CacheBlend: Fast Large Language Model Serving for RAG with Cached Knowledge Fusion

Large language models (LLMs) often incorporate multiple text chunks in their inputs to provide the necessary contexts. To speed up the prefill of the long LLM inputs, one can pre-compute the KV cache of a text and re-use the KV cache when the context is reused as the prefix of another LLM input. However, the reused text chunks are not always the input prefix, which makes precomputed KV caches not directly usable since they ignore the text's cross-attention with the preceding texts. Thus, the benefits of reusing KV caches remain largely unrealized. This paper tackles just one challenge: when an LLM input contains multiple text chunks, how to quickly combine their precomputed KV caches in order to achieve the same generation quality as the expensive full prefill (i.e., without reusing KV cache)? This challenge naturally arises in retrieval-augmented generation (RAG) where the input is supplemented with multiple retrieved texts as the context. We present CacheBlend, a scheme that reuses the precomputed KV caches, regardless prefix or not, and selectively recomputes the KV values of a small subset of tokens to partially update each reused KV cache. In the meantime, the small extra delay for recomputing some tokens can be pipelined with the retrieval of KV caches within the same job, allowing CacheBlend to store KV caches in slower devices with more storage capacity while retrieving them without increasing the inference delay. By comparing CacheBlend with the state-of-the-art KV cache reusing schemes on three open-source LLMs of various sizes and four popular benchmark datasets of different tasks, we show that CacheBlend reduces time-to-first-token (TTFT) by 2.2-3.3x and increases the inference throughput by 2.8-5x from full KV recompute without compromising generation quality. The code is available at https://github.com/LMCache/LMCache.

==> backups/1-introduction-0927.tex <==
\label{sec:intro}

\subsection{Motivation}
Nowadays, there have been an increasing number of software applications with the need of deploying deep neural networks (DNNs) to understand what is present in the images. Due to the heavy burden of designing and training such DNNs, many software developers use off-the-shelf machine learning (ML) APIs provided by many cloud service providers (\eg Google, Microsoft, Amazon) to reduce their development effort~\cite{wan2021machine}. However, the generic ML APIs might not be able to solve the tasks that the software intends to perform. 

When the service providers design the ML APIs, their goal is mainly to improve traditional class-wise accuracy metrics (\ie high average recall and precision)~\cite{wang2020multi} over all classes for large-scale datasets. However, when developers employ the ML APIs in their software, they care about whether ML APIs' outputs match their expectations (\ie as if the ML APIs' outputs are exactly the ground-truth labels). This gap in service providers' and software developers' purposes can lead to many software mis-behaviors, thus model adaptation is needed to provide a customized model that reduces software mis-behaviors as much as possible.





% Therefore, there is a need to adapt the ML APIs to directly optimize for producing correct software behaviors \cc{``ML APIs are xxx, while software are xxxx. Therefore, there is a need to adapt xxx''} 

To understand how and why optimizing class-wise accuracy does not necessarily lead to the correct software behaviors, we take the software application Smart can in Figure~\ref{fig:app_example} as an example. This application defines three lists to classify trash into categories. It calls Google's multi-label classification API to get the labels that describe the content in the image. The application then compares the output labels, ranked with descending order of confidence scores, with the three lists and returns the corresponding judgment if the outputs intersect with one of the lists. 
% goes through the output labels, and executes a branch if an output label is included in its corresponding pre-defined list. 

% and 
% then performs a post-processing step which executes one of \emph{Recycle, Compost, } and \emph{Donate} branches if the output labels contain any of the keywords specified in the pre-defined list \code{Recycle, Compost, Donate} \cc{``the pre-defined list'', you need to explain what is recycle, as it means a branch in the last reference} .


This simple post-processing step incurs potential software mis-behaviors even with a highly reliable ML API. For example, consider an input image (trash\_image) with ground-truth labels specified in the figure. The multi-label classification API returns an ordered list of labels, ranked in descending order of confidence scores. If we measure the outputs according to traditional recall and precision, this output yields a recall of 100\% and a precision of 80\%. Nevertheless, this output is completely wrong from the view of the software.  
According to the ground-truth labels, the correct branch to be executed is the one that returns ``This belongs to Compost'', since the only intersection between the ground-truth labels and the three lists is the one associated with the \emph{Compost} branch. However, the API's outputs lead to the program executing the branch which returns ``This belongs to Recycle. ''

% where its ground-truth labels include \emph{['Alcoholic beverage', \textcolor{red}{``Glass''}, 'Cocktail', 'Liqueur', 'Stemware'] }, and the API outputs are \emph{['Stemware', \textcolor{cyan}{``Food''}, 'Cocktail', 'Alcoholic beverage', 'Liqueur', 'Wine', \textcolor{red}{``Glass''}]}\cc{Maybe create a figure with a concrete image example and show the list (use color to show overlaps). 
% \yh{}
% Reader have to work hard to understand what is going on here }. This output yields a per-example recall of 100\% and precision of 71.5\%, while this prediction will be considered completely wrong from the view of the software. To be more specific, the correct branch to be executed, according to the ground-truth labels, should be \textcolor{red}{Recycle}. However, the labels generated by the ML API will lead to executing the branch which returns Compost. 
% \cc{This is not reason, but a detailed version of ``software considers it wrong''. Maybe use another way to describe this fact. Also, ``human-labeled ground-truth label'' and ``expected'' seem come out of blue. Suddenly human appears, and there is an expectation. You may just say the correct branch is xxx, according the ground-truth label} 

% This example demonstrates a common pattern of the mismatch between the generic tasks that the ML APIs are designed for and the specific tasks the software intends to perform. 
This is not the only case where the ML APIs' outputs lead to wrong software behaviors. When the software developers use the ML APIs in specific scenarios (\eg performing garbage classification), errors made by the ML APIs have different levels of severity: errors that lead to wrong software behaviors are more damaging than others. For example, false positives that lead to the program executing the wrong program branches, such as the ``Glass'' prediction that leads to the Recycle branch, are more devastating than false positives that are not included in the pre-defined lists associated with wrong program branches. 
Thus, an ideal solution for using ML APIs in the software is to customize the DNNs behind the ML APIs to reduce the errors that lead to wrong software behaviors. 
% \cc{Please say it is ideal solution. Maybe sth. like ``An ideal solution is to automatically adapt the network behind ML API to the task software performs''} 
% \cc{This paragraph is very strange, and does not provide any additional information. We usually say sth. like ``this example shows a common feature of xxxx'' or ``this is not the only example. A number of xxxx''} \cc{What gap? and how to define the gap? You need to introduce it first. Actually, I prefer you define the second half of this sentence as the gap}


% \emph{Automatically} adapting the ML APIs is important since the developers that call the ML APIs typically lack the knowledge of ML model training, or they do not have the compute resource to afford model training. 
% \cc{I move this sentence to this paragraph. Please change this sentence starting from sth. like ``Automation is important as ....''}

Automatically adapting the ML APIs has many challenges. 

\begin{itemize}

\item First, automatic model adaptation is hard. We need to infer the software-specific task from the software. The software developers did not explicitly specify the specific tasks they are performing and are not able to specify the specific tasks in the format that can be directly used to optimize the DNNs behind the ML APIs. 

% from the software about the specific task. 
% why infer? Users didn't explicitly specify the tasks, and they are non-experts, so they are not able to specify the tasks in the form that can be directly used to optimize for DNNs' accuracy 
% It is unrealistic to provide extra input for model adaptation (\eg manuals for performing model re-training) at the software developers' end. The main reason is that the software developers who call the ML APIs are typically non-experts in ML, thus it is hard for them to provide an effective model adaptation strategy. 


\item Secondly, model adaptation needs to be very efficient. As the software developers typically lack the computation resources to perform model training, model adaptation has to happen on the cloud service providers' side. Thus, it is important to provide a quick way of adapting models which reduces errors leading to wrong software behaviors with minimum training cost. 


% such that the number of damaging errors leading to incorrect software behaviors can be reduced most effectively (\ie incurring minimal training cost).  

% \item We performed empirical study on the applications that use ML APIs performing image classification tasks to affect the control flow of the software. We found that a common pattern 


% \item Machine Learning (ML) offers effective ML APIs to a wide range of cognition tasks. Many cloud providers offer ML APIs, supported by underlying Deep Neural Networks (DNNs), that perform well on generic tasks (\eg image classification). These ML APIs are utilized in a wide range of software applications for different specific tasks. However, the ML APIs are not adapted to achieve the application specific tasks, leading to many software misbehaviors.
    % \item List an application such that why/how high class-wise accuracy does not lead to correct software behavior or vice versa and cite~\cite{wan2022automated} to illustrate that there are many such applications. 
    % \ref{fig:app_example} is an example software that incorporates Google \code{label\_detection} API, which outputs all the existing labels in the input image. If we consider traditional class-wise F1 score of the application, the ML API can achieve 
    % \item Here we define the software achieving correct behaviors if the outputs of the ML APIs lead to the same software behavior as if the ground-truth is returned.  
    % \item Explain why the accuracy of the software would be low: the service providers train the ML models aiming to maximize class-wise accuracy, while the software developers need to ensure correct software behavior given the ML API outputs.  
    % \begin{itemize}
    %     \item the service providers pre-train the ML models that support the ML APIs with large-scale datasets (\eg Open Images dataset), aiming at providing good class-wise accuracy. \cc{Do you want to emphasis that they have different optimization goals?}
    %     \item When software developers use the ML APIs in their software, they expect the ML APIs to output classes that lead to the correct software behavior (\ie same software behavior as what the ground-truth leads to) \cc{What's the different between point2 \& 3?} 
    %     \item The pre-trained ML models may make mistakes that lead to the wrong software behavior
    % \end{itemize}
    

    % \item Automatically adapting the ML APIs to the software is important: (1) The developers who use the ML APIs are usually not experts in ML, thus may not know how to adapt the models (2) The developers do not have an affordable way to support model adaptation. 
    % \yh{mention why automation is important}
    % \yh{Emphasize that the problem is important}
    
    
    
    % \item However, when the developers use the ML APIs in their software, they are either unaware of the mismatch between ML APIs' accuracy and software's accuracy, or they do not have an affordable way to adapt the ML APIs to fit the software application they are writing.  \yh{Define affordable: 1. developers do not need to provide training data 2. they do not need to specify what are the context that can be digested by the DNNs to improve accuracy. }
    % \item Automatically adapting the ML APIs to the software is challenging. 
    % \begin{itemize}
    %     \item No existing benchmark has shown that there is a discrepancy between the outputs resulting in high class-wise accuracies and the ones leading to the correct software behaviors

    %     % (prior works either (1) only study ML APIs themselves (2) realize the low accuracy of ML APIs in the software~\cite{wan2021machine} (3) do not understand why the ML APIs do not work when applying to the software (SW only cares about branch prediction are correct) )
    %     % \item Need to transform cognition task into math expression 
    %     % create the template 
    %     \item Need to extract software specific cognitive task automatically and transform the extracted software context into mathematical expression that enables ML API adaptation
    %     \item Need to adapt the ML APIs efficiently 
       
    % \end{itemize}
    
    
    
    
    
    % \yh{To adapt the ML solutions to the software, software developers face many issues... (or accuracy decrease) or say adaptation is very important}
    % \yh{why do adaptation ? if not, will cause accuracy decrease. }
    
    % \yh{Developers did not realize this issue or they do not have an affordable way to adapt}
    
    % \yh{List an example}
    
    
    % \yh{Automatically adapt to the software is challenging. }
    

   
\end{itemize}
Existing works have performed model customization in different scenarios. 
They either directly input (\eg the classes that need to be classified)~\cite{kim2021pool, cao2021thia} or specify the specific tasks through a fixed program interface (\eg SQL)~\cite{kang2018blazeit}, and adjust the models, by training specialized models or reorganize different pre-trained model components, based on the specific tasks. Another line of work observes run-time data distribution and customizes the model to fit the specific content in the data. 

\begin{figure}
   \centering
\begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
Recycle = ['plastic', 'wood', 'glass', 'paper', 'cardboard', 'metal', 'aluminum', 'tin', 'carton']
Compost = ['food', 'produce', 'snack']
Donate = ['clothing', 'jacket', 'shirt', 'pants', 'footwear', 'shoe']
image = types.Image(content=trash_image)
response = client.label_detection(image=image)
for obj in response.label_annotations:
  if obj.name in Recycle:
    return 'It is recyclable.'
  if obj.name in Compost:
    return 'It is compostable.'
  if obj.name in Donate:
    return 'It is donatable.'
\end{lstlisting}
\includegraphics[width=.99\linewidth]{figs/app_example2.pdf}
    \caption{Heapsortcypher, a smart can application \cite{xxx} using Google Cloud API.}
    \label{fig:app_example}
    
\end{figure}
\subsection{Contributions} 
\begin{itemize}
%  \item We present \tool, which is an end-to-end system which automatically extracts software context from the applications that incorporate ML APIs, and adapt the ML models to improve the software accuracy. 
\item Studied a wide range of software applications that incorporate image classification APIs, and identified that one of the common software-specific tasks is mapping fine-grained ML API output classes to program branches. 
\item Automatically extracts the software-specific task from the code the software developers write, and transforms it into a mathematical expression that can adapt the ML APIs to the software. 
% Defined a template to automatically transform the code that the software developers write into mathematical expression that can adapt the ML APIs to the software. 
% \item defined the template and the transformation to math expression 
\item Leveraged two ways of model adaptation with the defined software context that (1) changes the training data distribution to reflect the subset of classes that the users care about; (2) modifies training loss function to directly optimize for the software-specific task. 
% \item Compared the ways of model adaptation in terms of accuracy improvement and training cost on \todo{X} real applications using ML APIs.

% defined two types of software context that can improve the accuracy of the software: (1) Data distribution context; (2) Subset of classes context. 

% \item Developed a tool to automatically extract the defined context from the Python code written by software developers 


\end{itemize}

==> backups/1-introduction-1004.tex <==
\label{sec:intro}

% \subsection{Motivation}

% \kt{It is not common to put subsections inside introduction (I'm not sure if it is common in SE community though)}
Nowadays, there have been an increasing number of software applications with the need of deploying deep neural networks (DNNs) to understand what is present in the input. Due to the heavy burden of designing and training such DNNs
% \kt{need citations here}
, many software developers use off-the-shelf machine learning (ML) APIs provided by many cloud service providers (\eg Google, Microsoft, Amazon) to reduce their development effort~\cite{wan2021machine}.  However, the generic ML APIs with good accuracy might lead to misbehaviors when applied to the software.
% \kt{The argument ``the software misbehavior is because that APIs are agnostic to software'' is an important argument and it directly leads to your key contribution. You bring this point too quick without much support, making this argument sounds trivial. I would suggest we postpone the mentioning of this point and just say a general ML API with good performance can lead to a lot of software behavior.}
% \yh{example: use the figure 1 example }
% \yh{existing works cost reduction by leveraging e.g., model compression 

% correct software misbehaviors by improving the ml models  =>  }

To illustrate how ML APIs with good accuracy may lead to software misbehaviors,
% how and why optimizing class-wise accuracy does not necessarily lead to the correct software behaviors,
% \kt{Maybe discribe the software behavior following the processing order of the software, like input -> API -> labels -> list -> output}
we take the software application \emph{Heapsortcypher} in Figure~\ref{fig:app_example} as an example. The application takes an image as input, and calls Google's multi-label classification API to get the labels that describe the content in the image. This application then goes through a post-processing step which classifies the ML APIs' outputs into categories of garbage. The application pre-defines three lists, \emph{Recycle, Compost, and Donate}. It then checks the output labels (\eg [Glass, Candy, Snack, Confectionery, Lollipop]), ranked with descending order of confidence scores, and searches for the first label (\eg Glass) that matches any of the labels in the three pre-defined lists. Then it executes the branch that corresponds to the found pre-defined list (\eg the one that outputs returns ``It is recyclable. '').
% the corresponding judgment if the outputs intersect with one of the lists. 

% and 
% then performs a post-processing step which executes one of \emph{Recycle, Compost, } and \emph{Donate} branches if the output labels contain any of the keywords specified in the pre-defined list \code{Recycle, Compost, Donate} \cc{``the pre-defined list'', you need to explain what is recycle, as it means a branch in the last reference} .


This simple post-processing step incurs potential software mis-behaviors even with an ML API that is able to correctly identify most of the classes.
% \kt{80\% recall does not sound like highly reliable. Also, ``highly reliable'' is vague. Maybe just say ``even when the ML API correctly identifies most of the classes''.} 
 Figure~\ref{fig:app_example2} shows a concrete example of how \emph{Heapsortcypher} works.  
% \cc{Maybe directly say that ``the bottom of Figure 1 shows a concrete example'', instead repeating what we have introduced earlier} 
 Given the outputs of the ML API, if we use traditional recall and precision as the metrics~\cite{wang2020multi}, this output yields a recall of 100\% and a precision of 80\%. Nevertheless, this output is completely wrong from the view of the software. 
According to the ground-truth labels, the correct branch to be executed is the one that returns ``It is compostable. '', since the only intersection between the ground-truth labels and the three lists is the one associated with the \emph{Compost} branch. However, the API's outputs lead to the program executing the branch which returns ``It is recyclable. '' \kt{From a system guy's perspective, I guess it is better  to highlight the cost of such software misbehavior. I'm not sure if this is needed in SE conference though.}
% \cc{P4 \& 5 have duplicate description}
%\cc{Maybe create a figure with a concrete image example and show the list (use color to show overlaps). 
% \yh{}
% Reader have to work hard to understand what is going on here }. This output yields a per-example recall of 100\% and precision of 71.5\%, while this prediction will be considered completely wrong from the view of the software. To be more specific, the correct branch to be executed, according to the ground-truth labels, should be \textcolor{red}{Recycle}. However, the labels generated by the ML API will lead to executing the branch which returns Compost. 
% \cc{This is not reason, but a detailed version of ``software considers it wrong''. Maybe use another way to describe this fact. Also, ``human-labeled ground-truth label'' and ``expected'' seem come out of blue. Suddenly human appears, and there is an expectation. You may just say the correct branch is xxx, according the ground-truth label} 

% This example demonstrates a common pattern of the mismatch between the generic tasks that the ML APIs are designed for and the specific tasks the software intends to perform. 
\kt{It is a cool empirical finding. The current way of giving this point is a bit too direct, and unintentionally trigger the reader to downplay the importance of this finding. Maybe back this finding up with more empirical evidence.} \yh{systematically find on Github}
This example represents a common usage pattern of ML APIs in software: developers specify a subset of labels that they care about in the specific application, such as the classes in different garbage categories, and how they plan to use the labels, such as which sets of labels trigger the same program branches. Under such usage patterns, ML API mis-predictions can have different levels of severity: errors that lead to wrong software behaviors are more damaging than others.\kt{You are somewhat downplaying an important new point (errors have different severity) by ``hiding'' it inside the para that seems to introducing the common usage pattern of ML API. Make this point clear by giving it a new paragraph.}  
% \cc{need connection. This example represents a common usage pattern of ML API:xxxx. Under such usage pattern, ML API mis-prediction have different level of damages to the software. xxx (not all API errors would lead to failure)}
For example, when the developer write the code as shown in Figure~\ref{fig:app_example}, false positives that lead to the program executing the wrong program branches, such as the ``Glass'' prediction that leads to the Recycle branch, are more devastating than false positives that do not affect the behavior of the software. 


\kt{Maybe contrast this design point with the one-size-fit-for-all design point.}Thus, an ideal solution for using ML APIs in the software is to customize the DNNs such that they are aware of the errors that lead to software misbehaviors. On this front, we want to 
% \cc{``we want''. It's still the motivation section, not contribution} 
re-train the DNNs behind the ML APIs with a re-constructed loss function that reflects the subset of labels the software cares about and the most damaging errors. For example, given the code structure in Figure~\ref{fig:app_example}, the re-constructed loss function will incur penalty only if the DNN makes mistakes that lead to wrong program branch (\eg ``Glass'' appearing in the outputs), and ignores any other types of errors that do not affect the software behavior(\eg the DNNs being confused between ``Snack'' and ``Food'', both belonging to the pre-defined list associated with \emph{Compost} branch).  
% \cc{Please say it is ideal solution. Maybe sth. like ``An ideal solution is to automatically adapt the network behind ML API to the task software performs''} 
% \cc{This paragraph is very strange, and does not provide any additional information. We usually say sth. like ``this example shows a common feature of xxxx'' or ``this is not the only example. A number of xxxx''} \cc{What gap? and how to define the gap? You need to introduce it first. Actually, I prefer you define the second half of this sentence as the gap}


% \emph{Automatically} adapting the ML APIs is important since the developers that call the ML APIs typically lack the knowledge of ML model training, or they do not have the compute resource to afford model training. 
% \cc{I move this sentence to this paragraph. Please change this sentence starting from sth. like ``Automation is important as ....''}

% \kt{As I learned from Junchen, in general, when introducing related works, it is better to suggest what we are going to do, but do not say it directly.}
Existing work proposes solutions to improve ML models on specific tasks without the knowledge of the software. 
% \kt{Adapting ML models sounds a bit abrupt. Maybe say ``existing work improves the performance of ML API by adapting the ML model.}
% \kt{Also, for me it feels early for us to mention ``optimizing without the knowledge of the software'' as the definition and importance of software knowledge is unclear here.}
% One line of work customizes the DNNs based on run-time data statistics and still optimizes for the same tasks (\eg image classification)~\cite{kim2021pool, cao2021thia, anderson2019physical}. Another line of work trains specialized models performing the tasks specified through a subset of SQL queries, such as aggregation and limit ~\cite{kang2018blazeit, kang2017noscope}.

\kt{Saying that we are targeting a different problem sounds like we are not picking the correct related work for our problem. Maybe try to say previous work are solving the same problem with the wrong assumption.}
However, we are tackling a different problem than these prior work. Firstly, as software developers typically write Python code to use the ML APIs, instead of declarative\kt{declarative is a ``noise'' here. It's better for us to focus on the popularity of the language here.} languages such as SQL.\kt{Previous work use SQL is not immediately clear to the reader.}
Second of all, the operations that can be expressed in SQL queries that the prior work optimizes for are limited (\eg aggregation, limit)\kt{People tend to not directly care about the limit of operations. Maybe link to what people care, like SQL limits what the \textbf{software can do}, and give a real (at least seemingly real) example to convince people a true need of software cannot be expressed by SQL.}, while there are a wider range of operations that can be expressed by Python. For example, aggregation or limit queries cannot specify subsets of labels can have the same effects on the final program behaviors. Thirdly, in order to use the these systems that optimize for SQL queries, users need to translate their code into SQL queries, which incurs an extra development burden for the users.\kt{For me, this point is essentially the same as the first point. The effect of choosing a programming language that people don't use is forcing the user to ``tranlate'' their code to another language.} Lastly, these approaches cannot guide the ML APIs to produce outputs that lead to correct software behaviors\kt{Personally I feel like this is the most fundamental reason. Putting it at the last is kind of downplaying this point.}\kt{I guess maybe you are referring that these works cannot fix the misbehavior of the software as they are just compressing the model, not improving the model. ``Software behavior'' and ``ground-truth labels'' are noise.} (\ie as if the ground-truth labels are returned), as they only optimize for inference delay. 

% When the service providers design the ML APIs, their goal is mainly to improve traditional class-wise accuracy metrics (\ie high average recall and precision)~\cite{wang2020multi} over all classes for large-scale datasets. However, when developers employ the ML APIs in their software, they care about whether ML APIs' outputs match their expectations (\ie as if the ML APIs' outputs are exactly the ground-truth labels). This gap in service providers' and software developers' purposes can lead to many software mis-behaviors, thus model adaptation is needed to provide a customized model that reduces software mis-behaviors as much as possible.


\kt{Maybe contrast this design point with the one-size-fit-for-all design point.}Thus, an ideal solution for using ML APIs in the software is to customize the DNNs such that they are aware of the errors that lead to software misbehaviors. On this front, we want to 
% \cc{``we want''. It's still the motivation section, not contribution} 
re-train the DNNs behind the ML APIs with a re-constructed loss function that reflects the subset of labels the software cares about and the most damaging errors. For example, given the code structure in Figure~\ref{fig:app_example}, the re-constructed loss function will incur penalty only if the DNN makes mistakes that lead to wrong program branch (\eg ``Glass'' appearing in the outputs), and ignores any other types of errors that do not affect the software behavior(\eg the DNNs being confused between ``Snack'' and ``Food'', both belonging to the pre-defined list associated with \emph{Compost} branch).  
% \cc{Please say it is ideal solution. Maybe sth. like ``An ideal solution is to automatically adapt the network behind ML API to the task software performs''} 
% \cc{This paragraph is very strange, and does not provide any additional information. We usually say sth. like ``this example shows a common feature of xxxx'' or ``this is not the only example. A number of xxxx''} \cc{What gap? and how to define the gap? You need to introduce it first. Actually, I prefer you define the second half of this sentence as the gap}


% \emph{Automatically} adapting the ML APIs is important since the developers that call the ML APIs typically lack the knowledge of ML model training, or they do not have the compute resource to afford model training. 
% \cc{I move this sentence to this paragraph. Please change this sentence starting from sth. like ``Automation is important as ....''}

Automatically adapting the DNNs behind ML APIs to fit the software's need has many challenges. 

\begin{itemize}

\item First, automatic model adaptation is hard. We need to automatically extract information embedded in the code structure that indicates how the software plans to use the labels. We also need to transform the information extracted from the software into loss functions that can directly be applied to optimize the DNNs. 


% from the software about the specific task. 
% why infer? Users didn't explicitly specify the tasks, and they are non-experts, so they are not able to specify the tasks in the form that can be directly used to optimize for DNNs' accuracy 
% It is unrealistic to provide extra input for model adaptation (\eg manuals for performing model re-training) at the software developers' end. The main reason is that the software developers who call the ML APIs are typically non-experts in ML, thus it is hard for them to provide an effective model adaptation strategy. 


\item Secondly, model adaptation needs to be very efficient. Given how the interface of the ML APIs is designed, the software developers who call the ML APIs are not able to adapt the DNNs behind the ML APIs. Thus, model adaptation has to happen on the cloud service providers' side, and it is important to provide a quick way of adapting models which reduces errors leading to wrong software behaviors with minimum training cost. 


% such that the number of damaging errors leading to incorrect software behaviors can be reduced most effectively (\ie incurring minimal training cost).  

% \item We performed empirical study on the applications that use ML APIs performing image classification tasks to affect the control flow of the software. We found that a common pattern 


% \item Machine Learning (ML) offers effective ML APIs to a wide range of cognition tasks. Many cloud providers offer ML APIs, supported by underlying Deep Neural Networks (DNNs), that perform well on generic tasks (\eg image classification). These ML APIs are utilized in a wide range of software applications for different specific tasks. However, the ML APIs are not adapted to achieve the application specific tasks, leading to many software misbehaviors.
    % \item List an application such that why/how high class-wise accuracy does not lead to correct software behavior or vice versa and cite~\cite{wan2022automated} to illustrate that there are many such applications. 
    % \ref{fig:app_example} is an example software that incorporates Google \code{label\_detection} API, which outputs all the existing labels in the input image. If we consider traditional class-wise F1 score of the application, the ML API can achieve 
    % \item Here we define the software achieving correct behaviors if the outputs of the ML APIs lead to the same software behavior as if the ground-truth is returned.  
    % \item Explain why the accuracy of the software would be low: the service providers train the ML models aiming to maximize class-wise accuracy, while the software developers need to ensure correct software behavior given the ML API outputs.  
    % \begin{itemize}
    %     \item the service providers pre-train the ML models that support the ML APIs with large-scale datasets (\eg Open Images dataset), aiming at providing good class-wise accuracy. \cc{Do you want to emphasis that they have different optimization goals?}
    %     \item When software developers use the ML APIs in their software, they expect the ML APIs to output classes that lead to the correct software behavior (\ie same software behavior as what the ground-truth leads to) \cc{What's the different between point2 \& 3?} 
    %     \item The pre-trained ML models may make mistakes that lead to the wrong software behavior
    % \end{itemize}
    

    % \item Automatically adapting the ML APIs to the software is important: (1) The developers who use the ML APIs are usually not experts in ML, thus may not know how to adapt the models (2) The developers do not have an affordable way to support model adaptation. 
    % \yh{mention why automation is important}
    % \yh{Emphasize that the problem is important}
    
    
    
    % \item However, when the developers use the ML APIs in their software, they are either unaware of the mismatch between ML APIs' accuracy and software's accuracy, or they do not have an affordable way to adapt the ML APIs to fit the software application they are writing.  \yh{Define affordable: 1. developers do not need to provide training data 2. they do not need to specify what are the context that can be digested by the DNNs to improve accuracy. }
    % \item Automatically adapting the ML APIs to the software is challenging. 
    % \begin{itemize}
    %     \item No existing benchmark has shown that there is a discrepancy between the outputs resulting in high class-wise accuracies and the ones leading to the correct software behaviors

    %     % (prior works either (1) only study ML APIs themselves (2) realize the low accuracy of ML APIs in the software~\cite{wan2021machine} (3) do not understand why the ML APIs do not work when applying to the software (SW only cares about branch prediction are correct) )
    %     % \item Need to transform cognition task into math expression 
    %     % create the template 
    %     \item Need to extract software specific cognitive task automatically and transform the extracted software context into mathematical expression that enables ML API adaptation
    %     \item Need to adapt the ML APIs efficiently 
       
    % \end{itemize}
    
    
    
    
    
    % \yh{To adapt the ML solutions to the software, software developers face many issues... (or accuracy decrease) or say adaptation is very important}
    % \yh{why do adaptation ? if not, will cause accuracy decrease. }
    
    % \yh{Developers did not realize this issue or they do not have an affordable way to adapt}
    
    % \yh{List an example}
    
    
    % \yh{Automatically adapt to the software is challenging. }
    

   
\end{itemize}
% Existing works have performed model customization in different scenarios. 
% They either directly input (\eg the classes that need to be classified)~\cite{kim2021pool, cao2021thia} or specify the specific tasks through a fixed program interface (\eg SQL)~\cite{kang2018blazeit}, and adjust the models, by training specialized models or reorganize different pre-trained model components, based on the specific tasks. Another line of work observes run-time data distribution and customizes the model to fit the specific content in the data. 

\begin{figure}
\begin{subfigure}{0.45\textwidth}    
         \centering
         \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
Recycle = ['plastic', 'wood', 'glass', 'paper', 'cardboard', 'metal', 'aluminum', 'tin', 'carton']
Compost = ['food', 'produce', 'snack']
Donate = ['clothing', 'jacket', 'shirt', 'pants', 'footwear', 'shoe']
image = types.Image(content=trash_image)
response = client.label_detection(image=image)
for obj in response.label_annotations:
  if obj.name in Recycle:
    return 'It is recyclable.'
    if obj.name in Compost:
    return 'It is compostable.'
  if obj.name in Donate:
    return 'It is donatable.'
    \end{lstlisting}
\subcaption{The software implementation}
\label{fig:app_example}
% \includegraphics[width=.99\linewidth]{figs/app_example2.pdf}
    \end{subfigure}
 \hfill
    \begin{subfigure}{0.45\textwidth}  
        \includegraphics[width=\linewidth]{figs/app_example2.pdf}
        \subcaption[]{A concrete example. }
        \label{fig:app_example2}
    \end{subfigure}
    \caption{Heapsortcypher, a garbage classification application \cite{heapsort} using Google Cloud API.}
\end{figure}

\subsection{Contributions} 
 We present \tool, which helps the cloud service providers, who offer the ML APIs, to automatically adapt the ML APIs to the applications the developers write. 

To understand common tasks software developers intend to perform, we conduct an empirical study on the applications using Google's \code{label\_detection} in a recently published benchmark suite studying ML software~\cite{wan2021machine}, a multi-label image classification API. We focus on 19 applications whose control flow decisions are affected by ML APIs' outputs, for example, the software will print out a warning if the outputs contain ``Gun'' or ``Fire'', and do nothing otherwise. We found that a common pattern of the code structures for these applications is triggering the same program actions for sets of labels, such as returning the same message for labels specified in the same pre-defined list. For example, labels specified in the \emph{Compost} list, including ``Food'', ``Produce'', and ``Snack'', triggers the same program behavior (\ie returning the message ``This is recyclable''). However, different applications have different specific ways of triggering program behaviors based on pre-defined lists. We generalized three levels of abstraction from the code structures of the applications in the benchmark suite: (1) labels that will trigger the same program behaviors; (2) whether the final program output is exclusively 
 
\begin{itemize}

\item Perform program analysis to extract the information needed to perform model adaptation, including the subset of labels that the software cares about, and the sets of labels that are considered equivalent by the software. We also re-constructed loss functions using the extracted information to directly reflect the damaging errors that are not acceptable by the software. 
% Defined a template to automatically transform the code that the software developers write into mathematical expression that can adapt the ML APIs to the software. 
% \item defined the template and the transformation to math expression 
\item Re-train the DNNs behind the ML APIs with the re-constructed loss function, and systematically measure the improvement in the rate of software mis-behaviors on \todo{X} open-source applications invoking ML APIs. 
% \item Compared the ways of model adaptation in terms of accuracy improvement and training cost on \todo{X} real applications using ML APIs.

% defined two types of software context that can improve the accuracy of the software: (1) Data distribution context; (2) Subset of classes context. 

% \item Developed a tool to automatically extract the defined context from the Python code written by software developers 


\end{itemize}

==> backups/1-introduction-1106.tex <==
\label{sec:intro}

\subsection{Motivation}
\kt{I would suggest listing the first sentence of each para as bullet points here. It is important to iterate on the structure and the logic (instead of the language details) first.}

% \kt{It is not common to put subsections inside introduction (I'm not sure if it is common in SE community though)}
% \begin{itemize}
%     \item increasing number of software applications use off-the-shelf ML APIs to understand what is present in the input. However, the generic ML APIs with good accuracy might make small mistakes leading to software misbehaviors
%     \item Illustrate how small mistakes could lead to software misbehaviors with the application example 
%     \item This 
% \end{itemize}
There have been an increasing number of software applications with the need of deploying deep neural networks (DNNs) to understand what is present in the input. Due to the heavy burden of designing and training such DNNs
% \kt{need citations here}
, many software developers use off-the-shelf machine learning (ML) APIs provided by many cloud service providers (\eg Google, Microsoft, Amazon) to reduce their development effort~\cite{wan2021machine}.  However, the accuracy of generic ML APIs misaligns with software correctness\shan{This sentence needs rewording. Not clearly what it tries to deliver.}. 
% \kt{The argument ``the software misbehavior is because that APIs are agnostic to software'' is an important argument and it directly leads to your key contribution. You bring this point too quick without much support, making this argument sounds trivial. I would suggest we postpone the mentioning of this point and just say a general ML API with good performance can lead to a lot of software behavior.}
% \yh{example: use the figure 1 example }
% \yh{existing works cost reduction by leveraging e.g., model compression 

% correct software misbehaviors by improving the ml models  =>  }

To illustrate how ML APIs with good accuracy may lead to software misbehaviors\shan{This opening sentence is a bit odd: it seems to fit our OOPSLA submission better, don't you think so? Furthermore, even with your tool and ML APIs with increased accuracy, the software may still misbehave, right?},
% how and why optimizing class-wise accuracy does not necessarily lead to the correct software behaviors,
% \kt{Maybe discribe the software behavior following the processing order of the software, like input -> API -> labels -> list -> output}
we take the software application \emph{Heapsortcypher} in Figure~\ref{fig:app_example} as an example. It takes a trash image as input, and invokes \code{label\_detection}, Google's multi-label classification API, to get the labels that describe the content in the image. It then goes through a post-processing step which classifies the ML APIs' outputs into categories of garbage. Heapsortcypher pre-defines three lists, \emph{Recycle, Compost, and Donate}. It checks the output labels (\eg [Glass, Candy, Snack, Confectionery, Lollipop]), ranked with descending order of confidence scores, and searches for the first label (\eg Glass) that matches any of the labels in the three pre-defined lists. Finally it executes the branch that corresponds to the found pre-defined list (\eg the one that outputs returns ``It is recyclable. '').
% the corresponding judgment if the outputs intersect with one of the lists. 

% and 
% then performs a post-processing step which executes one of \emph{Recycle, Compost, } and \emph{Donate} branches if the output labels contain any of the keywords specified in the pre-defined list \code{Recycle, Compost, Donate} \cc{``the pre-defined list'', you need to explain what is recycle, as it means a branch in the last reference} .


This simple post-processing step incurs potential software mis-behaviors even with an ML API that only mis-classifies one class, as shown in Figure~\ref{fig:input_example_top_wrong}.
% \kt{80\% recall does not sound like highly reliable. Also, ``highly reliable'' is vague. Maybe just say ``even when the ML API correctly identifies most of the classes''.} 
% Figure~\ref{fig:app_example2} shows a concrete example of how \emph{Heapsortcypher} works.  
% \cc{Maybe directly say that ``the bottom of Figure 1 shows a concrete example'', instead repeating what we have introduced earlier} 
% Given the outputs of the ML API, if we use traditional recall and precision as the metrics~\cite{wang2020multi}, this output yields a recall of 100\% and a precision of 80\%. Nevertheless, this output is completely wrong from the view of the software. 
% According to the ground-truth labels, the correct branch to be executed is the one that returns ``It is compostable. '', since the only intersection between the ground-truth labels and the three lists is the one associated with the \emph{Compost} branch. However, the API's outputs lead to the program executing the branch which returns ``It is recyclable. '' 
Given a candy image, the ML API wrongly returns the label ``Glass''. This mistake is minor in terms of the multi-label classification task~\cite{wang2020multi}: it  finds all the objects in the input image while recognizing an extra wrong object ``Glass'', providing a recall of 100\% and a precision of 80\%\shan{I don't understand how you get these numbers: 100\% and 80\%.}. However, it leads to a completely wrong software behavior. While this image belongs to \emph{compostable} branch, the software wrongly executes the \emph{recyclable} branch as \code{Recycle} list contains the first API output label ``Glass''.

\shan{After I finished reading the above two paragraphs, I finally saw what you are trying to tell the readers. I guess you are trying to say that not all mistakes of an ML API are equally important for a software application. Is that what you are trying to say? You need to clearly present what messages you want to deliver BEFORE you present examples. You cannot ask readers to summarize/infer what you mean AFTER they read the example.}


% \cc{I changed the description. Please proof read}

% \kt{From a system guy's perspective, I guess it is better  to highlight the cost of such software misbehavior. I'm not sure if this is needed in SE conference though.}
% \cc{P4 \& 5 have duplicate description}
%\cc{Maybe create a figure with a concrete image example and show the list (use color to show overlaps). 
% \yh{}

% \kt{It is a cool empirical finding. The current way of giving this point is a bit too direct, and unintentionally trigger the reader to downplay the importance of this finding. Maybe back this finding up with more empirical evidence.}
\kt{I would expect you saying this type of error is a common error. People do not directly care about the common usage pattern of ML API.}
% This example represents a common error pattern of applying ML APIs in software: developers specify a subset of labels that they care about, such as \code{Recycle}, \code{Compost}, and \emph{Donate} lists, and how they use the labels, such as these three lists correspond to three software branches. 
% We perform an empirical study to study the common patterns of the applications in the benchmark suite~\cite{wan2021machine}, focusing on the applications whose program behaviors are affected by the ML APIs' outputs\footnote{We study these applications as they reflect non-trivial ways of using ML APIs. If the applications directly return the APIs' outputs, they do not provide extra information for us to perform adaptation. }. We find that it is common for applications to pre-define one or more lists of labels, and execute different branches by comparing the output labels with the lists. \kt{People may wonder what happened to the remaining 40\% applications.} 
% \kt{It would be better to separate these two important points {\footnotesize (This pattern is common \& mispredictions have different levels of severity)} into two paragraphs.}
This example represents a common phenomenon in ML software. The reason is that the ML APIs are optimized for generic accuracy over a large number of classes, but the ML software has a different focus and priority: it cares about whether the ML API can produce outputs leading to correct control flow decisions\shan{I think it is a bit too early to mention control flow here. Please think and rephrase.}. 

The way the ML software is typically written can cause accurate ML APIs' outputs to lead to wrong control flow decisions\shan{?????What? Am I in the wrong paper? This sentence seems to fit our OOPSLA submission but does NOT fit here AT ALL. Your example so far is about wrong API result; it is NOT about accurate API result that leads to software failure. I am very confused.}. Specifically,  developers usually specify a subset of labels that they care about, such as \code{Recycle}, \code{Compost}, and \emph{Donate} lists, and how they use the labels, such as these three lists correspond to three software branches. Under such code patterns, ML API mis-predictions have different levels of severity: errors that lead to wrong software behaviors are more damaging than others\shan{No, it is not about which one is more damaging. Some mis-prediction simply has NO damage at all. Right?}. For example, in Heapsortcypher, the confusion within the lists, such as misclassifying a ``Food'' image to ``Produce'', is less damaging \shan{Again, when you say ``less damaging'', you are implying there exists some damage. But, that is not true here. mis-classifying food to produce has no damage to the software at all!} than across the list, such as misclassifying a ``Food'' image to ``Glass'', as only the latter would lead to a wrong control flow decision.



% Under such code patterns, ML API mis-predictions have different levels of severity: errors that lead to wrong software behaviors are more damaging than others. For example, in Heapsortcypher, the confusion within the lists, such as misclassifying a ``Food'' image to ``Produce'', is less damaging than across the list, such as misclassifying a ``Food'' image to ``Glass'', as only the latter would lead to a wrong execution path.
% \cc{Please explain the effect of mis-classification inside list and outside list} \yh{Done}
% \kt{You are somewhat downplaying an important new point (errors have different severity) by ``hiding'' it inside the para that seems to introducing the common usage pattern of ML API. Make this point clear by giving it a new paragraph.}  
% For example, when the developer write the code as shown in Figure~\ref{fig:app_example}, false positives that lead to the program executing the wrong program branches, such as the ``Glass'' prediction that leads to the Recycle branch, are more devastating than false positives that do not affect the behavior of the software. 


% \kt{Maybe contrast this design point with the one-size-fit-for-all design point.}
% \kt{``customize the DNNs'' is a surprise. Maybe give more rationales to justify why customizing DNN instead of something like redesigning the API interface.}
% \cc{Be aware of software behavior? aim to improve software correctness?} \yh{Done} \kt{This issue is not solved yet. I guess Chengcheng questions these two things because they are vague. Maybe try to answer what kind of concrete software behavior are you aim to improving/what is software correctness/what kind of software correctness are you trying to improve.}

Thus, instead of providing a generic ML API that could be applied to all software, an ideal solution is to customize the DNNs behind ML API for each software, while keeping the same interface\shan{How do you define interface? If you really keep the same interface, how do you collect the software control flow information for the API provider?}. In this way, the ML API is aware of how the ML APIs' outputs affect the software behavior and is optimized to provide outputs that ensure\shan{no way you can ensure} software behaves as if the ground-truth of the input is returned by the ML APIs. Meanwhile, the developers would not be bothered to modify their software to fit the adaptation. 
% On this front, we want to re-train these DNNs behind the ML APIs with a re-constructed loss function\kt{Justify this design choice.} that reflects the subset of labels the software cares about and the most damaging errors. For example, given the code structure in Figure~\ref{fig:app_example}, the re-constructed loss function will incur penalty only if the DNN makes mistakes that lead to wrong program branch (\eg ``Glass'' appearing in the outputs), and ignores any other types of errors that do not affect the software behavior(\eg the DNNs being confused between ``Snack'' and ``Food'', both belonging to the pre-defined list associated with \emph{Compost} branch).   \cc{This is solution. So I comment it out. I'll put them in Section 1.2}

% \cc{Please say it is ideal solution. Maybe sth. like ``An ideal solution is to automatically adapt the network behind ML API to the task software performs''} 
% \cc{This paragraph is very strange, and does not provide any additional information. We usually say sth. like ``this example shows a common feature of xxxx'' or ``this is not the only example. A number of xxxx''} \cc{What gap? and how to define the gap? You need to introduce it first. Actually, I prefer you define the second half of this sentence as the gap}


% \emph{Automatically} adapting the ML APIs is important since the developers that call the ML APIs typically lack the knowledge of ML model training, or they do not have the compute resource to afford model training. 
% \cc{I move this sentence to this paragraph. Please change this sentence starting from sth. like ``Automation is important as ....''}

% \kt{As I learned from Junchen, in general, when introducing related works, it is better to suggest what we are going to do, but do not say it directly.}
% \kt{This paragraph is tooooo long. Maybe illustrate these two line of works in two paragraphs?}
% \cc{``To the best of our knowledge, we are the first to study xxx problem.'' Can we claim something like this? If not, maybe starts with ``Existing work cannot tackle our problem. They improve xxxx without the knowledge of software.'' } \yh{I mentioned we are tackling a different problem, is this ok? }
% \kt{Adapting ML models sounds a bit abrupt. Maybe say ``existing work improves the performance of ML API by adapting the ML model.}
% \kt{Also, for me it feels early for us to mention ``optimizing without the knowledge of the software'' as the definition and importance of software knowledge is unclear here.}

% Existing work proposes solutions to improve the performance or accuracy of ML models without the knowledge of the software. However, we are tackling a different problem than these prior work. 
% One line of work optimizes the ML APIs' query accuracy or cost by adaptively choosing a sequential strategy to invoke available APIs within a resource budget ~\cite{chen2020frugalml, chen2022frugalmct}. 
% These work requires modifications on the developers' side, such as changing the code to apply the most accurate API. 

% Another line of work trains specialized models performing the tasks specified through a subset of SQL queries, such as aggregation and limit, such that the inference delay is reduced ~\cite{kang2018blazeit, kang2017noscope}. 
% The problem we are targeting at is different from this line of work for the following reasons. Firstly, these approaches cannot guide the ML APIs to produce outputs that lead to correct software behaviors, as they only optimize for inference delay instead of improving the model. Secondly, a great number of existing applications on GitHub calling ML APIs are written in Python~\cite{wan2021machine} instead of SQL. Thirdly, the operations that can be expressed in SQL queries that the prior work optimizes for are limited. For example, the SQL queries that are optimized by these work can only count average number of objects among all the video frames, or selecting limited number of frames that meet several constraints. Nevertheless, there are a wider range of operations that can be expressed by Python. For example, aggregation or limit queries cannot specify subsets of labels can have the same effects on the final program behaviors. 
% Lastly, in order to use the these systems that optimize for SQL queries, users need to translate their code into SQL queries, which incurs an extra development burden for the users.


Existing work proposes solutions to improve the performance or accuracy of ML models in software applications.
However, we found that existing solutions are not desirable as they add extra burden on the developers.
Specifically, one line of works focus on improving accuracy of ML task itself by modifying the software call to the ML APIs~\cite{chen2020frugalml, chen2022frugalmct}. 
Given a resource budget, they adaptively invokes several ML APIs from different cloud providers and ensemble their results. 
However, this approach require changing the software implementation in order to call different ML APIs, thus creating extra burden to the developers\shan{I find this argument very weak: the change required sounds very minimal and can be easily wrapped inside a library call. More importantly, I feel there are much more fundamental differences between your work and this previous work and yet you didn't mention.}.
Another line of work aims to reduce latency by compressing DNNs to perform a specialized task defined by a subset of SQL syntax~\cite{kang2018blazeit, kang2017noscope}. 
However, this approach cannot correct the software misbehavior triggered by wrong DNN output (as the DNN compression reduces the DNN latency while keeping the DNN ouput the same). 
Besides, this approach adds extra developer effort to reimplement their software logic (which is typically written in Python~\cite{wan2021machine}) using SQL syntax.
% In addition, they focus on SQL, while we study real-world applications written in general purpose language like Python~\cite{wan2021machine}, which supports much more operations.

Our goal is to \textit{automatically} adapting the DNNs behind the ML API \textit{without extra developer effort}.
\shan{Just like my comments in the abstract, I feel you still didn't make it very clear about your assumption. What is your assumption about what you have access to and what you can change? This assumption is VERY different from our OOPSLA submission, right? That is why you need to clearly explain your problem statement and assumption here.}

% \kt{Saying that we are targeting a different problem sounds like we are not picking the correct related work for our problem. Maybe try to say previous work are solving the same problem with the wrong assumption.}


% as software developers typically write Python code to use the ML APIs, instead of declarative\kt{declarative is a ``noise'' here. It's better for us to focus on the popularity of the language here.} languages such as SQL.\kt{Previous work use SQL is not immediately clear to the reader.}
% \kt{People tend to not directly care about the limit of operations. Maybe link to what people care, like SQL limits what the \textbf{software can do}, and give a real (at least seemingly real) example to convince people a true need of software cannot be expressed by SQL.}, 
% \kt{For me, this point is essentially the same as the first point. The effect of choosing a programming language that people don't use is forcing the user to ``tranlate'' their code to another language.}  \kt{Personally I feel like this is the most fundamental reason. Putting it at the last is kind of downplaying this point.}\kt{I guess maybe you are referring that these works cannot fix the misbehavior of the software as they are just compressing the model, not improving the model. ``Software behavior'' and ``ground-truth labels'' are noise.} 


% \cc{Please say it is ideal solution. Maybe sth. like ``An ideal solution is to automatically adapt the network behind ML API to the task software performs''} 
% \cc{This paragraph is very strange, and does not provide any additional information. We usually say sth. like ``this example shows a common feature of xxxx'' or ``this is not the only example. A number of xxxx''} \cc{What gap? and how to define the gap? You need to introduce it first. Actually, I prefer you define the second half of this sentence as the gap}


% \emph{Automatically} adapting the ML APIs is important since the developers that call the ML APIs typically lack the knowledge of ML model training, or they do not have the compute resource to afford model training. 
% \cc{I move this sentence to this paragraph. Please change this sentence starting from sth. like ``Automation is important as ....''}

% As a result, we need an approach that automatically adapts the ML models behind ML APIs such that they are aware of the damaging errors that will lead to software misbehaviors\cc{This sentence belongs to P5. It also looks like a repletion of P5-sentence1}.

Automatically adapting the ML models faces several challenges. 



\emph{Firstly}, automatic model adaptation is hard. Aiming to help non-expert developers, an automatic approach that minimizes developer effort is desired. To achieve such automatic adaptation, we need to understand how software uses ML API output label and the severity of different types of mis-predictions. We also need to translate these information to a DNN-understandable format for adaptation, such as a loss function, which is inherently hard due to rich code syntax. 
% \cc{Yuhan, please proof read}

% Automation is necessary because the application developers using the ML APIs typically lack expertise in ML, thus may not be able to efficiently perform model adaptation. We need to automatically extract information\kt{vague} embedded in the code structure that indicates how the software plans to use ML APIs' output labels. We also need to transform the information extracted from the software into loss functions that can directly be applied to optimize the DNNs.  
% \cc{why automation? please explain} \yh{added. }


% from the software about the specific task. 
% why infer? Users didn't explicitly specify the tasks, and they are non-experts, so they are not able to specify the tasks in the form that can be directly used to optimize for DNNs' accuracy 
% It is unrealistic to provide extra input for model adaptation (\eg manuals for performing model re-training) at the software developers' end. The main reason is that the software developers who call the ML APIs are typically non-experts in ML, thus it is hard for them to provide an effective model adaptation strategy. 


\emph{Secondly}, model adaptation needs to be very efficient. 
 Since we need to re-train the ML model for each software application, model adaptation should be fast. Moreover, software applications may change time to time during the development procedure, thus adapting the ML models quickly can greatly save the time and operation cost of re-training. 
 \shan{I guess we also assume that we cannot obtain new training data from application developers.}
 % \kt{Another reason is that your approach needs to train different DNNs for different softwares, so the training need to be cheap.}
% Given how the interface of the ML APIs is designed, the software developers who call the ML APIs are not able to adapt the DNNs behind the ML APIs. Thus, model adaptation has to happen on the cloud service providers' side, and it is important to provide a quick way of adapting models which reduces errors leading to wrong software behaviors with minimum training cost. \cc{It does not matter whether developer or service provider pay the training cost. Actually, service providers could charge more on developer if training takes more time. You may say (1) software may change time by time during development (2) a fast adaptation could save time and operation cost} 


% such that the number of damaging errors leading to incorrect software behaviors can be reduced most effectively (\ie incurring minimal training cost).  

% \item We performed empirical study on the applications that use ML APIs performing image classification tasks to affect the control flow of the software. We found that a common pattern 


% \item Machine Learning (ML) offers effective ML APIs to a wide range of cognition tasks. Many cloud providers offer ML APIs, supported by underlying Deep Neural Networks (DNNs), that perform well on generic tasks (\eg image classification). These ML APIs are utilized in a wide range of software applications for different specific tasks. However, the ML APIs are not adapted to achieve the application specific tasks, leading to many software misbehaviors.
    % \item List an application such that why/how high class-wise accuracy does not lead to correct software behavior or vice versa and cite~\cite{wan2022automated} to illustrate that there are many such applications. 
    % \ref{fig:app_example} is an example software that incorporates Google \code{label\_detection} API, which outputs all the existing labels in the input image. If we consider traditional class-wise F1 score of the application, the ML API can achieve 
    % \item Here we define the software achieving correct behaviors if the outputs of the ML APIs lead to the same software behavior as if the ground-truth is returned.  
    % \item Explain why the accuracy of the software would be low: the service providers train the ML models aiming to maximize class-wise accuracy, while the software developers need to ensure correct software behavior given the ML API outputs.  
    % \begin{itemize}
    %     \item the service providers pre-train the ML models that support the ML APIs with large-scale datasets (\eg Open Images dataset), aiming at providing good class-wise accuracy. \cc{Do you want to emphasis that they have different optimization goals?}
    %     \item When software developers use the ML APIs in their software, they expect the ML APIs to output classes that lead to the correct software behavior (\ie same software behavior as what the ground-truth leads to) \cc{What's the different between point2 \& 3?} 
    %     \item The pre-trained ML models may make mistakes that lead to the wrong software behavior
    % \end{itemize}
    

    % \item Automatically adapting the ML APIs to the software is important: (1) The developers who use the ML APIs are usually not experts in ML, thus may not know how to adapt the models (2) The developers do not have an affordable way to support model adaptation. 
    % \yh{mention why automation is important}
    % \yh{Emphasize that the problem is important}
    
    
    
    % \item However, when the developers use the ML APIs in their software, they are either unaware of the mismatch between ML APIs' accuracy and software's accuracy, or they do not have an affordable way to adapt the ML APIs to fit the software application they are writing.  \yh{Define affordable: 1. developers do not need to provide training data 2. they do not need to specify what are the context that can be digested by the DNNs to improve accuracy. }
    % \item Automatically adapting the ML APIs to the software is challenging. 
    % \begin{itemize}
    %     \item No existing benchmark has shown that there is a discrepancy between the outputs resulting in high class-wise accuracies and the ones leading to the correct software behaviors

    %     % (prior works either (1) only study ML APIs themselves (2) realize the low accuracy of ML APIs in the software~\cite{wan2021machine} (3) do not understand why the ML APIs do not work when applying to the software (SW only cares about branch prediction are correct) )
    %     % \item Need to transform cognition task into math expression 
    %     % create the template 
    %     \item Need to extract software specific cognitive task automatically and transform the extracted software context into mathematical expression that enables ML API adaptation
    %     \item Need to adapt the ML APIs efficiently 
       
    % \end{itemize}
    
    
    
    
    
    % \yh{To adapt the ML solutions to the software, software developers face many issues... (or accuracy decrease) or say adaptation is very important}
    % \yh{why do adaptation ? if not, will cause accuracy decrease. }
    
    % \yh{Developers did not realize this issue or they do not have an affordable way to adapt}
    
    % \yh{List an example}
    
    
    % \yh{Automatically adapt to the software is challenging. }
    

   

% Existing works have performed model customization in different scenarios. 
% They either directly input (\eg the classes that need to be classified)~\cite{kim2021pool, cao2021thia} or specify the specific tasks through a fixed program interface (\eg SQL)~\cite{kang2018blazeit}, and adjust the models, by training specialized models or reorganize different pre-trained model components, based on the specific tasks. Another line of work observes run-time data distribution and customizes the model to fit the specific content in the data. 

\begin{figure}
\begin{subfigure}{0.45\textwidth}    
         \centering
         \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
Recycle = ['Plastic', 'Wood', 'Glass', 'Paper', 'Cardboard', 'Metal', 'Aluminum', 'Tin', 'Carton']
Compost = ['Food', 'Produce', 'Snack']
Donate = ['Clothing', 'Jacket', 'Shirt', 'Pants', 'Footwear', 'Shoe']
image = types.Image(content=trash_image)
response = client.label_detection(image=image)
for obj in response.label_annotations:
  if obj.name in Recycle:
    return 'It is recyclable.'
  elif obj.name in Compost:
    return 'It is compostable.'
  elif obj.name in Donate:
    return 'It is donatable.'
return 'It is others.'
\end{lstlisting}
%          \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% Recycle = ['Plastic', 'Wood', 'Glass', 'Paper', 'Cardboard', 'Metal', 'Aluminum', 'Tin', 'Carton']
% Compost = ['Food', 'Produce', 'Snack']
% Donate = ['Clothing', 'Jacket', 'Shirt', 'Pants', 'Footwear', 'Shoe']
% image = types.Image(content=trash_image)
% response = client.label_detection(image=image)
% Predictions = []
% for obj in response.label_annotations:
%   Predictions.append(obj.name)
% if any([label in Recycle for label in Predictions]):
%   return 'It is recyclable.'
% elif any([label in Compost for label in Predictions]):
%   return 'It is compostable.'
% elif any([label in Donate for label in Predictions]):
%   return 'It is donatable.'
%     \end{lstlisting}
\subcaption{The software implementation}
\label{fig:app_example}
% \includegraphics[width=.99\linewidth]{figs/app_example2.pdf}
    \end{subfigure}
 \hfill
    \begin{subfigure}{0.45\textwidth}  
        \includegraphics[width=\linewidth]{figs/app_example2.pdf}
        \subcaption[]{Including an extra wrong\shan{???What do you mean by missing???} recognition ``Glass'' leads to software mis-behavior. The arrows starting from the Ground-truth labels are the correct software control flow decision (\ie as if the ground-truth labels are output by the ML API). In this example, the correct control flow is executing the branch associated with the Compost list, because the ground-truth labels only have an intersection with the Compost list. \shan{This caption is very difficult for readers to understand.}}
        \label{fig:input_example_top_wrong}
    \end{subfigure}
    %     \begin{subfigure}{0.45\textwidth}  
    %     \includegraphics[width=\linewidth]{figs/input_example_top_label_correct.pdf}
    %     \subcaption[]{Mis-classifying the label ``Wood'' does not lead to software mis-behavior. }
    %     \label{fig:input_example_top_correct}
    % \end{subfigure}
    % \caption{Heapsortcypher, a garbage classification application \cite{heapsort} using Google Cloud API. 
    % \kt{The key in this figure is the contrast between highly accurate API output and wrong software misbehavior. Maybe not calling the ideal API output as ``ground-truth''? It is better for your point to come across without letting the reader to parse what does ``ground-truth'' means, and realize that this image comes from your dataset and it is an image annotated with ground-truth label.}\cc{It's fine. We just take it literally: the correct answer.}
    % }
\label{fig:app_example_entire}
\end{figure}


\subsection{Contributions} 
%\kt{I would expect contributions to be some short and condensed bullet points.}\cc{Let's first make a long version and then decide how to compress it.}


% We present \tool, which helps the cloud service providers to automatically re-train the ML models behind the ML APIs to the applications the developers write, so as to reduce the software mis-behaviors incurred by the ML APIs' outputs.
% \cc{I changed the description. Please proof read} \yh{we are not helping developers, our solution happens on the cloud service providers' side. }

% We find that the code structures reflect the severity of different API mis-predictions.
% For example, in Figure~\ref{fig:app_example}, labels in the \emph{Recycle} list and labels in the \emph{Compost} list trigger different program behaviors. Therefore, given an input image only containing labels in the \emph{Recycle} list, it is a severe error if the ML API outputs labels in the \emph{Compost} list. \cc{This paragraph should belong to empirical study} 

To understand how real world applications use ML APIs\shan{This opening sentence is toooo generic. I could have used it in all recent papers from our group. If I am a reviewer, I would wonder ``haven't people already conducted tons of study to understand how applications use ML APIs? Why do you need to study again?????''. What EXACTLY was not understood before and hence you want to understand?}, we conduct an empirical study on a recently published ML software benchmark suite~\cite{wan2021machine}. We found five code structure patterns of how ML software post-process ML APIs' outputs, and derived three types of abstractions to characterize how the control flows are affected by ML APIs' outputs (details are in Section~\ref{sec:empirical})\shan{Again, why isn't this already covered by previous work?}.  
% We focus on 19 applications which invokes Google \code{label\_detection} API to make control flow decisions. These applications use the ML APIs' outputs to determine which program branch to be executed, like Heapsortcypher in Figure~\ref{fig:app_example}. They typically define several lists of labels and program branches the application should execute when the ML APIs' output labels intersect with their associated pre-defined list. 

% To characterize the application's post-processing step of ML API outputs, we defined three types of abstraction: (1) the sets of labels that have equivalent effects on the control flow;  (2) whether the final output of the software is exclusively associated with only one program branch; and (3) whether errors made in some sets of labels can be disguised by correct predictions in other sets of labels.


% \cc{Do we want to mention mutually exclusive?}. 
% Specifying the values of the abstractions can uniquely identify how the applications are going to post-process the ML APIs' outputs. 

Guided by the empirical study, we propose \tool, an automated framework that adapts ML models behind the ML API to the software implementation while keeping the same API interface, so as to reduce software misbehaviors. Tackling automation challenge, it first perform static analysis on the Python source code to extract the abstractions from the software. \tool then re-constructed the loss function to reflect the different severity of mis-predictions on software correctness. Tackling efficiency challenge, \tool adopts fine-tuning approach to adapt the ML model behind ML API with minimum training costs.
\shan{I like this paragraph, but clearer than earlier paragraphs.}
% \cc{Can you map these solutions to challenges?} \yh{i put the second challenge in the evaluation part}
% \cc{The second half of sentence are evaluation} 



% We systematically measure the improvement in the rate of software mis-behaviors on 19 open-source applications that call multi-label image classification API.
We systematically evaluate \tool on 19 open-source applications that use multi-label image classification API to make control flow decision.
Our evaluation shows that the re-constructed loss function provides up to \todo{X\%} improvements in reduction of software mis-behaviors, whereas alternative approach only improves rate of software mis-behaviors by \todo{Y\%}. Our evaluation also shows that performing model adaptation with the re-constructed loss function can finish within \todo{Z} minutes.  \yh{Will update the numbers after I finish the evaluation section. }
% (1) labels that will trigger the same program behaviors; (2) whether the final software output is exclusively associated with only one program branch, for example, in the application example shown in Figure~\ref{fig:app_example}, the final output of the software is the message specified in one of the program branches; (3) whether different sets of labels triggering same program behaviors have different priority levels. 


==> backups/1-introduction.tex <==
\label{sec:intro}

\subsection{Motivation}

\begin{itemize}
    \item Nowadays, more and more software applications require the underlying software to understand what is present in the images with Deep Neural Networks (DNNs). As training such DNNs can be expensive, the software developers use off-the-shelf ML APIs to reduce their development effort~\cite{wan2021machine}. 
    % \item Machine Learning (ML) offers effective ML APIs to a wide range of cognition tasks. Many cloud providers offer ML APIs, supported by underlying Deep Neural Networks (DNNs), that perform well on generic tasks (\eg image classification). These ML APIs are utilized in a wide range of software applications for different specific tasks. However, the ML APIs are not adapted to achieve the application specific tasks, leading to many software misbehaviors.
    \item List an application such that why/how high class-wise accuracy does not lead to correct software behavior or vice versa and cite~\cite{wan2022automated} to illustrate that there are many such applications. 
    \ref{fig:app_example} is an example software that incorporates Google \code{label\_detection} API, which outputs all the existing labels in the input image. If we consider traditional class-wise F1 score of the application, the ML API can achieve 
    % \yh{List the number of applications on GitHub that employs ML APIs}
    \item Here we define the software achieving correct behaviors if the outputs of the ML APIs lead to the same software behavior as if the ground-truth is returned.  
    \item Explain why the accuracy of the software would be low: the service providers train the ML models aiming to maximize class-wise accuracy, while the software developers need to ensure correct software behavior given the ML API outputs.  
    % \begin{itemize}
    %     \item the service providers pre-train the ML models that support the ML APIs with large-scale datasets (\eg Open Images dataset), aiming at providing good class-wise accuracy. \cc{Do you want to emphasis that they have different optimization goals?}
    %     \item When software developers use the ML APIs in their software, they expect the ML APIs to output classes that lead to the correct software behavior (\ie same software behavior as what the ground-truth leads to) \cc{What's the different between point2 \& 3?} 
    %     \item The pre-trained ML models may make mistakes that lead to the wrong software behavior
    % \end{itemize}
    
     
    % \item Accordingly, there is a mismatch between how the developers measure the end-to-end accuracy of the software and the original accuracy of the ML APIs. Even though the ML APIs are supposed to have very high accuracy on the overall generic accuracy of the ML APIs, the overall accuracy of the software using the ML APIs may be lower than the accuracy of the original ML APIs. \yh{list example numbers. }
    \item An ideal case of utilizing the ML APIs is to adapt the ML APIs so that they are aware of the errors that are unacceptable by the software (\ie leading to wrong software control flow). 
    % \cc{Automation is mentioned in next bullect. In this bullet, you'd better talk about customization only.} 
    \item Automatically adapting the ML APIs to the software is important: (1) The developers who use the ML APIs are usually not experts in ML, thus may not know how to adapt the models (2) The developers do not have an affordable way to support model adaptation. 
    % \yh{mention why automation is important}
    % \yh{Emphasize that the problem is important}
    
    
    
    % \item However, when the developers use the ML APIs in their software, they are either unaware of the mismatch between ML APIs' accuracy and software's accuracy, or they do not have an affordable way to adapt the ML APIs to fit the software application they are writing.  \yh{Define affordable: 1. developers do not need to provide training data 2. they do not need to specify what are the context that can be digested by the DNNs to improve accuracy. }
    \item Automatically adapting the ML APIs to the software is challenging. 
    \begin{itemize}
        \item No existing benchmark has shown that there is a discrepancy between the outputs resulting in high class-wise accuracies and the ones leading to the correct software behaviors

        % (prior works either (1) only study ML APIs themselves (2) realize the low accuracy of ML APIs in the software~\cite{wan2021machine} (3) do not understand why the ML APIs do not work when applying to the software (SW only cares about branch prediction are correct) )
        % \item Need to transform cognition task into math expression 
        % create the template 
        \item Need to extract software specific cognitive task automatically and transform the extracted software context into mathematical expression that enables ML API adaptation
        \item Need to efficiently adapt the ML APIs 
       
    \end{itemize}
    
    \yh{why related works cannot handle }
    
    
    
    
    
    % \yh{To adapt the ML solutions to the software, software developers face many issues... (or accuracy decrease) or say adaptation is very important}
    % \yh{why do adaptation ? if not, will cause accuracy decrease. }
    
    % \yh{Developers did not realize this issue or they do not have an affordable way to adapt}
    
    % \yh{List an example}
    
    
    % \yh{Automatically adapt to the software is challenging. }
    
    
    % \item However, when the software developers incorporate the ML APIs in their software applications, they usually only care about specific context.  
    % \item To understand the specific context that the software developers usually focus on, consider the Smart Can application in Figure~\ref{fig:app_example}. Smart Can uses the Google \code{label\_detection} API to perform image classification on a user input photo. ... 
    % \item For the Smart Can application, the software developers only care about if the ML API is able to correctly recognize classes in the specified lists (\eg Plastic, Food etc.). 
    % \item Additionally, the end-to-end accuracy of the software does not equal to the accuracy of the ML API. 
    % \item These two fronts bring the opportunity to adapt the ML models to improve the accuracy of the software that incorporate the ML APIs. 
    % \item However, there are several open challenges in adapting the ML models to the software. 
    
%     1. How to define the context of the software?  \yh{What should be the context? what is the context that can be digested by the NN? }
% \begin{itemize}
%     \item The subset of classes specified in the software
% \end{itemize}
    
%     2. How to extract the context automatically? \yh{merge into the first one}
    
%     3. How to utilize the context? Re-train the underlying ML models
%     \begin{itemize}
%         \item Modify the training data distribution 
%         \item Modify the training loss
%         \item Modify the model architecture to directly predict the output of the software 
%     \end{itemize}
    
%     4. Affordable re-training (training time, training data)
    
   
\end{itemize}


\begin{figure}
   \centering
\begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
Recycle = ['plastic', 'wood', 'glass', 'paper', 'cardboard', 'metal', 'aluminum', 'tin', 'carton']
Compost = ['food', 'produce', 'snack']
Donate = ['clothing', 'jacket', 'shirt', 'pants', 'footwear', 'shoe']
image = types.Image(content=trash_image)
response = client.label_detection(image=image)
for obj in response.label_annotations:
  if obj.name in Recycle:
    return 'Recycle'
  if obj.name in Compost:
    return 'Compost'
  if obj.name in Donate:
    return 'Donate'
\end{lstlisting}
    \caption{heapsortcypher, a smart can application \cite{xxx} using Google Cloud API. \cc{TODO}}
    \label{fig:app_example}
\end{figure}

\subsection{Contributions} 
\begin{itemize}
%  \item We present \tool, which is an end-to-end system which automatically extracts software context from the applications that incorporate ML APIs, and adapt the ML models to improve the software accuracy. 
\item Studied a wide range of software applications that incorporate ML APIs, and identified that one of the common software context is mapping fine-grained ML API output classes to program branches. 
\item Defined a template to automatically transform the code that the software developers write into mathematical expression that can adapt the ML APIs to the software. 
% \item defined the template and the transformation to math expression 
\item Leveraged two ways of model adaptation with the defined software context that (1) changes the training data distribution to reflect the subset of classes that the users care about; (2) modifies training loss function to directly reflect the control flow of the software. 

% \item Compared the ways of model adaptation in terms of accuracy improvement and training cost on \todo{X} real applications using ML APIs.

% defined two types of software context that can improve the accuracy of the software: (1) Data distribution context; (2) Subset of classes context. 

% \item Developed a tool to automatically extract the defined context from the Python code written by software developers 


\end{itemize}

==> backups/2-2-empirical-1025.tex <==
\label{sec:empirical}

To understand how developers use ML API in real-world applications, we conduct an empirical study on ML software that invokes  ML APIs to make control flow decisions. \cc{I weakly remember that you plan to study Amazon APIs. Please revise it if I'm wrong}

% We observe that there are different ways for developers to specify how they plan to use the ML APIs' outputs to affect the control flow of ML software. 
% In order to understand the common patterns of the control flows of the ML software, we conduct an empirical study on ML software using Google's \code{label\_detection} API, which performs multi-label image classification.  
% From the case study, we summarize three types of abstractions for the code structures of the ML software. 



% \yh{ML API on OI or pretrained on OI}
\subsection{Methodology}

\subsubsection{Application selection}



% Google (benchmark, search), AWS (search)
We study 40 open-source ML software applications  whose control flows are affected by the output of a multi-label image classification API. These applications comes from two sources: (1) 19 applications come from a recently published, open-sourced benchmark suite for ML software~\cite{wan2021machine}; and (2) 21 applications comes from GitHub by random checking around 60 applications.
Among these applications, 29 of them use Google \code{label\_detection} API and 11 use Amazon \code{detect\_labels} API.

\yh{select applications using multi-label classification and object-detection APIs, because that's representative of the ML software }

% \cc{Maybe also add some statistics}


We do not study the applications that directly print out the ML APIs' outputs or store these outputs without post-processing. The tasks that these applications perform are the same as the task of ML API. Therefore, there is no need to adapt APIs to software. In addition, ML APIs are only loosely integrated into these applications, e.g., not interacting with other software components. We believe they do not represent the future direction of ML software.

\subsubsection{Test data selection}
TO-DO
\cc{It is weird to have a subsection that only has one subsubsection. How about we also introduce the open image data and ground-truth label?}




% We study the open-source applications from a recently published, open-sourced benchmark suite for ML software~\cite{wan2021machine}. We focus on applications whose control flows are affected by the ML APIs' outputs. We focus on 19 applications which invoke Google \code{label\_detection} API to make control flow decisions. These applications use the ML APIs' outputs to determine which program branch to be executed. For example, in the application example in Figure~\ref{fig:app_example}, the API output labels in Figure~\ref{fig:app_example2} will lead the software executing \code{return 'Recycle'} on line 8 because ``Glass'' is included in the \code{Recycle} list. We refer to the branch being executed, such as \code{return  `Recycle'}, when the if condition is satisfied, as \emph{if/then branch}. 
% To characterize the application's post-processing step of ML API outputs, we defined three types of abstraction: (1) the sets of labels that have equivalent effects on the control flow;  (2) whether the final output of the software is exclusively associated with only one program branch; and (3) whether errors made in some sets of labels can be disguised by correct predictions in other sets of labels.
% We do not study the applications that directly print out the ML APIs' outputs or store all the outputs in the databases, because these applications do not have mismatch between ML APIs' outputs and software's output thus do not have room for improvement. 




% \subsection{Common patterns of code structure of software utilizing ML APIs}
\subsection{Result summary}
Across all applications we studied, 48\% of them defines several whitelists and compares ML API output labels with them. 

Take Heapsortcypher (Figure~\ref{fig:app_example_entire}) as an example. It executes Line 8 when given a candy image, as the API output ``Glass'' is included in the \code{Recycle} list and thus fulfills the statement in Line 7. We refer to this executed branch as \emph{if/then branch}. Correspondingly, we refer to another branch that  not executes Line 8 as \emph{if/else branch}.
We refer to a list of labels (or classification category) leading to the same control flow decision as a \emph{whitelist}. \code{Recycle}, \code{Compost}, and \code{Donate} are the three whitelists, taking Heapsortcypher as an example.

% \cc{yuhan, please put terminologies (those used in Section 3) here. Make sure that you are only using the Heapsortcypher as an example}

While these applications typically uses whitelists to post-process ML API results, they vary in the way of using whitelists to make control flow decisions. Even with same whitelists and API inputs, the applications would behave differently according to its code structure. Next, we will introduce the common patterns observed in the studied applications.


% We find that these software typically pre-defines one or several lists of labels as branch conditions, and then maps the original output labels to the pre-defined lists which intersect with the labels. Then the software executes one or more \ifts that correspond to those mapped pre-defined lists. 
% In other words, all the labels specified in one list will lead to the same control flow decision. 

% We refer to the lists of labels leading to the same control flow decisions as \emph{whitelists} in the rest of the paper. For example, in the application example shown in Figure~\ref{fig:app_example}, the software defines three \emph{whitelists}, Recycle, Compost, and Donate. 



% They typically define several lists of labels and which one or more program branches the application should execute by comparing the API output labels and these lists. 
% They typically define several lists of labels and which one or more program branches the application should execute when the ML APIs' output labels intersect with their associated pre-defined list. 


\begin{figure}
    \centering
     \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}

\end{lstlisting}
    \caption{Software implementation. }
    \label{fig:app_example_non_mut}
\end{figure}


\subsection{Abstractions}
\label{sec:abstractions}
As summarized in Figure~\ref{fig:hierarchy} we define four types of abstractions to characterize the code structure. We will use several minimal templates to illustrate the four types of abstractions. 


\textbf{1) Number of whitelists.} The software specifies one \wl or multiple \wls. Particularly, as shown in Figure~\ref{fig:template1}, each whitelist is related to a particular software branch: the software will execute the corresponding \ift when the ML APIs' outputs intersect with the labels in the \wl. In the rest of the paper, we will refer to executing a branch as mapping API outputs to its corresponding whitelist.

\textbf{2) Type of mapping.} For the software specifying multiple \wls, there are two types of mapping from ML API outputs to whitelists: (i) the software executes all the \ifts when the API's outputs intersect with the \wls associated with the branch condition. In other words, the original output labels are mapped to several \wls; (ii) the software checks whitelists in a specific order, and only executes the lower-ranked \ifts when API outputs do not intersect with any higher-ranked whitelist, leading to at most one \ift to be executed. In other words, the original output labels are mapped to at most one \wl. 
% \cc{I changed it from multiple to several, so that it means 0 to N}

% For the software specifying multiple \wls, when the software checks if the output labels intersect with the \wls, there are two possible ways of checking: (i) the software executes all the \ifts when the API's outputs intersect with the \wls associated with the branch condition. In other words, the original output labels may be mapped to multiple \wls; (ii) the software checks the branch conditions in a specific order, and only executes the lower-ranked \ifts if the higher-ranked branch conditions are false, leading to at most one \ift to be executed. In other words, the original output labels are mapped to at most one \wl. 
% (i) the software executes at most one if/then branch when the API's outputs intersect with the \wl associated with the branch condition; (ii) the software executes all the if/then branches when the API's outputs intersect with the \wls associated with the branch condition. 
% For the software that specifies several \wls, some software will compare the ML APIs' outputs with the \wls, and break at a program branch once the outputs intersect with the \wl associated with the branch. In other words, the final output of the software is the message corresponding to with only one program branch. Other software compares the ML APIs' outputs with the \wls, and outputs all the messages 

\textbf{3)Type of output.} For the software which maps original output labels of the ML API to several \wls, it either construct the final output in a format of (i) set or (ii) list. In the latter, the final output is affected by the order of examination.
% For the software which maps original output labels of the ML API to several \wls, there are two possible ways for software to construct the final output:  (1) the software checks the output labels one by one, and add a \wl to a list if the output labels intersect with the \wl. Finally, the software outputs the list containing all the matched \wls. In this case, the order at which the \wls intersect with the output labels does matter; (2) the software checks the output labels one by one, and add a \wl to a set if the output labels intersect with the \wl. Finally, the software outputs the set containing all the matched \wls. In this case, the order at which the \wls intersect with the output labels does not matter.

\textbf{4) Order of examination.}  For the software specifying multiple \wls, the order of examining intersections between \wls and ML API outputs determines software behavior. If we reconstruct the examination into a two-level nested loop that iterates through \wls and API outputs, there naturally arises two types of loop structure: prioritize the specified \wls or the API output labels.
% For the software which executes at most one \ift, the order at which the software performs the checking on the branch conditions may either prioritize the specified \wls or the output labels. 
% As a result, for the software that prioritizes the order of the output labels, mis-classifications happened on the lower-ranked output labels do not matter, as long as the higher-ranked output labels can lead to the correct control flow decisions. Similarly, for the software that prioritizes \wls, mis-classifications happened on the lower-ranked \wl do not matter, as long as the . 

\begin{figure}
     \includegraphics[width=\linewidth]{figs/hierarchy.pdf}
    \caption{Common code patterns of ML software. The decision nodes (in blue) are abstractions defined in Section~\ref{sec:abstractions}. The leaf nodes (in green) are the type of code structures constructed with the sequence of decisions made at each decision node. }
\label{fig:hierarchy}
\end{figure}



\subsection{Common Code Patterns}
\label{sec:examples}
\yh{TODO: add connection to the abstractions} \cc{Also add how many applications belongs to each category}
Based on these four types of abstractions, Figure~\ref{fig:hierarchy} summarized all the possible code patterns in a structure of decision tree. Each decision nodes represent an abstraction. Each leaf node represents a code pattern constructed with the sequences of different decisions made at each decision node. While Figure~\ref{fig:hierarchy} illustrates six possibilities, our studied applications only contain four of them (green box in solid lines).

% Based on these four types of abstractions, we can characterize the common code structures as shown in Figure~\ref{fig:hierarchy}. Each decision node in the decision tree represents an abstraction as described in Section~\ref{sec:abstractions}. Each leaf node in the decision tree represents a type of code structure constructed with the sequences of different decisions made at each decision node. The leaf nodes are all the possible code structures constructed with the abstractions. However, we only found a subset of all the possible code structures in the benchmark suite. The existing types of code structures are shown in the leaf nodes with edges marked with solid lines, whereas the non-exisiting code structures are the leaf nodes with edges marked with dashed lines in Figure~\ref{fig:hierarchy}. We list four patterns of ML software. 
% software examples to illustrate the common patterns of how ML APIs' outputs affect ML software's control flow decisions. 

\subsubsection{Software pattern 1: T-or-F} This type of software only specifies one \wl which includes multiple labels, such that labels in the \wl have an equivalent effect on the software's control flow decisions. Around 35\% applications in our benchmark suite belongs to this category.

Figure~\ref{fig:app_example_level1} shows a carnivore identification application. It goes through all the predicted labels of an input photo, and executes the \ift \code{ return `It is an animal. '} if the predicted labels intersect with the pre-defined \wl Animal. In this example, mis-classifications within the pre-defined \wl Animal (\ie mis-classifying a dog image as ``Wolf'') do not lead to software misbehavior. Instead, the ML API only needs to guarantee that the input images that should lead the software executing the \ift corresponding to \wl Animal (\ie having ground-truth labels that intersect with the \wl Animal), are classified into at least one of labels specified in \wl  Animal. On the contrary, if an image contains a carnivore, while the API output do not include any label in the \wl (Figure~\ref{fig:input_example_tf_wrong}). 


To quantify the difference in the metrics of the ML API and the correctness of this software, the traditional F1 score of the ML API on the test dataset is 58\%, while only 43\% of the data correctly identified classes in the \code{Dog} \wl, leading to software behaviors as human expected. 


% percentage of data such that the software behaves as human expected is 43\%. 

% \cc{I found it awkward to say groud-truth label contains xxxx. Can we just say the image contains a carnivore?} 

% For example, in Figure~\ref{fig:app_example_level1}, the software goes through all the predicted labels of an input image, and executes the \ift \code{return `It is an animal. '} if the predicted labels intersect with the pre-defined \wl Animal. In this example, we can see that mis-classifications within the pre-defined \wl Animal do not matter, such as mis-classifying an input image with ground-truth label `Dog' to `Wolf'. Instead, the ML API only needs to guarantee that the input images that should lead the software executing the \ift corresponding to \wl Animal (\ie having ground-truth labels that intersect with the \wl Animal), are classified into at least one of labels specified in \wl  Animal. 

% For example, in Figure~\ref{fig:input_example_tf_wrong}, the ML API's output labels lead to incorrect control flow decision because the ground-truth of the input image include a label in the pre-defined \wl (\ie ``Carnivore''), while the output labels do not include any label in the \wl. 

\subsubsection{Software pattern 2: M-to-N-set} In our benchmark, 25\% software defines multiple \wls, and the \wls themselves are parallel to each other. In other words, all the \wls have equivalent priority and all the \wls that have an intersection with the output labels will be reflected in the final output of the software. In Figure~\ref{fig:app_example_non_mut}, the food classifier application invokes ML API to determine the existence of protein, fruit, and grain in a food image\cc{Yuhan, please make sure you introduce what this app is doing before talking about its code structure}. It iterates through the predicted labels of an input image, and executes all the \ifts whose corresponding branch conditions are satisfied. In this example, we can see that mis-classifications within any of the \wls could still lead to correct software behavior.

As shown in Figure~\ref{fig:input_example_mton_correct}, for an input image that includes pasta with meat,  mis-classifying ``Pasta'' to ``Noodle'' does not matter, because the ML API's outputs lead the software to correctly set \code{protein} and \code{grain} variables to \code{True}.
% \cc{Please directly say misclassify which label as which label. The same description already exists in the previous paragraph}. 
However, if an input image has ground-truth labels covering all of the \wls, the correct software behavior is setting \code{protein}, \code{fruit} and \code{grain} to \code{True}. Missing ``Bread'' in the output leads to wrong software behavior: only setting \code{protein} and \code{fruit} variables to \code{True}. 
% \cc{Same here, please describe the example. By looking at this paragraph, it could be applied to any example}.  
% \cc{yuhan, please make the format consistent. Some whitelist names are in code format, some are not}

We also quantitatively measure the difference in the metrics for the ML API and this ML Software's correctness after invoking the ML API. We see that the ML API's F1 score on the food classifier application is 73.88\%. However, only 54.72\% of the input images in which the ML API's output labels lead the software executing all the corresponding \ifts as human expected. 

\subsubsection{Software pattern 3: Priority-list} Around 10\% software defines multiple \wls, and checks the \wls one by one until finding the first one that intersects with output labels. For example, Aander-ETL (Figure~\ref{fig:priority_input_example}) specifies three \wls (\code{Monument, Construction, Person}) to classify tourist photos. It first checks if the output labels have an intersection with the \code{Monument} \wl, and executes the corresponding \ift if having an intersection. If the output labels do not intersect with \code{Monument}, the software compares the output labels with \code{Construction} and \code{Person} in a similar way. Under such software pattern, we can see that mis-classifications for labels inside any of the lower-ranked \wl will not lead to wrong control flow decisions if ML API correctly recognizes the existence of labels in the hig her-ranked \wls. 

In Figure~\ref{fig:input_example_priority_correct}, the software behaves correctly even when the API recognizes an extra incorrect label ``Mansion'' in the \wl \code{ Construction}, as API correctly recognize ``Ancient history'', which belongs to the highest-ranked \wl \code{ Monument}. However, in Figure~\ref{fig:input_example_priority_wrong},  only missing the label ``Landmark'' in the \wl \code{  Monument} can lead to completely incorrect software behavior: the software wrongly executes the \ift corresponding to the second-highest ranked \wl \code{ Construction} since it is the first \wl that intersects with the API's output labels.

We observe that the ML API's overall F1 score for the Anander-ETL software is 61\%, while only 54\% of API's output labels lead to the software executing the \ift corresponding to the highest-ranked \wl included in the input images. 

% for an input image with ground-truth labels that intersect with all the three \wls, the ML API's output labels lead to incorrect control flow decision because missing the label ``Landmark'' in the highest-ranked \wl makes the software executing the \ift corresponding to the second-highest ranked \wl. 


\subsubsection{Software pattern 4: Top-label} For APIs that produce multiple output labels, some software maps the output labels to control flow decisions in a specific order. Around 30\% applications fall in this category.
For example, Heapsortcypher (Figure~\ref{fig:app_example}) iterates through the API output labels that are ranked in descending order of their confidence scores and finds the first output label that intersects with any of the specified \wls. Then the software executes the corresponding \ift associated with the found \wl. Therefore, mis-classification for lower-ranked output labels will not lead to software misbehavior if the higher-ranked output intersects with \wls. 

As shown in Figure~\ref{fig:input_example_top_correct}, API correctly recognizes ``Produce'' for an image of apple on table, which intersects with \wl Compost. Therefore, even it wrongly outputs a lower-ranked label``Wood'' which belongs to another \wl, the software still makes a correct control flow decision. 






\begin{figure}
\begin{subfigure}{0.45\textwidth}    
    \centering
\begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
Dog = ['Dog','Mammal','Carnivore','Wolf']
image = types.Image(content=dog_image)
response = client.label_detection(image=image)
for obj in response.label_annotations:
  if obj.name in Dog:
    return 'It is a animal.'
return 'It belongs to others.'
\end{lstlisting}
    \caption{Code pattern: T-or-F. }
    \label{fig:app_example_level1}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/input_example_tf_wrong.pdf}
    \caption{Failing recognize the carnivore leads to software failure. }
    \label{fig:input_example_tf_wrong}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/app_input_example_level1.pdf}
    \caption{Mis-classifying a dog as wolf does not trigger software failure. }
    \label{fig:input_example_tf_correct}
\end{subfigure}
\caption{Dogecoin~\cite{food}, an application that classifies carnivore images.  }
\label{fig:tf_example}
\end{figure}



\begin{figure}
\begin{subfigure}{0.45\textwidth}    

    \centering
             \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
proteinfoods = ['Hamburger', 'Meat', 'Patty']
fruitfoods = ['Apple', 'Fruit', 'Orange']
grainfoods = ['Noodle', 'Pasta', 'Al dente']
image = types.Image(content=trash_image)
response = client.label_detection(image=image)
protein, fruit, grain = False, False, False
for obj in response.label_annotations:
  if obj.name in proteinfoods:
    protein = True
  if obj.name in fruitfoods:
    fruit = True
  if obj.name in grainfoods:
    grain = True
RENDER_TEMPLATE(protein, fruit, grain)
\end{lstlisting}
    \caption{Software implementation. }
    \label{fig:app_example_non_mut}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/input_example_mton_wrong.pdf}
    \caption{Failing to recognize ``Cheese'' leads to software mis-behavior. }
    \label{fig:input_example_mton_wrong}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/input_example_mton_correct.pdf}
    \caption{Mis-classifying ``Pasta'' to ``Noodle'' still leads to correct software behavior. }
    \label{fig:input_example_mton_correct}
\end{subfigure}
\caption{Food classifier~\cite{food}, an application that classifies food images.}
\end{figure}


\begin{figure}
    \centering
             \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
proteinfoods = ['Hamburger', 'Meat', 'Patty']
fruitfoods = ['Apple', 'Fruit', 'Orange']
grainfoods = ['Noodle', 'Pasta', 'Al dente']
image = types.Image(content=trash_image)
response = client.label_detection(image=image)
food_list = []
for obj in response.label_annotations:
  if obj.name in proteinfoods:
    food_list.append('protein')
  if obj.name in fruitfoods:
    food_list.append('fruit')
  if obj.name in grainfoods:
    food_list.append('grain')
return food_list
\end{lstlisting}
    \caption{An example software that maps original output labels of the ML APIs to a list of \wls.  }
    \label{fig:app_example_non_mut}
\end{figure}



\begin{figure}
\begin{subfigure}{0.45\textwidth}
        \centering
             \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
Monument = ['Landmark', 'Sculpture', 'Monument']
Construction = ['Building', 'Estate', 'Mansion']
Person = ['Human','Person',  'Lady']
image = types.Image(content=landmark_image)
response = client.label_detection(image=image)
Predictions = []
for obj in response.label_annotations:
  Predictions.append(obj.name)
if any([label in Monument for label in Predictions]):
  return 'It belongs to monument.'
elif any([label in Construction for label in Predictions]):
  return 'It is construction.'
elif any([label in Person for label in Predictions]):
  return 'It is person.'
\end{lstlisting}
    \caption{Software implementation. }
    \label{fig:app_example_priority}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/input_example_priority_wrong.pdf}
    \caption{Missing a label ``Landmark'' leads to software mis-behavior. }
    \label{fig:input_example_priority_wrong}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/input_example_priority_correct.pdf}
    \caption{Recognizing an extra wrong label ``Mansion'' still leads to correct software behavior. }
\label{fig:input_example_priority_correct}
\end{subfigure}
\caption{Aander-ETL~\cite{etl}, an application that classifies landmark images.  }
\label{fig:priority_input_example}
\end{figure}

\cc{Do we want to introduce the accuracy difference between API and software? And the room for improvement?}

==> backups/2-2-empirical-1110.tex <==
\label{sec:empirical}

To understand how developers use ML API in real-world applications\shan{As I commented in Introduction, this opening sentence has to be more precise. It is tooooo generic now.}, we conduct an empirical study on ML software that invokes  ML APIs to make control flow decisions. 

\shan{The overall feeling of this section is lack of motivation. As a reader, I keep asking myself: why do I care how many applications use whitelists? Why do I care how many types of abstraction you use to characterize code structure? Or, why do I care about the whatever code structure? It is not clear to me, as a reader, why any of these have ANYTHING to do with software correctness, with how to customize ML APIs for software. This is related to my comments of your over-general opening sentences. Please keep in mind that readers do NOT necessarily want to ``understand how developers use ML API''. In other words, there are many more readers who want to understand how to customize an ML API to improve software correctness than readers who want to know how many whitelists a software defines. As a reader and an (impatient) reviewer, I skip paragraphs and sections that do not motivate me.}

% \yh{ML API on OI or pretrained on OI}
\subsection{Methodology}

\subsubsection{Application selection}



% Google (benchmark, search), AWS (search)
We study 40 open-source ML software applications  whose control flows are affected by the output of \emph{a multi-label image classification API}. 

We do not study the applications that directly print out the ML APIs' outputs or store these outputs without post-processing. The tasks that these applications perform are the same as the task of ML API. Therefore, there is no need to adapt APIs to software. In addition, ML APIs are only loosely integrated into these applications, e.g., not interacting with other software components. We believe they do not represent the future direction of ML software.

The 40 applications come from two sources: (1) 19 applications, which post-process the ML APIs' outputs to make control flow decisions, come from a recently published, open-sourced benchmark suite for ML software~\cite{wan2021machine}\shan{Why do you pick these 19?}; and (2) 21 applications come from GitHub by random checking around 60 applications\shan{What exactly are you looking for when you randomly check? Why don't you use all these 60?}.
Among these applications, 29 use Google \code{label\_detection} API, and 11 use Amazon \code{detect\_labels} API.

% \cc{Maybe also add some statistics}



\subsubsection{Test data selection}
TO-DO
\cc{It is weird to have a subsection that only has one subsubsection. How about we also introduce the open image data and ground-truth label?}







% \subsection{Common patterns of code structure of software utilizing ML APIs}
\subsection{Result summary}
The 40 applications whose control flow decisions are affected by the ML APIs' outputs pre-define several \wls, and compare ML APIs' outputs with them to decide which if-branch edge to execute, which we refer to as making application decision. 


\shan{Without knowing your application selection criteria, I cannot interpret what this ``48\%'' implies. What does the remaining 52\% applications do? If all applications in your bencharmk suite use ML API output to affect control flow, how can there be no whitelist? Can you offer more explanation here about what exactly this 48\% mean?} \yh{Sorry 48\% was an out-dated number. All the 40 apps whose control flow are affected by the ML APIs' outputs do specify whitelists. }

Take Heapsortcypher (Figure~\ref{fig:app_example}) as an example. It executes Line 8 when given a garbage image, as the API output ``Glass'' is included in the \code{Recycle} list and thus fulfills the statement in Line 7. 
% We refer to this executed branch as \emph{if/then branch}. Correspondingly, we refer to another branch that  not executes Line 8 as \emph{if/else branch}\shan{what if there is if-elsif-then?}.
We refer to a list of classes (or classification category) defined in the code\shan{what labels? you mean outputs of an ML API?} leading to the same control flow decision as a \emph{whitelist}. \code{Recycle}, \code{Compost}, and \code{Donate} are the three whitelists, taking Heapsortcypher as an example\shan{This definition has a lot of flaws.
One quick question: based on your definition, aren't all labels minus those in Recycle, Compost, and Donate also a white list? Are they?
}.

% \cc{yuhan, please put terminologies (those used in Section 3) here. Make sure that you are only using the Heapsortcypher as an example}

While these applications typically use \wls to post-process ML API results, they vary in the way of using whitelists to make application decisions. Even with the same whitelists and API outputs, the applications would behave differently according to their code structure. Next, we will introduce the common patterns observed in the studied applications.


% We find that these software typically pre-defines one or several lists of labels as branch conditions, and then maps the original output labels to the pre-defined lists which intersect with the labels. Then the software executes one or more \ifts that correspond to those mapped pre-defined lists. 
% In other words, all the labels specified in one list will lead to the same control flow decision. 

% We refer to the lists of labels leading to the same control flow decisions as \emph{whitelists} in the rest of the paper. For example, in the application example shown in Figure~\ref{fig:app_example}, the software defines three \emph{whitelists}, Recycle, Compost, and Donate. 



% They typically define several lists of labels and which one or more program branches the application should execute by comparing the API output labels and these lists. 
% They typically define several lists of labels and which one or more program branches the application should execute when the ML APIs' output labels intersect with their associated pre-defined list. 


% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% ML_API_outputs = [X]
% if X == C1: 
%     return "B1"
% elif X == C2: 
%     return "B2"
% elif X == C3: 
%     return "B3"
% elif X == C4: 
%     return "B4"
% \end{lstlisting}
%     \caption{Minimal example showing an application without any post-processing on the ML API's output labels.  }
%     \label{fig:template_0}
% \end{figure}

% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% ML_API_outputs = [X]
% A = [C1, C2]
% if X in A: 
%     return "X"
% else:
%     return "Y"
% \end{lstlisting}
%     \caption{Minimal example showing an application that defines a single \wl.}
%     \label{fig:template_1}
% \end{figure}


% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% ML_API_outputs = [X1, X2]
% A = [c1, c2]
% B = [c3, c4]
% count = 1
% for W in [A, B]:
%     for x in [x1, x2, ...]:



% for x in [x1, x2, ...]:
%     for W in [A, B]:


% for W in [A, B]:
%     if x1 in W or x2 in W:
%         return "branch " + str(count)
%     if X2 in W:
%         return "branch " + str(count)
%     count += 1
% return "branch 3"
% \end{lstlisting}
%     \caption{Minimal example showing an application that defines a single \wl.}
%     \label{fig:template_2}
% \end{figure}

% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% ML_API_outputs = [X1, X2]
% A = [C1, C2]
% B = [C3, C4]
% for X in [X1, X2]:
%     if X in A:
%         return "branch 1"
%     if X in B:
%         return "branch 2"
% return "branch 3"
% \end{lstlisting}
%     \caption{Minimal example showing an application that defines a single \wl.}
%     \label{fig:template_3}
% \end{figure}




% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% ML_API_outputs = [X1, X2]
% W1 = [C1, C2]
% W2 = [C3]
% output = set()
% for X in ML_API_outputs:
%     if X in W1:
%         output.add("B1")
%     elif X in W2:
%         output.add("B2")
% return output 
% \end{lstlisting}
%     \caption{Minimal example showing an application that defines a single \wl.}
%     \label{fig:template_4}
% \end{figure}


\subsection{Abstractions}
\label{sec:abstractions}
As summarized in Figure~\ref{fig:hierarchy} we define four types of abstractions to characterize the code structure. 

% We denote the whole set of classes that the DNN behind the ML API is able to classify as $C=\{C_1, C_2, C_3, C_4, C_5, C_6\}$, and the labels that the input images contain as $G$. To start with, Figure~\ref{fig:template_0} shows a minimal example application without any post-processing of the ML APIs' output labels (\eg directly prints out the output labels). The application simply returns the direct output of the ML API. In other words, any one of the ML API's output classes will lead to the software executing its corresponding \ift. In the following section, we will use several minimal templates to illustrate four types of abstractions. 


% Applications may specify a \wl candidate, such that when the API's output labels intersect with the \wl, then the corresponding \ift will be executed, \code{return "B1"} in Figure~\ref{fig:template_1}. In the rest of the paper, we will refer to executing a \ift as mapping the API outputs to its corresponding \wl. In this case, mis-classifications inside the \wl do not matter, as long as the ML API output labels intersect with the \wl for images containing labels in \wl. 

% Applications may specify multiple \wls candidates, and check these whitelists one by one to find the first one that intersects with API result as shown in Figure~\ref{fig:template_2}. In this case, mis-classifications for lower-ranked \wls do not matter, as long as the output labels in higher-ranked whitelists lead to the correct control flow decision. 


\textbf{1) How many \wl candidates does the software define? } The software may specify one or several \wls candidates. Each \wl candidate is related to a particular software branch: the software will execute the corresponding \ift when the ML APIs' outputs intersect with the labels in the \wls candidates. In the rest of the paper, we will refer to executing the \ift as selecting its associated \wl.

\textbf{2) How are the \wls selected? } For the software specifying several \wls, there are three ways such that the \wls are selected: (1) the software checks the \wls in a specific order, and selects at most one \wl when the API outputs intersect with the \wl; (2) the software selects a set of \wls which intersect with API outputs; (3) the software selects an ordered list of \wls which intersect with API outputs. In this case, the order in which the API outputs appear and intersect with the \wls matters. 
 
% (i) the software executes all the \ifts when the API's outputs intersect with the \wls associated with the branch condition. In other words, the original output labels are mapped to several \wls; (ii) the software checks whitelists in a specific order, and only executes the lower-ranked \ifts when API outputs do not intersect with any higher-ranked whitelist, leading to at most one \ift to be executed. In other words, the original output labels are mapped to at most one \wl. 
% \cc{I changed it from multiple to several, so that it means 0 to N}

% For the software specifying multiple \wls, when the software checks if the output labels intersect with the \wls, there are two possible ways of checking: (i) the software executes all the \ifts when the API's outputs intersect with the \wls associated with the branch condition. In other words, the original output labels may be mapped to multiple \wls; (ii) the software checks the branch conditions in a specific order, and only executes the lower-ranked \ifts if the higher-ranked branch conditions are false, leading to at most one \ift to be executed. In other words, the original output labels are mapped to at most one \wl. 
% (i) the software executes at most one if/then branch when the API's outputs intersect with the \wl associated with the branch condition; (ii) the software executes all the if/then branches when the API's outputs intersect with the \wls associated with the branch condition. 
% For the software that specifies several \wls, some software will compare the ML APIs' outputs with the \wls, and break at a program branch once the outputs intersect with the \wl associated with the branch. In other words, the final output of the software is the message corresponding to with only one program branch. Other software compares the ML APIs' outputs with the \wls, and outputs all the messages 


\textbf{3) How is the order determined?}  For the software specifying multiple \wls, the order of examining intersections between \wls and ML API outputs determines software behavior. If we reconstruct the examination into a two-level nested loop that iterates through \wls and API outputs, there naturally arises two types of loop structure: prioritize the specified \wls or the API output labels.




\begin{figure}
     \includegraphics[width=\linewidth]{figs/hierarchy.pdf}
    \caption{Abstractions that characterize the code structure. The decision nodes (in blue) are abstractions defined in Section~\ref{sec:abstractions}. The leaf nodes (in green) are the type of code structures constructed with the sequence of decisions made at each decision node. }
\label{fig:hierarchy}
\end{figure}




\begin{figure*}
     \includegraphics[width=\linewidth]{figs/code.pdf}
    \caption{Examples of software such that the ML APIs' outputs affect the control flow decisions. }
\label{fig:code}
\end{figure*}



\subsection{Common Code Patterns}
\label{sec:examples}
\yh{Currently re-writing this section}
Based on these four types of abstractions, Figure~\ref{fig:hierarchy} summarized all the possible code patterns in a structure of a decision tree. Each decision nodes represent an abstraction. Each leaf node represents a code pattern constructed with the sequences of different decisions made at each decision node. While Figure~\ref{fig:hierarchy} illustrates six possibilities, our studied applications only contain four of them (green box in solid lines).

% Based on these four types of abstractions, we can characterize the common code structures as shown in Figure~\ref{fig:hierarchy}. Each decision node in the decision tree represents an abstraction as described in Section~\ref{sec:abstractions}. Each leaf node in the decision tree represents a type of code structure constructed with the sequences of different decisions made at each decision node. The leaf nodes are all the possible code structures constructed with the abstractions. However, we only found a subset of all the possible code structures in the benchmark suite. The existing types of code structures are shown in the leaf nodes with edges marked with solid lines, whereas the non-exisiting code structures are the leaf nodes with edges marked with dashed lines in Figure~\ref{fig:hierarchy}. We list four patterns of ML software. 
% software examples to illustrate the common patterns of how ML APIs' outputs affect ML software's control flow decisions. 

\subsubsection{Software pattern 1: T-or-F} This type of software only specifies one \wl which includes multiple labels, such that labels in the \wl have an equivalent effect on the software's control flow decisions. Around 35\% of applications in our benchmark suite belong to this category.

As shown in Figure~\ref{fig:code}(a), the application defines a \wl \code{A = [c1, c2]}, and goes through the outputs of the ML API. It  executes the if-branch edge \code{return "branch 1"} when it finds an output class belonging to \code{A}. We refer to executing the if-branch edge as selecting the \wl \code{ A} in the rest of the paper.  If none of the output classes belongs to \code{A}, the application executes the code \code{return "branch 2"}. We refer to executing the code when the ML API's outputs do not match any of the \wls as selecting \code{others}. 

In this application pattern, mis-classifications within the pre-defined \wl do not matter, as long as samples with ground-truth 
% shows a carnivore identification application. It goes through all the predicted labels of an input photo, and executes the \ift \code{ return `It is an animal. '} if the predicted labels intersect with the pre-defined \wl Animal. In this example, mis-classifications within the pre-defined \wl Animal (\ie mis-classifying a dog image as ``Wolf'') do not lead to software misbehavior. Instead, the ML API only needs to guarantee that the input images that should lead the software executing the \ift corresponding to \wl Animal (\ie having ground-truth labels that intersect with the \wl Animal), are classified into at least one of labels specified in \wl  Animal. On the contrary, if an image contains a carnivore, while the API output do not include any label in the \wl (Figure~\ref{fig:input_example_tf_wrong}). 


% To quantify the difference in the metrics of the ML API and the correctness of this software, the traditional F1 score of the ML API on the test dataset is 58\%, while only 43\% of the data correctly identified classes in the \code{Dog} \wl, leading to software behaviors as human expected. 


% percentage of data such that the software behaves as human expected is 43\%. 

% \cc{I found it awkward to say groud-truth label contains xxxx. Can we just say the image contains a carnivore?} 

% For example, in Figure~\ref{fig:app_example_level1}, the software goes through all the predicted labels of an input image, and executes the \ift \code{return `It is an animal. '} if the predicted labels intersect with the pre-defined \wl Animal. In this example, we can see that mis-classifications within the pre-defined \wl Animal do not matter, such as mis-classifying an input image with ground-truth label `Dog' to `Wolf'. Instead, the ML API only needs to guarantee that the input images that should lead the software executing the \ift corresponding to \wl Animal (\ie having ground-truth labels that intersect with the \wl Animal), are classified into at least one of labels specified in \wl  Animal. 

% For example, in Figure~\ref{fig:input_example_tf_wrong}, the ML API's output labels lead to incorrect control flow decision because the ground-truth of the input image include a label in the pre-defined \wl (\ie ``Carnivore''), while the output labels do not include any label in the \wl. 

\subsubsection{Software pattern 2: M-to-N-set} In our benchmark, 25\% software defines multiple \wls, and the \wls themselves are parallel to each other. In other words, all the \wls have equivalent priority and all the \wls that have an intersection with the output labels will be reflected in the final output of the software. In Figure~\ref{fig:app_example_non_mut}, the food classifier application invokes ML API to determine the existence of protein, fruit, and grain in a food image\cc{Yuhan, please make sure you introduce what this app is doing before talking about its code structure}. It iterates through the predicted labels of an input image, and executes all the \ifts whose corresponding branch conditions are satisfied. In this example, we can see that mis-classifications within any of the \wls could still lead to correct software behavior.

As shown in Figure~\ref{fig:input_example_mton_correct}, for an input image that includes pasta with meat,  mis-classifying ``Pasta'' to ``Noodle'' does not matter, because the ML API's outputs lead the software to correctly set \code{protein} and \code{grain} variables to \code{True}.
% \cc{Please directly say misclassify which label as which label. The same description already exists in the previous paragraph}. 
However, if an input image has ground-truth labels covering all of the \wls, the correct software behavior is setting \code{protein}, \code{fruit} and \code{grain} to \code{True}. Missing ``Bread'' in the output leads to wrong software behavior: only setting \code{protein} and \code{fruit} variables to \code{True}. 
\shan{This example's discussion is confusing. The phenomenon of mis-classifying pasta to noodle does not matter is not unique to this pattern; it applies to the first T-of-F pattern as well. I also don't understand why you emphasize 
``if an input ... has ground-truth labels covering all ...''. Even if the ground truth labels do not cover all but
instead only cover fruit and grain, wouldn't missing bread still a problem? None of your discussion here sounds 
unique to this pattern to me.}
% \cc{Same here, please describe the example. By looking at this paragraph, it could be applied to any example}.  
% \cc{yuhan, please make the format consistent. Some whitelist names are in code format, some are not}

% We also quantitatively measure the difference in the metrics for the ML API and this ML Software's correctness after invoking the ML API. We see that the ML API's F1 score on the food classifier application is 73.88\%. However, only 54.72\% of the input images in which the ML API's output labels lead the software executing all the corresponding \ifts as human expected. 

\subsubsection{Software pattern 3: Priority-list} Around 10\% software defines multiple \wls, and checks the \wls one by one until finding the first one that intersects with output labels. 



% For example, Aander-ETL (Figure~\ref{fig:priority_input_example}) specifies three \wls (\code{Monument, Construction, Person}) to classify tourist photos. It first checks if the output labels have an intersection with the \code{Monument} \wl, and executes the corresponding \ift if having an intersection. If the output labels do not intersect with \code{Monument}, the software compares the output labels with \code{Construction} and \code{Person} in a similar way. Under such software pattern, we can see that mis-classifications for labels inside any of the lower-ranked \wl will not lead to wrong control flow decisions if ML API correctly recognizes the existence of labels in the higher-ranked \wls. 

% In Figure~\ref{fig:input_example_priority_correct}, the software behaves correctly even when the API recognizes an extra incorrect label ``Mansion'' in the \wl \code{ Construction}, as API correctly recognize ``Ancient history'', which belongs to the highest-ranked \wl \code{ Monument}. However, in Figure~\ref{fig:input_example_priority_wrong},  only missing the label ``Landmark'' in the \wl \code{  Monument} can lead to completely incorrect software behavior: the software wrongly executes the \ift corresponding to the second-highest ranked \wl \code{ Construction} since it is the first \wl that intersects with the API's output labels.

% We observe that the ML API's overall F1 score for the Anander-ETL software is 61\%, while only 54\% of API's output labels lead to the software executing the \ift corresponding to the highest-ranked \wl included in the input images. 

% for an input image with ground-truth labels that intersect with all the three \wls, the ML API's output labels lead to incorrect control flow decision because missing the label ``Landmark'' in the highest-ranked \wl makes the software executing the \ift corresponding to the second-highest ranked \wl. 


\subsubsection{Software pattern 4: Top-label} For APIs that produce multiple output labels, some software maps the output labels to control flow decisions in a specific order\shan{???In pattern 3, software maps ... ``in a specific order'' as well.}. Around 30\% applications fall in this category.
For example, Heapsortcypher (Figure~\ref{fig:app_example}) iterates through the API output labels that are ranked in descending order of their confidence scores and finds the first output label that intersects with any of the specified \wls. Then the software executes the corresponding \ift associated with the found \wl. Therefore, mis-classification for lower-ranked output labels will not lead to software misbehavior if the higher-ranked output intersects with \wls. 

As shown in Figure~\ref{fig:input_example_top_correct}, API correctly recognizes ``Produce'' for an image of apple on table, which intersects with \wl Compost. Therefore, even it wrongly outputs a lower-ranked label``Wood'' which belongs to another \wl, the software still makes a correct control flow decision. 

\shan{What is the F1 score drop for this category?}






% \begin{figure}
% \begin{subfigure}{0.45\textwidth}    
%     \centering
% \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% Dog = ['Dog','Mammal','Carnivore','Wolf']
% image = types.Image(content=dog_image)
% response = client.label_detection(image=image)
% for obj in response.label_annotations:
%   if obj.name in Dog:
%     return 'It is a animal.'
% return 'It belongs to others.'
% \end{lstlisting}
%     \caption{Code pattern: T-or-F. }
%     \label{fig:app_example_level1}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/input_example_tf_wrong.pdf}
%     \caption{Failing recognize the carnivore leads to software failure. }
%     \label{fig:input_example_tf_wrong}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/app_input_example_level1.pdf}
%     \caption{Mis-classifying a dog as wolf does not trigger software failure. }
%     \label{fig:input_example_tf_correct}
% \end{subfigure}
% \caption{Dogecoin~\cite{food}, an application that classifies carnivore images.  }
% \label{fig:tf_example}
% \end{figure}



% \begin{figure}
% \begin{subfigure}{0.45\textwidth}    

%     \centering
%              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% proteinfoods = ['Hamburger', 'Meat', 'Patty']
% fruitfoods = ['Apple', 'Fruit', 'Orange']
% grainfoods = ['Noodle', 'Pasta', 'Al dente']
% image = types.Image(content=trash_image)
% response = client.label_detection(image=image)
% protein, fruit, grain = False, False, False
% for obj in response.label_annotations:
%   if obj.name in proteinfoods:
%     protein = True
%   if obj.name in fruitfoods:
%     fruit = True
%   if obj.name in grainfoods:
%     grain = True
% RENDER_TEMPLATE(protein, fruit, grain)
% \end{lstlisting}
%     \caption{Software implementation. }
%     \label{fig:app_example_non_mut}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/input_example_mton_wrong.pdf}
%     \caption{Failing to recognize ``Cheese'' leads to software mis-behavior. }
%     \label{fig:input_example_mton_wrong}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/input_example_mton_correct.pdf}
%     \caption{Mis-classifying ``Pasta'' to ``Noodle'' still leads to correct software behavior. }
%     \label{fig:input_example_mton_correct}
% \end{subfigure}
% \caption{Food classifier~\cite{food}, an application that classifies food images.}
% \end{figure}


% \begin{figure}
%     \centering
%              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% proteinfoods = ['Hamburger', 'Meat', 'Patty']
% fruitfoods = ['Apple', 'Fruit', 'Orange']
% grainfoods = ['Noodle', 'Pasta', 'Al dente']
% image = types.Image(content=trash_image)
% response = client.label_detection(image=image)
% food_list = []
% for obj in response.label_annotations:
%   if obj.name in proteinfoods:
%     food_list.append('protein')
%   if obj.name in fruitfoods:
%     food_list.append('fruit')
%   if obj.name in grainfoods:
%     food_list.append('grain')
% return food_list
% \end{lstlisting}
%     \caption{An example software that maps original output labels of the ML APIs to a list of \wls.  }
%     \label{fig:app_example_non_mut}
% \end{figure}



% \begin{figure}
% \begin{subfigure}{0.45\textwidth}
%         \centering
%              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% Monument = ['Landmark', 'Sculpture', 'Monument']
% Construction = ['Building', 'Estate', 'Mansion']
% Person = ['Human','Person',  'Lady']
% image = types.Image(content=landmark_image)
% response = client.label_detection(image=image)
% Predictions = []
% for obj in response.label_annotations:
%   Predictions.append(obj.name)
% if any([label in Monument for label in Predictions]):
%   return 'It belongs to monument.'
% elif any([label in Construction for label in Predictions]):
%   return 'It is construction.'
% elif any([label in Person for label in Predictions]):
%   return 'It is person.'
% \end{lstlisting}
%     \caption{Software implementation. }
%     \label{fig:app_example_priority}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/input_example_priority_wrong.pdf}
%     \caption{Missing a label ``Landmark'' leads to software mis-behavior. }
%     \label{fig:input_example_priority_wrong}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/input_example_priority_correct.pdf}
%     \caption{Recognizing an extra wrong label ``Mansion'' still leads to correct software behavior. }
% \label{fig:input_example_priority_correct}
% \end{subfigure}
% \caption{Aander-ETL~\cite{etl}, an application that classifies landmark images.  }
% \label{fig:priority_input_example}
% \end{figure}

% \cc{Do we want to introduce the accuracy difference between API and software? And the room for improvement?}

==> backups/2-2-empirical-1117.tex <==
\label{sec:empirical}

This section introduces how ML API influences the behavior of MLaaS applications and then motivates:  
(1) the need to customize the ML API backend for each application, and 
(2) common patterns in which ML API output affects an application's decision process.
\subsection{Definitions}

% In addition, ML APIs are only loosely integrated into these applications, e.g., not interacting with other software components. We believe they do not represent the future direction of ML software.

% The 40 applications come from two sources: (1) 19 applications, which post-process the ML APIs' outputs to make control flow decisions, come from a recently published, open-sourced benchmark suite for ML software~\cite{wan2021machine}\shan{Why do you pick these 19?}; and (2) 21 applications come from GitHub by random checking around 60 applications\shan{What exactly are you looking for when you randomly check? Why don't you use all these 60?}.
% Among these applications, 29 use Google \code{label\_detection} API, and 11 use Amazon \code{detect\_labels} API.

% \cc{Maybe also add some statistics}



% \subsubsection{Test data selection}
% TO-DO
% \cc{It is weird to have a subsection that only has one subsubsection. How about we also introduce the open image data and ground-truth label?}


\begin{figure}
     \includegraphics[width=.95\linewidth]{figs/motivate_2examples.pdf}
    \caption{Code snippets from two example applications. Branch conditions influenced by API output and the structures over the conditional branches are highlighted.}
\label{fig:2examples}
\end{figure}

\mypara{Preliminaries} We begin with basic definitions.
% We first define the terminologies used in our paper.



% \begin{itemize}
%     \item \emph{Application decision}: the control flow decision of  which ML-API-related branch edge to execute
%     \item \emph{Conditional branches}: the lists of classes the application pre-defines in their source code, such that classes in these lists will lead to the same application decision. \yh{needs polish}
%     \item Selecting a whitelist $A$: the process of executing the branch edge corresponding to whitelist A
%     \item Selecting \code{others}: the process of executing the branch edge for not selecting any \wls
%     \item \emph{Ground-truth decision}: the application decision led by the human-labeled ground-truth of the input
% \end{itemize}


\begin{packeditemize}
    \item {\em ML API output:} the output of the MLaaS in response to the invocation of a single input, \eg a list of classes describing the content of an input image or the scores indicating the sentiment of the input text.
    % \item \emph{Conditional branches}: the branch conditioned on the API outputs 
    \item \emph{Branch conditions:} once the application receives the API output, it uses the branch conditions to decide which branch or branches to execute based on the API outputs.
    % \item \emph{Target-edge:} the branch edge that is executed when the API outputs fulfill a branch condition.%predicate of containing certain values. It typically is the edge following \code{then} statement.
    % \item \emph{A-edge}: for applications that compare API outputs with arrays of classes (\eg \code{A, B, C}), we refer to the Target-edge that is executed when the branch condition using array \code{A} is fulfilled as \emph{A-edge}.
    % \item \emph{Otherwise-edge}: the edge that is executed when none of the Target-edge is executed. 
    % \item \emph{Fall-through edge}: The non-target edge of a branch.
    % \item \emph{Path}: A feasible combination of edges of all conditional branches.
    % \item \emph{Target-path}: A path that contains at least one target edge.
    
    % % \item \emph{Whitelist}: A whitelist is a set of all ML API outputs that lead software to execute its corresponding whitelist-path.
    % \item \emph{Otherwise-path}: A path without any target edge. \cc{Please feel free to remove any concepts that are needed}
    \item \emph{Application decision}: given particular ML API output, the branch or branches whose branch conditions are satisfied.\footnote{Here, it is implicitly assumed that the application decision is affected only by the ML API output on the current input, not previous API output. While this may not be universally true, it holds for all the real-world applications that we have studied.}
    % the decision of which \emph{Target-edge} or \emph{Otherwise-edge} to execute. 
    % \item Selecting a whitelist $A$: the process of executing the branch edge corresponding to whitelist A
    \item \emph{Ground-truth decision}: the application decision if the API output is  human-labeled ground-truth of the input. 
    % \item \emph{Critical errors}: the errors that lead the application to execute edges different from the ground-truth decisions.
\end{packeditemize}


\mypara{Software decision process}
Given these definitions, an application's {\em software decision process} is the logic that maps an ML API output to an application decision. 
The code snippet in Figure~\ref{fig:input_example} shows an example software decision process, which maps the output of a classification ML API on an image to the image's recycling categorization specific to this application.

\mypara{Critical and non-critical errors}
Importantly, each software decision process decides when different ML API outputs lead to the same ground-truth decision (defined above), \ie {\em non-critical} error of ML API output {\em vs.} when different ML API outputs lead to decisions different from the ground-truth decision, \ie {\em critical} error of ML API output.

As we will see, the key is that {\em not} all errors are critical and that the critical errors {\em vary} across applications (using the same ML API) due to their different application decision processes.
%Thus, each application's decision process, if used carefully, could be leveraged to improve ML API output to reduce wrong application decisions. 
In the remainder of the section, we first present a systematic taxonomy of application decision processes and then apply the taxonomy to analyze a range of real-world applications using commercial MLaaS ML APIs.
%However, to unleash such potential in practice, we first need a deep understanding on the software contexts of various applications using real MLaaS {\em in the wild}.
In this empirical analysis, we focus on two central questions:
\begin{packeditemize}
\item Among applications using the same ML API, how much they differ in their application decision processes, and 
\item Despite the application heterogeneity, whether common patterns emerge which might allow extraction of information regarding an application's decision process.
\end{packeditemize}



\begin{figure}
     \includegraphics[width=\linewidth]{figs/hierarchy.pdf}
    \caption{Key dimensions that differentiate the code structures. The decision nodes (in blue) are key dimensions. The leaf nodes (in green) are the type of code structures constructed with the sequence of decisions made at each decision node. }
\label{fig:hierarchy}
\end{figure}



%\subsection{\hspace{-0.2cm} How ML API affects conditional branches}
\subsection{How is an application decision process affected by ML API?}
%\subsection{Taxonomy on how ML APIs affect application decision process}

\jc{text in this section can be tightened..}

%For each of these applications in our study, its software context is determined along two dimensions
% An application decision process can be characterized in two dimensions:
Two application decision processes may differ along one (or both) of the following dimensions:
{\em (i)} how each branch condition uses ML API output, and
{\em (ii)} how the conditional branches are structured.


\yh{be more precise about the titles, ask questions, define it and measure it }

\mypara{Two types of API output-based branch conditions}
% We identify two types of conditional branches
Figure~\ref{fig:2examples} shows an illustrative example for each.
%\item{\em Class lists:} 
The first type is used when the API output is a label or a list of labels, and several pre-defined {\em class lists} are then used to check if the API output labels belong to which list.
The code snippet of \code{Heapsortcypher}~\cite{heapsort} in Figure~\ref{fig:2examples}(a), for example, calls MLaaS with an image and receives class labels as ML API output.
It then checks if the API output belongs to three lists of classes, \code{Recycle}, \code{Compost}, \code{Donate} as the branch conditions to decide which branch to execute.
For an input with ground-truth class \code{``Shirt''}, the ground-truth decision is to execute the \code{Donate} branch.
If the ML API output is \code{``Paper''}, it will be a critical error, because the application decision (the \code{Recycle} branch) deviates from the ground-truth decision, whereas, if the ML API output is \code{``Jacket''}, it is not a critical error since the application's decision remains the same as the ground-truth decision.
%For example, the branch conditions in the \code{Heapsortcypher} application check if each API output class belongs to one of the three pre-defined lists. 
% \shan{This example is already discussed in the Introduction.}

%\item{\em Value ranges:}



The second type of branch condition is used when the API output is a score, and several pre-defined {\em value ranges} are then used to check if the API output scores fall in which range. 
The code snippet of \code{FoodDelivery}~\cite{food-delivery} in Figure~\ref{fig:2examples}(b), for example, calls MLaaS with a text sentence and receives a sentiment score as the ML API output. 
It uses three branch conditions, each checking if the API output score lies in a certain range. 
Given an input sentence whose ground-truth label is ``positive'', the ground-truth decision will print \code{It's a positive sentence}, and a critical error in this case will be when the API outputs a score lower than 0.6 on this sentence. 

% \shan{I am not totally sure about this arrangement. We already motivated somewhat in Introduction. How about we put any extra examples to a bit later when we discuss our empirical study result? It will also help move the pace faster into the empirical study.}
%As shown in the \code{FoodDelivery} application in Figure~\ref{fig:input_example}(b), it calls Google's \code{analyze\_sentiment} API to output a score indicating the emotional opinion of the input text. 
%The branch condition checks whether the score is over 0.6 (\ie the text is positive) or below 0.3 (\ie the text is negative), or otherwise (neutral). 
%\end{packeditemize}



%While these concepts may sound high-level, let us make them more concrete using two real-world applications, \code{Heapsortcypher} (Figure~\ref{fig:input_example}(a)) and \code{Food-delivery} (Figure~\ref{fig:input_example}(b)).
%
%\begin{packeditemize}
%\item 
%
%%\shan{This example is already discussed in the Introduction.}
%
%\item 
%%\shan{I am not totally sure about this arrangement. We already motivated somewhat in Introduction. How about we put any extra examples to a bit later when we discuss our empirical study result? It will also help move the pace faster into the empirical study.}
%\end{packeditemize}


\begin{figure*}
     \includegraphics[width=\linewidth]{figs/code.pdf}
    \caption{Examples of software such that the ML APIs' outputs affect the control flow decisions. }
\label{fig:code}
\end{figure*}


\mypara{Common structures over conditional branches}
Given the conditional branches, the way these branches are structured can also greatly affects the application decision process.
The structures over conditional branches differ along three key dimensions.
(1) the {\em number of conditional branches}; 
(2) the {\em number of executed branches} (for applications with several conditional branches, the application can either execute the first satisfied branch or all branches that satisfy the branch conditions); and finally
(3) the {\em order of examination}---when there are multiple elements in an ML API output {\em and} multiple conditional branches, an application can choose to examine each element one by one against the conditional branches (\ie examining the $1^{\textrm{st}}$ element in API output against all branch conditions before moving to the $2^{\textrm{nd}}$ element, and so forth) or examine all elements against each conditional branch (\ie examining all elements against the $1^{\textrm{st}}$ branch condition, then all elements against the $2^{\textrm{nd}}$ condition, and so forth). 
%\begin{packeditemize}
%\item {\em Number of conditional branches:} The applications may define one or several branch conditions. 
%\item {\em Number of executed branches:} For applications with several conditional branches, the application can either execute the first satisfied branch or all branches that satisify the branch conditions. 
%\item {\em Order of examination:}  
%When there are multiple elements in an ML API output {\em and} multiple conditional branches, an application can choose to examine each element one by one against the conditional branches (\ie examining the $1^{\textrm{st}}$ element in API output against all branch conditions before moving to the $2^{\textrm{nd}}$ element, and so forth) or examine all elements against each conditional branch (\ie examining all elements against the $1^{\textrm{st}}$ branch condition, then all elements against the $2^{\textrm{nd}}$ condition, and so forth). 
%%Applications that execute at most one branch  may either iterate through branch conditions first or the API outputs first in a two-level for loop. 
%\end{packeditemize}

With these dimensions, we identify four structures over conditional branches (Figure~\ref{fig:hierarchy}). 
Figure~\ref{fig:code} depicts a simple illustrative example of each structure.
\jc{we need to replace these names with macros. they will definitely be changed.}
\jc{yuhan, can you explain these categories using the three dimensions just introduced? what's the point of introducing the dimensions without actually using them?}
\begin{packeditemize}
\item {\em T-or-F:} Figure~\ref{fig:code}(a) is an example code structure where the first key dimension is only one branch condition. The application checks if the API outputs intersect with the list \code{A}. If so, it executes the branch \code{return "branch 1"}, otherwise, the branch \code{return "branch 2"} is executed. 
\item {\em M-to-N-set:}  Figure~\ref{fig:code}(b) is an example where it falls into the category of (1) defining more than one branch condition at the first key dimension; (2) executing a set of branches at the second key dimension.  The application defines two branch conditions in the for loop. If any of the branch conditions are fulfilled, the branch will be executed (\ie adding the message corresponding to the branch to the final output set). 
\item {\em Priority-list:} This type of applications define several class lists, and check the class lists in order until finding the first one that intersects with the API outputs. Figure~\ref{fig:code}(c) is an example of this code structure, and it falls into the category of (1) defining more than one branch condition at the first key dimension; (2) executing at most one branch; (3) first enumerate the branch conditions first at the third key dimension. 
\item {\em Top-label:} This type of applications iterate over the API outputs until finding one that intersects with any of the defined class lists, as shown in Figure~\ref{fig:code}(d). 
\end{packeditemize}





% \mypara{Software context}
% Given these definitions, we define the software context of an application as the {\em critical errors} on the ML API output that will lead to different application decisions than the ground-truth decisions\shan{???I don't quite get it}.
% While these applications may sound high-level, let us make them more concrete using two real-world applications, \code{Heapsortcypher} (Figure~\ref{fig:input_example}(a)) and \code{Food-delivery} (Figure~\ref{fig:input_example}(b)).

% \begin{packeditemize}
% \item 
% The code snippet of \code{Heapsortcypher} in Figure~\ref{fig:input_example}(a) calls MLaaS with an image and receives class labels as ML API output.
% It then checks if the API output belongs to three lists of classes, \code{Recycle}, \code{Compost}, \code{Donate} as the branch conditions to decide which branch to execute.
% % , so that 
% % % s. Each of the branch conditions 
% % checks if the API output belongs to the list of classes associated with the branch. 
% For an input with ground-truth class \code{``Shirt''}, the ground-truth decision is to execute the \code{Donate} branch.
% % \emph{Target-edge} associated with the \code{Donate} list. 
% If the ML API output is \code{``Paper''}, it will be a critical error, because the application decision will be the \code{Recycle} branch, deviating from the ground-truth decision.
% % is executing the \emph{Target-edge} associated with the \code{Recycle} list. This application decision deviates from the ground-truth decision, thus forming a critical error. 
% Nevertheless, if the ML API output is 
% % mis-classifies the Shirt image to 
% \code{``Jacket''}, it is not a critical error since the application's decision remains the same as the ground-truth decision.
% % is still executing the \emph{Target-edge} associated with the \code{Donate} edge.
% \shan{This example is already discussed in the Introduction.}

% \item The code snippet of \code{FoodDelivery} in Figure~\ref{fig:input_example}(b) calls MLaaS with a sentence and receives a sentiment score as the ML API output. 
% It uses three branch conditions, each checking
% % . Each branch condition checks 
% if the API output score lies in a range. Given an input sentence whose ground-truth label is ``positive'', the ground-truth decision will execute the branch that prints \code{It's a positive sentence}, and a critical error in this case will be when the API outputs a score lower than 0.6 on this sentence. 
% \shan{I am not totally sure about this arrangement. We already motivated somewhat in Introduction. How about we put any extra examples to a bit later when we discuss our empirical study result? It will also help move the pace faster into the empirical study.}
% \end{packeditemize}

% Importantly, these examples show that {\em not} all errors are critical errors, and thus such per-application software context, if used carefully, could improve ML API output to reduce wrong application decisions. 
% However, to unleash such potential in practice, we first need a deep understanding on the software contexts of various applications using real MLaaS {\em in the wild}.


% \mypara{An empirical study over real MLaaS applications}
% To this end, in the remainder of this section, we run an empirical study over 77 open-source applications which collectively use 6 ML APIs.
% These applications are selected from a recently published benchmark suite~\cite{wan2021machine}.
% We keep all applications except those that directly print out or store the ML API outputs without post-processing (for these applications, by definition any errors of API output will be critical).

% Our empirical analysis focuses two central questions:
% (1) among applications using the same ML API, how much they differ in their software context (critical errors), and 
% (2) despite the application heterogeneity, whether common patterns emerge which might allow automatic extraction of software context.  



% \subsection{\hspace{-0.2cm} Use of API output in conditional branches}


% For each of these applications in our study, its software context is determined along two dimensions
% {\em (i)} the branch conditions that use API output, and
% {\em (ii)} the structure over the branch conditions.Two applications' software contexts can differ along either or both dimensions. 

% \mypara{Use of API output in branch conditions}
% Depending on the API output, we identify two types of conditional branches. 
% \begin{packeditemize}
% \item{\em Class lists:} The first type is used when the API output is a label or a list of labels, and it checks if the API output labels belong to several pre-defined lists of classes.
% For example, the branch conditions in the \code{Heapsortcypher} application check if each API output class belongs to one of the three pre-defined lists. 
% \item{\em Value ranges:}
% The second type of branch condition is used when the API output is a score, and it  then checks if the API output scores fall in several pre-defined value ranges. 
% As shown in the \code{FoodDelivery} application in Figure~\ref{fig:input_example}(b), it calls Google's \code{analyze\_sentiment} API to output a score indicating the emotional opinion of the input text. 
% The branch condition checks whether the score is over 0.6 (\ie the text is positive) or below 0.3 (\ie the text is negative), or otherwise (neutral). 
% \end{packeditemize}


% \mypara{Structures of conditional branches}
% Given the API output and conditional branches, the way these conditional branches are structured can also greatly affect the application decision.
% The structures of conditional branches differ along three key dimensions, shown in Figure~\ref{fig:hierarchy}:
% \begin{packeditemize}
% \item Number of branch conditions: The applications may define one or several branch conditions. 
% \item Number of executed branches: For applications that define several branch conditions, the application can either execute at most one branch or execute a set of branches that fulfill the branch conditions. 
% \item Order of examination:  Applications that execute at most one branch  may either iterate through branch conditions first or the API outputs first in a two-level for loop. 
% \end{packeditemize}

% Along these dimensions, we carefully categorize the conditional branch structure of each application in our study.
% Four common structures emerge.
% \begin{packeditemize}
% \item T-or-F: As shown in Figure~\ref{fig:code}(a), the application defines one branch condition to check if the API outputs intersect with the list \code{A}. If so, it executes the branch \code{return "branch 1"}, otherwise, the branch \code{return "branch 2"} is executed. 
% \item M-to-N-set: As shown in Figure~\ref{fig:code}(b), the application defines two branch conditions in the for loop. If any of the branch conditions are fulfilled, the branch will be executed (\ie adding the message corresponding to the branch to the final output set). 
% \item Priority-list: This type of applications define several class lists, and check the class lists in order until finding the first one that intersects with the API outputs. Figure~\ref{fig:code}(c) is an example of this code structure.  
% \item Top-label: This type of applications iterate over the API outputs until finding one that intersects with any of the defined class lists, as shown in Figure~\ref{fig:code}(d). 
% \end{packeditemize}

















\subsection{\hspace{-0.25cm}Empirical study of application heterogeneity}


{\em As a consequence of the application decision processes, not all errors are critical.
And because each application has unique conditional branches and its structure over these branches, their critical errors are greatly different. 
}

\mypara{An empirical study over real MLaaS applications}
To this end, in the remainder of this section, we run an empirical study over 77 open-source applications which collectively use 6 ML APIs.
These applications are selected from a recently published benchmark suite~\cite{wan2021machine}.
We keep all applications except those that directly print out or store the ML API outputs without post-processing (for these applications, by definition, any errors of API output will be equally critical, so there is little room for improvement by customizing the model based on critical errors.)

\mypara{How code structures affect critical errors of API output}
If a misclassification occurs within a class list associated to the same conditional branch, then it is not a critical error. 
But it would be a critical error, if an image is misclassified with a label in the class list of a different conditional branch than the ground-truth label.

Even with the same branch conditions, the critical errors can differ depending on the structure of the conditional branches.

Take the code structures in Figure~\ref{fig:code} as an example. Figure~\ref{fig:code}(b)(c)(d) defines two same class lists. Given an input  with ground-truth class \code{c1} and API outputs \code{[c3, c1]}. The ground-truth decision is execute the branch corresponding to \code{A}. For M-to-N-set, this API output leads the execution of branches corresponding to class lists \code{A} and \code{B}, thus forming a critical error. However, for Priority-list, this API output correctly leads the application to execute the branch corresponding to \code{A}. On the other hand, Top-label iterates over the outputs and breaks at the branch corresponding to \code{B}, which is also a critical error for the application. 


% \jc{Yuhan, please fill in}

\mypara{Empirical observations on application heterogeneity}
Figure~\ref{tab:stats} enumerates the conditional branches used in the applications under our study and assigns each application to one of the aforementioned structures. 
We make three empirical observations.
\begin{packeditemize}
\item In each application, {\em the number of pre-defined class lists and value ranges are relatively small}, indicating a potential for MLaaS to increase accuracy on specific classes by customizing (retraining) the ML models behind ML API. 
Collectively, set of classes in the class lists is relatively small compared to the number of classes in a typical classification training dataset (\eg 9605 classes in OpenImages~\cite{openimages} or 1000 classes in ImageNet~\cite{5206848}). 
\item More importantly, there are {\em very few overlaps among the branch conditions of different applications}, making a case for {\em per-application} customization of ML API backend model.
Specifically, among all (826 \footnote{We separately count the pairs for the 40 Vision tasks and 5 NLP entity recognition task, and 36 NLP text classification tasks as they do not share label sets}) pairs of applications with class-list-based branch conditions, only 71 of them overlap by more than one classes between their class lists. 
Similarly, among the 381 classes that appear in at least one application's branch conditions, only 16 of them appear in more than three applications.
\item Similarly, the structure over the conditional branches also varies greatly across applications, though four common patterns are enough to cover them. Out of the applications we study, 32\% of applications are T-or-F, 23\% of them fall into the pattern of M-to-N-set, 8\% of them are M-to-N-set, and the rest of them are Top-label.
% \jc{a few words on this}
\end{packeditemize}



% \mypara{An empirical study over real MLaaS applications}
% % Given the rich syntax that can be expressed by Python, critical errors for applications in the wild can be very different.
% % To understand common types of software context that affect the application decisions, we first perform 
% To this end, in the remainder of this section, we run an empirical study over 78 open-source applications  whose application decisions 
% % control flow decisions 
% which collectively use \fillme ML APIs.
% These applications are from a recently published benchmark suite~\cite{wan2021machine}~\footnote{
% We ignore applications that directly print out the ML API outputs or store these outputs without post-processing, and thus by definition any errors of API output will be critical.
% % The tasks that these applications perform are the same as the task of ML API. Therefore, there is no need to adapt APIs to software. 
% }. 
% These applications cover a wide range of use cases, from \fillme to \fillme. 



% % Google (benchmark, search), AWS (search)

% % \begin{definition}[Application decision]\label{def:app_decision}
        
% % \end{definition}

% % These applications compare the ML API's output classes with the applications' pre-defined lists of classes, and decide which if-branch edge to execute. We refer to this process as making \textit{application decisions} and the pre-defined lists of class as \wls. 



% % \shan{Without knowing your application selection criteria, I cannot interpret what this ``48\%'' implies. What does the remaining 52\% applications do? If all applications in your bencharmk suite use ML API output to affect control flow, how can there be no whitelist? Can you offer more explanation here about what exactly this 48\% mean?} \yh{Sorry 48\% was an out-dated number. All the 40 apps whose control flow are affected by the ML APIs' outputs do specify whitelists. }

% % The application goes through a list of conditional branches based on API outputs, whether a branch is executed is determined by if the API outputs matches with the branch condition or not 

% % \yh{use sentiment analysis, the way to map conditional branch to app decisions is different }


% % The application defines three \wls, \code{Recycle, Compost, Donate}. 
% % The human labeled ground-truth of the input image is ``Shirt'', so the ground-truth decision is executing the if-branch edge \code{return donate(trash\_image)}, which we refer to as selecting the \code{Donate} whitelist. 
% % Furthermore, if the ML API's outputs lead the application to make the decision of executing the code \code{return "It is others." }, such as outputting class ``Dog'', we refer to this decision as selecting \code{others}. 

% % We refer to this executed branch as \emph{if/then branch}. Correspondingly, we refer to another branch that  not executes Line 8 as \emph{if/else branch}\shan{what if there is if-elsif-then?}.
% % We refer to a list of classes (or classification categories) defined in the code\shan{what labels? you mean outputs of an ML API?} leading to the same control flow decision as a \emph{whitelist}. \code{Recycle}, \code{Compost}, and \code{Donate} are the three whitelists, taking Heapsortcypher as an example
% \shan{This definition has a lot of flaws.
% One quick question: based on your definition, aren't all labels minus those in Recycle, Compost, and Donate also a white list? Are they?
% }

% % \cc{yuhan, please put terminologies (those used in Section 3) here. Make sure that you are only using the Heapsortcypher as an example}

% % While these applications typically use \wls to post-process ML API results, they vary in the way of using whitelists to make application decisions. Even with the same whitelists and API outputs, the applications would behave differently according to their code structure. Next, we will introduce the common patterns observed in the studied applications.

% % We find that the common software context consists of two components: (1) Types of branch conditions (\eg checking if the API output belongs to a list of classes), details described in Section~\ref{sec:content}; (2) The organization of conditional branches, details in Section~\ref{sec:org}. 




% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% sentiment_text = types.Document(content = a_piece_of_text)
% annotations = client.analyze_sentiment(document=sentiment_text)
% sentiment_score = annotations.document_sentiment.score
% if sentiment_score < 0.3:
%     print("It's a negative sentence!")
% elif sentiment_score > 0.6:
%     print("It's a positive sentence!")
% else:
%     print("It's a neutral sentence!")
% \end{lstlisting}
%     \caption{The code snippet in the app \code{FoodDelivery}~\cite{food-delivery} calls Google's analyze\_sentiment API to determine the sentiment of a given text.}
%     \label{fig:sentiment}
% \end{figure}


% \subsection{Types of the branch conditions}
% \label{sec:content}
% % \yh{2.1 => what does the context entail, 2.2 and 2.3, differs from ...., but follows a set of common structure, not arbitrary }

% Our study reveals two types of conditional branches, comparing the API outputs with lists of classes, or setting ranges to branch the API outputs. 

% \subsubsection{Lists of classes} 


% % \begin{figure}
% %      \includegraphics[width=.8\linewidth]{figs/stats.pdf}
% %     \caption{ The number of classes included in the lists used to make application decisions. }
% % \label{fig:stats}
% % \end{figure}


% The Applications calling APIs that output categorical results (\eg image classification) 
% pre-define lists of classes, and compare the API outputs with the lists, to make the application decision. For example, the branch conditions in the \code{Heapsortcypher} application check if the API output class belongs to one of the three pre-defined lists. We observe that the lists the applications define typically cover only a very small subset of whole label set. In Figure~\ref{fig:stats}, we summarized the number of classes included in the lists used to make application decisions in our study. Out of the 9605 \yh{double check this number} classes that are covered in Google's classification API, the lists of classes used by the applications to make decisions include less than 20 classes.

% Since the ML API  is typically optimized on a much wider range of classes, the focus on the small subsets classes defined by the applications indicates great room for improvement on the ML API. 


% \subsubsection{Setting ranges}

% Some  applications  call APIs that output floating point values. As shown in the \code{Cloud-computing} application in Figure~\ref{fig:sentiment}, it calls Google's \code{analyze\_sentiment} API to output a score indicating the emotional opinion of the input text, where a score closer to 1 indicates the text is more positive, and a score closer to -1 is more negative. In this case, the  branch condition is checking if the predicted score falls into a specific range. 



% \subsection{How the branch conditions are organized}
% \label{sec:org}

% % \yh{Can those branch conditions directly determine how the application decisions, how the branches are structured => affects the critical errors}
% % \yh{Bad news: there's no one structure, good news: a handful of structures }
% A thoughtful reader may wonder: Does identifying the content of the branch conditions enough to determine the application decisions?


% % Can the branch conditions themselves enough to  determine the application decisions? 

% The answer is no. Our study reveals that even when the content of the branch conditions are the same (\ie defining the same lists of classes as branch conditions), the application decision may still be different based on how the  branch conditions are organized 

% Fortunately, we can classify different organization of branch conditions into a handful of categories. To illustrate the different ways the organization of conditional branches affects the application decision, we begin with defining three key abstractions.


% \subsubsection{Key Abstractions}
% \label{sec:abstractions}
% As summarized in Figure~\ref{fig:hierarchy} we define three types of abstractions to characterize the code structure. 


% \textbf{1) Number of branch conditions } The applications may define one or several branch conditions. If the applications only define one branch condition, whether to execute the branch or not only depends on if API outputs fulfill the only branch condition or not. On the other hand, for applications that define several branch conditions, the application decisions are also affected by other aspects. 
% % The software may specify one or several \wls candidates. Each \wl candidate is related to a particular software branch: the software will execute the corresponding \ift when the ML APIs' outputs intersect with the labels in the \wls candidates. In the rest of the paper, we will refer to executing the \ift as selecting its associated \wl.

% \textbf{2) Number of executed target-paths} Applications that define more than one branch condition can either (1) execute at most one branch; (2) execute the set of branches that fulfill 
%  their branch conditions. 



% \textbf{3) Order of examination}  Applications that execute at most one branch define a two-level nested loop to determine the branch to execute. The applications may iterate through branch conditions in the outer loop or the API outputs in the outer loop. 
% % For the software specifying multiple \wls, the order of examining intersections between \wls and ML API outputs determines software behavior. If we reconstruct the examination into a two-level nested loop that iterates through \wls and API outputs, there naturally arises two types of loop structure: prioritize the specified \wls or the API output labels.


% \begin{figure}
%      \includegraphics[width=\linewidth]{figs/hierarchy.pdf}
%     \caption{Abstractions that characterize the code structure. The decision nodes (in blue) are abstractions defined in Section~\ref{sec:abstractions}. The leaf nodes (in green) are the type of code structures constructed with the sequence of decisions made at each decision node. }
% \label{fig:hierarchy}
% \end{figure}



% \subsubsection{Common branch condition structures}
% \label{sec:examples}

% Based on these three types of abstractions, we can classify the common code structures into four categories shown in Figure~\ref{fig:hierarchy}. Each decision node represents an abstraction. Each leaf node represents a structure of branch conditions constructed with the sequences of different decisions made at each decision node. 

% In the following section, we explain the common branch condition structures with simple code snippets. 

% \subsubsection{Branch condition structure 1: T-or-F} The applications with this pattern only specifies one branch condition on the API outputs. Around 32\% of applications in our benchmark suite belong to this category.

% As shown in Figure~\ref{fig:code}(a), the application defines one branch condition to check if the API output belongs to the pre-defined list \code{A}. 

% \textbf{Input example} In this application pattern, given inputs with ground-truth decision of executing the \code{A} branch, the critical error is failing to include any of classes in \code{A} in API outputs.


% \subsubsection{Branch condition structure 2: M-to-N-set} 
% \label{sec:m_to_n}
% In our benchmark, 23\% applications define several branch conditions, and execute the set of branches whose branch conditions are fulfilled based on API outputs. 

% As shown in Figure~\ref{fig:code}(b), the application iterates over the API outputs with a for loop. Inside the for loop, two branch conditions are defined to check if the API output belongs to the lists \code{A} or \code{B}. If the API output belongs to the list \code{A}, the branch \code{final\_output.add("branch 1")} is executed. If the API output belongs to the list \code{B}, the branch \code{final\_output.add("branch 2")} is executed. 

% \textbf{Input example} In this case, given an input  whose ground-truth is \code{c1}, the ground-truth decision is only executing the branch \code{final\_output.add("branch 1")}. When the API outputs \code{[c3, c1]}, both \code{final\_output.add("branch 1")} and \code{final\_output.add("branch 2")} are executed. This output forms a critical error in M-to-N-set. 



% % defines two \wls, \code{A} and \code{B}, and iterates through the ML API's outputs, and adds the string \code{"branch 1"} to the final output set if the outputs intersect with the whitelist \code{A}, and adds the string \code{"branch 2"} to the final output set if the outputs intersect with the whitelist \code{B}. 

% % In this pattern, mis-classifications inside \ do not matter, as long as the ML API's output classes include at least one class in the \wls that should be selected in the ground-truth decision, and not include any class in the \wls that are not in ground-truth decision. 

% % \yh{
% % Given the ground-truth is [Bread, Cheese]

% % Critical errors: failed to include any class in Grainfoods and Proteinfoods, and including any one class in fruitfoods

% % }


% \subsubsection{Branch condition structure 3: Priority-list}
% \label{sec:priority}Around 8\% software defines multiple branch conditions, and check the branch conditions one-by-one until the API outputs fulfill the condition. If none of the conditions are fulfilled, the branch \code{return ``branch 3''} is executed. 

% For example, in Figure~\ref{fig:code}(c), the application defines two lists of classes,  \code{A} and \code{B}, and iterates over the two lists. If any of the API outputs belongs to \code{A}, the application makes the decision of executing the branch \code{return "branch 1"}. If not, the application checks if the API outputs intersect with \code{B}. If the API outputs do not intersect with either \code{A} or \code{B}, the branch \code{return "branch 3"} is then executed. 

% \textbf{Input example} With the same example discussed in Section~\ref{sec:m_to_n}, given an input with ground-truth \code{c1}, the ground-truth decision is executing the branch \code{return "branch 1"}. However, when the API outputs \code{[c3, c1]}, only the branch  \code{return "branch 1"} is executed because the API outputs intersect with \code{A}. This API output, thus do not lead to a critical error for Priority-list. 


% % For example, in Figure~\ref{fig:code}(c), the application defines two \wls, \code{A} and \code{B}, and \code{A} has higher priority than \code{B}. The application uses a nested loop that first iterates through the \wls, and then the output classes. The three possible decisions this application may make are: (1) selecting whitelist \code{A} if the ML API's outputs intersect with \code{A}; (2) selecting whitelist \code{B} if the ML API's outputs do not intersect with \code{A} and intersects with \code{B}; (3) selecting \code{others} if the ML API's outputs do not intersect with either \code{A} or \code{B}.

% % In this pattern, mis-classifications within the for labels inside any of the lower-ranked \wl will not lead to wrong application decisions if ML API correctly recognizes the existence of classes in the higher-ranked \wls. 

% % \yh{
% % Given the ground truth is [Building]

% % critical errors: including any class in monument 

% % }



% \subsubsection{Branch condition structure 4: Top-label}
% \label{sec:top_label}
% Applications that belong to this pattern make decisions by checking the ML API's output classes one by one until finding the first class that fulfills a branch condition. \shan{???In pattern 3, software maps ... ``in a specific order'' as well.}. Around 37\% of applications fall into this category.

% For example, as shown in Figure~\ref{fig:code}(d), the  application defines two lists of classes, and iterates over API outputs. If the first output, \code{x1}, belongs to any of the lists, the corresponding branch will be executed. If not, the application checks if the second output, \code{x2}, matches any one of the two lists or not. If none of the API outputs matches the two lists, the branch will be executed. 

% \textbf{Input example} With the same example discussed in Section~\ref{sec:priority}, different from Priority-list, the API outputs \code{[c3, c1]} lead the execution of the branch \code{return "branch 2"}.  This API output, thus incurs a critical error for Top-label. 

% %  the application defines two \wls, \code{A} and \code{B}. The application defines a nested for loop that first iterates through the output classes (\ie [\code{x1}, \code{x2}]), and then the \wls. If \code{x1} intersects with any of the \wls, the application selects the corresponding one. If \code{x1} does not match with any of the \wls, then the application checks if \code{x2} belongs to any of the \wls. Otherwise, it selects \code{others}. 

% % In this pattern, mis-classifications for classes ranked lower in the ML API's outputs do not matter, as long as the classes that rank higher leads to correct application decisions. 

% % \yh{Pie chart showing some statistics  }

% \subsubsection{Summary}

% In short, in these different structures of branch conditions, even when the branch conditions are the same (\eg checking if the API outputs interest with lists of classes), the same API outputs can lead to different application decisions. As a result, the patterns of critical errors can be very different for these different structures. 

% Although we use examples whose branch conditions are lists of classes, applications whose branch conditions are based on the range of the output scores also fall in the branch condition structures described in Section~\ref{sec:priority} or Section~\ref{sec:top_label}. 
% % \shan{What is the F1 score drop for this category?}

% \subsection{Summary of findings}

% To summarize, the real applications covered in our study reveal that there is a rich set of \emph{software context}. This motivates the need for customizing the ML API to incorporate the different \emph{software context}. 

% Luckily, although there is a rich set of \emph{software context}, the context is \emph{not} arbitrary. We can express the context in a format that combines the content and the structure of the branch condition, which can be extracted from the applications' source code.  
% % \yh{\textbf{Why we need to customize}}



% % \begin{figure}
% % \begin{subfigure}{0.45\textwidth}    
% %     \centering
% % \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% % Dog = ['Dog','Mammal','Carnivore','Wolf']
% % image = types.Image(content=dog_image)
% % response = client.label_detection(image=image)
% % for obj in response.label_annotations:
% %   if obj.name in Dog:
% %     return 'It is a animal.'
% % return 'It belongs to others.'
% % \end{lstlisting}
% %     \caption{Code pattern: T-or-F. }
% %     \label{fig:app_example_level1}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/input_example_tf_wrong.pdf}
% %     \caption{Failing recognize the carnivore leads to software failure. }
% %     \label{fig:input_example_tf_wrong}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/app_input_example_level1.pdf}
% %     \caption{Mis-classifying a dog as wolf does not trigger software failure. }
% %     \label{fig:input_example_tf_correct}
% % \end{subfigure}
% % \caption{Dogecoin~\cite{food}, an application that classifies carnivore images.  }
% % \label{fig:tf_example}
% % \end{figure}



% % \begin{figure}
% % \begin{subfigure}{0.45\textwidth}    

% %     \centering
% %              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% % proteinfoods = ['Hamburger', 'Meat', 'Patty']
% % fruitfoods = ['Apple', 'Fruit', 'Orange']
% % grainfoods = ['Noodle', 'Pasta', 'Al dente']
% % image = types.Image(content=trash_image)
% % response = client.label_detection(image=image)
% % protein, fruit, grain = False, False, False
% % for obj in response.label_annotations:
% %   if obj.name in proteinfoods:
% %     protein = True
% %   if obj.name in fruitfoods:
% %     fruit = True
% %   if obj.name in grainfoods:
% %     grain = True
% % RENDER_TEMPLATE(protein, fruit, grain)
% % \end{lstlisting}
% %     \caption{Software implementation. }
% %     \label{fig:app_example_non_mut}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/input_example_mton_wrong.pdf}
% %     \caption{Failing to recognize ``Cheese'' leads to software mis-behavior. }
% %     \label{fig:input_example_mton_wrong}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/input_example_mton_correct.pdf}
% %     \caption{Mis-classifying ``Pasta'' to ``Noodle'' still leads to correct software behavior. }
% %     \label{fig:input_example_mton_correct}
% % \end{subfigure}
% % \caption{Food classifier~\cite{food}, an application that classifies food images.}
% % \end{figure}


% % \begin{figure}
% %     \centering
% %              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% % proteinfoods = ['Hamburger', 'Meat', 'Patty']
% % fruitfoods = ['Apple', 'Fruit', 'Orange']
% % grainfoods = ['Noodle', 'Pasta', 'Al dente']
% % image = types.Image(content=trash_image)
% % response = client.label_detection(image=image)
% % food_list = []
% % for obj in response.label_annotations:
% %   if obj.name in proteinfoods:
% %     food_list.append('protein')
% %   if obj.name in fruitfoods:
% %     food_list.append('fruit')
% %   if obj.name in grainfoods:
% %     food_list.append('grain')
% % return food_list
% % \end{lstlisting}
% %     \caption{An example software that maps original output labels of the ML APIs to a list of \wls.  }
% %     \label{fig:app_example_non_mut}
% % \end{figure}



% % \begin{figure}
% % \begin{subfigure}{0.45\textwidth}
% %         \centering
% %              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% % Monument = ['Landmark', 'Sculpture', 'Monument']
% % Construction = ['Building', 'Estate', 'Mansion']
% % Person = ['Human','Person',  'Lady']
% % image = types.Image(content=landmark_image)
% % response = client.label_detection(image=image)
% % Predictions = []
% % for obj in response.label_annotations:
% %   Predictions.append(obj.name)
% % if any([label in Monument for label in Predictions]):
% %   return 'It belongs to monument.'
% % elif any([label in Construction for label in Predictions]):
% %   return 'It is construction.'
% % elif any([label in Person for label in Predictions]):
% %   return 'It is person.'
% % \end{lstlisting}
% %     \caption{Software implementation. }
% %     \label{fig:app_example_priority}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/input_example_priority_wrong.pdf}
% %     \caption{Missing a label ``Landmark'' leads to software mis-behavior. }
% %     \label{fig:input_example_priority_wrong}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/input_example_priority_correct.pdf}
% %     \caption{Recognizing an extra wrong label ``Mansion'' still leads to correct software behavior. }
% % \label{fig:input_example_priority_correct}
% % \end{subfigure}
% % \caption{Aander-ETL~\cite{etl}, an application that classifies landmark images.  }
% % \label{fig:priority_input_example}
% % \end{figure}

% % \cc{Do we want to introduce the accuracy difference between API and software? And the room for improvement?}

==> backups/3-method-1123.tex <==
\label{sec:method}

\subsection{System architecture}

\begin{figure}
     \includegraphics[width=\linewidth]{figs/system_overview.pdf}
    \caption{System architecture of \tool. }
\label{fig:system}
\end{figure}
% \mypara{Main components}

% \mypara{Extracted Software decision process}

Figure~\ref{fig:system} shows the overall system architecture of \tool.
In the offline stage, the developers run a parser plugin locally, which extracted the software decision process from the application source code. The extracted software decision process is displayed in JSON format, consisting of: (1) the content of class lists used in branch conditions; (2) whether the application is making multi-select or multi-choice decisions; (3) the order of examination for applications making multi-choice decisions. Then, the developers will upload the JSON of software decision process to the MLaaS backend. On the MLaaS backend side, \tool will re-train the ML model by re-sampling the training data with a more focus on the classes appeared in the applications, and constucting loss functions which directly penalize the critical errors.

% In the online stage, 




% which consists of a parser plugin, an ML model re-training scheme run in the offline stage, and in the online stage, \tool selects the customized ML model based on applications' credentials, and run inference with the customized model.  


% 3.2: given the extracted json, how should we re-train teh model 
% 3.3. how to extract
% 3.4: how to change the run-time interface

% \tool is an automated framework that adapts the DNN behind the ML APIs, such that the number of software mis-behaviors can be greatly reduced when applied to an ML software. 

% \tool first performs static analysis to extract the code structure of the applications invoking MLaaS to understand how the software uses the ML API outputs to make application decisions. Then \tool constructs loss functions that penalize the critical errors of the applications. Finally, \tool re-trains the DNNs behind the ML APIs with the constructed loss function, without modifying the output interface of the ML APIs. 

% In this section, we will introduce how \tool performs static analysis and constructs the loss functions for the applications. 


% \subsection{Understanding Software Context}

% \subsection{Notations}
% \yh{not 3.2 }
% Denote the total number of classes that the DNN behind the ML API can classify as $n$, and the whole set of classes is $C=\{C_1, C_2, ..., C_n\}$.  We define the symbols in our problem setting as follows:

% \begin{itemize}
%     \item $I$: the input image
%     \item $G=\{G_1, ..., G_a\}$: ground truth label set of $I$, where $G_i \in C$ for $1 \leq i \leq a$
%     \item $T$: the prediction threshold of the DNN behind the ML API
%     \item $O=\{O_1, O_2, ..., O_b\}$: the predicted classes over the prediction threshold $T$, where $P_i \in C$ for $1 \leq i \leq b$
%     \item $P=\{p_1, p_2, ..., p_b\}$: the corresponding probability for the predicted classes
    
    
% \end{itemize}



\subsection{How to customize the ML model in the ML API backend}

We first start with introducing the re-training scheme in \tool. 


\yh{Outline of this section: 
1. first list the goal in math (or text): minimize the incorrect app decisions
2. a naive re-training scheme is to use a training data that  focuses on classes appeared in the apps 3. why this design is not good: it can only solve xxx, but not xxx 4. describe our loss function }
% \yh{goal: minimize the incorrect app decisions; what we have: extracted software decision process (key dimensions) }
As shown in our empirical study in Section~\ref{sec:empirical}, we find the software decision process can be characterized by two aspects: (1) the class list(s) or value ranges that are used in branch conditions (2) the structures of the branch conditions.

In this section, we will describe how we incorporate the software decision process in the loss function. Our optimization is composed of two steps: (1) clustering the training data to focus on classes appearing in the branch conditions; (2) constructing the loss functions to be aware of the software decision process. Our objective is to incur a high penalty on critical errors, and no penalty if the errors make no impact on the application. 


To begin with, we first introduce the loss function traditionally used in multi-label image classification.


The binary cross-entropy loss function used in multi-label classification task~\cite{ASL} is denoted as:
\begin{equation}
    L_{bce}  = -\frac{1}{n}\sum_{i=1}^n{(y_i\log(p_i) + (1 - y_i)\log(1 - p_i))} \,,
\end{equation}
where $y_i = 1$ if class $i$ is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. $p_i$ is the predicted probability for class $i$. 
% \begin{itemize}
%     \item  $y_i = 1$ if the $i^{th}$ class is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. 
%     \item $p_i$ is the predicted probability for the $i^{th}$ class.
% \end{itemize}
% where $y_i$ indicates whether the $i^{th}$ class exists in the input sample $I$ or not. In other words, $y_i = 1$ if the $i^{th}$ class exists in the input $I$, and $y_i = 0$ otherwise. \cc{It is still one sentence, so please do not start a new paragraph}


\subsubsection{Clustering training data}


To achieve the first step, one approach is to assign different weights to samples with ground-truth decisions of executing the \code{Others} branch and non-\code{Others} branches.  
We take a simple example to illustrate this approach. An application  defines one branch condition to check if the API outputs intersect with a class list $W_1$. $W_1$ is a non-empty subset of the whole label set $C$ that the DNN is able to classify. 
 The original fraction of images in the training data whose ground-truth  decisions are executing the \code{$W_1$}-branch (\ie $G \cap W \neq \emptyset$), which we refer to as \code{$W_1$}-samples,  is $A$. 
 % \cc{This sentence is very hard to read. Can we use phrase like ``which we refer to as $W$-images''?} 
The fraction of images whose ground-truth decisions are executing the \code{other}-branch is $1-A$,  which we refer to as \code{others}-samples. If we want to balance the distribution between $W$-samples and \code{others}-samples, we can use a loss function that assigns higher weights to \code{W}-samples:

\begin{equation}
    L_D = y_1 \cdot \frac{1}{A} \cdot L_{bce} + (1-y_1)\cdot A \cdot L_{bce} \,,
\end{equation}
where $y_1$ indicates whether this sample is a \code{$W$}-sample or not. In other words, $y_1 = 1$ when the sample is a \code{$W$}-sample ($G \cap W \neq \emptyset$), and $y_1 = 0$ otherwise ($G \cap W = \emptyset$). 
% \cc{This example seems to be T-or-F. Could we use consistency description as Section 3.4.2? }


% In this way, samples whose ground-truth decisions are selecting the \wl and those whose ground-truth decisions are selecting \code{others} are taking the same effect during training, instead of biasing towards either selecting the \wl or selecting \code{others}. 
In this way, \code{$W$}-samples and \code{others}-samples are taking the same effect during training, instead of biasing towards either \code{W} or \code{others}. 

% We construct loss functions for each type of software represented by the software examples shown in section~\ref{sec:empirical}. \cc{Maybe say some high-level ideas, more intuition}

\subsubsection{Branch condition structure 1: T-or-F} 

For the software that defines only one branch condition, checking if the output labels $O$ intersect with a class list $W_1$. We penalize the critical errors: (1) all the classes in $W_1$ are not included in top predictions for \code{$W_1$}-samples; or (2) at least one class in $W_1$ are included in top predictions for \code{others}-samples.



% \begin{equation}
% \left\{
% \begin{split}
%     L_{W_1} &= y_1 \cdot \textrm{S}(\theta - P_1) + (1-y_1) \cdot \textrm{S}(P_1 - \theta) \\
%     P_1 &= xxx 
% \end{split}
% \right.
% \cc{Another format}
% \end{equation}

% \kt{$L_{W_i} = y_i (p_i\succ \theta) + (1-y_i) (\theta \succ p_i)$, where $y_1$ indicates whether ground truth contains classes inside $WL_1$ (in other word, ???=1, ???=0), $p_1$ is the maximum probability among white list 1 (\ie $WL_1$) and $\theta$ is the threshold used inside the ML API}.
% \cc{Some equations have numbers, some do not. Please make them consistent}

% \begin{itemize}
%     \item $y_1$ \cc{yuhan, this part is not finished yet}
% \end{itemize}

\begin{equation}
    L_{W_1} =y_1 \cdot \textrm{S}(\theta - P_1) + (1-y_1) \cdot \textrm{S}(P_1 - \theta) \,,
\label{eq:loss}
\end{equation}
where
$y_1$ indicates whether this sample is a \code{$W_1$}-sample or not. 
In other words, $y_1 = 1$ if the sample is a \code{$W_1$}-sample, and $y_1=0$ if the sample is a \code{others}-sample. $\theta$ is the prediction threshold, where classes whose predicted probability will be included in the output label list. $P_1$ is the maximum probability of classes in $W_1$ (\ie $P_1 = max_{c \in W_1} p_c  $). $S(x)$ is the Sigmoid function $\frac{1}{1+e^{-k x}}$, which we will denote as $S$ in the rest of the paper. 



Ideally, we want the loss function to be a step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{no penalty} when $P_1$ is greater than $\theta$ for  \code{$W_1$}-samples. However, to make the loss function differentiable, we use the Sigmoid function to approximate the step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{a low penalty} otherwise, for \code{$W_1$}-samples. Similarly for \code{other}-samples. 


% For example, in the example\cc{yuhan, please read these five words again to see what's the problem...} software shown in Figure~\ref{fig:tf_example}, given a prediction threshold of 0.5, when the probability scores of the labels in the specified \wl are $\langle0.2, 0.3, 0.4, 0.9\rangle$ for Dog, Mammal, Carnivore, and Wolf respectively in Figure~\ref{fig:input_example_tf_correct}, the penalty incurred by the loss function is 0.40. On the other hand, in Figure~\ref{fig:input_example_tf_wrong}, where the ground-truth labels include one of the labels in the \wl, thus the ML API should output at least one label in the \wl in order to produce the correct control flow decision. When the probability scores for  Dog, Mammal, Carnivore, and Wolf are $\langle0.2, 0.3, 0.35, 0.3\rangle$\cc{I use parenthesis to make them look like lists instead of random number. yuhan, could also change other places?} respectively, leading to none of the labels in the \wl being output, the penalty incurred by the loss function is 0.537. 


\subsubsection{Branch condition structure 2: M-to-N-set} 

 In M-to-N-set, several branch conditions are defined, each checking if a class list intersects with the API output $O$. All the fulfilled branches will be executed. We denote all the $m$ class lists the application uses in branch conditions as {$W_1$, ..., $W_m$}. In this pattern, the ground-truth  decisions is executing \emph{all} the branches whose class lists  intersect with the ground-truth labels. 

We derive the following loss function for M-to-N-set:
\begin{equation}
    L = \sum_{i=1,\cdots,m} y_i \cdot \textrm{S}(\theta - P_i) + (1-y_i) \cdot \textrm{S}(P_i - \theta) \,,
\end{equation}
where $y_i$ indicates whether  $W_i$ is among the branches the ground-truth decision executes, in other words, $y_i = 1$ if $G \cap W_i \neq \emptyset$, and $y_i = 0$ otherwise. Similar to Equation~\ref{eq:loss}, $P_i$ is the maximum probability of classes belonging to $W_i$ (\ie $P_i = max_{c \in W_i} p_c$). 

 Only if the application decisions led by $O$ exactly match with the ground-truth decisions, the penalty will be low.
 % \cc{be low or be zero? should we also mention the probability differences?}. 


% \kt{$\sum_{i=1,\cdots,N} L_{W_i}$}



\subsubsection{Branch condition structure 3: Priority-list}

Priority-list defines several branch conditions, and each of them is associated with a class list $W_i$. The application checks the branch conditions from highest to lowest priority until finding the first one whose class list intersects with API output labels $O$. Let $W_i$ (where $1 \leq i \leq m$) denote the class lists used in branch conditions, where class lists with smaller $i$ indicate higher priority. Let $W$ denote the union of the classes in all the whitelists, in other words, $W = \cup^{m}_{i=1}W_i$. The ground-truth decision  is executing the highest priority branch whose associated class list intersects with the ground-truth classes $G$. 

We derive the loss function as:
\begin{equation}
\begin{split}
    L = y_i \cdot \textrm{S} (\max(\theta, P_{k^{-}})  - P_k ) + 
    (1-y_i) \cdot \textrm{S}(P - \theta) \,,
\end{split}
\end{equation}
where $y_i = 1$ when the ground-truth decision is executing one of the branches in $\{ W_1, \cdots, W_m\}$ (\ie $G \cap W \neq \emptyset$), and  $y_i = 0$ when the ground-truth decision is executing the \code{others} branch. 
$k$ is the index of the highest-priority branch whose class list intersects with the ground-truth classes (\ie $k = \min \{i|WL_i \cap G \neq \emptyset\}$). $P_k$ is the maximum predicted probability for classes belonging to $W_k$, and $P_{k^{-}}$ is the maximum predicted probability out of the classes belonging to higher priority branches than the ground-truth branch (\ie $k^{-} = \min \{i | W_i \cap (G \setminus W ) \neq \emptyset \textrm{ and } i < k \}$). $P$ is the maximum probability of the classes belonging to $W$. 

Given this loss function, only if the highest-priority branch whose class list intersects with the predicted classes $O$ is the ground-truth decision, the penalty will be low. 

% \begin{equation*}
%     \footnotesize
%     \begin{split}
%     L(O, G) &=  \begin{cases}
%    P \Big( T, \max\limits_{c \in W} p_c \Big ), & G \cap W = \emptyset \\
%      P \Big( \max\limits_{c \in WL_k } p_c, T \Big ) + P\Big( \max\limits_{c \in WL_k} p_c, \max\limits_{c \in W \setminus WL_k} p_c \Big ), & G \cap W \neq \emptyset \\
% \end{cases}\\
% k &= \min \{i|WL_i \cap G \neq \emptyset\}
%     \end{split}
% \end{equation*}
% \kt{$L_{W_k}$, where $k=???$}


% Given this loss function, we can ensure that: (1) for images with ground-truth labels intersecting with at least one \wl, as long as the \wls that intersect with the output labels are not the one that ranked highest among those intersecting with the ground-truth labels, the penalty incurred by the loss function will be large; (2) for images with ground-truth labels that do not have an intersection with any of the \wls, as long as the output labels intersect with the labels in any of the \wls, the penalty incurred by the loss function will be large. 


% For example, in the example software \cc{I prefer directly writing down software name (if we already introduce it) or describe what type of software, e.g. trash classification application. It's hard for people to recall what happens only with the figure number} shown in Figure~\ref{fig:priority_input_example}, the prediction threshold is 0.5. In the input example in Figure~\ref{fig:input_example_priority_correct}, the probability scores of the labels in the Monument \wl are 0.2, 0.3 and 0.1 respectively, and the probability scores of the labels in the Construction \wl are 0.8, 0.2, 0.05, and the probability scores of the labels in the Person \wl are 0.45, 0.4, 0.2. The penalty incurred by the loss function is $Sigmoid(0.5-0.8)$ + $Sigmoid(0.45-0.8)$ = 0.8388. 

% On the other hand, in the input example in Figure~\ref{fig:input_example_priority_wrong}, the probability scores of the labels in the Monument \wl are 0.3, 0.2 and 0.15 respectively, and the probability scores of the labels in the Construction \wl are 0.7, 0.2, 0.1, and the probability scores of the labels in the Person \wl are 0.45, 0.8, 0.2. The penalty incurred by the loss function is $Sigmoid(0.5-0.3)$ + $Sigmoid(0.8-0.3)$ = 1.17. The penalty, in this case, is greater than the penalty in Figure~\ref{fig:input_example_priority_correct}, because labels in the highest-ranked \wl intersecting with the ground-truth labels do not appear in the output. 

\subsubsection{Branch condition structure 4: Top-label}

Top-label defines several branch conditions, and associates with each of them with a class list $W_i$, similar to Priority-list. However, unlike Priority-list, it checks the \emph{API output labels} one by one until one of them intersects with any of the class lists. Similar to the previous section, $W$ is the union of classes in all the defined class lists. We denote the classes belonging to class lists intersecting with ground-truth classes as $W^+ = \bigcup_{W_i \cap G \neq \emptyset} W_i$, and the classes belonging to \wls that do not intersect with ground-truth classes as $W^- = W \setminus W^+$.
 
In this pattern, the ground-truth decision is to execute the branch condition  whose class list  intersects with the ground-truth classes. 

We derive the loss function as:
\begin{equation}
    L = y_i \cdot S(\max(P^{-}, \theta) - P^{+}) + (1-y_i) \cdot S(P^- - \theta) \,,
\end{equation}
where $y_i  = 1$ indicates that the ground-truth decision is executing one of the branches in \{$W_1$, $W_2$, ...$W_m$\}, and $y_i = 0$ indicates the ground-truth decision is selecting \code{others}, similarly to the previous section. $P^{+}$ is the maximum probability out of classes in $W^+$ (\ie $P^+ = \max_{c \in W^+ } p_c$), and $P^-$ is the maximum probability out of classes in $W^-$ (\ie $P^- = \max_{c \in W^- } p_c$). 
% \begin{equation*}
%     \footnotesize
%     L(O, G) =  \begin{cases}
%    P \Big( T, \max_{c \in W} p_c \Big ), & G \cap W = \emptyset \\
%      P \Big( \max_{c \in G \cap W } p_c, T \Big ) + P\Big( T, \max_{c \in W \setminus G } p_c \Big ), & G \cap W \neq \emptyset \\
% \end{cases}
% \end{equation*}

% \kt{$L_W$, where $W={\bigcap_{W_i \cup G\neq \phi} W_i}$ is ....}

Given this loss function, we can ensure that only when the first class encountered in the predicted labels, that belongs to $W$, is one of the classes in the ground-truth decision, the penalty would be low. 




\subsection{How to extract the software decision process}
% How we use sym-ex to get info, and which info 
\yh{Change all the whitelists}
To extract software context, we conduct an offline static analysis to detect code patterns introduced in Section~\ref{sec:empirical}. 
Particularly, we focus on the control-flow structures that are directly affected by ML API results. 

Given a code location of ML API invocation, \tool analyzes all the if-branches that have dependency on the ML API's output. For each combination of branch decisions, \tool adopts symbolic execution engine DSE~\cite{irlbeck2015deconstructing} and CVC5 constraint solver~\cite{cvc5} to find all the API outputs that lead to these decisions, which is the corresponding \wl.
If the software specifies only 1 branch condition, \tool reports pattern T-or-F. Otherwise, \tool analyzes the code structure to determine the pattern. % according to Figure~\ref{fig:hierarchy}:

\emph{How is the whitelist selected?} \tool analyzes all the statements inside the edges of an ML-API-related if-branch. If the software terminates all the examinations inside one of the branch edges (e.g., a break statement inside the loop and a return statement inside a function body), \tool regards that it as ``select 1 whitelist'' and further examines the order. 
If there is no such termination, \tool determines it is a M-to-N-set structure. 
% If there is no such termination, \tool determines whether it is pattern M-to-N-set or M-to-N-list according to the data structure of function returned value.

\emph{How is the order determined?} \tool finds all the loop structures and the equivalent statements outside the ML-API-related if-branches. It analysis their nested levels and the data dependency relationship of their iterators. 
If the software does not contain any loop iterating ML API's output or \wls, \tool stops examination and reports an absence of code pattern. 
If an inner (outer) loop iterates the ML API's output and the outer (inner) loop iterates the \wls, \tool regards it as pattern Priority-list (Top-label).  Note that, if the software contains multiple nested loops iterating the same variable, \tool focuses on the innermost one.


\subsection{How to change the MLaaS run-time backend}


% \subsection{Network Architecture}
% How we change the architecture of pre-trained model (freezing some part of the model)


% \subsection{Dataset Construction}



==> backups/3-method-1126.tex <==
\label{sec:method}

\subsection{Key components and workflow}

\begin{figure}
     \includegraphics[width=\linewidth]{figs/system_overview.pdf}
    \caption{System architecture of \tool. 
    % \jc{the overall flow looks ok, but there are so many minor issues in this figure. just to name a few: 
    % (1) where is "cloud service" coming from? 
    % (2) (a) and (b) shouldn't be distinguished (see comment in 3.1).
    % (3) i thought we decided to drop the arrow of giving the parser to developer?
    % (4) why "software context" is still used?
    % (5) user is not running python code! they run real apps
    % (6) why calling it "prediction" instead of API output?
    % (7) what's "model inference code"? if it's simply selecting the right model to run, we shouldn't introduce a new term.
    % (8) the three customized models should be put side by side (either all vertically or horizontally),
    % (9) why calling them "adapted" ML model? if the term we always use is "customized", then stick to that.}
    % \jc{in general, EVERY word must be picked very carefully, which you clearly didn't do :)}
    \yh{fixed comments, I'm calling it ML-model outputs instead of API outputs because the outputs comes before the ``output interface'', thus it's not API outputs yet}
    \jc{sorry i disagree. again, don't introduce new terms unless really necessary, which i don't think is the case. why dont you change the figure, to move the output and input the left of the model output interface, which should also be changed to "ML API"?}
    \jc{and don't let arrows overlap with arrows or lines (e.g., Model pool, Select)}
    }
\label{fig:system}
\end{figure}
% \mypara{Main components}

% \mypara{Extracted Software decision process}
Guided by the empirical study in \S~\ref{sec:empirical}, we propose \tool, an optimization framework that extracts the software decision process of the applications querying the MLaaS, and customizes the ML-model in the MLaaS backend. 
% summarizes the overall workflow of \tool.


As shown in Figure~\ref{fig:system}, when the application is being developed, 
% \jc{the term offline is new. the contrast between offline and online is overcomplicating. can we say something like when the application is being developed?}
besides the existing development procedure, the developers also run an MLaaS-provided parser plugin on their own machines, 
% \jc{the ``parser'' comes from nowhere. who provides it? even a simple ``MLaaS-provided parser'' is better}
% \jc{``locally'' has many meanings. pick a more precise term}, 
which extracts a summary of the software decision process
% \jc{maybe we need a different term; ``key features'' invites unnecessary confusion when used in an ML-related paper. how about a ``summary of the application's decision process''?}
% \jc{``extracts xxx from app into a file'' sounds wrong. shouldn't it be ``extract xxx from an app and uploads it as a file to xxx''?} 
from the application source code (details in \S~\ref{sec:extract}), and uploads it as a file to the MLaaS backend. In the MLaaS backend, \tool constructs a loss function based on the uploaded file, re-trains the ML-model with the constructed loss function, and adds the re-trained ML-model into the model pool (details in \S~\ref{sec:loss}). 
Finally, 
% \jc{the last phrase can be deleted}
an application queries the MLaaS with inputs via the existing interface,  
the MLaaS backend selects and runs inference with the customized ML-model(details in \S~\ref{sec:runtime}). 
% \jc{the separation among the three stages (``developer'', ``retraining'' and ``run-time'') is unnecessarily complicating the flow, and it introduces unnecessary terms, like ``run-time''. }

\jc{when introducing the flow, shouldn't we also highlight what we DO change and what we do NOT change?}

% The software decision process extracted from the Python source code, is composed of the key features characterizing it.\cc{This sentence does not provide additional information. Also, we could mention python in the implementation section} 

\jc{please don't explain a concept together with an application. you should always explain the concept first, and THEN use an example to explain it in a specific context.}
The summary of the software decision process consists of three aspects: (1) what are the target classes?  (2) what is the type of decision out of \emph{True-False}, \emph{Multi-Choice}, or \emph{Multi-Select}? (3) if the application makes a \emph{Multi-Choice} decision, how does the application reach a decision? 
These three aspects can uniquely identify which errors are critical or non-critical to the applications. Identifying the critical errors, as discussed in \S~\ref{sec:empirical}, which vary greatly across applications, provides us with great opportunities to customize the ML-models per application. 

Take the garbage classification application in Figure~\ref{fig:code}(a) as an example to illustrate. The summary of the software decision process for this application contains: (1) the three target classes \code{Recycle}, \code{Compost}, \code{Donate}; (2) a \emph{Multi-Choice} decision; (3) it follows the \emph{API-output order} to reach the \emph{Multi-Choice} decision.  

\jc{this last sentence is important but quite misleading. first of all, these features don't uniquely describe a decision process (e.g., they dont say what decisions will be made for each branch). instead, they specify what errors are critical and what errors are not critical.
second, you didn't say WHY they SHOULD be used by \tool to customize the ML model.}


\begin{comment}
\jc{this definition is extremely important and should be elevated. i suggest explain it in a separate paragraph. so you will have two paragraphs: one explain the overall workflow, and the second explains what's extracted from the source code and used to customize ML-model. it's important to keep the 1st para short.} 
\jc{it should be explained more formally, probably with a simple example, and the terms (e.g., multi-select vs. multi-choice) should be tightly connected to when they are first defined. remember, many reviewers may have skipped (or missed) their definitions in section 2.} 
\jc{moreover, i wouldn't mention JSON at the beginning. the exact format (not the content in the file) seems secondary to me}
\jc{what about score ranges? we need a way to explain all cases under consideration} 
% used in branch conditions; (2) whether the application is making multi-select or multi-choice decisions; (3) the order of examination for applications making multi-choice decisions. Then, the developers will upload the JSON of software decision process to the MLaaS backend. On the MLaaS backend side, \tool will re-train the ML model by re-sampling the training data with a more focus on the classes appeared in the applications, and constucting loss functions which directly penalize the critical errors.
\jc{i wouldn't distinguish training data resampling and loss function as two separate steps. last time we met as a group, we decided to say changing loss function is all that's needed, though the real implementation does resampling to speedup training. i like this idea, so the distinction should be secondary.} 

\jc{regarding the terminology, the parser doesn't extract the entire application decision process, it merely extracts the key features of the application decision process, which include xxx}



\jc{now this is too low-level when explaining the workflow. here, you can just say ``each time an application calls the ML API, the ML API backend will select the ML-model model customized for the application, ...''}
% the applications submit inference request to the ML API with input and the credential, like 

\jc{two meta comments: 1. Yuhan, you should read the terms used in the new Section 2 and use them consistently in section 3.
2. when writing 3.1, please make sure that every important term appears with a forward pointer to a later subsection that explains it in detail as well as a pointer to Figure 4}
\end{comment}

% which consists of a parser plugin, an ML model re-training scheme run in the offline stage, and in the online stage, \tool selects the customized ML model based on applications' credentials, and run inference with the customized model.  


% 3.2: given the extracted json, how should we re-train teh model 
% 3.3. how to extract
% 3.4: how to change the run-time interface

% \tool is an automated framework that adapts the ML-model behind the ML APIs, such that the number of software mis-behaviors can be greatly reduced when applied to an ML software. 

% \tool first performs static analysis to extract the code structure of the applications invoking MLaaS to understand how the software uses the ML API outputs to make application decisions. Then \tool constructs loss functions that penalize the critical errors of the applications. Finally, \tool re-trains the ML-models behind the ML APIs with the constructed loss function, without modifying the output interface of the ML APIs. 

% In this section, we will introduce how \tool performs static analysis and constructs the loss functions for the applications. 


% \subsection{Understanding Software Context}

% \subsection{Notations}
% \yh{not 3.2 }
% Denote the total number of classes that the ML-model behind the ML API can classify as $n$, and the whole set of classes is $C=\{C_1, C_2, ..., C_n\}$.  We define the symbols in our problem setting as follows:

% \begin{itemize}
%     \item $I$: the input image
%     \item $G=\{G_1, ..., G_a\}$: ground truth label set of $I$, where $G_i \in C$ for $1 \leq i \leq a$
%     \item $T$: the prediction threshold of the DNN behind the ML API
%     \item $O=\{O_1, O_2, ..., O_b\}$: the predicted classes over the prediction threshold $T$, where $P_i \in C$ for $1 \leq i \leq b$
%     \item $P=\{p_1, p_2, ..., p_b\}$: the corresponding probability for the predicted classes
    
    
% \end{itemize}



% \subsection{How to customize the ML model in the MLaaS backend}
\subsection{Customizing ML model for an application decision process}
\label{sec:loss}
As introduced in \S~\ref{sec:empirical},  applications in the wild differ greatly in their software decision processes. 
% For example, they may  define different number of target classes or include only a small subset of labels of the whole label set in their target classes and so on. 
This heterogeneity can lead to differences in critical errors\jc{remind people what critical errors are?} across applications. 
It is possible for an ML API error to be non-critical for one application, while critical for another. Thus, customizing the DNN in the MLaaS backend is important in order to incorporate the differences in software decision processes across applications.
\jc{the whole first paragraph is redundant to 3.1. this para should highlight why we start by explaining the step of DNN retraining}

The customization goal is to minimize the critical errors for each application.
% caused by ML API errors. 
Formally, the software decision process can be viewed as $\z = \Decision(\API(\x))$, where $\x$ is the input to the API, $\API(\x)$ is the ML API output, and $\Decision$ is the post-processing the application performs to make decisions based on API outputs. 
Let $\x_i\in \X$ denote the $i^{th}$ input, where $1 \leq i \leq M$, to the ML API, and $\hat{y_i}$ denote its ground-truth label. 
% $API(x_i)$ is a list of probabilities for label-based API (\eg image or text classification), 
% [$p_1, p_2, \dots, p_n$], for every label in the whole label set, and a score $O_i$ for score-based API (\eg sentiment analysis API). 
Formally, our customization goal is:
% Let $\mathds{1}_{x}$ denote the indicator function, where $\mathds{1}_{x} = 1$ when $x$ is \emph{True} and 0 otherwise. Therefore, the customization goal is:

\begin{equation}
    \min |\{x_i \in X | Decision(API(x_i)) \neq Decision(y_i)\}|
    \label{eq:goal}
\end{equation}

With this customization goal, together with the observation that applications typically heavily cluster on a small subset of labels in mind, we naturally come up with a \emph{strawman} of customization: re-train the ML-model with a re-sampled training dataset, which clusters on the labels appearing in the target classes of the application. 
While the original model is optimized to minimize average label-wise errors across a wide range of labels\footnote{Traditionally, the loss function minimizes the average error between the predicted probability and ground-truth labels for every class, which we refer to as average label-wise errors. } (\eg 9605 labels in Open Images~\cite{ASL}), this strawman approach can reduce the label-wise errors of labels belonging to the target classes. However, it is unaware that applications may make different decisions, including \emph{True-False}, \emph{Multi-select}, and \emph{Multi-choice}, and how these decisions affect the severity of ML API errors. 

Fortunately, the loss function used in ML-model training provides a \emph{differentiable} way to capture the incorrectness of the ML-model's predictions with respect to the ground-truth. In addition, we formulate the software decision process in a structured format. This allows \tool to translate it into a loss function with the goal of both clustering on labels in target classes and directly minimizing the critical errors (Equation~\ref{eq:goal}). 
% \yh{Why they fails and we do not fail }
% \yh{add general recipe }
Compared to the strawman which may spare energy penalizing non-critical errors, such as penalizing mis-classifications within the target classes, 
our solution only focuses on penalizing the critical ones, such as mis-classifications across target classes. 





As illustrated in \S~\ref{sec:empirical}, the critical errors in the applications can differ greatly for different target classes, types of decisions, and order of examination. As a result, we construct different loss functions, with the unified goal of minimizing critical errors, for each type of applications. 

A general recipe for our loss function is formulated as:

\begin{equation}
    L_i = H_{o}(\hat{y_i}) \cdot S(\theta-G(y_i)) + \sum_{j=1}^{m} H_j(\hat{y_i}) \cdot S(F(y_i)-G_j(y_i))  
\end{equation}

\mypara{True-False} This type of application defines only one target class, checking if the API outputs match with
% \cc{I suspect ``intersect'' is a better praise, as we the API output includes a list of items}
it. We denote the labels included in the target class as $W_1$. Therefore, the corresponding loss function is:
\begin{equation}
    L = y_i\cdot \frac{M}{N_1}  \cdot \textrm{S}(\theta - P_1) + (1-y_i) \cdot \frac{M}{M-N_1} \textrm{S}(P_1 - \theta) \,,
\label{eq:loss}
\end{equation}
where $y_i = 1$ when the ground-truth of the input intersects with the target class $W_1$, and $y_i=0$ otherwise. $\theta$ is the prediction threshold, where output labels whose predicted probability are greater than it will be included in the output label list. $P_1$ is the maximum probability of labels in $W_1$ (\ie $P_1 = max_{c \in W_1} p_c  $). $S(x)$ is the Sigmoid function $\frac{1}{1+e^{-k x}}$, which we will keep the notation in the rest of the paper. $N_1$ is the total number of inputs in the training dataset whose ground-truth decision is the target class (\ie $N_1 = \sum\limits_{j=1}^{M}\mathds{1}_{\hat{y_j}\cap W_1 \neq \emptyset}$), denoted as target-inputs. The inputs whose ground-truth decision is selecting the non-target class are denoted as non-target-inputs. 


% With this loss function, \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{a low penalty} otherwise, for \code{$W_1$}-inputs. Similarly for \code{other}-inputs. 

Ideally, we want the loss function to be a step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{no penalty} when $P_1$ is greater than $\theta$ for target-inputs. However, to make the loss function differentiable, we use the Sigmoid function to approximate the step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{a low penalty} otherwise, for target-inputs. Similarly for non-target-inputs. 

Furthermore, to achieve the effect of clustering on labels in $W_1$, the loss function applies a weight of $\frac{M}{N_1}$ on target-inputs, and a weight of $\frac{M}{M-N_1}$. Therefore, the number of target-inputs and non-target-inputs are effectively balanced, instead of biasing towards either the target class or non-target class. 

\mypara{Multi-Select} This type of application defines several target classes, $\{W_1, W_2, \dots, W_m\}$, and multiple selections are allowed about which class(es) the ML API output belongs to. We construct the following loss function:

\begin{equation}
    L = \frac{M}{N_i}\sum_{j=1}^{m} y_i \cdot \textrm{S}(\theta - P_j) + (1-y_i) \cdot \textrm{S}(P_j - \theta) \,,
\label{eq:multi-select}
\end{equation}
where $y_i$ indicates whether this input belongs to the $j^{th}$ target class $W_j$, $y_i = 1$ when $\hat{y_i} \cap W_j \neq \emptyset$, and $y_i = 0$ otherwise. Similar to Equation~\ref{eq:loss}, $P_j$ is the maximum probability of classes belonging to $W_j$ (\ie $P_j = max_{c \in W_j} p_c$). Let $\mathbb{W} = \bigcup\limits_{j=1}^{m} W_j$ denote the union of all the target classes defined in the application, and $\mathcal{W}_i = \bigcup_{W_j \cap  \hat{y_i} \neq \emptyset} W_j $ denote the union of all the ground-truth target classes for the $i^{th}$ input (same notation used in the rest of the section). 
When $\hat{y_i} \cap \mathbb{W} \neq \emptyset$, $N_i$ is the total number of inputs in the training data belonging to $\mathcal{W}_i$ (\ie $N_i = \sum\limits_{j=1}^{M}\mathds{1}_{\hat{y_j}\cap \mathcal{W}_i \neq \emptyset}$); otherwise, $N_i$ denotes the total number of non-target-inputs (\ie $N_i = \sum\limits_{j=1}^{M}\mathds{1}_{\hat{y_i} \cap \mathbb{W} = \emptyset}$), the same notation will be used throughout this section. Similarly to Equation~\ref{eq:loss}, the weight $\frac{M}{N_i}$ is used to achieve the effect of balancing each of the target classes and non-target class.

With this loss function, only if the application decisions led by the ML API outputs exactly match with the ground-truth decisions, the penalty will be low.

\mypara{Multi-Choice API-output order} This type of application defines several target classes, and starts with checking if the first API output label matches with any of the classes. If so, the rest of the labels are skipped. Otherwise, later labels will be checked. We construct the following loss function:
 \begin{equation}
    L = \frac{M}{N_i} \Bigl( y_i \cdot S(\max(P^{-}, \theta) - P^{+}) + (1-y_i) \cdot S(P^- - \theta) \Bigr) \,,
\label{eq:api_output}
\end{equation}
where $y_i  = 1$ indicates ground-truth labels intersect with $\mathbb{W}$, and $y_i=0$ otherwise. $P^{+}$ is the maximum probability out of classes in $\mathcal{W}_i$ (\ie $P^+ = \max_{c \in \mathcal{W}_i } p_c$), and $P^-$ is the maximum probability out of classes in the incorrect target classes (\ie $P^- = \max_{c \in (\mathbb{W} \setminus \mathcal{W}_i) } p_c$). 

Therefore, the loss function ensures only if the first output label encountered belonging to any of the target classes, matches with the ground-truth class, the penalty will be low. 

\mypara{Multi-Choice application-choice order} This type of application starts with checking if the first target class matches with any output label before moving to the next class. We construct the following loss function for this type:

\begin{equation}
\begin{split}
    L = \frac{M}{N_i} \Bigl( y_i \cdot \textrm{S} (\max(\theta, P_{k^{-}})  - P_k ) + 
    (1-y_i) \cdot \textrm{S}(P - \theta) \Bigr) \,,
\end{split}
\label{eq:app_choice}
\end{equation}

Similarly to Equation~\ref{eq:api_output},  $y_i  = 1$ indicates ground-truth labels intersect with $\mathbb{W}$, and $y_i=0$ otherwise. $k$ is the index of the highest-priority target class that intersects with the ground-truth labels (\ie $k = \min \{j|W_j \cap \hat{y_i} \neq \emptyset\}$). $P_k$ is the maximum probability for labels belonging to $W_k$, and $P_{k^{-}}$ is the maximum probability out of the labels belonging to higher priority classes than the ground-truth class (\ie$W_{k^{-}} = \bigcup_{\{j|\hat{y_i} \cap W_j \neq \emptyset  \textrm{ and }  j < k \}} W_j$ and $P_{k^{-}} = \max_{c\in W_{k^{-}} }p_c$). $P$ is the maximum probability of the classes belonging to $\mathbb{W}$. 


This loss function ensure that only if the first target class that matches with any of the output labels is the ground-truth class, the penalty incurred by the loss function will be low. 


\mypara{Value-ranges} For APIs outputting scores, such as the sentiment analysis API, application check whether the score lies in defined value ranges. The loss function we construct is:

\begin{equation}
    L = \frac{M}{N_i} \cdot \Bigl( S(l_i - O_i) + S(O_i - h_i) \Bigr) \,,
\end{equation}
where $l_i$ is the lower bound of the ground-truth  value range, and $h_i$ is the upper bound of the ground-truth value range. $N_i$ is defined similarly to previous sections. 

Therefore, the penalty incurred by the loss function will be low only when the API output score lies in the ground-truth value ranges.
% Given this loss function, we can ensure that only when the first class encountered in the predicted labels, that belongs to $W$, is one of the classes in the ground-truth decision, the penalty would be low. 




\jc{
an example outline of this subsection (each bullet is a para)
\begin{itemize}
\item why we start with this? the key step is customizing ML-model for each application.
\item what's the goal
\item what's a strawman (resampling training data)? and why is it not good (doesn't distinct multi-choice vs multi-option and order of examination)? (this para must be short). if room, also bring up some prior work that also does this
\item our idea: rewriting loss function. give a general recipe of how this is done
\item why is it better? (this should directly contrast with the strawman)
\item more case-by-case explanation.
\end{itemize}
}

\jc{regarding how to explain the goal, you can expand the following: formally an application can be viewed as $z=Decision(Model(x))$. for a given decision process $Decision$, the goal is to minimize $Decision(Model(x_i))\neq Decision(\hat{y_i})$ over a set of $x_i$, where $\hat{y_i}$ is the ground truth label of $x_i$.}



% \mypara{Notations} 
% Denote the total number of classes that the ML-model behind the ML API can classify as $n$, and the whole set of classes is $C=\{C_1, C_2, ..., C_n\}$.  We define the symbols in our problem setting as follows. 
% \begin{itemize}
%     \item $I$: the input image
%     \item $G=\{G_1, ..., G_a\}$: ground truth label set of $I$, where $G_i \in C$ for $1 \leq i \leq a$
%     \item $T$: the prediction threshold of the ML-model behind the ML API
%     \item $O=\{O_1, O_2, ..., O_b\}$: the predicted classes over the prediction threshold $T$, where $P_i \in C$ for $1 \leq i \leq b$
%     \item $P=\{p_1, p_2, ..., p_b\}$: the corresponding probability for the predicted classes
    
    
% \end{itemize}

% \mypara{Customization goal} For T-or-F, we want to minimize the critical errors which are caused by the API outputs that lead to the  execution of the \emph{False} branch, when the statement should be \emph{True} according to the ground-truth, and vice versa. With the above notations, our goal can be written as:

% \begin{equation}
% \begin{aligned}
% \min \sum\limits_{i=1}^{M}( y_i \cdot \mathds{1}_{\theta - P} + (1-y_i) \cdot \mathds{1}_{P-\theta} )
% \end{aligned}
% \end{equation}

% Where $\mathds{1}_{x} = 1$ when $x > 0$, and 0 otherwise. $y_i = 1$ if the $i^{th}$ input belongs to the class list defined in the branch condition, which we denote as $W$. $\theta$ is the prediction threshold, where classes whose predicted probability is higher than the threshold will be included in the output label list. $P$ is the maximum probability of classes in $W$, in other words, $P = max_{c \in W} p_c$.
% there are two types of critical errors: (1) for inputs whose statement in the branch condition is \emph{True} according to the ground-truth, which we refer to as \emph{target-inputs}, the API outputs lead the application selecting the \emph{False} branch; (2) for inputs whose statement is \emph{False}, the API outputs lead the application selecting the \emph{True} branch. To minimize incorrect application decisions, we want: 




% \yh{Outline of this section: 
% 1. first list the goal in math (or text): minimize the incorrect app decisions
% 2. a naive re-training scheme is to use a training data that  focuses on classes appeared in the apps 3. why this design is not good: it can only solve xxx, but not xxx 4. describe our loss function }
% \yh{goal: minimize the incorrect app decisions; what we have: extracted software decision process (key dimensions) }
% As shown in our empirical study in Section~\ref{sec:empirical}, we find the software decision process can be characterized by two aspects: (1) the class list(s) or value ranges that are used in branch conditions (2) the structures of the branch conditions.

% In this section, we will describe how we incorporate the software decision process in the loss function. Our optimization is composed of two steps: (1) clustering the training data to focus on classes appearing in the branch conditions; (2) constructing the loss functions to be aware of the software decision process. Our objective is to incur a high penalty on critical errors, and no penalty if the errors make no impact on the application. 


% To begin with, we first introduce the loss function traditionally used in multi-label image classification.


% The binary cross-entropy loss function used in multi-label classification task~\cite{ASL} is denoted as:
% \begin{equation}
%     L_{bce}  = -\frac{1}{n}\sum_{i=1}^n{(y_i\log(p_i) + (1 - y_i)\log(1 - p_i))} \,,
% \end{equation}
% where $y_i = 1$ if class $i$ is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. $p_i$ is the predicted probability for class $i$. 
% \begin{itemize}
%     \item  $y_i = 1$ if the $i^{th}$ class is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. 
%     \item $p_i$ is the predicted probability for the $i^{th}$ class.
% \end{itemize}
% where $y_i$ indicates whether the $i^{th}$ class exists in the input input $I$ or not. In other words, $y_i = 1$ if the $i^{th}$ class exists in the input $I$, and $y_i = 0$ otherwise. \cc{It is still one sentence, so please do not start a new paragraph}


% \subsubsection{Clustering training data}


% To achieve the first step, one approach is to assign different weights to inputs with ground-truth decisions of executing the \code{Others} branch and non-\code{Others} branches.  
% We take a simple example to illustrate this approach. An application  defines one branch condition to check if the API outputs intersect with a class list $W_1$. $W_1$ is a non-empty subset of the whole label set $C$ that the ML-model is able to classify. 
%  The original fraction of images in the training data whose ground-truth  decisions are executing the \code{$W_1$}-branch (\ie $G \cap W \neq \emptyset$), which we refer to as \code{$W_1$}-inputs,  is $A$. 
%  % \cc{This sentence is very hard to read. Can we use phrase like ``which we refer to as $W$-images''?} 
% The fraction of images whose ground-truth decisions are executing the \code{other}-branch is $1-A$,  which we refer to as \code{others}-inputs. If we want to balance the distribution between $W$-inputs and \code{others}-inputs, we can use a loss function that assigns higher weights to \code{W}-inputs:

% \begin{equation}
%     L_D = y_1 \cdot \frac{1}{A} \cdot L_{bce} + (1-y_1)\cdot A \cdot L_{bce} \,,
% \end{equation}
% where $y_1$ indicates whether this input is a \code{$W$}-input or not. In other words, $y_1 = 1$ when the input is a \code{$W$}-input ($G \cap W \neq \emptyset$), and $y_1 = 0$ otherwise ($G \cap W = \emptyset$). 

% In this way, \code{$W$}-inputs and \code{others}-inputs are taking the same effect during training, instead of biasing towards either \code{W} or \code{others}. 

% % We construct loss functions for each type of software represented by the software examples shown in section~\ref{sec:empirical}. \cc{Maybe say some high-level ideas, more intuition}

% \subsubsection{Branch condition structure 1: T-or-F} 

% For the software that defines only one branch condition, checking if the output labels $O$ intersect with a class list $W_1$. We penalize the critical errors: (1) all the classes in $W_1$ are not included in top predictions for \code{$W_1$}-inputs; or (2) at least one class in $W_1$ are included in top predictions for \code{others}-inputs.




% \begin{equation}
%     L_{W_1} =y_1 \cdot \textrm{S}(\theta - P_1) + (1-y_1) \cdot \textrm{S}(P_1 - \theta) \,,
% \label{eq:loss}
% \end{equation}
% where
% $y_1$ indicates whether this input is a \code{$W_1$}-input or not. 
% In other words, $y_1 = 1$ if the input is a \code{$W_1$}-input, and $y_1=0$ if the input is a \code{others}-input. $\theta$ is the prediction threshold, where classes whose predicted probability will be included in the output label list. $P_1$ is the maximum probability of classes in $W_1$ (\ie $P_1 = max_{c \in W_1} p_c  $). $S(x)$ is the Sigmoid function $\frac{1}{1+e^{-k x}}$, which we will denote as $S$ in the rest of the paper. 



% Ideally, we want the loss function to be a step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{no penalty} when $P_1$ is greater than $\theta$ for  \code{$W_1$}-inputs. However, to make the loss function differentiable, we use the Sigmoid function to approximate the step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{a low penalty} otherwise, for \code{$W_1$}-inputs. Similarly for \code{other}-inputs. 



% \subsubsection{Branch condition structure 2: M-to-N-set} 

%  In M-to-N-set, several branch conditions are defined, each checking if a class list intersects with the API output $O$. All the fulfilled branches will be executed. We denote all the $m$ class lists the application uses in branch conditions as {$W_1$, ..., $W_m$}. In this pattern, the ground-truth  decisions is executing \emph{all} the branches whose class lists  intersect with the ground-truth labels. 

% We derive the following loss function for M-to-N-set:
% \begin{equation}
%     L = \sum_{i=1,\cdots,m} y_i \cdot \textrm{S}(\theta - P_i) + (1-y_i) \cdot \textrm{S}(P_i - \theta) \,,
% \end{equation}
% where $y_i$ indicates whether  $W_i$ is among the branches the ground-truth decision executes, in other words, $y_i = 1$ if $G \cap W_i \neq \emptyset$, and $y_i = 0$ otherwise. Similar to Equation~\ref{eq:loss}, $P_i$ is the maximum probability of classes belonging to $W_i$ (\ie $P_i = max_{c \in W_i} p_c$). 

%  Only if the application decisions led by $O$ exactly match with the ground-truth decisions, the penalty will be low.


% % \kt{$\sum_{i=1,\cdots,N} L_{W_i}$}



% \subsubsection{Branch condition structure 3: Priority-list}

% Priority-list defines several branch conditions, and each of them is associated with a class list $W_i$. The application checks the branch conditions from highest to lowest priority until finding the first one whose class list intersects with API output labels $O$. Let $W_i$ (where $1 \leq i \leq m$) denote the class lists used in branch conditions, where class lists with smaller $i$ indicate higher priority. Let $W$ denote the union of the classes in all the whitelists, in other words, $W = \cup^{m}_{i=1}W_i$. The ground-truth decision  is executing the highest priority branch whose associated class list intersects with the ground-truth classes $G$. 

% We derive the loss function as:
% \begin{equation}
% \begin{split}
%     L = y_i \cdot \textrm{S} (\max(\theta, P_{k^{-}})  - P_k ) + 
%     (1-y_i) \cdot \textrm{S}(P - \theta) \,,
% \end{split}
% \end{equation}
% where $y_i = 1$ when the ground-truth decision is executing one of the branches in $\{ W_1, \cdots, W_m\}$ (\ie $G \cap W \neq \emptyset$), and  $y_i = 0$ when the ground-truth decision is executing the \code{others} branch. 
% $k$ is the index of the highest-priority branch whose class list intersects with the ground-truth classes (\ie $k = \min \{i|WL_i \cap G \neq \emptyset\}$). $P_k$ is the maximum predicted probability for classes belonging to $W_k$, and $P_{k^{-}}$ is the maximum predicted probability out of the classes belonging to higher priority branches than the ground-truth branch (\ie $k^{-} = \min \{i | W_i \cap (G \setminus W ) \neq \emptyset \textrm{ and } i < k \}$). $P$ is the maximum probability of the classes belonging to $W$. 

% Given this loss function, only if the highest-priority branch whose class list intersects with the predicted classes $O$ is the ground-truth decision, the penalty will be low. 


% \subsubsection{Branch condition structure 4: Top-label}

% Top-label defines several branch conditions, and associates with each of them with a class list $W_i$, similar to Priority-list. However, unlike Priority-list, it checks the \emph{API output labels} one by one until one of them intersects with any of the class lists. Similar to the previous section, $W$ is the union of classes in all the defined class lists. We denote the classes belonging to class lists intersecting with ground-truth classes as $W^+ = \bigcup_{W_i \cap G \neq \emptyset} W_i$, and the classes belonging to \wls that do not intersect with ground-truth classes as $W^- = W \setminus W^+$.
 
% In this pattern, the ground-truth decision is to execute the branch condition  whose class list  intersects with the ground-truth classes. 

% We derive the loss function as:
% \begin{equation}
%     L = y_i \cdot S(\max(P^{-}, \theta) - P^{+}) + (1-y_i) \cdot S(P^- - \theta) \,,
% \end{equation}
% where $y_i  = 1$ indicates that the ground-truth decision is executing one of the branches in \{$W_1$, $W_2$, ...$W_m$\}, and $y_i = 0$ indicates the ground-truth decision is selecting \code{others}, similarly to the previous section. $P^{+}$ is the maximum probability out of classes in $W^+$ (\ie $P^+ = \max_{c \in W^+ } p_c$), and $P^-$ is the maximum probability out of classes in $W^-$ (\ie $P^- = \max_{c \in W^- } p_c$). 


% Given this loss function, we can ensure that only when the first class encountered in the predicted labels, that belongs to $W$, is one of the classes in the ground-truth decision, the penalty would be low. 




\subsection{How to extract the software decision process}
\label{sec:extract}
% How we use sym-ex to get info, and which info 
\yh{Change all the whitelists}
To extract software decision process, we conduct an offline static analysis to detect code patterns introduced in Section~\ref{sec:empirical}. 
Particularly, we focus on the control-flow structures that are directly affected by ML API results. 

Given a code location of ML API invocation, \tool analyzes all the if-branches that have dependency on the ML API's output. For each combination of branch decisions, \tool adopts symbolic execution engine DSE~\cite{irlbeck2015deconstructing} and CVC5 constraint solver~\cite{cvc5} to find all the API outputs that lead to these decisions, which is the corresponding \wl.
If the software specifies only 1 branch condition, \tool reports pattern True-False. Otherwise, \tool analyzes the code structure to determine the pattern. % according to Figure~\ref{fig:hierarchy}:

\emph{Whether multi-select or multi-choice?} \tool analyzes all the statements inside the edges of an ML-API-related if-branch. If the software terminates all the examinations inside one of the branch edges (e.g., a break statement inside the loop and a return statement inside a function body), \tool regards that it as a multi-choice and further examines the order. 
If there is no such termination, \tool determines it is multi-select structure. 


\emph{How is the order determined?} \tool finds all the loop structures and the equivalent statements outside the ML-API-related if-branches. It analysis their nested levels and the data dependency relationship of their iterators. 
If the software does not contain any loop iterating ML API's output or application choices, \tool stops examination and reports an absence of code pattern. 
If an inner (outer) loop iterates the ML API's output and the outer (inner) loop iterates the application choices, \tool regards it as pattern Application-choice order (API-output order).  Note that, if the software contains multiple nested loops iterating the same variable, \tool focuses on the innermost one.


\subsection{How to change the MLaaS run-time backend}
\label{sec:runtime}



==> backups/3-method-1129.tex <==
\label{sec:method}

Guided by the empirical study in \S\ref{sec:empirical}, this section presents \tool, an optimization framework that customizes ML models of the MLaaS backend for the decision processes of different applications.

\subsection{Key components and workflow}
\label{sec:overall}
\begin{figure}
     \includegraphics[width=\linewidth]{figs/system_overview.pdf}
    \caption{System architecture of \tool. 
    % \jc{the overall flow looks ok, but there are so many minor issues in this figure. just to name a few: 
    % (1) where is "cloud service" coming from? 
    % (2) (a) and (b) shouldn't be distinguished (see comment in 3.1).
    % (3) i thought we decided to drop the arrow of giving the parser to developer?
    % (4) why "software context" is still used?
    % (5) user is not running python code! they run real apps
    % (6) why calling it "prediction" instead of API output?
    % (7) what's "model inference code"? if it's simply selecting the right model to run, we shouldn't introduce a new term.
    % (8) the three customized models should be put side by side (either all vertically or horizontally),
    % (9) why calling them "adapted" ML model? if the term we always use is "customized", then stick to that.}
    % \jc{in general, EVERY word must be picked very carefully, which you clearly didn't do :)}
    % \yh{fixed comments, I'm calling it ML model outputs instead of API outputs because the outputs comes before the ``output interface'', thus it's not API outputs yet}
    % \jc{sorry i disagree. again, don't introduce new terms unless really necessary, which i don't think is the case. why dont you change the figure, to move the output and input the left of the model output interface, which should also be changed to "ML API"?}
    % \jc{and don't let arrows overlap with arrows or lines (e.g., Model pool, Select)}
    }
\label{fig:system}
\end{figure}
% \mypara{Main components}

% \mypara{Extracted application's decision process}
% the application's decision process of the applications querying the MLaaS, and customizes the ML model in the MLaaS backend.
% summarizes the overall workflow of \tool.


\mypara{Workflow}
Figure~\ref{fig:system} depicts \tool's high-level workflow. 
When the developers publish an application \App, they first run a parser script provided by \tool on \App's source code to extract its {\em decision-process summary} (explained shortly), and then upload the summary to \tool's MLaaS backend (details in \S\ref{sec:extract}). 
In the backend, \tool uses the received decision-process summary to construct a new loss function, such that when the ML model is re-trained using the new loss function, it will produce inference results that yield fewer application decision failures for the application \App (details in \S\ref{sec:loss}).
\tool then adds the new ML model to a pool of customized ML models. 
% \jc{the last phrase can be deleted}
When a user of application \App queries the MLaaS backend with an input via the existing ML API, the backend will select the ML model customized for \App and return the inference result of the selected ML model (details in \S\ref{sec:runtime}).


\begin{comment}
When the application is being developed, 
% \jc{the term offline is new. the contrast between offline and online is overcomplicating. can we say something like when the application is being developed?}
besides the existing development procedure, the developers also run an MLaaS-provided parser plugin on their own machines, 
% \jc{the ``parser'' comes from nowhere. who provides it? even a simple ``MLaaS-provided parser'' is better}
% \jc{``locally'' has many meanings. pick a more precise term}, 
which extracts a summary of the application's decision process
% \jc{maybe we need a different term; ``key features'' invites unnecessary confusion when used in an ML-related paper. how about a ``summary of the application's decision process''?}
% \jc{``extracts xxx from app into a file'' sounds wrong. shouldn't it be ``extract xxx from an app and uploads it as a file to xxx''?} 
from the application source code (details in \S\ref{sec:extract}), and uploads it as a file to the MLaaS backend. 
\end{comment}




% \jc{the separation among the three stages (``developer'', ``re-training'' and ``run-time'') is unnecessarily complicating the flow, and it introduces unnecessary terms, like ``run-time''. }

% \jc{when introducing the flow, shouldn't we also highlight what we DO change and what we do NOT change?}

% The application's decision process extracted from the Python source code, is composed of the key features characterizing it.\cc{This sentence does not provide additional information. Also, we could mention python in the implementation section} 

% \jc{please don't explain a concept together with an application. you should always explain the concept first, and THEN use an example to explain it in a specific context.}

\smallskip
\noindent
The {\bf \summary} extracted from an application includes three pieces of information: 
\begin{packeditemize}
\item the values included in each target class; \yh{double check}
\item the type of decision (\ie \emph{True-False}, \emph{Multi-Choice}, or \emph{Multi-Select});
\item the matching order over the target classes, if the application makes a \emph{Multi-Choice} decision.
\end{packeditemize}
These three pieces of information can uniquely identify which errors are critical and which are non-critical to the application, which provides vital information to customize the ML model for the application, as elaborated in \S\ref{sec:loss}. 
% vary greatly across applications, 
% provides us with great opportunities to customize the ML models per application. 

To give a concrete example, the \summary of the garbage classification application in Figure~\ref{fig:code}(a) contains
(1) the three target classes (each being a list of labels): \code{Recycle}, \code{Compost}, and \code{Donate}; (2) the \emph{Multi-Choice} type of decision; and 
(3) it follows the \emph{API-output order} to reach the \emph{Multi-Choice} decision.  


\mypara{What is changed, what is not}
It is important to notice that \tool does {\em not} change the ML API or the source code or the executable of the application.
% \jc{check the term with shan/chengcheng}
That said, \tool does change two things. 
First, the application developers need to run \tool's parser script to extract the decision-process summary.
Second, \tool modifies the MLaaS backend to re-train an ML model per application (instead of serving the same model to all applications) and selects the right ML model to serve each query.
% When the application queries the MLaaS, 
% a model selector module is added in the backend to choose the ML model customized to the application, based on the application ID incorporated in the identification credential.

% \jc{this last sentence is important but quite misleading. first of all, these features don't uniquely describe a decision process (e.g., they dont say what decisions will be made for each branch). instead, they specify what errors are critical and what errors are not critical.
% second, you didn't say WHY they SHOULD be used by \tool to customize the ML model.}


\begin{comment}
\jc{this definition is extremely important and should be elevated. i suggest explain it in a separate paragraph. so you will have two paragraphs: one explain the overall workflow, and the second explains what's extracted from the source code and used to customize ML model. it's important to keep the 1st para short.} 
\jc{it should be explained more formally, probably with a simple example, and the terms (e.g., multi-select vs. multi-choice) should be tightly connected to when they are first defined. remember, many reviewers may have skipped (or missed) their definitions in section 2.} 
\jc{moreover, i wouldn't mention JSON at the beginning. the exact format (not the content in the file) seems secondary to me}
\jc{what about score ranges? we need a way to explain all cases under consideration} 
% used in branch conditions; (2) whether the application is making multi-select or multi-choice decisions; (3) the order of examination for applications making multi-choice decisions. Then, the developers will upload the JSON of application's decision process to the MLaaS backend. On the MLaaS backend side, \tool will re-train the ML model by re-sampling the training data with a more focus on the classes appeared in the applications, and constucting loss functions which directly penalize the critical errors.
\jc{i wouldn't distinguish training data resampling and loss function as two separate steps. last time we met as a group, we decided to say changing loss function is all that's needed, though the real implementation does resampling to speedup training. i like this idea, so the distinction should be secondary.} 

\jc{regarding the terminology, the parser doesn't extract the entire application decision process, it merely extracts the key features of the application decision process, which include xxx}



\jc{now this is too low-level when explaining the workflow. here, you can just say ``each time an application calls the ML API, the ML API backend will select the ML model model customized for the application, ...''}
% the applications submit inference request to the ML API with input and the credential, like 

\jc{two meta comments: 1. Yuhan, you should read the terms used in the new Section 2 and use them consistently in section 3.
2. when writing 3.1, please make sure that every important term appears with a forward pointer to a later subsection that explains it in detail as well as a pointer to Figure 4}
\end{comment}

% which consists of a parser plugin, an ML model re-training scheme run in the offline stage, and in the online stage, \tool selects the customized ML model based on applications' credentials, and run inference with the customized model.  


% 3.2: given the extracted json, how should we re-train teh model 
% 3.3. how to extract
% 3.4: how to change the run-time interface

% \tool is an automated framework that adapts the ML model behind the ML APIs, such that the number of software mis-behaviors can be greatly reduced when applied to an ML software. 

% \tool first performs static analysis to extract the code structure of the applications invoking MLaaS to understand how the software uses the ML API outputs to make application decisions. Then \tool constructs loss functions that penalize the critical errors of the applications. Finally, \tool re-trains the ML models behind the ML APIs with the constructed loss function, without modifying the output interface of the ML APIs. 

% In this section, we will introduce how \tool performs static analysis and constructs the loss functions for the applications. 


% \subsection{Understanding Software Context}

% \subsection{Notations}
% \yh{not 3.2 }
% Denote the total number of classes that the ML model behind the ML API can classify as $n$, and the whole set of classes is $C=\{C_1, C_2, ..., C_n\}$.  We define the symbols in our problem setting as follows:

% \begin{itemize}
%     \item $I$: the input image
%     \item $G=\{G_1, ..., G_a\}$: ground truth label set of $I$, where $G_i \in C$ for $1 \leq i \leq a$
%     \item $T$: the prediction threshold of the DNN behind the ML API
%     \item $O=\{O_1, O_2, ..., O_b\}$: the predicted classes over the prediction threshold $T$, where $P_i \in C$ for $1 \leq i \leq b$
%     \item $P=\{p_1, p_2, ..., p_b\}$: the corresponding probability for the predicted classes
    
    
% \end{itemize}



% \subsection{How to customize the ML model in the MLaaS backend}
\subsection{Customizing ML model for an application decision process}
\label{sec:loss}
% As introduced in \S\ref{sec:empirical},  applications in the wild differ greatly in their application's decision processes. 
% % For example, they may  define different number of target classes or include only a small subset of labels of the whole label set in their target classes and so on. 
% This heterogeneity can lead to differences in critical errors\jc{remind people what critical errors are?} across applications. 
% It is possible for an ML API error to be non-critical for one application, while critical for another. Thus, customizing the DNN in the MLaaS backend is important in order to incorporate the differences in application's decision processes across applications.
% \jc{the whole first paragraph is redundant to 3.1. this para should highlight why we start by explaining the step of DNN re-training}

% Model re-training has been widely adopted in ML to update the generic pre-trained ML models to work for related but different tasks~\cite{mullapudi2019online,ekya}. In model re-training, the model is initialized from a pre-trained model, and  its model parameters are updated based on the goal of the new task.
The idea of model re-training has been widely adopted in ML to update the generic pre-trained ML models to work for related but different tasks~\cite{mullapudi2019online,ekya}. The key challenge is how to formulate the customized optimization goal and design re-training strategy to efficiently achieve high  accuracy on different tasks.
\shan{Reading this sentence, as a picky reviewer, I would start worrying about the novelty of this work over model re-training work. The next sentence ``In our problem setting'' reads quite similar to the previous sentences. Is it possible to rephrase so that the difference is more obvious?}  \cc{Done. I feel the last sentence actually do not provide new information. So I deleted it.}
% In our problem setting, we want to initialize from a pre-trained model for the original ML task (\eg image or text classification), and re-train it with our customization goal.  
  

Our {\bf customization goal} is to minimize the critical errors for each application.
% caused by ML API errors. 
If we view the application's decision process  as $\z = \Decision(\API(\x))$, where $\x$ is the input to the API, $\API(\x)$ is the ML API output, and $\Decision$ is the post-processing the application performs to make decisions based on API outputs. 
Let $\x_i\in \X$ denote the $i^{th}$ input to the ML API, and $\hat{y_i}$ denote its ground-truth label. 
% $API(x_i)$ is a list of probabilities for label-based API (\eg image or text classification), 
% [$p_1, p_2, \dots, p_n$], for every label in the whole label set, and a score $O_i$ for score-based API (\eg sentiment analysis API). 
Formally, our customization goal is written as:
% Let $\mathds{1}_{x}$ denote the indicator function, where $\mathds{1}_{x} = 1$ when $x$ is \emph{True} and 0 otherwise. Therefore, the customization goal is:

\begin{equation}
    \min |\{x_i \in X | Decision(API(x_i)) \neq Decision(\hat{y_i})\}|
    \label{eq:goal}
\end{equation}


A common practice in ML is to utilize the loss function to express the optimization goal~\cite{celoss}. For example, the Binary Cross Entropy loss is used in image or text classification tasks, and Mean Squared Error loss is used in regression tasks. 

% Take classification task as an example, the Binary Cross Entropy loss is defined as:

% \begin{equation}
%     L_{BCE}(y_i) = \sum_{j=1}^{n} -\hat{y_{i, j}} \cdot log(y_{i,j}) - (1-\hat{y_{i,j}}) \cdot log(1-y_{i,j})
%     \label{eq:bce}
% \end{equation}
% where $y_i$ is the output of the ML model on the $i^{th}$ input, which is a list of probabilities. The higher the probability at the $j^{th}$ index is, the more confident the model is about the existence of the $j^{th}$ label in the input.  $\hat{y_i}$ is the ground truth for the $i^{th}$ input. $\hat{y_{i,j}} = 1$ if the $j^{th}$ label is in the ground truth of the $i^{th}$ input. Intuitively, this loss function incurs a high penalty when the $j^{th}$ label is present in the ground truth, but the model outputs a low probability for it, and vice versa. 

The question we want to answer is,  \emph{how to design a loss function that can achieve our customization goal?}

\mypara{Strawman}With the observation that applications typically heavily cluster on a small subset of labels appearing in the target classes(\S\ref{sec:empirical}), we naively come up with a \emph{strawman} of loss function design: assigning higher penalties to errors made by the ML model on inputs whose ground-truth decisions are selecting the target classes. 

% \begin{equation}
% L(y_i) = w_i \cdot T_i \cdot L_{BCE}(y_i) + (1-T_i) \cdot L_{BCE}(y_i)
% \end{equation}
% where $w_i$ is a large weight (\eg $w_i = 20$), and $T_i = 1$ if the ground-truth labels of the $i^{th}$ sample overlap with the applications' target classes, and 0 otherwise. 


% Intuitively, this \emph{strawman} loss function is compatible with our goal since it prioritizes the reduction of the loss on the samples belonging to the target classes than the non-target ones. 

Take the classification task  as an example to illustrate this idea. 
The ML model predicts a list of probabilities for an input, in which the $j^{th}$ element describes how confident the model is about whether the $j^{th}$  label exists in the input. 
The ground truth is a list, where the $j^{th}$ element is 1 if the $j^{th}$ label exists in the input, and 0 otherwise. 
The pre-trained model is trained to reduce the \emph{average} errors between the probabilities and the ground truth across a wide range of labels (\eg 9605 labels in Open Images~\cite{ASL}).
On the other hand, 
this strawman approach can prioritize the reduction of errors on the inputs whose ground-truth decisions are selecting the target classes. 
However, the strawman penalizes mis-classifications within one target class, such as mis-classifying a paper image into plastic in the garbage classification application example in Figure~\ref{fig:code}(a), and this type of errors are non-critical to the application.
% because the strawman is unaware that different applications may make different decisions given the same output (\eg \emph{True-False}, \emph{Multi-select}, and \emph{Multi-choice}) and how these decisions affect the severity of ML model errors
\shan{This last sentence is not clear.}. 

\mypara{New loss function}We propose a new loss function directly constructed from the \summary.
% \yh{Why they fails and we do not fail }
% \yh{add general recipe }
Compared to the strawman which may spare energy penalizing non-critical errors\shan{?? what exactly are non-critical errors spared by strawman?} \yh{I put in the last para: \ie mis-classifications within one target class}, 
our proposed solution only focuses on penalizing the critical ones. 
Specifically, two types of critical errors are being penalized\shan{I don't understand the (1) and (2) presented below}: 
(1)\shan{Hmm, what does this mean?}\emph{all} the labels in a target class have low probabilities in the prediction, but ground-truth decision selects it. 
(2) \emph{at least one of} the labels in a target class has a high probability, but ground-truth decision does not select it.

\tool's  loss function uses the Sigmoid function (\ie $Sigmoid(y) = \frac{1}{1+e^{k\cdot y}}$) to penalize the critical errors. The intuition behind using the Sigmoid function is that it provides a differentiable way to incur a high penalty when $y >0$\shan{what is y?}, and a low penalty otherwise, which appropriately fits our needs. 

% , such as mis-classifications across target classes. 
% For example, the strawman penalizes mis-classifications within the target classes, which are non-critical, while 



Formally, the loss function can be written as:

\begin{align*}
L_{i} &= 
\overbrace{ \sum_{j \in \{ \textrm{selected target classes}\}} ~\textrm{Sigmoid}(\F(y_i)-M_j(y_i))
}^{\substack{\text{\sf \footnotesize {Penalize low probability for the selected target class
	}} 
}} \\ &+ 
\overbrace{\sum_{j \in \{ \textrm{unselected target classes}\}} \textrm{Sigmoid}(M_j(y_i)-\Q(y_i) )
}^{\substack{\text{\sf \footnotesize {Penalize high probability for the unselected target class
	}} 
}} \label{eq:loss}
\end{align*}
where $M_j(y)$ is the \emph{maximum} probability in $y$ at indices that belong to the $j^{th}$ target class.  $\Q(y), \F(y)$ are two scores that differ by different types of applications. Generally, $ \F(y) > M_j(y)$ or $ M_j(y) > \Q(y)$ suggest that $y$ leads to an incorrect decision, otherwise, a correct decision is made\shan{hmmm, too complicated for me to understand} \yh{Working on how to make this clearer now}. 
% where $H_o(y) = 1$ if $y$ leads to the selection of the non-target class, and $H_o(y) = 0$ otherwise. $H_j(y) = 1$ if $y$ leads to the selection of the $j^{th}$ target class, and  $H_j(y) = 0$ otherwise. $Q_j(y) = 0$ for applications making \emph{Multi-Choice} decisions in API-output order, and $Q_j(y) = 1-H_j(y)$ otherwise. 
% $\theta$ is the prediction threshold of ML model, where any labels whose predicted probability is higher than it will be included in the output. $G_j(y)$ is the maximum probability in $y$ at indices that belong to the $j^{th}$ target class. $G(y) = max_{j \in \{1, \dots, m\}} (G_j(y))$ is the maximum probability in $y$ at indices belonging to all the target classes. $\F(y) = max$($\theta$, maximum probability in  $y$ at the indices that belong to any ground-truth unselected target class(es)). 

% In order to achieve the goal of re-sampling the training data,  our loss function assigns a weight $\frac{M}{N_i}$, where $M$ is the total number of data in the original training dataset, and $N_i$ is the number of training samples whose ground-truth labels overlap with the ground-truth target class(es) of the $i^{th}$ input. This weight, intuitively,  alleviates the effect of class skews in the original dataset by assigning higher weight to less dominant target classes, and lower weight for more dominant ones. 
% \yh{care more about the target classes} 


% M is the total number of data in the original training dataset. $N_i$ is the total number of data whose ground-truth selected target class(es) overlap with the ground-truth target class(es) of the $i^{th}$ input.  

As we have seen in \S\ref{sec:empirical}, the critical errors can vary greatly across different types of application's decision processes. Thus, in order to accurately capture the critical errors, we design different loss functions for each type of decision process. 

% Next, we describe the loss function for each type of decision process case-by-case. 


\mypara{True-False} In \emph{True-False} decision, only one target class is defined, and the application checks if the API output matches with it. 
Denote the prediction threshold of the ML model as $\theta$, where all the labels whose probabilities are higher than it will be included in the output. 
In this case, $\F(y) = \theta$, and $\Q(y) = \theta$. \shan{I understand the next few sentences, but I don't understand why F(y) is $\theta$, and 
Q(y) is $\theta$. I went back to read the $L_i$ formula, but still don't understand.}
For an input whose ground-truth decision selects the target class, a high penalty will be incurred if none of the labels in the target class appear in the output. 
% Thus, when the maximum probability for labels belonging to the 
On the other hand, for an input whose ground-truth decision selects the non-target class, a high penalty will be incurred  when there is at least one label in the target class included in the output. 

\mypara{Multi-Select} As for \emph{Multi-Select} decision, multiple selections are allowed about which target class(es) the ML API output matches with. 
In this case, the ground-truth target class(es) are those which overlap with the ground-truth labels of the input. 
$\F(y) = \theta$ and $\Q(y) = \theta$ for this type. 
The loss function will incur a high penalty when there are ground-truth target class(es) whose maximum probability is lower than $\theta$, 
or when there are target class(es) unselected by ground-truth whose maximum probability is higher than the $\theta$. 
\shan{Is Multi-Select's loss function essentially the same as True-False? Or, maybe you can tell me what exactly is the difference between them?}


% Denote the output of the ML model on the $i^{th}$ input as [$y_{i, 1}, \dots, y_{i,n}$]


\mypara{Multi-Choice application choice order} This type of application reaches only one selection by checking if the highest-priority target class matches with the output labels, if not, it moves on to the next target class, and so on. In this case, the ground-truth target class is the highest priority class out of those overlapping with its ground-truth labels. $\F(y) = max(\theta$, \textrm{maximum probability in $y$ at indices of unselected target class(es)}), and $\Q(y) = \theta$. Take the example in Figure~\ref{fig:loss} to illustrate. The application defines three target classes. Given an input image whose ground-truth label is \code{``Mansion''}, the ground-truth target class is the second one. In this example, $\F(y_i) = max(\theta, M_1(y_i)) = 0.8$ because the first target class has higher priority than the ground-truth target class. $\Q(y_i) = 0.5$ in this example. Thus, the penalty incurred by the loss function is Sigmoid(0.8-0.5) + Sigmoid(0.8-0.7) + Sigmoid(0.4-0.5). 
 
We can see that the loss function will incur a high penalty if any target class(es) with higher priority than the ground-truth target class are included in the output. 


\begin{figure}
     \includegraphics[width=\linewidth]{figs/loss.pdf}
    \caption{Illustration of \tool's loss function.
    }
\label{fig:loss}
\end{figure}


\mypara{Multi-Choice API output order} In this case, similar to the application choice order, only one selection is allowed. However, the application reaches a decision by checking if the first output label matches with any of the target classes, if not, it moves on to the next output label. 
In this case, the ground-truth target classes are those  overlapping with ground-truth labels. 
$\F(y) = max(\theta, $ maximum probability in $y$ at indices of unselected target classes by ground-truth decision), and $\Q(y) = $ the maximum probability in $y$ at indices of the ground-truth target classes.  
Thus, for the ground-truth target class, only if the maximum probability of it  is smaller than the maximum probability of unselected target class(es) or the prediction threshold, a high penalty will be incurred by the loss function. 


\mypara{Value ranges} As for APIs that output a score $y_i$ to describe the input, applications typically define $m$ value ranges as target classes to make decisions, where the lower bound of the $j^{th}$ value range is denoted as $l_j$ and the upper bound of the $j^{th}$ value range is denoted as $u_j$. The loss function commonly used to optimize for this type of regression task is the Mean Squared Error loss defined as follows:

\begin{equation}
    L_{MSE}(y_i) = (y_i - g_i)^2
\end{equation}
where $g_i$ is the ground truth. 

We construct the following loss function:

\begin{align*}
L(y_i) &= 
\overbrace{ ~\textrm{Sigmoid}(l_j-y_i)
}^{\substack{\text{\sf \footnotesize {Penalize the output if lower than ground-truth lower bound
	}} 
}} \\ &+ 
\overbrace{\textrm{Sigmoid}(y_i-u_j )
}^{\substack{\text{\sf \footnotesize {Penalize the output if higher than ground-truth upper bound
	}} 
}} \label{eq:}
\end{align*}
where $u_j$ and $l_j$ are the upper and lower bound of the value range the ground-truth score selects. 

Similar to the idea of the loss function we construct for classification tasks, compared to the Mean Squared Error loss which penalizes the score $y_i$ if it is not equal to the ground truth,  \tool's proposed loss function only penalizes the score if it falls out of the range that ground truth lies in. 
% MSE loss, borrow the idea 
 

% \jc{
% an example outline of this subsection (each bullet is a para)
% \begin{itemize}
% \item why we start with this? the key step is customizing ML model for each application.
% \item what's the goal
% \item what's a strawman (resampling training data)? and why is it not good (doesn't distinct multi-choice vs multi-option and order of examination)? (this para must be short). if room, also bring up some prior work that also does this
% \item our idea: rewriting loss function. give a general recipe of how this is done
% \item why is it better? (this should directly contrast with the strawman)
% \item more case-by-case explanation.
% \end{itemize}
% }

% \jc{regarding how to explain the goal, you can expand the following: formally an application can be viewed as $z=Decision(Model(x))$. for a given decision process $Decision$, the goal is to minimize $Decision(Model(x_i))\neq Decision(\hat{y_i})$ over a set of $x_i$, where $\hat{y_i}$ is the ground truth label of $x_i$.}



% \mypara{Notations} 
% Denote the total number of classes that the ML model behind the ML API can classify as $n$, and the whole set of classes is $C=\{C_1, C_2, ..., C_n\}$.  We define the symbols in our problem setting as follows. 
% \begin{itemize}
%     \item $I$: the input image
%     \item $G=\{G_1, ..., G_a\}$: ground truth label set of $I$, where $G_i \in C$ for $1 \leq i \leq a$
%     \item $T$: the prediction threshold of the ML model behind the ML API
%     \item $O=\{O_1, O_2, ..., O_b\}$: the predicted classes over the prediction threshold $T$, where $P_i \in C$ for $1 \leq i \leq b$
%     \item $P=\{p_1, p_2, ..., p_b\}$: the corresponding probability for the predicted classes
    
    
% \end{itemize}

% \mypara{Customization goal} For T-or-F, we want to minimize the critical errors which are caused by the API outputs that lead to the  execution of the \emph{False} branch, when the statement should be \emph{True} according to the ground-truth, and vice versa. With the above notations, our goal can be written as:

% \begin{equation}
% \begin{aligned}
% \min \sum\limits_{i=1}^{M}( y_i \cdot \mathds{1}_{\theta - P} + (1-y_i) \cdot \mathds{1}_{P-\theta} )
% \end{aligned}
% \end{equation}

% Where $\mathds{1}_{x} = 1$ when $x > 0$, and 0 otherwise. $y_i = 1$ if the $i^{th}$ input belongs to the class list defined in the branch condition, which we denote as $W$. $\theta$ is the prediction threshold, where classes whose predicted probability is higher than the threshold will be included in the output label list. $P$ is the maximum probability of classes in $W$, in other words, $P = max_{c \in W} p_c$.
% there are two types of critical errors: (1) for inputs whose statement in the branch condition is \emph{True} according to the ground-truth, which we refer to as \emph{target-inputs}, the API outputs lead the application selecting the \emph{False} branch; (2) for inputs whose statement is \emph{False}, the API outputs lead the application selecting the \emph{True} branch. To minimize incorrect application decisions, we want: 




% \yh{Outline of this section: 
% 1. first list the goal in math (or text): minimize the incorrect app decisions
% 2. a naive re-training scheme is to use a training data that  focuses on classes appeared in the apps 3. why this design is not good: it can only solve xxx, but not xxx 4. describe our loss function }
% \yh{goal: minimize the incorrect app decisions; what we have: extracted application's decision process (key dimensions) }
% As shown in our empirical study in Section~\ref{sec:empirical}, we find the application's decision process can be characterized by two aspects: (1) the class list(s) or value ranges that are used in branch conditions (2) the structures of the branch conditions.

% In this section, we will describe how we incorporate the application's decision process in the loss function. Our optimization is composed of two steps: (1) clustering the training data to focus on classes appearing in the branch conditions; (2) constructing the loss functions to be aware of the application's decision process. Our objective is to incur a high penalty on critical errors, and no penalty if the errors make no impact on the application. 


% To begin with, we first introduce the loss function traditionally used in multi-label image classification.


% The binary cross-entropy loss function used in multi-label classification task~\cite{ASL} is denoted as:
% \begin{equation}
%     L_{bce}  = -\frac{1}{n}\sum_{i=1}^n{(y_i\log(p_i) + (1 - y_i)\log(1 - p_i))} \,,
% \end{equation}
% where $y_i = 1$ if class $i$ is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. $p_i$ is the predicted probability for class $i$. 
% \begin{itemize}
%     \item  $y_i = 1$ if the $i^{th}$ class is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. 
%     \item $p_i$ is the predicted probability for the $i^{th}$ class.
% \end{itemize}
% where $y_i$ indicates whether the $i^{th}$ class exists in the input input $I$ or not. In other words, $y_i = 1$ if the $i^{th}$ class exists in the input $I$, and $y_i = 0$ otherwise. \cc{It is still one sentence, so please do not start a new paragraph}


% \subsubsection{Clustering training data}


% To achieve the first step, one approach is to assign different weights to inputs with ground-truth decisions of executing the \code{Others} branch and non-\code{Others} branches.  
% We take a simple example to illustrate this approach. An application  defines one branch condition to check if the API outputs intersect with a class list $W_1$. $W_1$ is a non-empty subset of the whole label set $C$ that the ML model is able to classify. 
%  The original fraction of images in the training data whose ground-truth  decisions are executing the \code{$W_1$}-branch (\ie $G \cap W \neq \emptyset$), which we refer to as \code{$W_1$}-inputs,  is $A$. 
%  % \cc{This sentence is very hard to read. Can we use phrase like ``which we refer to as $W$-images''?} 
% The fraction of images whose ground-truth decisions are executing the \code{other}-branch is $1-A$,  which we refer to as \code{others}-inputs. If we want to balance the distribution between $W$-inputs and \code{others}-inputs, we can use a loss function that assigns higher weights to \code{W}-inputs:

% \begin{equation}
%     L_D = y_1 \cdot \frac{1}{A} \cdot L_{bce} + (1-y_1)\cdot A \cdot L_{bce} \,,
% \end{equation}
% where $y_1$ indicates whether this input is a \code{$W$}-input or not. In other words, $y_1 = 1$ when the input is a \code{$W$}-input ($G \cap W \neq \emptyset$), and $y_1 = 0$ otherwise ($G \cap W = \emptyset$). 

% In this way, \code{$W$}-inputs and \code{others}-inputs are taking the same effect during training, instead of biasing towards either \code{W} or \code{others}. 

% % We construct loss functions for each type of software represented by the software examples shown in section~\ref{sec:empirical}. \cc{Maybe say some high-level ideas, more intuition}

% \subsubsection{Branch condition structure 1: T-or-F} 

% For the software that defines only one branch condition, checking if the output labels $O$ intersect with a class list $W_1$. We penalize the critical errors: (1) all the classes in $W_1$ are not included in top predictions for \code{$W_1$}-inputs; or (2) at least one class in $W_1$ are included in top predictions for \code{others}-inputs.




% \begin{equation}
%     L_{W_1} =y_1 \cdot \textrm{S}(\theta - P_1) + (1-y_1) \cdot \textrm{S}(P_1 - \theta) \,,
% \label{eq:loss}
% \end{equation}
% where
% $y_1$ indicates whether this input is a \code{$W_1$}-input or not. 
% In other words, $y_1 = 1$ if the input is a \code{$W_1$}-input, and $y_1=0$ if the input is a \code{others}-input. $\theta$ is the prediction threshold, where classes whose predicted probability will be included in the output label list. $P_1$ is the maximum probability of classes in $W_1$ (\ie $P_1 = max_{c \in W_1} p_c  $). $S(x)$ is the Sigmoid function $\frac{1}{1+e^{-k x}}$, which we will denote as $S$ in the rest of the paper. 



% Ideally, we want the loss function to be a step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{no penalty} when $P_1$ is greater than $\theta$ for  \code{$W_1$}-inputs. However, to make the loss function differentiable, we use the Sigmoid function to approximate the step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{a low penalty} otherwise, for \code{$W_1$}-inputs. Similarly for \code{other}-inputs. 



% \subsubsection{Branch condition structure 2: M-to-N-set} 

%  In M-to-N-set, several branch conditions are defined, each checking if a class list intersects with the API output $O$. All the fulfilled branches will be executed. We denote all the $m$ class lists the application uses in branch conditions as {$W_1$, ..., $W_m$}. In this pattern, the ground-truth  decisions is executing \emph{all} the branches whose class lists  intersect with the ground-truth labels. 

% We derive the following loss function for M-to-N-set:
% \begin{equation}
%     L = \sum_{i=1,\cdots,m} y_i \cdot \textrm{S}(\theta - P_i) + (1-y_i) \cdot \textrm{S}(P_i - \theta) \,,
% \end{equation}
% where $y_i$ indicates whether  $W_i$ is among the branches the ground-truth decision executes, in other words, $y_i = 1$ if $G \cap W_i \neq \emptyset$, and $y_i = 0$ otherwise. Similar to Equation~\ref{eq:loss}, $P_i$ is the maximum probability of classes belonging to $W_i$ (\ie $P_i = max_{c \in W_i} p_c$). 

%  Only if the application decisions led by $O$ exactly match with the ground-truth decisions, the penalty will be low.


% % \kt{$\sum_{i=1,\cdots,N} L_{W_i}$}



% \subsubsection{Branch condition structure 3: Priority-list}

% Priority-list defines several branch conditions, and each of them is associated with a class list $W_i$. The application checks the branch conditions from highest to lowest priority until finding the first one whose class list intersects with API output labels $O$. Let $W_i$ (where $1 \leq i \leq m$) denote the class lists used in branch conditions, where class lists with smaller $i$ indicate higher priority. Let $W$ denote the union of the classes in all the whitelists, in other words, $W = \cup^{m}_{i=1}W_i$. The ground-truth decision  is executing the highest priority branch whose associated class list intersects with the ground-truth classes $G$. 

% We derive the loss function as:
% \begin{equation}
% \begin{split}
%     L = y_i \cdot \textrm{S} (\max(\theta, P_{k^{-}})  - P_k ) + 
%     (1-y_i) \cdot \textrm{S}(P - \theta) \,,
% \end{split}
% \end{equation}
% where $y_i = 1$ when the ground-truth decision is executing one of the branches in $\{ W_1, \cdots, W_m\}$ (\ie $G \cap W \neq \emptyset$), and  $y_i = 0$ when the ground-truth decision is executing the \code{others} branch. 
% $k$ is the index of the highest-priority branch whose class list intersects with the ground-truth classes (\ie $k = \min \{i|WL_i \cap G \neq \emptyset\}$). $P_k$ is the maximum predicted probability for classes belonging to $W_k$, and $P_{k^{-}}$ is the maximum predicted probability out of the classes belonging to higher priority branches than the ground-truth branch (\ie $k^{-} = \min \{i | W_i \cap (G \setminus W ) \neq \emptyset \textrm{ and } i < k \}$). $P$ is the maximum probability of the classes belonging to $W$. 

% Given this loss function, only if the highest-priority branch whose class list intersects with the predicted classes $O$ is the ground-truth decision, the penalty will be low. 


% \subsubsection{Branch condition structure 4: Top-label}

% Top-label defines several branch conditions, and associates with each of them with a class list $W_i$, similar to Priority-list. However, unlike Priority-list, it checks the \emph{API output labels} one by one until one of them intersects with any of the class lists. Similar to the previous section, $W$ is the union of classes in all the defined class lists. We denote the classes belonging to class lists intersecting with ground-truth classes as $W^+ = \bigcup_{W_i \cap G \neq \emptyset} W_i$, and the classes belonging to \wls that do not intersect with ground-truth classes as $W^- = W \setminus W^+$.
 
% In this pattern, the ground-truth decision is to execute the branch condition  whose class list  intersects with the ground-truth classes. 

% We derive the loss function as:
% \begin{equation}
%     L = y_i \cdot S(\max(P^{-}, \theta) - P^{+}) + (1-y_i) \cdot S(P^- - \theta) \,,
% \end{equation}
% where $y_i  = 1$ indicates that the ground-truth decision is executing one of the branches in \{$W_1$, $W_2$, ...$W_m$\}, and $y_i = 0$ indicates the ground-truth decision is selecting \code{others}, similarly to the previous section. $P^{+}$ is the maximum probability out of classes in $W^+$ (\ie $P^+ = \max_{c \in W^+ } p_c$), and $P^-$ is the maximum probability out of classes in $W^-$ (\ie $P^- = \max_{c \in W^- } p_c$). 


% Given this loss function, we can ensure that only when the first class encountered in the predicted labels, that belongs to $W$, is one of the classes in the ground-truth decision, the penalty would be low. 




\subsection{How to extract the application's decision process}
\label{sec:extract}
% How we use sym-ex to get info, and which info 
% \yh{Change all the whitelists}
To extract application's decision process, we conduct an offline static analysis to detect code patterns introduced in Section~\ref{sec:empirical}. 
Particularly, we focus on the control-flow structures that are directly affected by ML API results. 

Given a code location of ML API invocation, \tool analyzes all the if-branches that have dependency on the ML API's output. 
\shan{hmmm, I feel your paper discussion so far has never talked about ``combination of branch decisions''. I don't have a clear picture about how it would fit our taxonomy ...}\cc{Updated}
Particularly, we focus on the branch conditions that software compares ML API output with certain values to make selection decisions, which are typically reflected by whether executing the target branch edge.
For each possible software decisions, \tool adopts standard symbolic execution to find all the API outputs that lead to these decisions, which is the corresponding target class.
If the software specifies only one target class\shan{what exactly does this mean ...}\cc{Done}, \tool reports pattern True-False. Otherwise, \tool analyzes the code structure to determine the pattern. % according to Figure~\ref{fig:hierarchy}:

\emph{Whether multi-select or multi-choice?} \tool analyzes all the statements inside the edges of an \shan{What is the definition of ML-API-related if-branch? I know we probably already used this phrase before. However, here, we are talking about static analysis, so we need to be particularly precise.}\cc{Done} if-branch that compares ML API output with target class. If the software exits the examination process after making a selection \shan{no no no. This is not a precise PL language. I don't know what you mean by ``terminates all examination inside one ...''. If you are doing control flow analysis here, you need to use control flow language to describe your algorithm.}\cc{How about this?} (\eg a break statement inside the loop and a return statement inside a function body), \tool regards that it as a multi-choice and further examines the order. 
If there is no such exit\shan{``termination'' usually refers to the termination of a program.}\cc{Done}, \tool determines it is multi-select structure. 


\emph{How is the order determined?} \tool finds all the loop structures\shan{??? what are ``equivalent statements''???}\cc{Removed. I put that phrase just in case there are other statements that lead to loop-like control flow} outside the ML-API-related if-branches. It analysis their nested levels and the data dependency relationship of their iterators -- due to Python syntax, the loop structure typically directly specify the list/set to be iterated (\eg~\code{for iterator in list}).
If the software does not contain any loop iterating ML API's output or application choices, \tool stops examination and reports an absence of code pattern. 
If an inner (outer) loop iterates\shan{how do you even know what variables a loop ``iterates'' through??? For example, in LLVM, index variables are identified for certain simple loops, but not all. I cannot believe you can identify what variables a loop ``iterates'' through for any type of loops. There must be unwritten assumptions here.}\cc{There's a widely-used Python syntax \code{for iter in list}. } the ML API's output and the outer (inner) loop iterates the application choices, \tool regards it as pattern Application-choice order (API-output order).  Note that, if the software contains multiple nested loops iterating the same variable, \tool focuses on the innermost one.


\subsection{How to integrate \tool in the MLaaS backend}
\label{sec:runtime}
TO-DO
To apply the \tool in xx,  we still keep the ML API, when users 

\tool modifies the MLaaS backend to serve the customized ML model per application. 
The MLaaS backend, as described in \S\ref{sec:overall}, adds the ML model to a model pool.
As depicted in Figure~\ref{fig:system}, when a user of an application queries the ML API, same as existing ML API querying, he/she first sets up a per-application authentication credential~\cite{google-cloud}, which is used for billing purposes. Then, when the user feeds the input to the ML API, the backend of MLaaS probes the model pool of customized ML models, selects the right model customized to the 

==> outline1.tex <==


% \subsection{Caching policy}
% \begin{itemize}
% \item what's wrong if we use a naive method to decide where to store kv cache? give a concrete example.
% \item what are the factors that might affect the delay and cost
% \item cost model
% \item delay model
% \item validation with real numbers
% \item how the models can inform the placement of kv caches (revisit the earlier example)
% \end{itemize}

% \subsection{KV cache Preloading}
% \begin{itemize}
% \item opportunity: kv cache can be loaded into CPU memory even before prefill starts. we can leverage it while the job is waiting in the queue
% \item give an example of how this can help.
% \item In scheduling algorithms, we add a new state that deprioritizes jobs when GPU is busy and KV cache is loading. 
% \end{itemize}





==> sec_abstract_v1.tex <==
\begin{abstract}
\jiayi{The title can be more general}

Large language models (LLMs) are extensively leveraged to answer complex queries that depend on domain-specific or user-provided knowledge outside training data. 
To achieve this, many LLMs rely on retrieval-augmented generation (RAG). 
In RAG, external data will be retrieved in the form of text segments from outside sources (\eg document repositories, cloud databases).
These text segments will then be concatenated and prepended to the user prompt to be pre-processed by the LLM before generation, a stage called prefill.
During prefill, the LLM computes the KV cache for the entire input, which demands extensive computation and could become the bottleneck. 
Even though different queries might share some text segments in their prompts (\eg system prompt for chatbots) and reusing the KV cache for shared text segments could greatly alleviate the prefill bottleneck, 
to realize this we face two key challenges in practice: 
(1) the KV cache to be reused must be from texts at the beginning of the input prompt, 
%which is not the case for current RAG as texts segments follow one another in the input, 
and
(2) the performance gain of reusing KV cache varies depending on models in use, storage devices, and reuse frequency. 
%\hc{The above seems  long but I cant compress any further}

To address these challenges, we present \name, the first context KV cache reuse system that efficiently stores, loads, and fuses KV caches of multiple text segments into one KV cache inside GPU memory ready to generate response. 
First, \name uses a KV cache fusor to merge multiple segments' KV cache with minimal quality drop. 
Second, a KV cache storage manager is deployed to smartly incorporate non-volatile storage devices into the caching system to minimizes delay while keeping cost under a budget. 
In our evaluation, we compare \name with other systems over a broad spectrum of delay, generation quality, cost, and throughput. 
Across xx datasets, \name is able to reduce average inference delay by \fillme x with only \fillme reduction in quality. 
It is also able to reduce cost by \fillme x or increase throughput by \fillme x when compared with other cache reusing baselines.


\end{abstract}

==> sec_background_v1.tex <==
\section{Background and Motivation}

\subsection{LLM Inference}
\label{subsec:transformer}
%\jiayi{we need to explain the math of attention since i need torefer it in the following sections}


%\hc{the key here is to explain how prefill could be fast but is costly too. I think people with LLM experience may have preassumption that prefilling is fast while decoding is slow.}
Current LLMs mainly utilize transformers~\cite{vaswani2023attention,brown2020language, palm} as the basic model architecture. 
A transformer takes input tokens (\ie a word, or a part of a word) and predicts future tokens in an autoregressive manner. 
In general, after receiving the input tokens, the LLM first goes through a prefill phase which computes the relationships between each tokens in the user prompt by transforming them into key (K) and value (V) vectors ({\em KV cache}) for future use. After prefilling is complete, the model enters an iterative decoding phase. In each iteration, the model predicts the next token with current KV cache and appends the new key and value vectors to the KV cache for the next iteration. This process repeats until End-of-Sentence (EOS) token is generated.

For each layer in the prefilling phase, the tokens are first transformed into query (Q), key (K), and value (V) vectors. 
Then it takes the dot product of query and key vectors between each token and use them as weights to calculate the weighted average of value vectors. 
These weighted averages then go through multiple neural layers to obtain the tokens for next layer. 
The key and value vectors are kept inside GPU memory after prefilling and will be used together with the new token's query vector to predict the next token.

\jc{can we not say prefill is fast? prefill on several thousands of tokens will take about several seconds to over 10 sec. this is definitely not fast. can someone update it with some real numbers?}
Since the prefilling process is highly parallelizable, it is usually considered much faster than decoding. For example, as shown in Figure \ref{fig:time_vs_len_bsz}, for Mistral-7B served on an A40 GPU, prefilling \textasciitilde 1500 tokens takes the same amount of time as decoding 10 tokens. However, prefilling phase could still become the bottleneck when the input prompt is long and/or the request rate is high (since concurrent requests can be batched in decoding phase).

\yh{The prefill phase can be slow,  especially when the input is long. 
For example, prefilling an input of 4K tokens takes 700ms for Mistral-7B, when served on one A40 GPU.
Larger LLMs require an even longer prefilling delay. 
Specifically, for Llama-70B, it takes 5.8 seconds to prefill an input of 4K tokens on one A40 GPU. 
Compared to the decoding phase, which only takes 10ms to decode one token, the prefill phase can become the bottleneck. 
}

\begin{figure}
\centering
     \includegraphics[width=.95\columnwidth]{figs/text_comparison.pdf}
    \tightcaption{Text comparison} 
    \label{fig:text_comparison}
\end{figure}

\begin{figure}
\centering
     \includegraphics[width=.95\columnwidth]{figs/attn_comparison.pdf}
    \tightcaption{\jiayi{add some explanation}\jiayi{Please add boxes to indicate cross attention and internal attention}\jiayi{improve this visualization by not focusing on the internal attention in second chunk}}
    \label{fig:attn_comparison}
\end{figure}


\subsection{LLM serving with substantial text redundancies}
 \label{subsec:redundancy}
% \hc{I am leaving this here since Jiayi and Siddhant probably knows much more about how people use RAG}
%\sr{For many applications (like RAG), it is useful to have a system which supports the reuse of contexts, as recomputation of many (long) contexts is expensive in terms of computation\cite{context_reuse}. As workloads get more complex, it is common to have contexts in RAG pipelines upto ${\sim}1M$ tokens\cite{1m_context} In such scenarios, it is natural to reuse the shared KV cache between all requests which reuse these long contexts. Such requests might be different questions from the same set of contexts or queries from different users about the same topics (like code documentation)\cite{su2024arks}.

%Some contexts maybe resused with significant time gaps (different users might query the same code documentation over several hours), which makes it important to store the KV cache of such contexts for longer times. Also, the size of the KV cache increases linearly with the sie of the prompt (GPT-3 generates a 4.5MB KV cache for each token) and prompts containing 1000s of tokens will produce several GBs of KV cache\cite{gao2024attentionstore}.

%Finally RAG consists of retrieving and adding relevant context chunks to the prompt. Most RAG applications today tend to use multiple small chunk sizes (upto 1024 tokens) for output generation\cite{chunk_stats_1, chunk_stats_2}. A common method of adding the context chunks to the prompt is simply concatenating them sequentially to the prompt. When the number of retrieved contexts chunks sizes are small, this becomes an obvious choice as the overall context window doesn't exceed the size of the model's window and the output generation is fast. When larger contexts are present, there exist other methods to combine the retreived contexts (like Refine, Map Reduce or Map Rerank) but these are often slower as they involve multiple calls to the LLM\cite{langchain, compare_chains}.}

%\sr{\textit{Hanchen please add approprriate conclusions above}}

% \begin{itemize}
% \item many appalications (RAG) are wildly popular. show several examples, see this link for some inspiration: \url{https://chat.openai.com/share/607cf54f-2180-4a66-a177-bb6cb2352864}
% % have requests that share a lot of context chunks. 
% \item a few characteristics of this workload:
% \item first, long text chunks are reused (100s or 1,000s of tokens). \\
% $\Rightarrow$ kv caches are much bigger than usual length of chat prefix (can we get some numbers from shareGPT?).
% \item second, chunks shared across separate requests, possibly from different users.\\
% $\Rightarrow$ unlike chatbot apps, a text chunk may be re-used over a long period of time.
% \item third, the input chunks are not supposed to be processed separately. \\ 
% $\Rightarrow$ input concatenates multiple chunks.
% alternatives are either slower (like refine) or have lower quality (like MapReduce and ReRank). (need Siddhant's help on this!)
% \end{itemize}

%\hc{siddhant is finishing this by Sunday morning}

%\jiayi{The motivation for more chunks should be two-fold: (1) the related info might not reside in the first chunk; (2) some tasks (e.g., reasoning, comparison, summary) do need more chunks}

%\jiayi{We should convey three points here: (1) multiple documents should be retrieved; long, (2) these documents should be read jointly, (3) prefix ratio is low}

\jc{somewhere in this subsec, we need to clarify our focus is the inference on the retrieved chunks, rather than which chunks to retrieve}
Many popular LLM applications often encounter the case when input prompts contain a substantial portion of constantly recurring texts. We define these recurring and reusable texts as text redundancies in LLM inputs. 
Text redundancies can be found in AI agents where agents are always prompted with templated instructions \cite{Significant_Gravitas_AutoGPT, pmlr-v162-huang22a, qin2023tool}. 
Such redundancies also exist in chat histories that are stored, partially modified and constantly reused \cite{packer2023memgpt, wu2024secgpt}. 
A typical and popular category of such applications is Retrival Augmented Generation (RAG) \cite{lewis2021retrievalaugmented}. 

Existing research has shown enormous benefits of utilizing RAG pipeline LLMs in many aspects, such as alleviating hallucination issues\cite{mao2020generation, ram-etal-2023-context} and provding more privacy and security control over proprietary information\cite{gao2023retrievalaugmented}. 
A common RAG paradigm usually contains three stages: indexing (preprocessing the text chunks), retrieving the text chunks, and generating. A toy RAG example is shown in Figure \ref{fig:text_comparison}. The user gave a query of \textit{"How many goals did Messi score more than Cristiano Ronaldo at FIFA World Cups?"}. A RAG retriever will retrieve text chunks including two players' career statistics inside the pre-built text database. In the generation stage, the retrieved texts and the user question are combined and fed into LLM. In this case, the career satistics regarding Messi and Ronaldo are known in advance and are expected to be reused when there come similar queries (e.g., \textit{"Who scored more than five goals at FIFA World Cups?"}).



\begin{figure}
\centering
    \subfloat[Musique]
        {\includegraphics[width=0.49\columnwidth]{figs/musique_acc_motivation.pdf}\label{fig:rag_acc_1}}
    \subfloat[2WikiMQA]
        {\includegraphics[width=0.49\columnwidth]{figs/2wiki_f1_motivation.pdf}\label{fig:rag_acc_2}}
    \tightcaption{Accuracy increases as more chunks are retrieved}
    \label{fig:overlap}
\end{figure}



\begin{figure}
\centering
     \includegraphics[width=.95\columnwidth]{figs/time_prefix.pdf}
    \tightcaption{TTFT grows as more chunks are retrieved (assuming cache already in GPU), \jiayi{we should also have a fig for cache not in GPU, in that fig, ours can be the same as optimal}} 
    \label{fig:time_prefix}
\end{figure}

The above toy example is an idealized scenario. Real-world RAG workloads require more and longer chunks to include enough information in the context. For example, the actual text information in the toy example could be "Messi is one of the only six men played in five World Cups alongside Antonio Carbajal.... He has scored 13 goals at FIFA World Cups in total". In this case, we need bigger chunk length to retain the semantic coherence. And the retriever might need to retrieve more than two chunks in order to retrieve the scoring information about Messi and Ronaldo. In addition, some tasks innately require multiple text chunks (e.g., summarization, multihop reasoning). To be more concrete, we use a popular multi-hop reasoning dataset Musique~\cite{???} and a multi-document question-answering dataset~\cite{2wikimqa}, where we retrieve chunks of size 128 tokens (a popular number)~\cite{jan_chunksize} and evaluate the generation quality by increasing the number of chunks. As shown in both figures (Figure \ref{fig:rag_acc_1}, \ref{fig:rag_acc_2}), accuracy increases significantly as more chunks are retrieved. Note that only reading these chunks jointly can lead to such accuracy improvement as the LLM requires information from multiple chunks to reason about the steps in the required answer generation. Therefore, we believe there are always use cases where 

\textbf{\em Multiple chunks should be read jointly.}
%\sr{We should add here that we need more chunks because what matters is the total input text to the LLM which should have all the facts}. 

However, incorporating longer contexts in the LLM input inevitably increases the context processing time. Such overhead can be alleviated by reusing the recurring prefixes of contexts' KV cache. However, even assuming contexts are used strictly at the begining of the input or the texts before contexts (e.g., system prompt, user instruction, chat history) are fixed and pre-known, the prefix ratio will eventually become low as more text chunks are retrieved, which constrains the benefits of KV reuse. As shown in Figure \ref{fig:time_prefix}, assuming the precomputed KV cache is in (or already loaded to) GPU, the benifits of prefix reuse soon become negligible as more chunks are retrieved. Therefore, it's apparent that

\textbf{\em Prefix caching is limiting.}

%Note that the grey line in Figure \ref{fig:time_prefix} shows the maximum potential of KV cache reuse. The overhead in this optimal imaginary scenraio is only prefilling the last token (assuming the KV cache is already in GPU and can be directly reused). In reality, we cannot expect the KV cache always reside in GPU. \jiayi{somehow empirically show this, a lot of KV cache. also show the loading overhead somehow}. Therefore, 

%\textbf{\em KV cache needs to be stored and loaded efficiently.}

%Further, . As shown in Figure \fillme, scattered (more ). That is, if we only . Therefore, the potential for reusing the KV cache could be constrained by a finite and fixed storage capacity (e.g., CPU DRAM, Local SSD).


%For example, to build a RAG pipeline for open-domain question answering, we can use wikipedia as our external knowledge base. In the indexing stage, we need to first parse the wikipedia pages and load the texts into smaller chunks. Chunking is necessary in that LLMs have a max input limit, and longer context inputs inevitably increase the response delay due to longer prefilling time. In addition, irrevalent information can also degrade the genration accuracy\cite{chen2023benchmarking, liu2023lost}. An embedding model (e.g., BERT\cite{turc2019}, BGE\cite{bge_embedding}) is then used to encode the text chunks into vectors. Lastly, an index is created for each text chunk and the corresponding embedding and raw text are stored as a key-value pair. In the retrieval stage, relavent text chunks are retrieved based on the similarity between their emeddings and the embedding of the given user query. The retrieved text chunks and the user query is toghether fed to the LLM as input.

%\S\ref{subsec:redundancy} (reuse opprortunities exist and can be benefitial), context augmented generation could have very long input length. In these cases, naively following the original logic could incur great cost in prefill phase. In order to solve this problem, a promising solution emerges: instead of recomputing the long context every time a request arrives at the server, we could store the pre-computed KV cache corresponding to different contexts and load them into GPU memory when needed. 

%This optimization requires a new module that is currently missing in the current LLM serving ecosystem. Ideally, this KV cache management module is able to perform the following tasks:
%\begin{itemize}
%    \item Storage of as many reusable contexts as possible with minimal cost.  
%    \item On-demand loading of the KV caches with minimal delay. 
%    \item Ability to combine KV caches of different contexts for future inference. 
%\end{itemize}

%These three tasks are essential to accomadate the different use cases of context-generated LLM discussed in \S\ref{subsec:cases}. After the retriever \hc{please explain in 2.2 about how the retriever works} fetches the documents


% \begin{itemize}
% \item for these retrieval-based apos, an opportunity emerges to minimize prefill by reusing kv cache. 
% \item we need a new module that stores and loads KV caches efficiently. 
% \begin{itemize}
%     \item storing kv caches of potentially reused text chunks
%     \item on-demand loading the kv caches of reused text chunks
%     \item update kv caches to include the cross-attention among the text chunks
% \end{itemize}
% \item a few words on the potential benefits: higher throughput and lower delay
% \end{itemize}


\subsection{Challenges and prior attempts}
In the last section, we have discussed the potential of KV reuse to relieve the prefil bottleneck. Many prior works have focused on prefix reusing to reduce this overhead. vLLM\cite{kwon2023efficient} innately supports prefix reuse within a batch, which can be easily extended to cross-request scenario (e.g., offload the KV cache to CPU). %ChunkedAttention\cite{ye2024chunkattention} futher optimizes attention computation when multiple requests in a batch share the same prefix.
SGLang\cite{sglang} uses a tree-like structure and an LRU policy to maximize the commonly shared prefixes among concurrent requests.
RAGCache\cite{jin2024ragcache} extends a similar tree structure and further optimizes the cache eviction policy, enabling prefix reuse among different requests.

However, in these works, the benefits of KV reuse only exist when reuse takes place at prefix position.
Therefore, to build a more flexible system that maximizes the potential of KV reuse at any positions, the key challenge is  

 \textbf{\em How to combine the independently precomputed KV cache of different text chunks effectively and efficiently?}

An easily thought of solution is to naively concatenate the KV vectors of multiple text chunks. \promptcache\cite{gim2023prompt} follows this line of thought by simply concatenating KV vectors of recurring text chunks with the help of buffers to ensure positional accuracy. For example, if we are to concatenate chunks \(C_{1}\) and \(C_{2}\), the KV vectors of \(C_{2}\) needs to be cached as \((l*buffer, C_{2})\) where \(l\) is the length of the buffer and should be greater or equal than the length of \(C_{1}\). This naive concatenation strategy has two innate problems. First, cross-attenton between \(C_{1}\) and \(C_2\) is completely ignored (Figure \ref{fig:attn_comparison}). As a consequence, such ignorance might fail to address the relationship between the two text chunks, degrading generation quality (Figure \ref{fig:text_comparison}). Second, precomputation at fixed positions (with buffers) only allows the resuse of the same texts at similar positions. The KV vectors of the text chunk have to be precomputed multiple times and saved in multiple copies (with different buffer lengths) in order to be reused at any position. We will address these two problems in the next section \ref{sec:merge}.

%In addition to combine, \jiayi{Can we somehow naturally mention the difficulty in loading here}


 %As mentioned in \S\ref{subsec:cases}, the retriever fetches text chunks from various sources and uses them together as a whole piece of context for inference. Reusing KV vectors of these recurring text chunks can lead to fewer context processing computation. However, the self-attention mechanism, which allows a token to pay attention to its subsequent tokens, makes KV vectors only reusable when the recurring text is a prefix of the context. 
 
 %\jiayi{I have pushed naive concat to the next part.}

 
 %The naive prefill phase will recompute the KV cache for this new concatenated context and capture the relationships between each token. However, during the offline precomputation, each chunk's KV cache was assumed to be the only context in inference. Thus, the KV cache for an individual chunk does not contain its tokens' relationship with tokens in other chunks. For example, \hc{Lets put a graph to show the two challenges, this is the first part. two sentences related but could not be understood if not taken together} As a consequence, if we naively concatenate the KV caches together, the generation quality drops significantly (shown later in \S\ref{}).

%Second, how do we determine where to store the KV cache while the benefit of reusing varies widely depending on model, storage device type, and reuse frequency? For a fixed length text segment, the fastest yet cheaper than prefill storing location for its KV cache varies widely with different model and reuse frequency. How do we determine where to place one KV cache given the abundance of storage device available remains unclear.

%{\em Challenge \#2: How do we determine where to store the KV cache under a cost budget while the benefit of reusing varies widely depending on model, optimizations enabled?}

%\jiayi{should be store and load now. please drop this chalenge and makes it as a natural consequence of KV reuse (e.g., we can reuse more kv cache, therefore we nned to store more)}

% In a retrieval based LLM application, different text segments could have very different reuse frequency depending on the popularity of the content inside. If we choose a high end storage device for a rarely reused KV cache, the storage cost could easily rise above the original prefill.

%Since different storage devices vary widely in throughput and cost, it is important to choose an appropriate storage setup to minimize delay.
%However, this option is dependent on the model we are serving as well as optimizations available.

%We show an cost analysis for running Llama-7B, 34B, and 70B with KV cache 8-bit compression enabled on AWS platform in Fig. \ref{fig:motiv-models} with different provided storage types. This is due to different models' KV cache sizes vary widely due to architecture difference. 

%Moreover, the abundant compression and quantizations available also affects the optimal storage devices we want to us. As shown on Fig. \ref{fig:motiv-quantizations}, storing Llama 70B's KV cache in FP16 on a 100MBps S3 storage increases delay by xxxX. If the developer uses S3 without choosing to do 8-bit quantization, all requests that loads from this tier will suffer from extra TTFT. Moreover, there are more available KV compression methods that potentially induces more loss, based on the developers' tolerance of loss in the application, we need to build this caching system with different compression methods in consideration.

% \begin{figure}
%     \centering
%     \includegraphics[width=.95\columnwidth]{figs/store_challenge_model.jpeg}
%     \caption{With 8-bit quantization, Llama 7B, 34B and 70B have different delay-prefill over cost curve\jiayi{Is it Mistral 7b or llama 7b?}}
%     \label{fig:motiv-models}
% \end{figure}

% Thus, for a KV cache reuse system, a wide range of KV caches could be stored. In order to save cost, we need to store many of them in cheaper non-volatile memory devices such as SSD or hard disk. These different devices vary in cost and throughput. And loading multiple contexts in the same time could cause contention for IO throughput, which makes loading delay more than recomputation. Moreover, due to the different designs of LLM models, caching their KV cache size brings differnet extents of benefit when compared with recomputation. For example, recomputation with llama 7B is 4x faster than llama 70B, but its KV cache is even twice as big as 70B! This disparity means that under the same reuse frequency, storing KV cache of Llama 70B could potentially be 8x more worth than storing llama 7B KV cache. Given this disparity in model to be served and storage types that could be utilized, it remains unclear how do we create a system to handle this complexity.


% \begin{figure}
%     \centering
%     \includegraphics[width=.95\columnwidth]{figs/store_challeng_opt.jpeg}
%     \caption{Using Llama 70B, storage device utility curve also varies with optimization enabled}
%     \label{fig:motiv-quantizations}
% \end{figure}


% \begin{itemize}
% \item first, when the reused text chunk isn't a prefix but follows different texts, its KV cache won't be able to capture its cross-attention with various preceding texts, so it can't be directly reused. 
% \begin{itemize}
%     \item
% \end{itemize}
% \item second, compared to storing common prompt prefixes for which CPU memory is enough, storing the KV caches of all potentially reused text chunks needs much more storage space. 
% \begin{itemize}
%     \item 
% \end{itemize}
% \end{itemize}





% \subsection{Why not existing solutions?}
% \label{subsec:existing solutions}
% A lot of work has been done in the intersection between LLM and systems. We discuss the most related ones in this part and explain why they are not sufficient to solve the two challenges.

% Many prior works have adopted prefix reusing to reduce KV cache prefilling. ChunkedAttention\cite{ye2024chunkattention} optimizes attention computation when multiple requests in a batch share the same prefix.
% SGLang\cite{sglang} uses tree-like structure and use LRU policy to reuse the KV vectors of commonly shared prefixes across different requests. However, these methods only utilize limited GPU and CPU memory to cache KV cache generated by temporal approximate requests. \jiayi{Can we focus on "prefix" instead of "multi-tier" in this para.?} as mentioned earlier (\jiayi{or show here}), prefix-only caching is too limiting \hc{We should explain what prefix reuse does, and show the result Jiayi put earlier (prefix ratio is low in RAG)}.

% A straightforward solution is to naively concatenate the KV vectors of multiple text chunks. \promptcache\cite{gim2023prompt} follows this line of thought by simply concatenating KV vectors of recurring text chunks with the help of buffers to ensure positional accuracy. For example, if we are to concatenate chunks \(C_{1}\) and \(C_{2}\), the KV vectors of \(C_{2}\) needs to be cached as \((l*buffer, C_{2})\) where \(l\) is the length of the buffer and should be greater or equal than the length of \(C_{1}\). This naive concatenation strategy has two innate problems. First, cross-attenton between \(C_{1}\) and \(C_2\) is completely ignored (Figure \ref{fig:attn_comparison}). As a consequence, the generation quality drops significantly (Figure \ref{fig:text_comparison}). Second, precomputation at fixed positions (with buffers) only allows the resuse of the same texts at similar positions. The KV vectors of the text chunk have to be precomputed multiple times and saved in multiple copies (with different buffer lengths) in order to be reused at any position. We will address these two problems in section \ref{sec:merge}. 

% Many existing systems also offloads KV caches to CPU or storage devices to increase throughput. 
% vLLM~\cite{?} uses CPU to store KV caches when GPU memory is not enough to store all KV cache page. 
% FlexGen~\cite{?} designs offloading strategy for both model weights and KV cache to optimize throughput under constrained resources. 
% InfiniteLLM~\cite{?} shares CPU memory across datacenter to accomadate long requests. 
% However, these systems only offload KV cache within a single request and only reuses KV cache for the unfinished job in its current queue. 
% \hc{rag cache and attention store needs to be mentioned}
% \qz{system reviewers not familiar with LLMs would be smashed when they read all these related work; make a table summarizing prior work's limitations and compare with METIS (to-do)}

% It is possible to extend them to multi-tier storage and reuse them across requests. But their current design will fail under such scenarios. If KV cache is offloaded to cheap storage devices, the delay incurred when re-loading this KV cache back to GPU could be very high. Moreover, loading different context from the same device could cause contention for the limited throughput/bandwidth. 
% \qz{focus on why existing offloading strategies cannot be easily adapted for multi-tier storage and multi-request KV cache reuse}
% \begin{itemize}
% \item previous systems are not designed for this concept \\

% \item for challenge 1, some prior systems cache prefixes across requests
% \begin{itemize}
% \item examples: vllm, chunkedattention, gslang
% \item they also reuse kv across requests.
% \item but limited benefit in RAG
% \end{itemize}

% \item better solution is modular caching: such as promptcache. 
% \item however, it can't handle cross-attention. give an example! 
% \item explain the cross-attention and how promptcache may have missed it.\\

% \item for challenge 2: some systems (distkv-llm, flexgen, vllm) also cache more kv than one gpu can
% \item but they only manage kv cache within a single job, so most kv caches are in gpu, and even if a kv cache is offloaded, we know when it's used

% \item can we extend them to storing kv caches across jobs? yes, but they do not optimize the cost-delay trade-offs when storing the kv cache on cheaper yet slower storage, like local or remote storage. The delay also would be higher
% \end{itemize}




==> sec_impl_v1.tex <==
\section{Implementation}\label{sec:impl}
We implement \name on top of vLLM with about 3K lines of code in Python based on PyTorch v2.0.

\mypara{Integrating Fusor into LLM serving engine}
\name performs the partial prefill process in a layer-wise manner through three interfaces:

\begin{packeditemize}
\item \texttt{fetch\_kv(text, layer\_id) -> KVCache}: given a piece of text and a layer id, \name fetches the corresponding KV cache from KV store into the GPU. Returns -1 if the KV cache is not in the system.
\item \texttt{prefill\_layer(input\_dict, KVCache) -> output\_dict}: \name takes in the input and KV cache of this layer and performs the partial prefill process for this particular layer. The output is used as the input for the next layer.
\item \texttt{synchronize()}: \name requires sychronization before prefilling every layer to make sure the KV cache of this layer has already been loaded into the GPU.
\end{packeditemize}

We implement these three interfaces inside vLLMs. For \texttt{fetch\_kv}, we first calculate the hash of the text and search if it is inside the KV store system. If it is present, we call \texttt{torch.load()} to load it into GPU memory if KV cache is on disk or use \texttt{torch.cuda()} if the KV cache is inside CPU memory. For \texttt{prefill\_layer}, we implement this interface on top of the orginal \texttt{layer} function in vLLM that performs one layer of prefill. Three key-value pairs are recorded in the \texttt{input\_dict}: (1) the original input data \texttt{input\_org} required for prefilling an LLM layer (e.g., input\_tensor, input\_metadata), (2) a \texttt{check\_flag} indicating whether \HCA tokens will be selected in this layer, and (3) \texttt{HKVD\_indices} that tracking the current indices of \HCA tokens. If \texttt{check\_flag} is set to \texttt{True}, the input tokens with the largest deviation between the newly computed KV cache and the loaded KV cache will be selected as the \HCA tokens. In the \texttt{output\_dict}, the \texttt{HKVD\_indices} will be updated and the related data in \texttt{input\_org} will also be updated (e.g., the input\_tensor is indexed by the \texttt{HKVD\_indices}). If \texttt{check\_flag} is \texttt{False}, partial prefill will only be performed on the current \HCA tokens indicated by \texttt{HKVD\_indices}. Note that only the KV cache of the \HCA tokens will be computed and updated at each layer.

\name performs the layer-wise partial prefill iteratively over all layers. In iteration \(i\), two threads are used to pipeline the computation (\texttt{prefill\_layer}) of layer \(i\) and the KV cache loading (\texttt{fetch\_kv}) of the next layer \(i+1\). The interface \texttt{synchronize} is called before \texttt{prefill\_layer} to make sure the KV cache needed for prefilling this layer has already been loaded in GPU.


% \name performs the selective recomputation
% through two modifications to the inference code. In the model executor module, for each supported model class (ex. Llama), we add a loading mechanism in the {\em forward} function. This forward function fetches the raw KV caches of next layers of the chunks from KV store, and sends a status flag to the attention backend.

% Inside the {\em xformers} attention backend module, we first check the status flag. If the status flag is in check mode, then we will perform full recomputation for that layer. After recomputation, we will compare the ground-truth KV cache with the loaded KV cache, identify the token positions with high KV deviations, and save them as a mask. If the status flag is in partial prefill mode, then we will use the previous mask to choose a subset of token to perform attention matrix multiplication with the other KV values from previous layer. After this step, we will replace the old KV values in the layer with the newly computed ones.

\mypara{Managing KV cache}
\name manages the KV caches in the following manner:
If KV cache is not inside the system and is recomputed by the LLM engine in the runtime, we will move the KV cache into CPU by \texttt{torch.cpu()} and open a thread to write it back to disk in the background with \texttt{torch.save()}. The default KV storage position is extra CPU memory and user-allocated SSD space, with the potential to use S3 object storage. During the \texttt{fetch\_kv}, we go through through three hash tables from the highest to the lowest to fetch KV cache. 


%Moreover, since KV cache in vLLM are organized in a GPU page table, we need to transform loaded KV cache to 32-token blocks. For this end, we use {\em load\_and\_reshape} to take the key and value tensors, reshape them to 32-token groups, and put them on to the preallocated GPU space inside vLLM.


==> sec_intro_v1.tex <==
\section{Introduction}

Large language models (LLMs) have become widely adopted for their remarkable  capabilities, applications in personal assistance, AI healthcare~\cite{llm-app-1,llm-app-2,llm-app-3,llm-app-4}. In order to improve on the accuracy and reliability of these generative model, there is an increasing interest in builindg Retrieval-Augmented-Generation (RAG) pipelines.~\cite{???} RAG supplements the user prompt with context texts containing essential information for answering the question. During RAG, the most common pipeline begins with a retriever that fetches multiple text segments based on user request from the text database. These documents are then concatenated together and prepended to the prompt to form the input. The LLM model first go through a prefilling phase, which uses attention layers to process the input tokens and produces a complete KV cache. Then in the decoding phase, LLM iteratively predicts the next token with current KV cache and appends the KV tensor of the newly generated token to the KV cache for next iteration.


% \jc{why don't we just spell out RAG clearly and upfront and say it's very popular. 
% then in the next para, say because the retrieved docs form long contexts, prefill is slow and expensive, etc}

% \jc{then at the end, we can try to generalize it a bit and say these properties are not unique to RAG}

% For executing intricate tasks, it is common for users or applications to initiate LLM interactions with extensive contexts that may span thousands of tokens or more. This paper treats such extensive preambles provided to various LLM inputs as a context. These context supplements user prompts with domain-knowledge to help LLM generate responses with specific knowledge not contained in the original pretrained model.




\jc{let's be consistent about the terminology: each input consists of multiple text segments, and each text segment can be a retrieved document (or a chunk of a document) and a user query. currently, we use terms like context, text, or chunk all referring to the same concept ``segment''. just try to be consistent. }

\jc{text before this point can be much shorter. within .25 of a page. just leave the key points. details can be moved to section 2 or 3}

Although LLM prefill is highly parallelizable and thousands of tokens could be prefilled in less than 10 seconds, it is very costly due the extensive computation and GPU cycles needed. For example, It takes one second to prefill only \fillme KB of text. Previous system~\cite{distserve} could use 4 GPUs for prefill while 2 for decoding. In these context augmented generations, since the contexts are very long but not necessarily the generated answers~\cite{?}\hc{we need rag application examples}, prefill could be the main bottleneck in RAG systems.

Fortunately, across many LLM applications, the contexts retrieved could often be shared across different LLM inputs. For examples, if a financial LLM service receives two request from the user for one company: ``Analyze Amazon's liquidity position at the end of the last fiscal year.'' and ``Evaluate the Amazon's profitability trends over the last year'' . 
Both of the requests are likely to use the company's income statement as context.  
Similarly, for the legal assistant application, two requests ``What are the responsibilities of a landlord regarding property maintenance?'' and  ``Can a tenant withhold rent if the landlord fails to make necessary repairs?'' both require tenant-landlord laws to generate the answers. \jc{in RAG, the input would be several segments of relevant texts from the income statements or landlord laws, rather than one single document. if we don't highlight this, people may be misled to think about prefix caching} 

For these settings where input texts are reused chunks, {\em if} we could store and reuse the KV caches of these reused texts, we {\em could} greatly increase the system throughput since the main computation bottleneck of prefill is resolved. 
\jc{if we are serious about showing the potential, we need more stats than just throughput improvement. what about delay? what about amount of computation? what about the data size inflation that need to be stored? i'd love to see some ballpark numbers before seeing the challenges.}Through a simple experiment, we should the throughput could increase by ??x if the GPU cycles do not need to be spent on prefill. 


However, building this system is not easy. Two key challenges arise for such a system. 
\begin{itemize}
    \item How to reuse the precomputed KV cache when it is not the prefix? In this new system, the text chunks used are not always the prefix of the LLM input.\jc{this needs to be explained way earlier, i.e., when we introduce RAG as the main use case in the first couple of paragraphs. we can then refer to it here} This breaks the assumption of the original KV cache and fails to capture this text's relationship with the previous ones.\jc{why don't we directly say cross-attention? it's a good idea to mention it even before formally defining it.} Thus, the KV caches could not be directly reused and requires modification to ensure generation quality. 
    \item \hc{I am changing this to multi model, multi tier}How could we keep all KV caches of reusable text chunks on cheaper and slower devices while ensuring the loading is still fast enough? Storing KV cache of all potentially reused text chunks demands much more storage spaces than only common prefix. We potentially want to store less frequently used KV caches to cheaper devices including SSD and HDD to reduce the cost. But naive loading from cheap storages like HDD will increase delays to more than recomputation.
\end{itemize}

To address these challenges, we present \name \footnote{\name is the goddess of knowledge in Greek Mythology. Our system manages the knowledge sources of LLM, the KV caches of contexts.}, the first context KV cache storing and loading system for LLMs to efficiently yet correctly retrieve knowledge without the costly prefill process. Our system mainly comprises of two parts,  a KV cache combiner and a multi-tier storage system with loading controller.

To address challenge 1, the KV cache combiner takes in individual text chunks' KV cache and partially recompute the cross-attention between these chunks to reconstruct a consistent KV cache with minimal overhead. 

To address challenge 2, our multi-tier storage accomodates the potential use frequency differences among different text chunks, while the loading controller dynamically optimizes loading delay based on the IO and GPU availablity. 

We implemented \name on top of VLLM with xx lines of python and xx lines of CUDA. We evaluated our methods with exisiting LLM serving systems and outperforming them in dimensions of throughput, delay, quality, and cost. Here is the summary: 
\begin{itemize}
    \item Comparing with the state of art methods for KV reuse in CPU and GPU , our end to end system is able to increase throughput by ???X with minimal drop in generation quality.   
    \item Comparing with state of the art KV cache reusing system and recompute baseline, our KV combiner are able to increase Rouge F1 score by ??x or reduce delay by ??x.
    \item Comparing with storage with a single tier, we achieve ??x lower cost under same level of delay and xx lower delay under same level of cost. Moreover, our optimizer reduces ??X delay over multi-tier storage with LRU policy.
\end{itemize}

In conclusion, our contributions are to:

\begin{itemize}
    \item design and implemented the first KV cache storing and loading system targeting the prefill bottleneck for context augmented LLM generation.
    
    \item proposed selective recomputation methods that efficiently combine precomputed KV caches with ??x less delay under only 0.005 F1 drop.
    \item extended KV caching to multi-tier storage and designed loading controller that reduces delay by ??x with Max Flow Solver.

\end{itemize}




% \begin{itemize}
% \item LLM prefill is costly, both in delay and in throughput. 
% it takes one second to prefill only \fillme KB of text. 
% cite recent papers on prefill being a bottleneck.
% \item fortunately, across many LLM apps, it's common that an LLM input contains multiple reused long text chunks shared across different LLM inputs. give several RAG examples, such as news/financial doc analysis.
% \item for these settings where most input texts are reused chunks, that {\em if} we store and reuse the KV caches of all reused texts, we {\em could} greatly reduce delays and improve throughput. need some concrete numbers to give people some sense (some forward pointers).
% \item however, two key challenges arise. 
% first, when the reused text chunk isn't a prefix but follows different texts, its KV cache won't be able to capture its cross-attention with various preceding texts, so it can't be directly reused. 
% \begin{itemize}
%     \item {\em challenge 1: how to reuse the precomputed KV cache of a text chunk when it follows a given text?}
% \end{itemize}
% \item second, compared to storing common prompt prefixes for which CPU memory is enough, storing the KV caches of all potentially reused text chunks needs much more storage space. 
% \begin{itemize}
%     \item {\em challenge 2: how to store all KV caches of reusable text chunks on cheaper yet slower storage while ensuring KV caches can still be loaded fast enough?}
% \end{itemize}
% \item to address these challenges, we present \name, a new module for LLM serving system that efficiently stores and loads multiple chunks of KV caches needed for the inference. 
% (forward point \S\ref{sec:store})
% (mention that the latest work doesn't consider cross-attention, which is prevalent for longer text chunks.)
% \item to address challenge 1, \name incorporates the cross-attention between a stored KV cache with the new preceding text, by selectively recomputing a small fraction of the KV cache values. 
% (forward point \S\ref{sec:merge})
% \item to address challenge 2, \name maintains a low delay of loading KV caches from slower and cheaper storage, by prefetching the KV caches even when the request's still in the queue and selectively storing and loading KV cache only when reducing both delay and cost. 

% \item we've implemented \name on top of Sarathi/DistServe.
% our eval compares \name with vLLM or FlexGen's KV cache management (the state-of-the-art scheme for storing KV cache in GPU and CPU memories) and with PromptCache (the state-of-the-art scheme for reusing non-prefix KV cache). here's a summary:
% \begin{itemize}
%     \item \name achieves \fillme better generation quality in F1-score (for Q-A tasks) and Roug-L (for summarization) than PromptCache without increasing TTFT.
%     \item at the same generation quality, \name reduces TTFT by \fillme\%, increases throughput by \fillme\%, and reduces cost by \fillme\% compared to with KV cache only on prefix and existing KV cache management.
% \end{itemize}

% \end{itemize}

==> sec_intro_v2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


%\jiayi{We should place two graphs in the intro: (1)Normalized quality vs. TTFT (2) Cost savings }
\section{Introduction}

For their remarkable capabilities, large language models (LLMs) are widely used in personal assistance, AI healthcare, and question answering~\cite{llm-app-1,llm-app-2,llm-app-3,llm-app-4}. 
To ensure high response quality, applications often supplement the user query with additional {\em context} texts of domain knowledge or user-specific information~\cite{something might not be rag}.
For instance, in retrieval-augmented generation (RAG), 
% A typical type of such applications is retrieval-augmented generation (RAG). 
%Many RAG systems 
an application will begin with a retriever fetching multiple {\em text chunks} relevant to the query and then concatenate the text chunks and prepend them with the user query to form the final LLM input.
% based on sentence similarity with user request from the text database. 
%These {\em text segments} are then concatenated together and prepended to the request to constitute the final LLM input. 

While necessary for high response quality, the context text chunks also greatly increases the LLM input length and the {\em prefill} overhead during LLM inference. 
The LLM first uses the prefill phase to go through the entire LLM input to produce the {\em KV cache}---concatenated tensors associated with each input token that embeds the token's ``attention'' with all preceding tokens. 
The LLM must finish the prefill phase before it can use the KV cache to decode (generate) the response tokens. 
%The LLM model first goes through a {\em prefill} phase to produce a KV cache that represents the LLM's ``understanding'' of the input through the attention mechanism. 
%Then, in the decoding phase, LLM iteratively predicts the next token with the current KV cache and appends the KV vectors of the newly generated token to the KV cache for next iteration.
%\jc{i like the fact we put RAG as the primary use case, can we not start directly with RAG? it sounds a bit narrow. we can say many apps improve generation quality by putting multiple text chunks as context in the input, and then immediately say RAG is a popular example. } \jiayi{That's how I start sec 2.2. Do you think we should do similar thing here?}

% \jc{why don't we just spell out RAG clearly and upfront and say it's very popular. 
% then in the next para, say because the retrieved docs form long contexts, prefill is slow and expensive, etc}

% \jc{then at the end, we can try to generalize it a bit and say these properties are not unique to RAG}

% For executing intricate tasks, it is common for users or applications to initiate LLM interactions with extensive contexts that may span thousands of tokens or more. This paper treats such extensive preambles provided to various LLM inputs as a context. These context supplements user prompts with domain-knowledge to help LLM generate responses with specific knowledge not contained in the original pretrained model.




% \jc{let's be consistent about the terminology: each input consists of multiple text segments, and each text segment can be a retrieved document (or a chunk of a document) and a user query. currently, we use terms like context, text, or chunk all referring to the same concept ``segment''. just try to be consistent. }

% \jc{text before this point can be much shorter. within .25 of a page. just leave the key points. details can be moved to section 2 or 3}

%\begin{figure}
%\centering
%     \includegraphics[width=1\columnwidth]{figs/time_vs_len_bsz.pdf}
%    \tightcaption{Left: Right:. Non-prefix caching. Store KV cache vs. Full prefill \jc{replace this with a contrast between prefix caching and cachefuse}} 
%    \label{fig:time_vs_len_bsz}
%\end{figure}

\begin{figure}
\centering
     \includegraphics[width=.99\columnwidth]{figs/intro_contrast.pdf}
    \tightcaption{Contrast between prefill, prefix caching, and our partial KV update.}
    \label{fig:intro:contrast}
\end{figure}

Despite many optimizations, 
%Although LLM prefill has been extensively optimzed to parallelize on GPUs, 
the prefill delay and computation overhead grow at least linearly with the input length. 
% it is still very costly due the extensive GPU computation needed. 
%As shown in Figure \ref{fig:time_vs_len_bsz}, 
As a result, prefill can easily become the bottleneck of delay and throughput when the total input is long~\cite{distserve,sarathi,??,??}, such as LLM inputs in RAG which consist of multiple text chunks, each with hundreds of tokens. 
% prefill could easily become the inference bottleneck as the input length or batch size grows. In context-augmented LLM systems like RAG, since the text segments are usually long (upto thousands of tokens), prefill becomes the main bottleneck.
% \jc{the original sentence sounds repetitive. i merged them but please check if it is correct}
%For example, It takes four seconds of two A40 GPUs to only prefill a 4K token context with Llama-70B, while decoding could be batched to increase overall throughput. Previous system~\cite{distserve} could schedule mulitple GPUs to prefill for every GPU dedicated to decoding to compensate for the computation disproportionate compute needed. In the RAG pipelines,  since the text segments are very long but the output lengths may not necessarily be long, prefill becomes the main bottleneck in RAG LLM serving.
%\jc{i like the high-level point that prefill is a bottleneck, but the exact flow sounds quite confusing. for example, unless the reviewer is distserve author or really familiar with the work, they won't be able to understand the middle part. how about we give some concrete numbers on the high resource usage of prefill and throughput difference between prefill and decoding/generation? they seem to be mentioned in current text, but a reader may not directly get them.}
%\jiayi{see Figure \ref{fig:time_vs_len_bsz}}
%\jiayi{say prefill becomes dominant as length increases; decode can be batched; lead to potential optimization (KV reuse)}

So, {\em how to speed up the prefill of LLM inputs that contain {\bf multiple} context text chunks?} 
A few recent systems have noted that the context texts are often reused by many LLM inputs, giving rise to an opportunity to avoid the repeated prefill on the reused texts~\cite{cachegen,sglang,vllm,??,??,??}. 
These systems typically assume that the reused text is the prefix of the LLM input, and under this assumption, the KV cache of the prefix can be precomputed once and reused because the KV cache is not affected by the succeeding texts.

However, in many real-world tasks, LLM inputs need to be augmented by {\em multiple} (often at least three) text chunks, rather than one chunk, to provide different contexts that are necessary to answer the user query. 
For instance, \fillme
\jc{Jiayi, please fill in here}

With multiple text chunks, only one text chunk can be the prefix.
Although the other chunks' KV caches may have been pre-computed, even with corrected positional embedding~\cite{promptcache}, directly using their pre-computed KV caches can lead to wrong answers.
This is because these KV caches do not incorporate the cross-attention with the preceding text in the specific LLM input. (\S\ref{??} offers concrete examples). 

This paper tackles the question: when an LLM input includes multiple text chunks, {\em how to quickly combine their precomputed KV caches} in order to achieve the same generation quality as the expensive full prefill?

We present \name, a scheme that reuses most of the pre-computed KV cache of each non-prefix text chunk but dynamically selects and recomputes a small fraction of the values based on the specific preceding texts. 
The benefit of this {\em partial update} of KV cache is that we can  reuse the KV cache of {\em all} reused text chunks and also mostly recover the cross-attention between text chunks and thus can be used to generate responses that are of the same quality as full prefill without any caching.

The price for the benefit is an extra delay to update the KV of a small fraction of tokens and layers. 
Empirically, this fraction is less than 15\% in many cases, based on our tests over four public datasets for multi-document reasoning.
In other words, \name needs to do no more than $\sim$1/7 of the full prefill computation.

Though partial KV update increases delay, \name~{\em embraces} this delay by pipelining partial KV update with the retrieval of precomputed KV caches from slower devices with more storage capacity into GPU memory, {\em without} increasing the inference delay. 
Specifically, to partially update a KV cache at one layer, \name only needs the KV of the preceding layers to be available in the GPU. 
Though pipelining KV compute and fetching is not new, we note that by storing KV on cheaper storage devices, such as a separate storage server in the same cloud cluster, \name can store the KV cache of many more text chunks without more storage cost or longer delay than storing KV cache in GPU or CPU memory.

We implemented \name on top of vLLM. We evaluated our methods against exisiting LLM serving systems and find our system outperforming them in dimensions of throughput, delay, quality, and cost. \name is able to reduce delay by ?x with only ?\% drop in accuracy, a ?\% increase of state of the art method. Comparing with other KV cache reusing methods, \name could reduce delay by  while keeping cost saving xxx?\%.


\jc{junchen stops here}

\jc{old text below}

%Fortunately, the contexts retrieved are predetermined and can share many overlapping {\em text segments} across different LLM requests, leading to potential opportunities for optimization. 
Consider when a question-answering LLM trained on public datasets receives two user queries that require private knowledge from a company database: ``How many employees are there in each division of the company?" and ``How much revenue does each employee contribute to the company this year?"
% Consider when a question-answering LLM receives two user queries: ``What are the health benefits of a Mediterranean diet?" and ``Why is olive oil considered healthy?".
% The LLM might need to retrieve wikipedia pages under category ``Nutritional Science" to answer the first query and wikipedia pages under category ``Dietary Fats and Oils" to answer the second query, while these two categories could have a large number of overlapping pages. 
A document that records the names and division affiliations of all employees (as large as several gigabytes) would needed to be retrieved to answer both queries. 
In this case, loading this document once and sharing it across different inference requests could unlock substantial performance gain.
% In this case, loading overlapping wikipedia pages once and sharing them among different LLMs could unlock substantial performance gain.

Similarly, for a financial LLM service receiving two requests: ``Analyze Amazon's liquidity position at the end of the last fiscal year.'' and ``Which company has the highest profit in cloud service last year?'' . 
Although these two requests may need separate segments such as ``manual for liquidity position analysis" for the first one and other comanies' financial report for the second one, both requests are likely to use Amazon's annual financial report as a shared text segment.
% for the legal assistant application, two requests ``What are the responsibilities of a landlord regarding property maintenance?'' and  ``Can a tenant withhold rent if the landlord fails to make necessary repairs?'' both require tenant-landlord laws to generate the answers. \jc{in RAG, the input would be several segments of relevant texts from the income statements or landlord laws, rather than one single document. if we don't highlight this, people may be misled to think about prefix caching} 

For these settings where input texts are reused chunks, {\em if} we store and reuse the KV caches of these reused texts, we {\em could} greatly reduce the computation needed and speed up inference. For example, a 4K-token context in Llama-70B takes \textasciitilde 4s to run on 2 A40 GPUs. On the other hand, its KV cache is \textasciitilde 1.25GB if we save the tensors in FLOAT16. If we store this context's KV cache in local CPU DRAM with 10GB/s PCIe bandwidth ~\cite{ebsdata}%\jc{this 4GB/s number seems too high. do we have a pointer AND some good reason why it should be that high?}, 
loading this KV cache into GPU memory only takes \textasciitilde 0.1s. This could potentially speed up the context processing time by \textasciitilde 40x.
%If other concurrent requests have output length of 30 tokens with their prefill reduced too, we will be able to increase throughput by more than 16x. 

% \jc{if we are serious about showing the potential, we need more stats than just throughput improvement. what about delay? what about amount of computation? what about the data size inflation that need to be stored? i'd love to see some ballpark numbers before seeing the challenges.}Through a simple experiment, we should the throughput could increase by ??x if the GPU cycles do not need to be spent on prefill. 


However, such astonishing improvement can only be achieved in very limited scenarios. All reused texts need to be at the begining of the input. This is because KV cache of non-prefix tokens are affected by the previous tokens (e.g., another document, user input) through cross attention. A critical challenge lies in {\em developing a KV cache reusing system capable of accommodating non-prefix texts while managing the potentially vast size of KV caches}. Directly reusing the KV cache at non-prefix positions fails to help LLM synthesize multiple contexts together (Figure \ref{fig:text_comparison}). In addition, simply storing all KV cache in CPU DRAM is impractical (Figure \ref{fig:intro_storage}). Therefore, the system necessitates a solution that provides an economical storage space for the KV cache and ensures efficient cache delivery to the GPU for processing.  

%Second, the common approach of caching reuseable KV cache in CPU memory could not satisfy the growing number of text documents~\cite{prefix reuse papers, growing number of documents}. As shown in Fig \ref{fig:cachesize}, the CPU memories in a 2 * A100 instance is only able to accodomate 183 4K-token Llama-70B KV caches. While it is possible to attach more CPU memories or storage devices to the compute device, these devices vary widely in throughput and cost~\cite{fig:intro_storage} and it remains unlear how to utilize them economically and efficiently.

\begin{figure}
\centering
     \includegraphics[width=1\columnwidth]{figs/intro_storage_graph.pdf}
    \tightcaption{Instance CPU memory could not hold all Llama 70B 4K-token KV caches \hc{needs update. }\jiayi{maybe deleted}} 
    \label{fig:intro_storage}
\end{figure}


%\jc{it's still unclear to me why it's challenging to achieve the astonishing improvement of 11.4x delay speedup. is it because SSD is too expensive so most KV cache will be store in some remote server like S3? if so, how does addressing the 2nd challenge make most KV cache in SSD despite its limited space?} \hc{Updated, Do you think I need to add more?}

We present \name,
% {\name is the goddess of knowledge in Greek Mythology and our system manages the knowledge sources of LLM: KV cache of retrieved documents.} 
the first context KV cache management system that allows flexible KV reuse at non-prefix positions. \name achieves efficient and economical storing, loading, and fusing KV caches by the design of three components, a KV cache fusor and a KV cache manager, and a loading controller. Our KV cache fusor takes different segments' KV cache and recovers the cross attention between them by partially recomputating a small fraction of the KV vectors on-the-fly. In addition, the fusor is able to restore accurate positional embedding of the KV cache through a fast element-wise matrix multiplication, avioding the need to store KV cache at different positions. Our loading controller and KV cache manager help to deliver the raw KV cache for the fusor with a multi-tier storage system that allocates storage sizes economically based on the workload. Furthermore, we implemented three system optimizations to improve and extend \name: (1) pipelining computation with loading, (2) storage-aware request reordering, and (3) model-aware cache eviction for multi-model serving. 

We implemented \name on top of VLLM with xx lines of python and xx lines of CUDA. We evaluated our methods against exisiting LLM serving systems and find our system outperforming them in dimensions of throughput, delay, quality, and cost. \name is able to reduce delay by ?x with only ?\% drop in accuracy, a ?\% increase of state of the art method. Comparing with other KV cache reusing methods, \name could reduce delay by  while keeping cost saving xxx?\%.


In conclusion, our contributions are to:

\begin{itemize}
    \item design and implemented the first KV cache storing and loading system targeting the prefill bottleneck for context reuse systems.
    
    \item proposed selective recomputation framework that efficiently combines precomputed KV caches with 80-90\% less FLOPs compared with full recomputation while maintaining satisfying generation qulity (only \fillme F1 drop).

    \item KV cache manager (supports KV fusor efficiently, materialze the benefit of kv fusor) \jiayi{TODO}
    %\item designed KV cache manager that smartly allocates non-volatile storage devices based on model configuration that reduces xxx delay under constrained budget.

\end{itemize}




% \begin{itemize}
% \item LLM prefill is costly, both in delay and in throughput. 
% it takes one second to prefill only \fillme KB of text. 
% cite recent papers on prefill being a bottleneck.
% \item fortunately, across many LLM apps, it's common that an LLM input contains multiple reused long text chunks shared across different LLM inputs. give several RAG examples, such as news/financial doc analysis.
% \item for these settings where most input texts are reused chunks, that {\em if} we store and reuse the KV caches of all reused texts, we {\em could} greatly reduce delays and improve throughput. need some concrete numbers to give people some sense (some forward pointers).
% \item however, two key challenges arise. 
% first, when the reused text chunk isn't a prefix but follows different texts, its KV cache won't be able to capture its cross-attention with various preceding texts, so it can't be directly reused. 
% \begin{itemize}
%     \item {\em challenge 1: how to reuse the precomputed KV cache of a text chunk when it follows a given text?}
% \end{itemize}
% \item second, compared to storing common prompt prefixes for which CPU memory is enough, storing the KV caches of all potentially reused text chunks needs much more storage space. 
% \begin{itemize}
%     \item {\em challenge 2: how to store all KV caches of reusable text chunks on cheaper yet slower storage while ensuring KV caches can still be loaded fast enough?}
% \end{itemize}
% \item to address these challenges, we present \name, a new module for LLM serving system that efficiently stores and loads multiple chunks of KV caches needed for the inference. 
% (forward point \S\ref{sec:store})
% (mention that the latest work doesn't consider cross-attention, which is prevalent for longer text chunks.)
% \item to address challenge 1, \name incorporates the cross-attention between a stored KV cache with the new preceding text, by selectively recomputing a small fraction of the KV cache values. 
% (forward point \S\ref{sec:merge})
% \item to address challenge 2, \name maintains a low delay of loading KV caches from slower and cheaper storage, by prefetching the KV caches even when the request's still in the queue and selectively storing and loading KV cache only when reducing both delay and cost. 

% \item we've implemented \name on top of Sarathi/DistServe.
% our eval compares \name with vLLM or FlexGen's KV cache management (the state-of-the-art scheme for storing KV cache in GPU and CPU memories) and with PromptCache (the state-of-the-art scheme for reusing non-prefix KV cache). here's a summary:
% \begin{itemize}
%     \item \name achieves \fillme better generation quality in F1-score (for Q-A tasks) and Roug-L (for summarization) than PromptCache without increasing TTFT.
%     \item at the same generation quality, \name reduces TTFT by \fillme\%, increases throughput by \fillme\%, and reduces cost by \fillme\% compared to with KV cache only on prefix and existing KV cache management.
% \end{itemize}

% \end{itemize}

==> sec_motivation_v1.tex <==
\begin{figure}
\centering
     \includegraphics[width=.95\columnwidth]{figs/text_comparison.pdf}
    \tightcaption{Text comparison} 
    \label{fig:text_comparison}
\end{figure}

\begin{figure}
\centering
     \includegraphics[width=.95\columnwidth]{figs/attn_comparison.pdf}
    \tightcaption{\jiayi{add some explanation}\jiayi{Please add boxes to indicate cross attention and internal attention}\jiayi{improve this visualization by not focusing on the internal attention in second chunk}}
    \label{fig:attn_comparison}
\end{figure}

\section{Extended Motivation}
\label{sec:motivation}
% \hc{I think there is sth missing here. We are actually using storage devices as cache. This is actually a nontrivial idea and this is only rational because recomputation is so costly and long. We need to explain this here or otherwise reviewers in storage (many in SOSP) can get really confused.}
%\hc{I wonder if we want to change the content below?}
As mentioned in \S\ref{subsec:transformer}, prefilling phase could easily become the bottleneck in LLM inference as input length increases. A  \jiayi{Add some transition}

 \subsection{LLM serving with substantial text redundancies}
 \label{subsec:redundancy}
% \hc{I am leaving this here since Jiayi and Siddhant probably knows much more about how people use RAG}
%\sr{For many applications (like RAG), it is useful to have a system which supports the reuse of contexts, as recomputation of many (long) contexts is expensive in terms of computation\cite{context_reuse}. As workloads get more complex, it is common to have contexts in RAG pipelines upto ${\sim}1M$ tokens\cite{1m_context} In such scenarios, it is natural to reuse the shared KV cache between all requests which reuse these long contexts. Such requests might be different questions from the same set of contexts or queries from different users about the same topics (like code documentation)\cite{su2024arks}.

%Some contexts maybe resused with significant time gaps (different users might query the same code documentation over several hours), which makes it important to store the KV cache of such contexts for longer times. Also, the size of the KV cache increases linearly with the sie of the prompt (GPT-3 generates a 4.5MB KV cache for each token) and prompts containing 1000s of tokens will produce several GBs of KV cache\cite{gao2024attentionstore}.

%Finally RAG consists of retrieving and adding relevant context chunks to the prompt. Most RAG applications today tend to use multiple small chunk sizes (upto 1024 tokens) for output generation\cite{chunk_stats_1, chunk_stats_2}. A common method of adding the context chunks to the prompt is simply concatenating them sequentially to the prompt. When the number of retrieved contexts chunks sizes are small, this becomes an obvious choice as the overall context window doesn't exceed the size of the model's window and the output generation is fast. When larger contexts are present, there exist other methods to combine the retreived contexts (like Refine, Map Reduce or Map Rerank) but these are often slower as they involve multiple calls to the LLM\cite{langchain, compare_chains}.}

%\sr{\textit{Hanchen please add approprriate conclusions above}}

% \begin{itemize}
% \item many appalications (RAG) are wildly popular. show several examples, see this link for some inspiration: \url{https://chat.openai.com/share/607cf54f-2180-4a66-a177-bb6cb2352864}
% % have requests that share a lot of context chunks. 
% \item a few characteristics of this workload:
% \item first, long text chunks are reused (100s or 1,000s of tokens). \\
% $\Rightarrow$ kv caches are much bigger than usual length of chat prefix (can we get some numbers from shareGPT?).
% \item second, chunks shared across separate requests, possibly from different users.\\
% $\Rightarrow$ unlike chatbot apps, a text chunk may be re-used over a long period of time.
% \item third, the input chunks are not supposed to be processed separately. \\ 
% $\Rightarrow$ input concatenates multiple chunks.
% alternatives are either slower (like refine) or have lower quality (like MapReduce and ReRank). (need Siddhant's help on this!)
% \end{itemize}

%\hc{siddhant is finishing this by Sunday morning}

%\jiayi{The motivation for more chunks should be two-fold: (1) the related info might not reside in the first chunk; (2) some tasks (e.g., reasoning, comparison, summary) do need more chunks}

%\jiayi{We should convey three points here: (1) multiple documents should be retrieved; long, (2) these documents should be read jointly, (3) prefix ratio is low}

\jc{somewhere in this subsec, we need to clarify our focus is the inference on the retrieved chunks, rather than which chunks to retrieve}
Many popular LLM applications often encounter the case when input prompts contain a substantial portion of constantly recurring texts. We define these recurring and reusable texts as text redundancies in LLM inputs. 
Text redundancies can be found in AI agents where agents are always prompted with templated instructions \cite{Significant_Gravitas_AutoGPT, pmlr-v162-huang22a, qin2023tool}. 
Such redundancies also exist in chat histories that are stored, partially modified and constantly reused \cite{packer2023memgpt, wu2024secgpt}. 
A typical and popular category of such applications is Retrival Augmented Generation (RAG) \cite{lewis2021retrievalaugmented}. 

Existing research has shown enormous benefits of utilizing RAG pipeline LLMs in many aspects, such as alleviating hallucination issues\cite{mao2020generation, ram-etal-2023-context} and provding more privacy and security control over proprietary information\cite{gao2023retrievalaugmented}. 
A common RAG paradigm usually contains three stages: indexing (preprocessing the documents), retrieving the documents, and generating. A toy RAG example is shown in Figure \ref{fig:text_comparison}. The user gave a query of \textit{"How many goals did Messi score more than Cristiano Ronaldo at FIFA World Cups?"}. A RAG retriever will retrieve text chunks including two players' career statistics inside the pre-built text database. In the generation stage, the retrieved texts and the user question are combined and fed into LLM. In this case, the career satistics regarding Messi and Ronaldo are known in advance and are expected to be reused when there come similar queries (e.g., \textit{"Who scored more than five goals at FIFA World Cups?"}).

\begin{figure}
\centering
     \includegraphics[width=.95\columnwidth]{figs/rag_acc.pdf}
    \tightcaption{Accuracy increases as more chunks are retrieved \jiayi{can we have another dataset?}} 
    \label{fig:rag_acc}
\end{figure}

\begin{figure}
\centering
     \includegraphics[width=.95\columnwidth]{figs/time_prefix.pdf}
    \tightcaption{TTFT grows as more chunks are retrieved (assuming cache already in GPU), \jiayi{we should also have a fig for cache not in GPU, in that fig, ours can be the same as optimal}} 
    \label{fig:time_prefix}
\end{figure}

The above toy example is an idealized scenario. Real-world RAG workloads require more and longer chunks to include enough information in the context. For example, the actual text information in the toy example could be "Messi is one of the only six men played in five World Cups alongside Antonio Carbajal.... He has scored 13 goals at FIFA World Cups in total". In this case, we need bigger chunk length to retain the semantic coherence. And the retriever might need to retrieve more than two chunks in order to retrieve the scoring information about Messi and Ronaldo. In addition, some tasks innately require multiple text chunks (e.g., summarization, multihop reasoning). To be more concrete, we use a popular multihop reasoning dataset Musique\cite{???}, where we retrieve chunks of size 128 tokens (a popular number)\cite{jan_chunksize} and evaluate the generation quality by increasing the number of chunks. As shown in Figure \ref{fig:rag_acc}, accuracy can be doubled as more chunks are retrieved. Note that only reading these chunks jointly can lead to such accuracy improvement as the LLM requires information from multiple chunks to reason about the steps in the required answer generation. Therefore, we believe there are always use cases where 

\textbf{\em Multiple chunks should be read jointly.}
%\sr{We should add here that we need more chunks because what matters is the total input text to the LLM which should have all the facts}. 

However, incorporating longer contexts in the LLM input inevitably increases the context processing time. Such overhead can be alleviated by reusing the recurring prefixes of contexts' KV cache. However, even assuming contexts are used strictly at the begining of the input or the texts before contexts (e.g., system prompt, user instruction, chat history) are fixed and pre-known, the prefix ratio will eventually become low as more text chunks are retrieved, which constrains the benefits of KV reuse. As shown in Figure \ref{fig:time_prefix}, assuming the precomputed KV cache is in (or already loaded to) GPU, the benifits of prefix reuse soon become negligible as more chunks are retrieved. Therefore, it's apparent that

\textbf{\em Prefix caching is limiting.}

%Note that the grey line in Figure \ref{fig:time_prefix} shows the maximum potential of KV cache reuse. The overhead in this optimal imaginary scenraio is only prefilling the last token (assuming the KV cache is already in GPU and can be directly reused). In reality, we cannot expect the KV cache always reside in GPU. \jiayi{somehow empirically show this, a lot of KV cache. also show the loading overhead somehow}. Therefore, 

%\textbf{\em KV cache needs to be stored and loaded efficiently.}

%Further, . As shown in Figure \fillme, scattered (more ). That is, if we only . Therefore, the potential for reusing the KV cache could be constrained by a finite and fixed storage capacity (e.g., CPU DRAM, Local SSD).


%For example, to build a RAG pipeline for open-domain question answering, we can use wikipedia as our external knowledge base. In the indexing stage, we need to first parse the wikipedia pages and load the texts into smaller chunks. Chunking is necessary in that LLMs have a max input limit, and longer context inputs inevitably increase the response delay due to longer prefilling time. In addition, irrevalent information can also degrade the genration accuracy\cite{chen2023benchmarking, liu2023lost}. An embedding model (e.g., BERT\cite{turc2019}, BGE\cite{bge_embedding}) is then used to encode the text chunks into vectors. Lastly, an index is created for each text chunk and the corresponding embedding and raw text are stored as a key-value pair. In the retrieval stage, relavent text chunks are retrieved based on the similarity between their emeddings and the embedding of the given user query. The retrieved text chunks and the user query is toghether fed to the LLM as input.

%\S\ref{subsec:redundancy} (reuse opprortunities exist and can be benefitial), context augmented generation could have very long input length. In these cases, naively following the original logic could incur great cost in prefill phase. In order to solve this problem, a promising solution emerges: instead of recomputing the long context every time a request arrives at the server, we could store the pre-computed KV cache corresponding to different contexts and load them into GPU memory when needed. 

%This optimization requires a new module that is currently missing in the current LLM serving ecosystem. Ideally, this KV cache management module is able to perform the following tasks:
%\begin{itemize}
%    \item Storage of as many reusable contexts as possible with minimal cost.  
%    \item On-demand loading of the KV caches with minimal delay. 
%    \item Ability to combine KV caches of different contexts for future inference. 
%\end{itemize}

%These three tasks are essential to accomadate the different use cases of context-generated LLM discussed in \S\ref{subsec:cases}. After the retriever \hc{please explain in 2.2 about how the retriever works} fetches the documents


% \begin{itemize}
% \item for these retrieval-based apos, an opportunity emerges to minimize prefill by reusing kv cache. 
% \item we need a new module that stores and loads KV caches efficiently. 
% \begin{itemize}
%     \item storing kv caches of potentially reused text chunks
%     \item on-demand loading the kv caches of reused text chunks
%     \item update kv caches to include the cross-attention among the text chunks
% \end{itemize}
% \item a few words on the potential benefits: higher throughput and lower delay
% \end{itemize}


\subsection{Challenges and prior attempts}
In the last section, we have discussed the potential of KV reuse to relieve the prefil bottleneck. Many prior works have focused on prefix reusing to reduce this overhead. vLLM\cite{kwon2023efficient} innately supports prefix reuse within a batch, which can be easily extended to cross-request scnario (e.g., offload the KV cache to CPU). %ChunkedAttention\cite{ye2024chunkattention} futher optimizes attention computation when multiple requests in a batch share the same prefix.
SGLang\cite{sglang} uses a tree-like structure and an LRU policy to maximize the commonly shared prefixes among concurrent requests.
RAGCache\cite{jin2024ragcache} extends a similar tree structure and futher optimizes the cache eviction policy, enabling prefix reuse among different requests.

However, in these works, the benefits of KV reuse only exist when reuse takes place at prefix position.
Therefore, to build a more flexible system that maximizes the potential of KV resue at any positions, the key challenge is  

 \textbf{\em How to combine the independently precomputed KV cache of different text chunks effectively and efficiently?}

An easily thought of solution is to naively concatenate the KV vectors of multiple text chunks. \promptcache\cite{gim2023prompt} follows this line of thought by simply concatenating KV vectors of recurring text chunks with the help of buffers to ensure positional accuracy. For example, if we are to concatenate chunks \(C_{1}\) and \(C_{2}\), the KV vectors of \(C_{2}\) needs to be cached as \((l*buffer, C_{2})\) where \(l\) is the length of the buffer and should be greater or equal than the length of \(C_{1}\). This naive concatenation strategy has two innate problems. First, cross-attenton between \(C_{1}\) and \(C_2\) is completely ignored (Figure \ref{fig:attn_comparison}). As a consequence, the generation quality drops significantly (Figure \ref{fig:text_comparison}). Second, precomputation at fixed positions (with buffers) only allows the resuse of the same texts at similar positions. The KV vectors of the text chunk have to be precomputed multiple times and saved in multiple copies (with different buffer lengths) in order to be reused at any position. We will address these two problems in the next section \ref{sec:merge}.

In addition to combine, \jiayi{Can we somehow naturally mention the difficulty in loading here}


 %As mentioned in \S\ref{subsec:cases}, the retriever fetches text chunks from various sources and uses them together as a whole piece of context for inference. Reusing KV vectors of these recurring text chunks can lead to fewer context processing computation. However, the self-attention mechanism, which allows a token to pay attention to its subsequent tokens, makes KV vectors only reusable when the recurring text is a prefix of the context. 
 
 %\jiayi{I have pushed naive concat to the next part.}

 
 %The naive prefill phase will recompute the KV cache for this new concatenated context and capture the relationships between each token. However, during the offline precomputation, each chunk's KV cache was assumed to be the only context in inference. Thus, the KV cache for an individual chunk does not contain its tokens' relationship with tokens in other chunks. For example, \hc{Lets put a graph to show the two challenges, this is the first part. two sentences related but could not be understood if not taken together} As a consequence, if we naively concatenate the KV caches together, the generation quality drops significantly (shown later in \S\ref{}).

%Second, how do we determine where to store the KV cache while the benefit of reusing varies widely depending on model, storage device type, and reuse frequency? For a fixed length text segment, the fastest yet cheaper than prefill storing location for its KV cache varies widely with different model and reuse frequency. How do we determine where to place one KV cache given the abundance of storage device available remains unclear.

%{\em Challenge \#2: How do we determine where to store the KV cache under a cost budget while the benefit of reusing varies widely depending on model, optimizations enabled?}

%\jiayi{should be store and load now. please drop this chalenge and makes it as a natural consequence of KV reuse (e.g., we can reuse more kv cache, therefore we nned to store more)}

% In a retrieval based LLM application, different text segments could have very different reuse frequency depending on the popularity of the content inside. If we choose a high end storage device for a rarely reused KV cache, the storage cost could easily rise above the original prefill.

%Since different storage devices vary widely in throughput and cost, it is important to choose an appropriate storage setup to minimize delay.
%However, this option is dependent on the model we are serving as well as optimizations available.

%We show an cost analysis for running Llama-7B, 34B, and 70B with KV cache 8-bit compression enabled on AWS platform in Fig. \ref{fig:motiv-models} with different provided storage types. This is due to different models' KV cache sizes vary widely due to architecture difference. 

%Moreover, the abundant compression and quantizations available also affects the optimal storage devices we want to us. As shown on Fig. \ref{fig:motiv-quantizations}, storing Llama 70B's KV cache in FP16 on a 100MBps S3 storage increases delay by xxxX. If the developer uses S3 without choosing to do 8-bit quantization, all requests that loads from this tier will suffer from extra TTFT. Moreover, there are more available KV compression methods that potentially induces more loss, based on the developers' tolerance of loss in the application, we need to build this caching system with different compression methods in consideration.

% \begin{figure}
%     \centering
%     \includegraphics[width=.95\columnwidth]{figs/store_challenge_model.jpeg}
%     \caption{With 8-bit quantization, Llama 7B, 34B and 70B have different delay-prefill over cost curve\jiayi{Is it Mistral 7b or llama 7b?}}
%     \label{fig:motiv-models}
% \end{figure}

% Thus, for a KV cache reuse system, a wide range of KV caches could be stored. In order to save cost, we need to store many of them in cheaper non-volatile memory devices such as SSD or hard disk. These different devices vary in cost and throughput. And loading multiple contexts in the same time could cause contention for IO throughput, which makes loading delay more than recomputation. Moreover, due to the different designs of LLM models, caching their KV cache size brings differnet extents of benefit when compared with recomputation. For example, recomputation with llama 7B is 4x faster than llama 70B, but its KV cache is even twice as big as 70B! This disparity means that under the same reuse frequency, storing KV cache of Llama 70B could potentially be 8x more worth than storing llama 7B KV cache. Given this disparity in model to be served and storage types that could be utilized, it remains unclear how do we create a system to handle this complexity.


% \begin{figure}
%     \centering
%     \includegraphics[width=.95\columnwidth]{figs/store_challeng_opt.jpeg}
%     \caption{Using Llama 70B, storage device utility curve also varies with optimization enabled}
%     \label{fig:motiv-quantizations}
% \end{figure}


% \begin{itemize}
% \item first, when the reused text chunk isn't a prefix but follows different texts, its KV cache won't be able to capture its cross-attention with various preceding texts, so it can't be directly reused. 
% \begin{itemize}
%     \item
% \end{itemize}
% \item second, compared to storing common prompt prefixes for which CPU memory is enough, storing the KV caches of all potentially reused text chunks needs much more storage space. 
% \begin{itemize}
%     \item 
% \end{itemize}
% \end{itemize}





% \subsection{Why not existing solutions?}
% \label{subsec:existing solutions}
% A lot of work has been done in the intersection between LLM and systems. We discuss the most related ones in this part and explain why they are not sufficient to solve the two challenges.

% Many prior works have adopted prefix reusing to reduce KV cache prefilling. ChunkedAttention\cite{ye2024chunkattention} optimizes attention computation when multiple requests in a batch share the same prefix.
% SGLang\cite{sglang} uses tree-like structure and use LRU policy to reuse the KV vectors of commonly shared prefixes across different requests. However, these methods only utilize limited GPU and CPU memory to cache KV cache generated by temporal approximate requests. \jiayi{Can we focus on "prefix" instead of "multi-tier" in this para.?} as mentioned earlier (\jiayi{or show here}), prefix-only caching is too limiting \hc{We should explain what prefix reuse does, and show the result Jiayi put earlier (prefix ratio is low in RAG)}.

% A straightforward solution is to naively concatenate the KV vectors of multiple text chunks. \promptcache\cite{gim2023prompt} follows this line of thought by simply concatenating KV vectors of recurring text chunks with the help of buffers to ensure positional accuracy. For example, if we are to concatenate chunks \(C_{1}\) and \(C_{2}\), the KV vectors of \(C_{2}\) needs to be cached as \((l*buffer, C_{2})\) where \(l\) is the length of the buffer and should be greater or equal than the length of \(C_{1}\). This naive concatenation strategy has two innate problems. First, cross-attenton between \(C_{1}\) and \(C_2\) is completely ignored (Figure \ref{fig:attn_comparison}). As a consequence, the generation quality drops significantly (Figure \ref{fig:text_comparison}). Second, precomputation at fixed positions (with buffers) only allows the resuse of the same texts at similar positions. The KV vectors of the text chunk have to be precomputed multiple times and saved in multiple copies (with different buffer lengths) in order to be reused at any position. We will address these two problems in section \ref{sec:merge}. 

% Many existing systems also offloads KV caches to CPU or storage devices to increase throughput. 
% vLLM~\cite{?} uses CPU to store KV caches when GPU memory is not enough to store all KV cache page. 
% FlexGen~\cite{?} designs offloading strategy for both model weights and KV cache to optimize throughput under constrained resources. 
% InfiniteLLM~\cite{?} shares CPU memory across datacenter to accomadate long requests. 
% However, these systems only offload KV cache within a single request and only reuses KV cache for the unfinished job in its current queue. 
% \hc{rag cache and attention store needs to be mentioned}
% \qz{system reviewers not familiar with LLMs would be smashed when they read all these related work; make a table summarizing prior work's limitations and compare with METIS (to-do)}

% It is possible to extend them to multi-tier storage and reuse them across requests. But their current design will fail under such scenarios. If KV cache is offloaded to cheap storage devices, the delay incurred when re-loading this KV cache back to GPU could be very high. Moreover, loading different context from the same device could cause contention for the limited throughput/bandwidth. 
% \qz{focus on why existing offloading strategies cannot be easily adapted for multi-tier storage and multi-request KV cache reuse}
% \begin{itemize}
% \item previous systems are not designed for this concept \\

% \item for challenge 1, some prior systems cache prefixes across requests
% \begin{itemize}
% \item examples: vllm, chunkedattention, gslang
% \item they also reuse kv across requests.
% \item but limited benefit in RAG
% \end{itemize}

% \item better solution is modular caching: such as promptcache. 
% \item however, it can't handle cross-attention. give an example! 
% \item explain the cross-attention and how promptcache may have missed it.\\

% \item for challenge 2: some systems (distkv-llm, flexgen, vllm) also cache more kv than one gpu can
% \item but they only manage kv cache within a single job, so most kv caches are in gpu, and even if a kv cache is offloaded, we know when it's used

% \item can we extend them to storing kv caches across jobs? yes, but they do not optimize the cost-delay trade-offs when storing the kv cache on cheaper yet slower storage, like local or remote storage. The delay also would be higher
% \end{itemize}



==> sec_recompute_v1.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Fast Context Fusing by Selective Recomputation}
\label{sec:merge}


% \hc{Hi Jiayi, I think this part right now is too mathy. when we modify it later do you think the following is a better way? 1. How we capture the error by comparing first layer result and later layer result. Don't go too deep in attention mechanism, just tell them the specific way we determine loss with one-sentence insight (math intuition) in paper and put the actual calculation in appendix. 2. How we determine the recompute ratio and how we recompute. I assume this is token wise computation and pretty intuitive. 3. How we only save the KV cache before positional encoding and update them on the fly. We should say the exact math operation we are doing during recovery, but leave the proof in appendix}
% \jiayi{I think getting a bit mathy is okay for sec5. Reviewers probably will just look at the figures (or not) in sec 5 and 6 and jump to the eval section. But I do think this sec is a bit too long. Might need to move sth to appendix..}
% \begin{itemize}
% \item why only a few tokens' kv cache need to be updated? only a small fraction tokens have high cross-attention
% \item some empirical evidence (maybe goes back to the example in 3.2) 
% \item is this the same insight as sparse attention \\

% \item our idea: prefill but skipping most of the tokens and layers
% \item framework: no change to the overall workflow of prefill, but between two layers, select the {\em high cross-attention} tokens to recompute.
% \item we explain four aspects: 
% (1) how to select high cross-attention tokens between two layers, 
% (2) how to recompute high cross-attention tokens with minimum overhead, and
% (3) how to quickly calibrate positional encoding.
% \end{itemize}

In this section, we address the key challenge mentioned in the last section (\S\ref{sec:motivation}). 
Namely, we present how \name fuses {\bf \em multiple} reusable text chunks by recomputing a small fraction of KV cache at a subset of layers and tokens and dynamically recovering the positional information of the KV cache. 
%\jc{should we use KV vectors or KV caches? previous text uses KV cache, but I'm fine either way. Just make sure it's consistent.}
%\jc{swap the order. selective kv recompute should come before more efficient positional encoding}
In this way, \name can save compute by reusing the KV cache of all the text chunks without compromising generation quality.
%\jc{verbose.. just say "save compute or save GPU compute cycles"}
%\jc{can we just say no compromise on generation quality?}
%\jc{reusing most KV sounds vague. say KV of all reused text chunks. please be specific in other places too.}

In \S\ref{subsec:HCA}, we first note the sparsity of cross-attention, which implies that only a small fraction of tokens are affected by cross attention. Further, we measure the impact of cross attention by comparing the deviation between precomputed KV cache (without cross attention) and fully recomputed KV cache (with cross attention). To recover cross attention, we choose to recompute tokens with high KV deviation (HKVD tokens) and update the corresponding KV cache. However, such strategy does not save any compute as obataining KV deviation requires fully recomputed KV cache, therefore, requiring the expensive full prefill. To address this inefficiency, we propose a lightweight prediction-based algorithm to approximate the HKVD tokens. Then, in \S\ref{subsec:framework}, we explain mechanically how KV cache of HKVD tokens can be recomputed and updated efficiently with our novel partial prefill framework. Finally, in \S\ref{subsec:recover pos}, we present a method that quickly recovers the positional encoding of KV cache for a given position on the fly.

\jiayi{Above is a new outline structure}


\jiayi{Response to the comment at the end: The key chanllenge or technique is NOT using KV deviation to approximate cross attention because obtaining either the KV deviation (require the whole fully recomputed KV cache) or the attention matrix is expensive anyway (both require compute more than full prefill). Instead, the key challenge is to approximate KV deviations with a small amount of compute.}

%\jiayi{A natural question would be: why do we use KV deviation instead of directly using the deviation in the attention matrix? The answer is in two fold. (1) We didn't cache the precomputed attention matrix. Therefore, we can't compute the deviation. (2) Deviation in KV cache can reflect the errors in both cross attention and internal attention. The root cause of inaccurate internal attention is still cross attention. However, this might be somewhat contradictory to our sparsity claim. Therefore, I agree the internal attention thing should be dropped. Otherwise, we might need to change our sparsity claim a bit. Let me think about this.... and then reconstruct the following parts}

%\jc{the outline structure is not very clear. it's there but buried..  try to crystallize it.}
%We start with \jc{formally?}defining two types of attention: (1) internal attention\jc{is internal attention so important to be mentioned in preamble?} and (2) cross-attention (\S\ref{subsec:HCA}). \jc{need a transition here: so the key is to recompute the kv of tokens with high cross-attention with other tokens (any other tokens or the sum of other tokens?)? and explain briefly why it's hard to precisely know which tokens have high cross-attention}
%Moreover, we demonstrate how to \jc{approximately}identify tokens that are severely affected\jc{``severely affected'' sounds awkward. just say tokens that have ...} by high cross attention (HCA)\jc{dont introduce terms unless it'll be repeatedly reused right away} and why the recomputation of such tokens should be prioritized. 
%Then, in \S\ref{subsec:framework}, we explain how to perform "recomputation" mechanically during the LLM prefill phase and present a cascading token recomputation framework that enables de-facto compute savings\jc{i dont understand this phrase}, and thus reducing TTFT. 
%Then in \S\ref{subsec:prediction}, we illustrate a lightweight prediction-based HCA token selection method in order to maximize the number of recomputed HCA tokens under the cascading recomputation framework. 
%Finally, in \S\ref{subsec:recover pos}, we present a method that quickly recovers the positional encoding of KV cache .
%a more effective and also more efficient\jc{sounds handwavy, just say a scheme that quickly recovers xxx for a given position, etc} way of recovering positional encoding compared with \promptcache. %\name's overall framework is depicted in Figure \fillme. 

\subsection{Recovering cross attention with HKVD tokens}\label{subsec:HKVD}

\mypara{Sparsity of cross attention}
%\jiayi{The precoputed KV should still preserve some locality through cross attention. However, only a small fraction of tokens are still affected by cross attention.}
\jiayi{Working on a visualization (similar to scissorhands)}
Attention sparsity has been widely observed in the existing research \cite{liu2024scissorhands,h2o,choromanski2020rethinking,chen2021scatterbrain}. Namely, one token attends to only a small number of tokens, meaning that the attention score follows a power law distribution. Building upon this observation, we further zoom into cross attention as the independently precomputed KV cache only takes internal attention (within in each chunk) into account but misses any cross attention (between chunks). Fortunately, we find that cross attention is also sparse. Figure \fillme visulizes the amount of cross attention each token receives. It is clear that cross attention is only prevalent in a small fraction of tokens. In addition, Figure \fillme confirms this observation on a larger scale, showing the power law distribution of cross attention scores. 
%The sparsity observed in cross attention suggests the precomputed KV cache of most tokens could bear enough semantic meaning for the LLM to understand through internal attention. 


\mypara{Measuring cross attention with KV deviation}
%We note that KV deviations can be used to measure the impact of cross attention. 
Due to the sparsity of cross attention (\S\ref{sparse}), we expect only a small subset of tokens to be significanly affected by cross attention.
We use KV deviation to measure how much the precomputed KV cache is affected by cross attention (i.e., misses how much cross attention). KV deviation for token \(i\) at layer \(j\) is computed as \(||\{K_{ij},V_{ij}\}-\{K^{'}_{ij},V^{'}_{ij}\}||\) where \(\{K,V\}\) are the fully recomputed KV cache and \(\{K^{'},V^{'}\}\) are the precomputed KV cache containing errors (w/o any cross attention). %The intuition behind this is that KV cache . 
We use the two-chunk example  in \ref{subsec:existing solutions} (Figure \ref{fig:text_comparison}) to demonstrate why KV deviation can be used to measure cross attention. Assume there are two retrieved text chunks \(C_{1}\) and \(C_{2}\) whose KV cache is independently pecomputed, and assume there's a token \(i\) in \(C_{2}\). We start from layer \(j\). Denote the cross attention between \(C_{1}\) and token \(i\) as \(CrossAttn_{ij} \in \mathbb{R}^{1\times k}\) where \(k\) is the number of tokens preceding token \(i\) in total. Similarly, denote the attention within \(C_{2}\) between \(C^{'}_{2}\) (tokens in \(C_{2}\) and preceedig token \(i\)) and token \(i\) as \(InternalAttn_{ij}\). Then, the output of attention module at this layer \(j\), \(AttnOutput_{j} \in \mathbb{R}^{d}\) where \(d\) is the hidden dimension, is computed as \((V_{C_{1}},V_{C^{'}_{2}})(CrossAttn_{j}, InternalAttn_{j})^{T}\). This \(AttnOutput\) is then passed through several neural layers (MLP module) to form the input embedding of token \(i\) at the next layer \((j+1)\), denoted by \(x\). KV cache for token \(i\) at layer \((j+1)\) can be computed as \(\{k,v\}=\{W_{\{k,v\}}x\}\). Note that \(CrossAttn_{j}\) is essentially zero when KV cache is precomputed independently whereas \(InternalAttn_{j}\) can be preserved during precomputation.
%\jiayi{The fact is internal attention cannot be computed accurately but let's play down this}. 
Therefore, token \(i\) is expected to have high KV deviation if it receives high cross attention. To recover cross attention given a limited fraction of KV cache to be recomputed and updated, we should prioritize the recomptation over tokens with high KV deviations (HKVD tokens). Formally, HKVD tokens should be picked as 

%\begin{center}
\begin{gather}
    \mathop{\arg\max}\limits_{I} \sum_{i,j}||\{K_{ij},V_{ij}\}-\{K^{'}_{il},V^{'}_{ij}\}||I_{i,j}\nonumber\\
     \text{s.t.} \quad I_{i,j}=\{0,1\}, \sum_{i,j} I_{i,j} = rNL \nonumber 
\end{gather}
%\end{center}



where I is the dummy variable indicating whether token \(i\) at layer \(j\) is considered as an HKVD token, N and L are the total number of tokens and layers, and the fraction of HKVD tokens is limited by a fixed HKVD ratio \(r\).

\mypara{Inefficiency of identifying HKVD tokens}
 In the last \ref{HKVD}, we rely on KV deviations to identify HKVD tokens. However, obtaining the KV deviation \(||\{K,V\}-\{K^{'},V^{'}\}||\) fails to save any compute in that obaining \({K,V}\) in the first place needs full prefill. In the two-chunk \((C_{1}, C_{2})\) example, if fully recomputed KV cache is needed to select the HKVD tokens, then we are essentially performing full prefill for \(C_{2}\), falling back to prefix-only caching.

\mypara{Fast HKVD token selector with look-ahead prediction}
In order to achieve actual compute savings, we need to come up with a more efficient way of identifying HKVD tokens. Luckily, we observe that KV deviations in earlier layer can serve as a decent predictor for KV deviations in later layers. In this way, we no longer need to recompute all the KV cache to select HKVD tokens. Figure \ref{fig:overlap} shows the overlap between HKVD tokens in the second layer and the following layers. If we pick 15\% tokens as HKVD tokens, the overlap ratios between the HKVD tokens in the second layer and those in later layers are consistently over 60\%. While the overlap can be improved by picking HKVD tokens more frequently (e.g., in layer 2, 5, 15), we should note that the final goal is not to achieve high overlap. Figure \ref{fig:effect_attn_dev} shows the reduction in attention deviation between the partially recomputed attention matrix (at different HKVD ratios) and the fully recomputed attention matrix. Attention matrix here refers to the attention between the input contexts (e.g., \((C_{1},C_{2})\)) and the question afterwards. Attention deviation can be reduced by over 80\% with the 10-20\% HKVD tokens selected and recomputed. The final generation quality can also be maintained under a similar range of HKVD ratio (\S\ref{sec:eval}). The details on how to perform recomputation on the selected HKVD tokens are demonstrated in \S\ref{subsec:framework}.
 
 The explanation for the effectiveness of look-ahead prediction lies within the innate architecture of LLM. 
 %Recall from \S\ref{subsec:transformer} that each LLM layer consists of two basic components: attention module and MLP module. 
 Suppose the input vector of a token \(i\) at a given \(il\)-th layer is \(x\) with shape \([d,1]\). In the attention module, the accordant query, key and value vectors are obtained with \(q,k,v=W_{q,k,v}x\). We further assume this token is identified as an HKVD token due to its high KV deviation. Then, we can safely infer that the input vector \(x\) also has a high error, and therefore so do \(q\) and \(k\). The output error of attention module (with skip connection) for this token should remain high in that the output is computed as \(x+V(softmax(q^{T}K/\sqrt{d}))\). Note that \(K\) and \(V\) are the entire matrix with shape \([d,N]\). After the attention module, errors continue to propogate in a token-wise manner in the MLP module, resulting in a high input error for the next layer. Therefore, it is reasonable treat KV deviations in early layers as an early indicator of KV deviations in later layers.
 
 In addition, we observe the distribution of K deviatons and V deviations are very similar at every layer, meaning that tokens with high K deviations match with token with high V devations. This alignment is expected in that KV cache at each layer is computed as \(\{K,V\}=\{W_{\{k,v\}}X\}\) where X is the input embedding of this layer. Further, this can simplify the process of picking HKVD tokens even more in that we only need to obtain one of the K and V deviations. 

\jiayi{jiayi stopped here. Above is the latest version for 4.1}

\jiayi{Below is the old text}
\subsection{Identifying high cross attention tokens}
%\jiayi{I'm trying to refer back to the example/section we had earlier}
\label{subsec:HCA}
%\begin{itemize}
%\item define high cross-attention tokens
%\item why high kv deviation is a good indicator of high cross-attention
%\item how to choose the right fraction
%\end{itemize}

%Before trying to tackle the chanllenge
%\shan{\st{What is challenge \#1?}}
To start with, we first define two types of attention. Going back to the example in \ref{subsec:existing solutions} (Figure \ref{fig:text_comparison}), assume there are two retrieved text chunks \(C_{1}\) and \(C_{2}\). (1) Internal attention measures the attention within \(C_{2}\). For any token \(i\) in \(C_{2}\), internal attention is calculated as the sum of attention scores between token \(i\) and its preceding tokens in \(C_{2}\). Internal attention has been largely\jc{completely?} preserved in the independently precomputed KV vectors of \(C_{2}\). (2) Cross attention is the attention between \(C_{1}\) and \(C_{2}\). The cross attention of any token \(i\) in \(C_{2}\) can be computed as the sum of attention scores between token \(i\) and all tokens in \(C_{1}\). Precomputing KV vectors independently for tokens within a single document completely neglects cross attention, and thus, degrades the generation quality. 
\jc{define HCA tokens here?}

To maintain the generation quality while still saving compute, we aim to first identify tokens (HCA tokens) whose KV vectors are greatly affected by HCA, and then recover HCA by partially recomputing and updating the KV vectors of these HCA tokens\jc{why can recomputing kv of high-HCA tokens recover cross-attention? need a bit more hand-holding}. \jiayi{the intuitive message that "the recomputated tokens are aware of tokens in other chunks" should be delivered somehow}

\jc{aren't we supposed to explain why only a few tokens have HCA and thus whose KV need to be recomputed?}

\begin{figure}

\centering
    \subfloat[Yi-34B]
        {\includegraphics[width=0.5\columnwidth]{figs/overlap_34b.pdf}\label{fig:overlap_34b}}
    \subfloat[Llama-70B]
        {\includegraphics[width=0.5\columnwidth]{figs/overlap_70b.pdf}\label{fig:overlap_70b}}
    \tightcaption{Overlap}
    \label{fig:overlap}
\end{figure}


\vspace{\vspacesize}
\textbf{Identifying HCA tokens with KV deviations:}
KV deviation is used to measure the effect of HCA.\jc{this sentence doesn't make sense. rephrase please. maybe put the idea upfront: we observe that tokens with high KV deviation (maybe call them HKVD tokens?) (explained shortly) are likely to be HCA tokens. then explain what's KV deviation and show why KV deviation correlates with HCA, formally and empirically.} For token \(i\) at layer \(l\)\jc{use j as the layer index please}, the KV deviation is computed as \(\{K_{il},V_{il}\}-\{K^{'}_{il},V^{'}_{il}\}\) where \(\{K,V\}\) are the fully recomputed KV vectors and \(\{K^{'},V^{'}\}\) are the cached KV vectors containing errors (w/o any cross attention). \jc{can you give a formal definition of high KV deviation (HKVD) tokens?}

The insight of selecting HCA tokens based on KV deviations is driven by the interpretation that if the KV deviation of token \(i\) is high, then the cross attention and internal attention of this token is not accurately computed\jc{too vague}. The direct effect of cross attention is straightforward\jc{why?}. Ignoring cross-attention between \(C_{1}\) and \(C_{2}\) can lead to KV deviations in \(C_{2}\)\jc{sounds repetitive?}. \jc{im TOTALLY lost in this ``intuitive interpretation''. need to be rewritten}
Cross attention can also implicitly cause KV deviatons through internal attention. For example, assume token \(i\) is in \(C_{2}\). KV vectors of tokens preceeding token \(i\) (but still in the same text chunk \(C_{2}\)) are affected by cross attention from \(C_{1}\), and therefore can affect the KV vectors of token \(i\) through internal attention\jc{this sounds a bit weird. it seems to mean that as long as the cross-attention on one token is missed, all other ensuing tokens will also miss the cross-attention and thus all need to be recomputed? doesn't it contradict the sparsity claim? i'd drop this point to avoid confusion}. 

\vspace{\vspacesize}
\textbf{Sparsity of HCA: } \jiayi{TODO; 1. say attention is sparse with proper citations. 2. Say how, therefore, cross-attention is sparse.}
\jc{shouldn't this be BEFORE we bring up KV deviation?}

\vspace{\vspacesize}
\textbf{Inefficiency of identifying HCA tokens:}
%\jiayi{Getting kv devs and update with recomputed ones is inefficient. Hold "how to recompute" for a second.}
Based on the criterion (KV deviation) discussed above, a natural way to recover HCA is to first identify the HCA tokens with high KV deviations at each layer and then update the corresponding KV vectors with the fully recomputed ones. Due to the sparsity of HCA, only a small set of tokens are expected to be identified as HCA tokens. This strategy allows most cached KV vectors resuable but fails to save any computation for full recomputation is needed to obtain all the KV deviations. In the two-chunk \((C_{1}, C_{2})\) example, if fully recomputed KV vectors are needed to select the HCA tokens, then we are essentially performing full recomputation for \(C_{2}\), falling back to prefix-only caching.

\jc{Jiayi, it seems like you had a different flow in mind than we agreed on. 
The flow we agreed on was that HCA tokens are hard to identify because you need to compute the actual attention matrix which means full recompute, so we approximate them with HKVD tokens, which are naturally cheap to identify, layer by layer.
The flow you put here seems to say even HKVD tokens are not easy to compute. While I agree that HKVD is not straightforward at a first sight, I dont want to confuse the reviewers. In my view, HCA is fundamentally hard to compute cheaply, but HKVD can be cheaply computed with the right implementation}



\begin{figure}

\centering
    \subfloat[Normalized attention deviation]
        {\includegraphics[width=0.5\columnwidth]{figs/attn_dev.pdf}\label{fig:effect_attn_dev}}
    \subfloat[Normalized F1-score\jiayi{should plot four lines as in (a)}]
        {\includegraphics[width=0.5\columnwidth]{figs/mock_oracle_vs_predicted_recomp.PNG}\label{fig:effect_f1}}
    \tightcaption{Effectiveness of recomputation with HCA prediction\jiayi{Please rerun 34B curve in (1) if time}}
    \label{fig:effect}
\end{figure}



\vspace{\vspacesize}
\textbf{Fast HCA token selector with look-ahead prediction:}
\jiayi{we need some theoretical support on two things: (1) tokens with high KV error in early layer are more likely to have errors in later layers; (2) reduction in attenton deviation is guaranteed when tokens are recomputed}

 In order to achieve actual compute savings, we need to come up with a more efficient way of identifying HCA tokens. Luckily, we observe that KV errors in earlier layer can serve as a decent predictor for KV errors in later layers. In this way, we no longer need to recompute all the KV vectors to select HCA tokens. Figure \ref{fig:overlap} shows the overlap between HCA tokens in the second layer and the following layers. If we pick 15\% tokens as HCA tokens, the overlap ratios between the HCA tokens in the second layer and those in later layers are consistently over 60\%. While the overlap can be improved by picking HCA tokens more frequently (e.g., in layer 2, 5, 15), we should note that the final goal is not to achieve high overlap. Figure \ref{fig:effect_attn_dev} shows the reduction in attention deviation between the partially recomputed attention matrix (at different HCA ratios) and the fully recomputed attention matrix. Attention matrix here refers to the attention between the input contexts (e.g., \((C_{1},C_{2})\)) and the question afterwards. Attention deviation can be reduced by over 80\% with the 10-20\% HCA tokens selected and recomputed. The final generation quality can also be maintained under a similar range of HCA ratio (\S\ref{sec:eval}). The details on how to perform recomputation on the selected HCA tokens are demonstrated in \S\ref{subsec:framework}.
 
 The explanation for the effectiveness of look-ahead prediction lies within the innate architecture of LLM. Recall from \S\ref{subsec:transformer} that each LLM layer consists of two basic components: attention module and MLP module. Suppose the input vector of a token \(i\) at a given \(il\)-th layer is \(x\) with shape \([d,1]\). In the attention module, the accordant query, key and value vectors are obtained with \(q,k,v=W_{q,k,v}x\). We further assume this token is identified as an HCA token due to its high KV deviation. Then, we can safely infer that the input vector \(x\) also has an high error, and therefore so do \(q\) and \(k\). The output error of attention module (with skip connection) for this token should remain high in that the output is computed as \(x+V(softmax(q^{T}K/\sqrt{d}))\). Note that \(K\) and \(V\) are the entire matrix with shape \([d,N]\). After the attention module, errors continue to propogate in a token-wise manner in the MLP module, resulting in a high input error for the next layer. Therefore, it is reasonable treat KV deviations in early layers as an early indicator of KV deviations in later layers.
 
 In addition, we observe the distribution of K deviatons and V deviations are very similar at every layer, meaning that tokens with high K deviations match with token with high V devations. This alignment is expected in that KV cache at each layer is computed as \(\{K,V\}=\{W_{\{k,v\}}X\}\) where X is the input embedding of this layer. Further, this can simplify the process of picking HCA tokens even more in that we only need to obtain one of the K and V deviations. 

 \jiayi{Above is he old text.}

\subsection{A cascading partial prefill framework}
%\jiayi{This sec is not complete}
\label{subsec:framework}
% \begin{itemize}
% \item how to recompute the kv of selected tokens? \ie 10\% selected tokens take only 10\% prefill compute.
% \item give an illustrative figure showing how loading of kv cache into gpu can be pipelined with recomputation
% \end{itemize}

%\jiayi{Please start with summarizing the last para}

%\jiayi{Please try to make this first para clear enough in 5.1 so it does not need to be reiterated in 5.2}
%We denote the input of the first layer in the LLM as \(X_{1} \in \mathbb{R}^{N\times d}\) where \(N\) is the number of tokens and \(d\) is the hidden dimension. For simplicity, we assume all the \(N\) tokens are cached, meaning they already have KV vectors. Further, we use \(F_{i}: \mathbb{R}^{N\times d} \rightarrow \mathbb{R}^{n\times d}\) to denote the i-th layer of the LLM. To start with, we recompute everything in the first layer, namely \(F_{1}(X_{1})\), to obtain the input of the second layer \(X_{1}\) (the output of the first layer). Note that it's unecessary to update the KV vectors in the first layer in that they do not contain errors. More specifically, errors in K vectors in the first layer can be recovered by restoring positional encodings (\S\fillme). V vectors in the first layer are obtained by \(V = W_{V}{X_{1}}\) where \(X_{1}\) is only dependent on the input text. Therefore, V vectors in the first layer should contain no error in that the reused texts are the same. The actual KV update starts in the second layer. The fully recomputed KV vectors in the second layer are computed as \(K,V = W_{\{K,V\}}X_{1}\). \(K'\) and \(V'\) are used to represent the cached KV vectors. Errors in V vectors \(||v-v'||\) (\({v,v'}:[1,d]\in{V,V'}:[N,d]\)) are used to indicate KV errors for the fact that tokens with high V errors are largely overlapped with those with high K errors, and vice versa \jiayi{A figure or table should be shown here and a short explanation for the underlying reason}. A predefined and fixed ratio of cached KV vectors with greatest errors are replaced by the corresponding fully recomputed KV vectors. Subsequently, full recomputation for the second layer is needed to obtain the input of the third layer, namely, \(X_{3}=F_{2}(X_{2})\). The same process is repeated for each layer until the end of the LLM to update the KV cache in all layers.



%\begin{figure}

%\centering
%    \includegraphics[width=0.95\columnwidth]{figs/mock_saving_one_layer.pdf}
%    \tightcaption{latency one layer\jiayi{Not needed if no room, maybe just the below table and overall latency breakdown in eval sec}}
%    \label{fig:latency}
%\end{figure}

\begin{table}

\vspace{1.5mm}

\resizebox{0.99\linewidth}{!}{%
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{@{}cccccc@{}}
\toprule
% \normalsize
\textbf{Recomp Method}  & \textbf{Attn}  & \textbf{MLP} & \textbf{Recover pos} & \textbf{Predict (if nec)} & \textbf{Total (w. predict)}  \\ \midrule
Full Recomp  & 22.41 & 35.22 & NA & NA  & 58.12     \\
\midrule

15\% HCA ratio  & 3.75 & 7.13 & 0.10 & 1.94 & 11.25 (13.05) \\

\bottomrule
\end{tabular}

}
\label{tab:latency_breakdown}
\caption{Latency breakdown of Llama-70B (prefilling 4k tokens, one layer) on 2 A40s} 
\vspace{-1.5mm}
\end{table}



In this section, we introduce a novel partial prefill framework that only performs recomputation and updates the KV cache of HKVD tokens instead of all the tokens. 

%In this way, we are able to reduce the LLM layer's input shape from \([d,N]\) to a smaller shape \([d,n]\) (\(n < N\)) where \(N\) is the total number of tokens and \(n\) is the number of HCA tokens in this layer. The actual amount of compute saving in one layer is shown in Figure \ref{fig:saving_for_one_layer}\jiayi{show (in figure) flop reduction here}. 

%\jiayi{Do we need a pseudocode here?} 
To elaborate, we walk through how HKVD tokens are picked under the framework and how partial prefill is done on these HKVD tokens. Assume look-ahead prediction is performed only once at an early layer \(l\). Then, full recomputation is needed in the first \((l-1)\) layers, and HCA tokens are picked at layer \(l\). Namely, the input shape of the first \((l-1)\) layers is \([d,N]\) where \(N\) is the total number of input tokens. Starting from layer \(l\), the input shape will shrink to \([d,n]\) (\(n < N\)) where \(n\) is the number of HKVD tokens. This reduction in input shape can be done repetitively at multiple layers if more look-ahead predictions are performed, resulting in a even smaller input shape for the following layers. The actual amount of latency reduction (15\% HKVD ratio vs. full recomputation) in one layer is shown in Table \ref{tab:latency_breakdown} \jiayi{please fix this ref issue}. 

\jiayi{The following para should be updated, serving as a pointer to the next System Design section}
While our partial prefill framework effectively reduces compute expenses, it should be noted that it entails additional overhead in loading the KV cache to GPU. For example, assume (1) full recomutation of 1k tokens in Llama-70B takes \textasciitilde 1.1s, (2) partial recomputation (15\% HCA ratio) takes \textasciitilde 0.25s, (3) KV cache size is \textasciitilde 0.3GB. If the cache is loaded from disk (3GB/s bandwidth), loading time takes \textasciitilde 0.1s. However, the request does not require all the KV cache to be in GPU in order to start. Partial recomputation of one layer can already take place if the cached KV vectors of that specific layer are loaded to the GPU. Therefore, as shown in Figure \ref{fig:layer_pipeline}, the loading time can be hidden by layer-level pipelining. Bandwith could be lower such that the loading time cannot be hidden by recomputation anymore. In this case, we can leverage request-level pipeline (Figure \ref{fig:req_pipeline}) and KV cache compression techniques (e.g., CacheGen\cite{cachegen}, H2O\cite{h2o}). The design of KV storage and loading controller will be further discussed in \S\ref{sec:design}.





\begin{figure*}
\centering
    \includegraphics[width=1.9\columnwidth]{figs/overview.pdf}
    \tightcaption{\name system (green stared) in light of LLM context augmented generation for a single request. \name uses text provided by retriever, interacts with multiple storage devices, and provides KV cache on top of LLM inference engines. \hc{to be updated with simpler version}\yh{the loading controller needs to fetch the KV cache \#1-4 from the storage}}
    \label{fig:overview}
\end{figure*}




\subsection{On-the-fly recovery of positional encoding}
\label{subsec:recover pos}
%\jiayi{PromptCache will have more overhead when we assume cache is empty at the first place!!}
\jiayi{please explain and show the overhead of recovering positional encoding (at th end of this section)}
In the last sections (\S\ref{subsec:HKVD}, \S\ref{subsec:framework}), we omit the existence of positional encodings for the purpose of being focused on the idea of recomputation. However, as will be shown later in \S\ref{subsubsec:quality_assure}, accurate positional encodings are required to maintain generation quality. We typically focus on the recovery of the state-of-the-art positional encoding method: Rotary positional embedding (Rope) \cite{su2024roformer} \jiayi{ours can be applied to other PE method (e.g., AliBi, maybe show this in appendix)}. Note that \promptcache ensures positional accuracies by caching the resued texts at a limited fixed range of positions. Multiple caches are needed to allow KV vectors of the same text segment to be reused at different positions. This is neither effecient or effective. By contrast, our method of recovering positional encoding is not only more efficient (cached once, reused at any position) but also more effective (better positional accuracies). The comparison between \promptcache and our positional recovering method is shown in \S\ref{subsubsec:quality_assure}.

Here, for simplicity, we only demonstrate Rope and our positional recovering method in the two-dimensional scenario (Q vectors and K vectors only have two dimensions). Note that our positional recovery method can be generalized to the n-dimensional setting as shown in the \jiayi{Appendix}. Rope in the two-dimensional scenario is performed as the following:

\begin{equation}
q_{m}, k_{m}=
\begin{pmatrix}
\cos m\theta & -\sin m\theta\\
\sin m\theta & \cos m\theta\\
\end{pmatrix}
\{
\begin{pmatrix}
q_{[0]}\\
q_{[1]}\\
\end{pmatrix},
\begin{pmatrix}
k_{[0]}\\
k_{[1]}\\
\end{pmatrix}
\}
\label{formula: rope}
\end{equation}


where \(m\) indicates the absolute position and \(\theta\) is a predefined rotary constant. 

Rope is performed on Q vectors and K vectors in every layer of the LLM. However, we first focus on how Rope can be recovered in the first layer and then adapt the approach to the following layers. Q vectors can be ignored for now since only K vectors (and V vectors) are needed for inference. The reocovery of K vectors in the first layer is very straightforward. Instead of caching the \(k_{m}\) vector at position \(m\) (like how K vectors are cached during normal inference), we cache the K vector \(k\) without positional encoding, and then recover the positional encoding on-the-fly during the inference by multiplying \(k\) with the rotary matrix as shown in \ref{formula: rope}.

As for the following layers, the recovery of positional encoding can be performed exactly the same as in the first layer. Note that the input embedding \(x_{im}\) of the token \(i\) at position \(m\) in the first layer only depends on the token itself. Therefore, the corresponding K vector \(k_{i}\) (w.o. positional encoding) does not rely on the token's position \(m\). In order to show our positional recovery method can be applied to later layers, without loss of generality, we need to prove the input embedding of the second layer, or equivalently the output embedding \(x^{'}_{im}\) of the attention module in the first layer, is irrevalent to the token's absolute position \(m\). However, due to the attention module in the first layer, the attention output \(x^{'}_{im}\) is dependent on its previous tokens. More specifically, it depends on the previous tokens' K vectors (w. positional encoding), whose values depend on the absolute position \(m\) as shown in \ref{formula: rope}.

Proof in a two-token scenario should suffice. In addition to the token \(i\) at position \(m\), we assume there exists another token \(j\) at position \(m-n\) and denote its input embedding in the first layer as \(x_{j(m-n)}\). Note that the attention score between token \(i\) and token \(j\) is invariant with respect to the absolute position \(m\). Based on \ref{formula: rope},  attention score \(q_{im}k_{j(m-n)}\) should be computed as the following:

\begin{equation}
\begin{aligned}
{q}_{im} {k}_{j(m-n)}
&= q_{[0]i}k_{[0]j}\cos (m-m+n)\theta\\
& \quad +q_{[1]i}k_{[1]j}\cos (m-m+n)\theta \\
&= (q_{[0]i}k_{[0]j}+q_{[1]i}k_{[1]j})\cos n\theta \\
\end{aligned}
\label{formula: attn score invariance}
\end{equation}

where the attention score only depends on the relative position \(n\) between the two tokens instead of the absolute position \(m\). Recall from Formula \ref{formula: attn module} that the attention output \(x^{'}_{im}\) is the dot product between attention scores and V vectors. Since positional encoding does not affect the V vectors and we have shown that the attention scores are irrelevant to the abolute position \(m\), the attention output \(x^{'}_{im}\) should also be unrelated to the absolute position. Thus, we can cache the K vectors without positional and perform Rope when their actual absolute position is determined during the inference. As for V vectors, we simply cache them in the same way as how they are cached during normal inference. In this way, we are able to achieve "cached once, reused anywhere".
%\vspace{\vspacesize}
%\textbf{Recovery of Rope:}

==> sec_recompute_v2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Fast Context Fusing by Selective Recomputation}
\label{sec:merge}

In this section, we address the key challenge mentioned in the last section (\S\ref{sec:motivation}). 
Namely, we present how \name fuses {\bf \em multiple} reusable text chunks by recomputing a small fraction of KV cache at a subset of layers and tokens and dynamically recovering the positional information of the KV cache. 
In this way, \name can save compute by reusing the KV cache of all the text chunks without compromising generation quality.

%In \S\ref{subsec:HCA}, we first note that most cross attention can be recovered . Further, we measure the impact of cross attention by comparing the deviation between precomputed KV cache (without cross attention) and fully recomputed KV cache (with cross attention). To recover cross attention, we choose to recompute tokens with high KV deviation (HKVD tokens) and update the corresponding KV cache. However, such strategy does not save any compute as obataining KV deviation requires fully recomputed KV cache, therefore, requiring the expensive full prefill. To address this inefficiency, we propose a lightweight prediction-based algorithm to approximate the HKVD tokens. Then, in \S\ref{subsec:framework}, we explain mechanically how KV cache of HKVD tokens can be recomputed and updated efficiently with our novel partial prefill framework. Finally, in \S\ref{subsec:recover pos}, we present a method that quickly recovers the positional encoding of KV cache for a given position on the fly.


\begin{figure}

\centering
    \subfloat[]
        {\includegraphics[width=0.5\columnwidth]{figs/cdf1.pdf}\label{fig:cdf1}}
    \subfloat[]
        {\includegraphics[width=0.5\columnwidth]{figs/cdf2.pdf}\label{fig:cdf2}}
    \tightcaption{CDF of KV deviation}
    \label{fig:cdf_kv}
\end{figure}


\subsection{Recovering cross attention with HKVD tokens}\label{subsec:Recover cross}
As discussed in \ref{XXX}, the cross attention is completely missing in the independently computed KV caches. Our goal here is:

\begin{goal}
How to minimize deviation in cross attention (recover cross attention) with minimum compute?
\end{goal}

Attention deviation here is straightforwardly defined as the L2-norm of the difference between the precomputed attention matrix and the attention matrix obtained in full prefill. More specifically, deviation in cross attention measures the difference in the attention between chunks (i.e., bottom left part of the attention matrix as shown in Figure \ref{fig:xxx}). 

\subsubsection{Recvering cross attention with partial KV update}\label{subsubsec:recover with kv update}
\jiayi{Please remove the subsubsections}
Ignoring cross attention directly leads to inaccurate KV cache of tokens at non-prefix positions. In other words, all attention (including cross attention) can be recovered if all the KV cache are restored (same as full prefill). The below formula depicts the relationship between KV cache of token \(i\) (\(k_{i}\), \(v_{i}\)) at a given layer and the attention vector (\(m_{\widetilde{i}}\)) at the previous layer indicating the attention scores between token i and its preceding tokens at the previous layers:


%\begin{equation}
%\begin{aligned}
%k_{i}, v_{i}
%&= W_{\{k,v\}}(MLP(V_{\widetilde{i}}m_{\widetilde{i}}+x_{i})+%(V_{\widetilde{i}}m_{\widetilde{i}}+x_{i}))\\
%\end{aligned}
%\end{equation}

\begin{equation}
\begin{aligned}
k_{i}, v_{i}
&= W_{\{k,v\}}(C_{1}m_{\widetilde{i}}+c_{0})\\
\end{aligned}
\end{equation}

%\(V_{\widetilde{i}}\) is the V vectors of token i and its preceding tokens at the previous layer, and \(x_{i}\) is the input embedding of token \(i\) at the previous layer. \jiayi{We can hide V and x as constants}
where \(W_{\{k,v\}}\) is the projection matrix, \(C_{1}\) is a constant matrix and \(c_{0}\) is a constant vector. The detailed derivation is in Appendix \ref{XXX}. It is obvious that recovering the attention vector \(m_{\widetilde{i}}\) is equivalent as restoring the KV cache (\(k_{i}\), \(v_{i}\)). However, it is impossible to restore all the KV cache while still saving any compute. Therefore, given a limited amount of compute, we want to prioritize the restoration of KV cache of tokens who receive high cross attention score with tokens in the preceding chunks.


 
\begin{insight}
Recovering the cross attention of a token is equivalent as restoring the KV cache of the same token. Therefore, most cross attention can be recovered if the KV cache of high cross-attention (HCA) tokens are recovered.
\end{insight}


%Note that HCA tokens are aware of tokens (and their corresponding KV cache) in other chunks during partial prefill. In this way, most cross attention is expecteded to be recovered as HCA tokens receive high cross attention. 


\subsubsection{Sparsity of cross attention}\label{subsubsec:attn sparsity}
%\jiayi{The precoputed KV should still preserve some locality through cross attention. However, only a small fraction of tokens are still affected by cross attention.}
\jiayi{Working on a visualization (similar to scissorhands)}
Attention sparsity has been widely observed in the existing research \cite{liu2024scissorhands,h2o,choromanski2020rethinking,chen2021scatterbrain}. Namely, one token attends to only a small number of tokens, meaning that the attention score follows a power law distribution. Building upon this observation, we further zoom in on the cross attention. We adopt a similar definition on attention sparsity in \fillme. Fortunately, we find that 

\begin{insight}
Cross attention is sparse between chunks. Therefore, the number of HCA tokens need to be recompted to recover cross attention should be small.
\end{insight}

Figure \fillme compares the amount of internal attention and cross attention each token receives. It is clear that cross attention is only prevalent in a small fraction of tokens. In addition, Figure \fillme confirms this observation on a larger scale, showing the power law distribution of cross attention scores. 
%The sparsity observed in cross attention suggests the precomputed KV cache of most tokens could bear enough semantic meaning for the LLM to understand through internal attention. 


\subsubsection{Measuring cross attention with KV deviation}\label{subsubsec:kv dev}
\jiayi{please add a theoretical formula}
%We note that KV deviations can be used to measure the impact of cross attention. 
Due to the sparsity of cross attention (\S\ref{sparse}), we expect only a small subset of tokens to be significanly affected by cross attention. \jiayi{Needs a transition here to say why we do not use attention matrix}

\begin{insight}
High KV deviation (HKVD) tokens are highly correlated with HCA tokens. 
\end{insight}



KV deviation for token \(i\) at layer \(j\) is computed as \(||\{K_{ij},V_{ij}\}-\{K^{'}_{ij},V^{'}_{ij}\}||\) where \(\{K,V\}\) are the fully recomputed KV cache and \(\{K^{'},V^{'}\}\) are the precomputed KV cache containing errors (w/o any cross attention). High KV deviation (HKVD) tokens are simply defined as tokens with high KV deviations. In practice, we can use either K or V deviation as tokens with high K deviations are similar with tokens with high V devations. This alignment is expected in that KV cache at each layer is computed as \(\{K,V\}=\{W_{\{k,v\}}X\}\) where X is the input embedding of this layer. \jiayi{Find a good correlation metric here and show HKVD tokens are HCA tokens}.

\jiayi{Please shorten the following intuitive explanation}
We use the two-chunk example in \ref{subsec:existing solutions} (Figure \ref{fig:text_comparison}) to demonstrate why KV deviation can be used to measure cross attention. Assume there are two text chunks \(C_{1}\) and \(C_{2}\), and there's a token \(i\) in \(C_{2}\). We start from layer \(j\). Denote the cross attention between \(C_{1}\) and token \(i\) as \(CrossAttn_{ij} \in \mathbb{R}^{1\times k}\) where \(k\) is the number of tokens preceding token \(i\) in total. Similarly, denote the attention within \(C_{2}\) between \(C^{'}_{2}\) (tokens in \(C_{2}\) and preceedig token \(i\)) and token \(i\) as \(InternalAttn_{ij}\). Then, the output of attention module at this layer \(j\), \(AttnOutput_{j} \in \mathbb{R}^{d}\) where \(d\) is the hidden dimension, is computed as \((V_{C_{1}},V_{C^{'}_{2}})(CrossAttn_{j}, InternalAttn_{j})^{T}\). This \(AttnOutput\) is then passed through several neural layers (MLP module) to form the input embedding of token \(i\) at the next layer \((j+1)\), denoted by \(x\). KV cache for token \(i\) at layer \((j+1)\) can be computed as \(\{k,v\}=\{W_{\{k,v\}}x\}\). Note that \(CrossAttn_{j}\) is essentially zero when KV cache is precomputed independently whereas \(InternalAttn_{j}\) can be preserved during precomputation.
%\jiayi{The fact is internal attention cannot be computed accurately but let's play down this}. 
Therefore, token \(i\) is expected to have high KV deviation if it receives high cross attention. A more rigorous mathematical proof is presented in Appendix \ref{XXX}. \jiayi{add appendix}

%To recover cross attention given a limited fraction of KV cache to be recomputed and updated, we should prioritize the recomptation over tokens with high KV deviations (HKVD tokens). Formally, HKVD tokens should be picked as 

%\begin{center}
%\begin{gather}
%    \mathop{\arg\max}\limits_{I} \sum_{i,j}||\{K_{ij},V_{ij}\}-\{K^{'}_{il},V^{'}_{ij}\}||I_{i,j}\nonumber\\
%     \text{s.t.} \quad I_{i,j}=\{0,1\}, \sum_{i,j} I_{i,j} = rNL \nonumber 
%\end{gather}
%\end{center}



%where I is the dummy variable indicating whether token \(i\) at layer \(j\) is considered as an HKVD token, N and L are the total number of tokens and layers, and the fraction of HKVD tokens is limited by a fixed HKVD ratio \(r\).

%\mypara{Inefficiency of identifying HKVD tokens}
 %In the last \ref{HKVD}, we rely on KV deviations to identify HKVD tokens. However, obtaining the KV deviation \(||\{K,V\}-\{K^{'},V^{'}\}||\) fails to save any compute in that obaining \({K,V}\) in the first place needs full prefill. In the two-chunk \((C_{1}, C_{2})\) example, if fully recomputed KV cache is needed to select the HKVD tokens, then we are essentially performing full prefill for \(C_{2}\), falling back to prefix-only caching.

\begin{figure}

\centering
    \subfloat[]
        {\includegraphics[width=0.5\columnwidth]{figs/overlap_70b.pdf}\label{fig:overlap1}}
    \subfloat[]
        {\includegraphics[width=0.5\columnwidth]{figs/overlap_34b.pdf}\label{fig:overlap2}}
    \tightcaption{Overlap}
    \label{fig:overlap}
\end{figure}


\subsubsection{Fast layer-wise HKVD token selection}\label{subsubsec:select hkvd}
\jiayi{please add a theoretical formula}
In the last section (\S\ref{subsubsec:kv dev}), we rely on KV deviations to identify HKVD tokens. However, obtaining the KV deviation \(||\{K,V\}-\{K^{'},V^{'}\}||\) fails to save any compute in that obaining \({K,V}\) in the first place needs full prefill. Luckily, we observe that 

\begin{insight}
HKVD tokens at one layer is a superset of most HKVD tokens at the next layer
\end{insight}

\jiayi{it's more accurate to change "a superset of" to "highly correlated with", but the idea of "superset" is more compatible with our partial prefill framework introduced later}

In this way, we no longer need to recompute all the KV cache to select HKVD tokens. As shown in Figure \ref{XXX}, \jiayi{Show KV overlap between two consecutive layers}.

%Figure \ref{fig:overlap} shows the overlap between HKVD tokens in the second layer and the following layers. If we pick 15\% tokens as HKVD tokens, the overlap ratios between the HKVD tokens in the second layer and those in later layers are consistently over 60\%. While the overlap can be improved by picking HKVD tokens more frequently (e.g., in layer 2, 5, 15), we should note that the final goal is not to achieve high overlap. 

%Figure \ref{fig:effect_attn_dev} shows the reduction in attention deviation between the partially recomputed attention matrix (at different HKVD ratios) and the fully recomputed attention matrix. Attention matrix here refers to the attention between the input contexts (e.g., \((C_{1},C_{2})\)) and the question afterwards. Attention deviation can be reduced by over 80\% with the 10-20\% HKVD tokens selected and recomputed. The final generation quality can also be maintained under a similar range of HKVD ratio (\S\ref{sec:eval}). The details on how to perform recomputation on the selected HKVD tokens are demonstrated in \S\ref{subsec:framework}.
 
 An intuitive explanation for the effectiveness of this look-ahead prediction lies within the innate architecture of LLM. 
 %Recall from \S\ref{subsec:transformer} that each LLM layer consists of two basic components: attention module and MLP module. 
 Suppose the input vector of a token \(i\) at a given layer is \(x\) with shape \([d,1]\). In the attention module, the accordant query, key and value vectors are obtained with \(q,k,v=W_{q,k,v}x\). We further assume this token is identified as an HKVD token due to its high KV deviation. Then, we can safely infer that the input vector \(x\) also has a high error, and therefore so do \(q\) and \(k\). The output error of attention module (with skip connection) for this token should remain high in that the output is computed as \(x+V(softmax(q^{T}K/\sqrt{d}))\). Note that \(K\) and \(V\) are the entire matrix with shape \([d,N]\). After the attention module, errors continue to propogate in a token-wise manner in the MLP module, resulting in a high input error for the next layer. Therefore, it is reasonable to treat KV deviations in one layer as an decent indicator of KV deviations in later layers. A more detailed mathematical proof is explained in Appendix \ref{XXX}.
 
%Further, this can simplify the process of picking HKVD tokens even more in that we only need to obtain one of the K and V deviations. 


\begin{figure}

\centering
    \subfloat[Normalized attention deviation]
        {\includegraphics[width=0.5\columnwidth]{figs/attn_dev.pdf}\label{fig:effect_attn_dev}}
    \subfloat[Normalized F1-score\jiayi{should plot four lines as in (a)}]
        {\includegraphics[width=0.5\columnwidth]{figs/mock_oracle_vs_predicted_recomp.PNG}\label{fig:effect_f1}}
    \tightcaption{Effectiveness of recomputation with HCA prediction\jiayi{Please rerun 34B curve in (1) if time}}
    \label{fig:effect}
\end{figure}




\subsection{A cascading partial prefill framework}
%\jiayi{This sec is not complete}
\label{subsec:framework}

\jiayi{add a diagram, move the prediction here}
% \begin{itemize}
% \item how to recompute the kv of selected tokens? \ie 10\% selected tokens take only 10\% prefill compute.
% \item give an illustrative figure showing how loading of kv cache into gpu can be pipelined with recomputation
% \end{itemize}

%\jiayi{Please start with summarizing the last para}

%\jiayi{Please try to make this first para clear enough in 5.1 so it does not need to be reiterated in 5.2}
%We denote the input of the first layer in the LLM as \(X_{1} \in \mathbb{R}^{N\times d}\) where \(N\) is the number of tokens and \(d\) is the hidden dimension. For simplicity, we assume all the \(N\) tokens are cached, meaning they already have KV vectors. Further, we use \(F_{i}: \mathbb{R}^{N\times d} \rightarrow \mathbb{R}^{n\times d}\) to denote the i-th layer of the LLM. To start with, we recompute everything in the first layer, namely \(F_{1}(X_{1})\), to obtain the input of the second layer \(X_{1}\) (the output of the first layer). Note that it's unecessary to update the KV vectors in the first layer in that they do not contain errors. More specifically, errors in K vectors in the first layer can be recovered by restoring positional encodings (\S\fillme). V vectors in the first layer are obtained by \(V = W_{V}{X_{1}}\) where \(X_{1}\) is only dependent on the input text. Therefore, V vectors in the first layer should contain no error in that the reused texts are the same. The actual KV update starts in the second layer. The fully recomputed KV vectors in the second layer are computed as \(K,V = W_{\{K,V\}}X_{1}\). \(K'\) and \(V'\) are used to represent the cached KV vectors. Errors in V vectors \(||v-v'||\) (\({v,v'}:[1,d]\in{V,V'}:[N,d]\)) are used to indicate KV errors for the fact that tokens with high V errors are largely overlapped with those with high K errors, and vice versa \jiayi{A figure or table should be shown here and a short explanation for the underlying reason}. A predefined and fixed ratio of cached KV vectors with greatest errors are replaced by the corresponding fully recomputed KV vectors. Subsequently, full recomputation for the second layer is needed to obtain the input of the third layer, namely, \(X_{3}=F_{2}(X_{2})\). The same process is repeated for each layer until the end of the LLM to update the KV cache in all layers.



%\begin{figure}

%\centering
%    \includegraphics[width=0.95\columnwidth]{figs/mock_saving_one_layer.pdf}
%    \tightcaption{latency one layer\jiayi{Not needed if no room, maybe just the below table and overall latency breakdown in eval sec}}
%    \label{fig:latency}
%\end{figure}

\begin{table}

\vspace{1.5mm}

\resizebox{0.99\linewidth}{!}{%
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{@{}cccccc@{}}
\toprule
% \normalsize
\textbf{Recomp Method}  & \textbf{Attn}  & \textbf{MLP} & \textbf{Recover pos} & \textbf{Predict (if nec)} & \textbf{Total (w. predict)}  \\ \midrule
Full Recomp  & 22.41 & 35.22 & NA & NA  & 58.12     \\
\midrule

15\% HCA ratio  & 3.75 & 7.13 & 0.10 & 1.94 & 11.25 (13.05) \\

\bottomrule
\end{tabular}

}
\label{tab:latency_breakdown}
\caption{Latency breakdown of Llama-70B (prefilling 4k tokens, one layer) on 2 A40s} 
\vspace{-1.5mm}
\end{table}


In this section, we introduce a novel partial prefill framework that only performs recomputation and updates the KV cache of HKVD tokens instead of all the tokens. 

%In this way, we are able to reduce the LLM layer's input shape from \([d,N]\) to a smaller shape \([d,n]\) (\(n < N\)) where \(N\) is the total number of tokens and \(n\) is the number of HCA tokens in this layer. The actual amount of compute saving in one layer is shown in Figure \ref{fig:saving_for_one_layer}\jiayi{show (in figure) flop reduction here}. 

%\jiayi{Do we need a pseudocode here?} 
To elaborate, we walk through how HKVD tokens are picked under the framework and how partial prefill is done on these HKVD tokens. Assume look-ahead prediction is performed only once at an early layer \(l\). Then, full recomputation is needed in the first \((l-1)\) layers, and HKVD tokens are picked at layer \(l\). Namely, the input shape of the first \((l-1)\) layers is \([d,N]\) where \(N\) is the total number of input tokens. Starting from layer \(l\), the input shape will shrink to \([d,n]\) (\(n < N\)) where \(n\) is the number of HKVD tokens. This reduction in input shape can be done repetitively at multiple layers if more look-ahead predictions are performed, resulting in a even smaller input shape for the following layers. The actual amount of latency reduction (15\% HKVD ratio vs. full recomputation) in one layer is shown in Table \ref{tab:latency_breakdown}. 

While our partial prefill framework effectively reduces compute expenses, it should be noted that it entails additional overhead in loading the KV cache to GPU. However, the loading overhead can be hidden by the compute time with proper pipelining (\S\ref{sec:design}).

%For example, assume (1) full recomutation of 1k tokens in Llama-70B takes \textasciitilde 1.1s, (2) partial recomputation (15\% HCA ratio) takes \textasciitilde 0.25s, (3) KV cache size is \textasciitilde 0.3GB. If the cache is loaded from disk (3GB/s bandwidth), loading time takes \textasciitilde 0.1s. However, the request does not require all the KV cache to be in GPU in order to start. Partial recomputation of one layer can already take place if the cached KV vectors of that specific layer are loaded to the GPU. Therefore, as shown in Figure \ref{fig:layer_pipeline}, the loading time can be hidden by layer-level pipelining. Bandwith could be lower such that the loading time cannot be hidden by recomputation anymore. In this case, we can leverage request-level pipeline (Figure \ref{fig:req_pipeline}) and KV cache compression techniques (e.g., CacheGen\cite{cachegen}, H2O\cite{h2o}). The design of KV storage and loading controller will be further discussed in \S\ref{sec:design}.





\begin{figure*}
\centering
    \includegraphics[width=1.95\columnwidth]{figs/overview.pdf}
    \tightcaption{\name system (green stared) in light of LLM context augmented generation for a single request. \name uses text provided by retriever, interacts with multiple storage devices, and provides KV cache on top of LLM inference engines.}
    \label{fig:overview}
\end{figure*}




\subsection{On-the-fly recovery of positional encoding}
\label{subsec:recover pos}

In the last section (\S\ref{subsec:Recover cross}), we omit the existence of positional encoding for the purpose of being focused on how to recover cross attention. In this section, we propose a flexible and accurate position recovery method that allows a single piece of KV cache to be reused at different positions with a single element-wise matrix multipication at each layer. Typically, we focus on the recovery of the state-of-the-art positional encoding method: Rotary positional embedding (Rope) \cite{su2024roformer} \jiayi{add a footnote saying the method can be used for other relative positional encoding method}.

Here, for simplicity, we only demonstrate Rope and our position recovery method in the two-dimensional scenario (QKV vectors only have two dimensions). Note that our positional recovery method can be generalized to the n-dimensional setting as shown in the \jiayi{Appendix}. Rope in the two-dimensional scenario is performed as the following:

\begin{equation}
q_{m}, k_{m}=
\begin{pmatrix}
\cos m\theta & -\sin m\theta\\
\sin m\theta & \cos m\theta\\
\end{pmatrix}
\{
\begin{pmatrix}
q_{[0]}\\
q_{[1]}\\
\end{pmatrix},
\begin{pmatrix}
k_{[0]}\\
k_{[1]}\\
\end{pmatrix}
\}
\label{formula: rope}
\end{equation}


where \(m\) indicates the absolute position and \(\theta\) is a predefined rotary constant. Rope is performed on Q vectors and K vectors in every layer of the LLM. 

We start with the first layer. Q vectors can be ignored for now since only K vectors (and V vectors) are needed for inference. V vectors can also be ignored at the first layer in that positional encoding is not performed on V vectors. The reocovery of K vectors in the first layer is very straightforward. Instead of caching the \(k_{m}\) vector at position \(m\) (like how K vectors are cached during normal inference), we cache the K vector \(k\) without positional encoding, and then recover the positional encoding on-the-fly during the inference by multiplying \(k\) with the rotary matrix as shown in \ref{formula: rope}.

As for the following layers, the recovery of positional encoding can be performed exactly the same as in the first layer. Note that the input embedding \(x_{im}\) of the token \(i\) at position \(m\) in the first layer only depends on the token itself. Therefore, the corresponding K vector \(k_{i}\) (w.o. positional encoding) does not rely on the token's position \(m\). 
In order to show our positional recovery method can be applied to later layers, without loss of generality, we need to prove the input embedding of the second layer, or equivalently the output embedding \(x^{'}_{im}\) of the attention module in the first layer, is irrevalent to the token's absolute position \(m\). However, due to the attention module in the first layer, the attention output \(x^{'}_{im}\) is dependent on its previous tokens. More specifically, it depends on the previous tokens' K vectors (w. positional encoding), whose values depend on the absolute position \(m\) as shown in \ref{formula: rope}.

Proof in a two-token scenario should suffice. In addition to the token \(i\) at position \(m\), we assume there exists another token \(j\) at position \(m-n\) and denote its input embedding in the first layer as \(x_{j(m-n)}\). Note that the attention score between token \(i\) and token \(j\) is invariant with respect to the absolute position \(m\). Based on \ref{formula: rope},  attention score \(q_{im}k_{j(m-n)}\) should be computed as the following:

\begin{equation}
\begin{aligned}
{q}_{im} {k}_{j(m-n)}
&= q_{[0]i}k_{[0]j}\cos (m-m+n)\theta\\
& \quad +q_{[1]i}k_{[1]j}\cos (m-m+n)\theta \\
&= (q_{[0]i}k_{[0]j}+q_{[1]i}k_{[1]j})\cos n\theta \\
\end{aligned}
\label{formula: attn score invariance}
\end{equation}

where the attention score only depends on the relative position \(n\) between the two tokens instead of their absolute positions. Note that the attention output \(x^{'}_{im}\) should also be unrelated to the absolute positions as it is the dot product between attention scores and V vectors. Thus, we can cache the K vectors without positional encoding and perform Rope when their actual absolute position is determined during the inference. As for V vectors, we simply cache them in the same way as how they are cached during normal inference. In this way, we are able to achieve "cached once, reused anywhere".
%\vspace{\vspacesize}
%\textbf{Recovery of Rope:}
\jiayi{jiayi stopped here. Above is the latest version for 4}

==> sec_recompute_v3.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US

%\section{Fast Context Fusing by Selective Recomputation}
\section{Fast KV Cache Fusing}
\label{sec:merge}

A natural question then is how to have both the speed of module caching, referred to as {\em full KV reuse}, and the generation quality of prefix caching or full prefill, referred to as {\em full KV re-compute}. 
We formulate this goal in the following statement. 

\begin{goal}
When an LLM input includes multiple text chunks, how to {\em quickly} update their precomputed KV caches such that the resulting attention matrix (including the cross-attention between the chunks) has minimum difference with the one during the full KV re-compute. 
\end{goal}

%\jc{add a terminology table here}

\begin{table}[]
\small
\begin{tabular}{rl}
\hline
\textit{Notation} & \textit{Description} \\ \hline\hline
\begin{tabular}[c]{@{}r@{}}$\LayerIndex$ \\ $\TokenIndex$\\ $\ChunkIndex$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Layer index\\ Token index\\ Chunk index\end{tabular} \\ \hline
\begin{tabular}[c]{@{}r@{}}$\KV$\\ $\KV^{\Full}$\\ $\KV^{\Pre}$\\ $\KV^{\New}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}KV cache\\ Fully re-computed KV cache\\ Pre-computed KV cache\\ \name-updated KV cache\end{tabular} \\ \hline
\begin{tabular}[c]{@{}r@{}}$\KV[\LayerIndex]$\\ $\KV[\LayerIndex][\TokenIndex]$\end{tabular} & \begin{tabular}[c]{@{}l@{}}KV on layer $\LayerIndex$\\ KV on layer $\LayerIndex$ at token $\TokenIndex$\end{tabular} \\ \hline
\begin{tabular}[c]{@{}r@{}}$\Attention_{\LayerIndex}$\\ $\Attention_{\LayerIndex}[\TokenIndex,\TokenIndex']$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Attention Matrix on layer $\LayerIndex$\\ Attention Matrix on layer $\LayerIndex$ between token $\TokenIndex$ and $\TokenIndex'$\end{tabular} \\ \hline
$\CA_{\LayerIndex,\TokenIndex}$ & Aggregated Cross-Attention of token $\TokenIndex$ on layer $\LayerIndex$ \\ \hline\end{tabular}
\caption{Summary of terminology}
\label{tab:terminology}
\end{table}

To make it more rigorous, we formally define the terminologies as follows (Table~\ref{tab:terminolopgy}).
Given a KV cache $\KV$, we use $\KV[\LayerIndex]$ and $\KV[\LayerIndex][\TokenIndex]$ to denote the KV on layer $\LayerIndex$ and the KV on layer $\LayerIndex$ at token $\TokenIndex$, respectively.\footnote{For simplicity, we use KV and KV cache interchangeably.}
Given a KV cache $\KV$, we use $\Attention_{\LayerIndex}=\Func_\LayerIndex(\KV)$ to denote the resulting attention matrix on layer $\LayerIndex$.
For a given list of $\ChunkNum$ text chunks, we denote the KV cache after full KV re-compute (full prefill or prefix caching) as $\KV^{\Full}$.
%, where $\KV_{\ChunkIndex}^{\Full}$ is the precomputed KV cache of text chunk $\ChunkIndex$ ($1\leq\ChunkIndex\leq\ChunkNum$). 
We also denote the precomputed KV cache as $\KV^{\Pre}=[\KV_{1}^{\Pre},\dots,\KV_{\ChunkNum}^{\Pre}]$, where $\KV_{\ChunkIndex}^{\Pre}$ is the independently precomputed KV cache of text chunk $\ChunkIndex$, $1\leq\ChunkIndex\leq\ChunkNum$.

We can then frame our goal as how to quickly update the precomputed KV cache $\KV^{\Pre}$ to $\KV^{\New}$, such that the difference between the {\em partially updated} attention matrix $\Attention_{\LayerIndex}^{\New}=\Func_\LayerIndex(\KV^{\New})$ and the {\em fully recomputed} attention matrix $\Attention_{\LayerIndex}^{\Full}=\Func_\LayerIndex(\KV^{\Full})$ is minimum for all layer index $\LayerIndex$.
Since the difference between $\Attention_{\LayerIndex}^{\New}$ and $\Attention_{\LayerIndex}^{\Full}$ lies in the cross-attention between the chunks, 
%the attention matrix contains the cross-attention between the chunks, 
minimizing $||\Attention_{\LayerIndex}^{\New}-\Attention_{\LayerIndex}^{\Full}||$ effectively recovers the cross-attention to the same as full KV recompute.

%\subsection{Which tokens' KV should be recomputed?}

\subsection{Selective Re-computation of KV Cache}

To achieve the aforementioned goal, our design choice is to update the precomputed KV cache by {\em recomputing the KV of only a small subset of tokens}\footnote{We also need to update the positional encoding for all tokens, but as explained shortly in \S\ref{subsec:positional}, doing so incurs minimum overhead.} on each layer.
Specifically, by recomputing the token $\TokenIndex$ on layer $\LayerIndex$, we will make its values, $\KV[\LayerIndex][\TokenIndex]$, the same as what is in the full-prefilled KV, $\KV^{\Full}[\LayerIndex][\TokenIndex]$. 
We want to update $r\%$ of tokens per layer while maximally reduce $||\Attention_{\LayerIndex}^{\New}-\Attention_{\LayerIndex}^{\Full}||$.
%(\S\ref{subsec:??} will describe how to update the KV of a subset of tokens without changing the KV of other tokens.)

\vspace{0.2cm}
\noindent {\bf Question 1: Which tokens should be selected to recompute their KV?}
To answer it, we first define {\em \HCA} tokens at layer $\LayerIndex$ as the tokens who have the highest Aggregated Cross-Attentions. 
Here, the {\em Aggregated Cross-Attention}, or {\em \ACA}, of token $\TokenIndex$ on layer $\LayerIndex$, denoted as $\CA_{\LayerIndex,\TokenIndex}$, is the sum of fully-recomputed attention between token $\TokenIndex$ and any tokens in preceding chunks $\TokenIndex'$: $\CA_{\LayerIndex,\TokenIndex} = \sum_{\TokenIndex'\in\textrm{preceding chunks}}\Attention_{\LayerIndex}^{\Full}[\TokenIndex,\TokenIndex']$.
For instance, with three 100-token chunks, the \ACA of a token in the third chunk is the sum of its cross-attention with the 200 tokens in the preceding two chunks.

\begin{figure}[t]
\centering
	\includegraphics[width=.99\columnwidth]{figs/aca_illustrated.pdf}
    \tightcaption{Distribution of aggregated cross-attention (\ACA) of different tokens on one layer.}
    \label{fig:aca}
\end{figure}

With the notion of \HCA tokens, we have the following insight to help pick the tokens to recompute their KV.
%\jc{we need a visualization to help people understand the concepts}

\begin{insight}
A token with a higher aggregated cross-attention (\ACA) has a higher attention other tokens in preceding chunks, so recomputing the KV of \HCA tokens can better recover cross-attention.
%An HCA token has a high attention with other tokens in previous chunks, so recomputing its KV can greatly recover cross-attention.
%Recovering the cross attention of a token is equivalent as restoring the KV cache of the same token. Therefore, most cross attention can be recovered if the KV cache of high cross-attention (HCA) tokens are recovered.
\end{insight}

More rigorously, we can prove that recomputing the KV of token $\TokenIndex$ on layer $\LayerIndex$ directly reduces the cross-attention by its \ACA, $\CA_{\LayerIndex,\TokenIndex}$. (\S\ref{app:??} provides its proof.)
In other words, recomputing the KV of tokens with higher \ACA better recovers the cross-attention (or equivalently, reduce $||\Attention_{\LayerIndex}^{\New}-\Attention_{\LayerIndex}^{\Full}||$ more).
Thus, if we need to recompute the KV of, say 10\%, of tokens on each layer, we should choose the 10\% tokens with the highest \ACA, \ie top 10\% \HCA tokens.


Now that the most important tokens to recompute KV for are those \HCA tokens, we will tackle two natural questions. 

\vspace{0.2cm}
\noindent {\bf Question 2: Can recomputing the KV of a small subset of tokens recover most of the cross-attention?} 
That is, are there a small number of HCA tokens with much higher \ACA than others? 
Fortunately, the answer can be partly found in many recent works\cite{liu2024scissorhands,h2o,choromanski2020rethinking,chen2021scatterbrain} which have observed {\em attention sparsity} on many transformer models---each token attends to only a small number of preceding tokens, making the attention scores follow a power law distribution. 
Similar to the attention sparsity observation, we have the following insight.

\begin{insight}
Cross attention between different chunks (a subset of attention matrix) is sparse, so only a small number of tokens have very high Aggregated Cross Attention (\ACA), \ie recomputing the KV of a small subset of \HCA tokens can recover most of the cross-attention.
\end{insight}

\begin{figure}[t]
\centering
	\includegraphics[width=.99\columnwidth]{figs/ca_cdf.pdf}
    \tightcaption{Distribution of aggregated cross-attention (\ACA) of different tokens on one layer.\jiayi{Replotting this with our recomputation. Actually, I think using a separate graph might. The new graph should be the cdf containing only the recomputed ACA.}}
    \label{fig:acacdf}
\end{figure}

Figure~\ref{fig:acacdf} shows the distribution of \ACA of tokens on one layer from running \fillme \jiayi{150} inputs from the \fillme \jiayi{Musique} dataset on two different models.
We can see that a small fraction, about 10-15\%, of tokens have much higher \ACA than others, which empirically corroborates the sparsity of cross-attention.


\vspace{0.2cm}
\noindent {\bf Question 3: How to selectively recompute the KV for a subset of tokens (\HCA tokens) on every layer?}
The default implementation of LLM prefill does not support ``skipping'' tokens while only compute the KV of a subset of tokens. 
However, we can first {\em permute} the order of the tokens on each layer to move the \HCA tokens and separate them from other tokens whose KV does not need to be updated. 
The reason is the following insight, whose proof will be provided in \S\ref{??}.

\begin{insight}
The order of tokens on each layer does not affect the KV of each token.\jc{jiayi, this insight doesn't sound right. doesn't it mean you can arbitrarily shuffle the tokens and still get the same result?} \jiayi{A new version: The order of tokens on each layer does not affect the KV of each token if the attention mask is permuted accordingly}
\end{insight}

Once the \HCA tokens on a layer are moved together, the prefill computation can be done only on those tokens without affecting other tokens' KV.
Figure~\ref{??} illustrates this process.
So if only $r\%$ of tokens are selected as \HCA tokens, recomputing their KV only needs $r\%$ of computation overhead as a full prefill.

\vspace{0.2cm}
\noindent {\bf Question 4: How to identify the \HCA tokens without knowing the true attention matrix}
Naively, to identify the \HCA tokens, one must calculate the full attention matrix of every layer in the first place. 
Fortunately, the \HCA tokens on different layers are not independent. Instead, we have the following observation:

\begin{insight}
Tokens with higher \ACA on one layer are likely with higher \ACA on the next layer. 
%The \HCA tokens on one layer is likely a subset of \HCA tokens on the previous layer. 
\end{insight}

More specifically, on one layer $\LayerIndex$, if token $\TokenIndex$ has a higher \ACA than token $\TokenIndex'$, (\ie $\CA_{\LayerIndex, \TokenIndex}\geq\CA_{\LayerIndex, \TokenIndex}$), then on the the next layer $\LayerIndex+1$, token $\TokenIndex$ is likely to have a higher \ACA than token $\TokenIndex'$ (\ie $\CA_{\LayerIndex+1, \TokenIndex}\geq\CA_{\LayerIndex+1, \TokenIndex}$).
To put it concretely, if the top three \HCA tokens on the first layer are tokens 2, 3, and 5, these three tokens likely also have higher \ACA than most other tokens. 
Figure~\ref{fig:rankcorr} uses the same setting as Figure~\ref{fig:acacdf} and shows the Kendall's rank correlation scores between \ACA of the same token on two neighboring layers. 
The intuition behind this correlation is \fillme \jc{jiayi, please provide some explanation here}


\begin{figure}[t]
\centering
	\includegraphics[width=.99\columnwidth]{figs/ca_corr_bar_new.pdf}
    \tightcaption{Rank correlation of the Aggregated Cross-Attention (\ACA) per token between two consecutive layers.
    \jc{\st{mock figure. Jiayi, please update it with real numbers}}\jiayi{Scores don't look high enoug for now. Let me get figure 6 first then iterate on this}}
    \label{fig:rankcorr}
\end{figure}



Given the substantial correlation between the \ACA across layers, a straightforward solution, therefore, is that if we can  perform prefill on the first layer first, and pick the tokens with the highest \ACA as the \HCA tokens only update their KV on all other layers.
Since an LLM usually have over 30 layers, this process can save most of the compute compared to full KV re-compute. 
That said, using {\em only} the \ACA of different tokens on the first layer may not be statistically reliable to pick \HCA tokens of all layers, especially deeper layers. 

Instead, we opt for a {\em gradual filtering} scheme.
If on average we want to pick $r\%$ \HCA tokens per layer, we will pick $r_1\%$ tokens with the highest \ACA on the first layer as the \HCA tokens on the second layer, with $r_1$ being slightly higher than $r$.
Then we recompute the KV of these $r_1\%$ \HCA tokens on the second layer and pick $r_2\%$ tokens among them with the highest \ACA, with $r_2$ slightly less than $r_1$, as the \HCA tokens on the next layer, and so forth. 
Intuitively, this gradual-filtering scheme eventually picks the \HCA tokens that have not only relatively high \ACA on the first layer, but also a few other layers, which empirically is more statistically reliable to identify the \HCA tokens on each layers.  


%we only need to compute the \ACA of these three tokens on the next layer in order to pick its \HCA tokens. 

%As elaborated in \S\ref{subsec:modular}, the difference between the partially update attention matrix $\AttentionL{\LayerIndex}$ and the {\em fully recomputed} attention matrix $\AttentionL{\LayerIndex}^*$ 



\jc{junchen edit ends here}


\subsection{On-the-fly recovery of positional encoding}
\label{subsec:recover pos}

So far we have ignored the positional encoding so that we can focus on recovering cross attention. 
Next, we present a fast scheme to update the positional encoding of a KV cache when it is used at a different position than when it was pre-computed.
The only assumption is that the positional encoding method is Rotary positional embedding (Rope)~\cite{su2024roformer}, which has been used in many state-of-the-art LLMs\jc{some supporting evidence?}

%flexible and accurate position recovery method that allows a single piece of KV cache to be reused at different positions with a single element-wise matrix multipication at each layer. Typically, we focus on the recovery of the state-of-the-art positional encoding method: Rotary positional embedding (Rope) \cite{su2024roformer} \jiayi{add a footnote saying the method can be used for other relative positional encoding method}.

Here, for simplicity, we only demonstrate Rope and our position recovery method in the two-dimensional scenario (QKV vectors only have two dimensions). Note that our positional recovery method can be generalized to the n-dimensional setting as shown in the \jiayi{Appendix}. Rope in the two-dimensional scenario is performed as the following:

\begin{equation}
q_{m}, k_{m}=
\begin{pmatrix}
\cos m\theta & -\sin m\theta\\
\sin m\theta & \cos m\theta\\
\end{pmatrix}
\{
\begin{pmatrix}
q_{[0]}\\
q_{[1]}\\
\end{pmatrix},
\begin{pmatrix}
k_{[0]}\\
k_{[1]}\\
\end{pmatrix}
\}
\label{formula: rope}
\end{equation}


where \(m\) indicates the absolute position and \(\theta\) is a predefined rotary constant. Rope is performed on Q vectors and K vectors in every layer of the LLM. 

We start with the first layer. Q vectors can be ignored for now since only K vectors (and V vectors) are needed for inference. V vectors can also be ignored at the first layer in that positional encoding is not performed on V vectors. The reocovery of K vectors in the first layer is very straightforward. Instead of caching the \(k_{m}\) vector at position \(m\) (like how K vectors are cached during normal inference), we cache the K vector \(k\) without positional encoding, and then recover the positional encoding on-the-fly during the inference by multiplying \(k\) with the rotary matrix as shown in \ref{formula: rope}.

As for the following layers, the recovery of positional encoding can be performed exactly the same as in the first layer. Note that the input embedding \(x_{im}\) of the token \(i\) at position \(m\) in the first layer only depends on the token itself. Therefore, the corresponding K vector \(k_{i}\) (w.o. positional encoding) does not rely on the token's position \(m\). 
In order to show our positional recovery method can be applied to later layers, without loss of generality, we need to prove the input embedding of the second layer, or equivalently the output embedding \(x^{'}_{im}\) of the attention module in the first layer, is irrevalent to the token's absolute position \(m\). However, due to the attention module in the first layer, the attention output \(x^{'}_{im}\) is dependent on its previous tokens. More specifically, it depends on the previous tokens' K vectors (w. positional encoding), whose values depend on the absolute position \(m\) as shown in \ref{formula: rope}.

Proof in a two-token scenario should suffice. In addition to the token \(i\) at position \(m\), we assume there exists another token \(j\) at position \(m-n\) and denote its input embedding in the first layer as \(x_{j(m-n)}\). Note that the attention score between token \(i\) and token \(j\) is invariant with respect to the absolute position \(m\). Based on \ref{formula: rope},  attention score \(q_{im}k_{j(m-n)}\) should be computed as the following:

\begin{equation}
\begin{aligned}
{q}_{im} {k}_{j(m-n)}
&= q_{[0]i}k_{[0]j}\cos (m-m+n)\theta\\
& \quad +q_{[1]i}k_{[1]j}\cos (m-m+n)\theta \\
&= (q_{[0]i}k_{[0]j}+q_{[1]i}k_{[1]j})\cos n\theta \\
\end{aligned}
\label{formula: attn score invariance}
\end{equation}

where the attention score only depends on the relative position \(n\) between the two tokens instead of their absolute positions. Note that the attention output \(x^{'}_{im}\) should also be unrelated to the absolute positions as it is the dot product between attention scores and V vectors. Thus, we can cache the K vectors without positional encoding and perform Rope when their actual absolute position is determined during the inference. As for V vectors, we simply cache them in the same way as how they are cached during normal inference. In this way, we are able to achieve "cached once, reused anywhere".
%\vspace{\vspacesize}
%\textbf{Recovery of Rope:}
\jiayi{jiayi stopped here. Above is the latest version for 4}

==> sec_recompute_v4.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


%\section{Fast Context Fusing by Selective Recomputation}
\section{Fast KV Cache Fusing}
\label{sec:merge}

Given that {\em full KV re-compute} (\ie full prefill or prefix caching) can be too slow and {\em full KV reuse} (\ie modular caching) can have low quality, a natural question then is how to have both the low delay of full KV reuse {\em and} the high quality of full KV re-compute. 
Our goal therefore is the following:

\begin{goal}
When an LLM input includes multiple re-used text chunks, how to {\bf quickly} update their precomputed KV caches such that the resulting attention matrix, which includes the cross-attention between the chunks, has {\bf minimum difference} with the one produced by full KV re-compute. 
\end{goal}

To realize our goal, \name~{\em re-computes the KV of a selective subset of tokens} on each layer, while re-using other tokens' KV.\footnote{For simplicity, we use the terms KV and KV cache interchangeably.}
%\footnote{We also need to update the positional encoding for all tokens, but as explained shortly in \S\ref{subsec:positional}, doing so incurs minimum overhead.}
We explain how \name does so in three parts.
\S\ref{subsec:terminology} begins with the notations. 
\S\ref{subsec:partial-recompute} describes {\em how to re-compute} the KV of only a small subset of tokens with minimum overhead.
% (\S\ref{subsec:partial-recompute}).
Then \S\ref{subsec:token-selection} describes {\em how to select} the tokens on each layer whose KV will be re-computed.



\begin{table}[]
\small
\begin{tabular}{rl}
\hline
\textit{Notation} & \textit{Description} \\ \hline\hline
\begin{tabular}[c]{@{}r@{}}$\LayerIndex$ \\ $\TokenIndex$\\ $\ChunkIndex$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Layer index\\ Token index\\ Chunk index\end{tabular} \\ \hline
\begin{tabular}[c]{@{}r@{}}$\KV$\\ $\KV^{\Full}$\\ $\KV^{\Pre}$\\ $\KV^{\New}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}KV cache\\ Fully re-computed KV cache\\ Pre-computed KV cache\\ \name-updated KV cache\end{tabular} \\ \hline
\begin{tabular}[c]{@{}r@{}}$\KV[\LayerIndex]$\\ $\KV[\LayerIndex][\TokenIndex]$\end{tabular} & \begin{tabular}[c]{@{}l@{}}KV on layer $\LayerIndex$\\ KV on layer $\LayerIndex$ at token $\TokenIndex$\end{tabular} \\ \hline
\begin{tabular}[c]{@{}r@{}}$\Attention_{\LayerIndex}$\\ $\Attention_{\LayerIndex}[\TokenIndex]$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Attention matrix on layer $\LayerIndex$\\ Attention matrix on layer $\LayerIndex$ associated with token $\TokenIndex$\end{tabular} \\ \hline
%\begin{tabular}[c]{@{}r@{}}$\Attention_{\LayerIndex}$\\ $\Attention_{\LayerIndex}[\TokenIndex,\TokenIndex']$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Attention Matrix on layer $\LayerIndex$\\ Attention Matrix on layer $\LayerIndex$ between token $\TokenIndex$ and $\TokenIndex'$\end{tabular} \\ \hline
$\CA_{\LayerIndex,\TokenIndex}$ & Aggregated Cross-Attention of token $\TokenIndex$ on layer $\LayerIndex$ \\ \hline\end{tabular}
\caption{Summary of terminology}
\label{tab:terminology}
\end{table}

%\mypara{Terminology}

\subsection{Terminology}
\label{subsec:terminology}

Table~\ref{tab:terminology} summarizes the notations used in this section.
%To formally describe our goal, we begin with the notations used in this section (summarized in Table~\ref{tab:terminology}).
%For a given KV cache $\KV$, we use $\KV[\LayerIndex]$ and $\KV[\LayerIndex][\TokenIndex]$ to denote the KV on layer $\LayerIndex$ and the KV on layer $\LayerIndex$ at token $\TokenIndex$, respectively.\footnote{For simplicity, we use the terms KV and KV cache interchangeably.}
For a given list of $\ChunkNum$ text chunks, 
We use $\KV^{\Full}$ to denote the KV cache of full KV re-compute, $\KV^{\Pre}$ to denote the pre-computed KV cache,  and $\KV^{\New}$ to denote the \name-updated KV cache. 
Here, each of these KV caches is is a concatenation of KV caches $\KV_{\ChunkIndex}^{*}$ of different text chunks $\ChunkIndex$, $1\leq\ChunkIndex\leq\ChunkNum$.

We use $\Attention_{\LayerIndex}=\Func_\LayerIndex(\KV)$ to denote the attention matrix on layer $\LayerIndex$ of a KV cache $\KV$.
Within an attention matrix $\Attention$, we use $\Attention[\TokenIndex]$ to denote the submatrix of attention between one token $\TokenIndex$ and all preceding tokens.
Correspondingly, we use $\Attention_{\LayerIndex}^{\Full}=\Func_\LayerIndex(\KV^{\Full})$, $\Attention_{\LayerIndex}^{\Pre}=\Func_\LayerIndex(\KV^{\Pre})$, and $\Attention_{\LayerIndex}^{\New}=\Func_\LayerIndex(\KV^{\New})$ to denote the attention matrix of $\KV^{\Full}$, $\KV^{\Pre}$, and $\KV^{\New}$, respectively.

%We denote the precomputed KV cache as $\KV^{\Pre}=[\KV_{1}^{\Pre},\dots,\KV_{\ChunkNum}^{\Pre}]$, where $\KV_{\ChunkIndex}^{\Pre}$ is the independently precomputed KV cache of text chunk $\ChunkIndex$, $1\leq\ChunkIndex\leq\ChunkNum$.

\mypara{Attention Deviation}
Now, we define the {\em attention deviation} between a new KV cache $\KV$ and the fully re-computed $\KV^{\Full}$ on layer $\LayerIndex$ as the difference between attention matrices
$||\Attention-\Attention^{\Full}||$ (L2-norm).\footnote{We assume the $\KV$ has the same shape as $\KV^{\Full}$.}
Similarly, we can define the {\em token-wise attention deviation} of a token $\TokenIndex$ as $||\Attention[\TokenIndex]-\Attention^{\Full}[\TokenIndex]||$.

%$\Func_\LayerIndex(\KV)$ and $\Func_\LayerIndex(\KV^{\Full})$.\footnote{Assume $\KV$ has the same shape as $\KV^{\Full}$.}
%We measure the difference by L2-norm. 
Using these notations, our goal can be formulated as how to quickly update the precomputed KV cache $\KV^{\Pre}$ to the new KV cache $\KV^{\New}$, such that the attention deviation of any layer $\LayerIndex$, $||\Attention_{\LayerIndex}^{\New}-\Attention_{\LayerIndex}^{\Full}||$, is minimized. 
Note that the attention deviation between $\KV^{\Pre}$ and $\KV^{\Full}$ lies in the cross-attention between the chunks (\S\ref{??}), reducing the attention deviation effectively recovers the cross-attention to the same as full KV recompute.
%the attention matrix contains the cross-attention between the chunks, 


\begin{comment}

the difference between the new attention matrix $\Attention_{\LayerIndex}^{\New}=\Func_\LayerIndex(\KV^{\New})$ and the fully recomputed attention matrix $\Attention_{\LayerIndex}^{\Full}=\Func_\LayerIndex(\KV^{\Full})$ is minimized for all layers, \ie $\min ||\Attention_{\LayerIndex}^{\New}-\Attention_{\LayerIndex}^{\Full}||, \forall \LayerIndex$.



For a different KV cache $\KV$ (which has the same shape as $\KV^{\Full}$), we define the {\em attention deviation} on layer $\LayerIndex$ as the deviation between 
its attention matrix 
$\Func_\LayerIndex(\KV)$ and 
the full recomputed attention matrix 
$\Func_\LayerIndex(\KV^{\Full})$


$||\Attention_{\LayerIndex}-\Attention_{\LayerIndex}^{\Full}||=||\Func_\LayerIndex(\KV^{\New})-\Func_\LayerIndex(\KV^{\New})||$, the difference between 



After updating the pre-computed KV cache, we denote the new KV as $\KV^{\New}$, whose resulting attention matrix on layer $\LayerIndex$ is $\Attention_{\LayerIndex}^{\New}=\Func_\LayerIndex(\KV^{\New})$.



Formally, our goal is to quickly update the precomputed KV cache $\KV^{\Pre}$ to a {\em partially updated} KV cache $\KV^{\New}$, such that the difference between the new attention matrix $\Attention_{\LayerIndex}^{\New}=\Func_\LayerIndex(\KV^{\New})$ and the fully recomputed attention matrix $\Attention_{\LayerIndex}^{\Full}=\Func_\LayerIndex(\KV^{\Full})$ is minimized for all layers, \ie $\min ||\Attention_{\LayerIndex}^{\New}-\Attention_{\LayerIndex}^{\Full}||, \forall \LayerIndex$.



$||\Attention_{\LayerIndex}^{\New}-\Attention_{\LayerIndex}^{\Full})||$, is minimized for all layers $\LayerIndex$.
and the fully recomputed attention matrix $\Attention_{\LayerIndex}^{\Full}=\Func_\LayerIndex(\KV^{\Full})$ is minimum for all layer index $\LayerIndex$.
Since the difference between $\Attention_{\LayerIndex}^{\New}$ and $\Attention_{\LayerIndex}^{\Full}$ lies in the cross-attention between the chunks, 
%the attention matrix contains the cross-attention between the chunks, 
minimizing the attention matrix difference effectively recovers the cross-attention to the same as full KV recompute.

\end{comment}



\subsection{Selectively re-computing KV cache}
\label{subsec:partial-recompute}

%Then in \S\ref{subsec:token-selection}, we will 
%\item Which tokens should be selected to be re-computed (\S\ref{subsec:token-selection}).
%\end{packeditemize}

\begin{figure}[t]
\centering
	\includegraphics[width=.99\columnwidth]{figs/selective_recompute.pdf}
    \tightcaption{}
    \label{fig:selective_recompute}
\end{figure}


\mypara{Workflow} 
The default implementation of prefill (depicted in Figure~\ref{fig:selective_recompute}(a)) does not ``skip'' tokens while only compute the KV of a subset of tokens. 
Instead, on each layer $\LayerIndex$, we apply a mask on the input embedding (depicted in Figure~\ref{fig:selective_recompute}(b)) in order to reduce it to the a subset of tokens (selected by the logic explained shortly).
It transforms the reduced input embedding into the resulting $Q_{\LayerIndex}$, $K_{\LayerIndex}$ and $V_{\LayerIndex}$ vectors will also be restricted to the selected tokens. 
Next, it expands the $K_{\LayerIndex}$ vector and $V_{\LayerIndex}$ vector by reusing the KV cache entries associated with the tokens not selected for re-computation on layer $\LayerIndex$, so the resulting attention matrix will include the attention between the selected tokens and all preceding tokens. 
Finally, it runs the same attention module to produce the input embedding of the next layer. 
These changes make little assumption on the exact transformer process and can be integrated with many popular transformers (more details in \S\ref{sec:impl}).

\jc{Jiayi, please mention some papers that also do this}

\mypara{Benefits} This procedure has two benefits.
First, the compute overhead is now proportional to the number of selected tokens. 
This is because it only does the computations associated with the selected tokens. 
Thus, if we re-compute $r\%$ of tokens per layer, the total compute overhead will be $r\%$ of full prefill. 
Empirically, the prefill delay is also about $r\%$ of the full prefill (see \S\ref{subsec:eval:??}).

Second, the KV of the selected tokens are updated to capture the cross-attention between them and all of their preceding tokens. 
This is because although attention matrix on each layer only has the entries of the selected tokens, it includes their attention with all preceding tokens, both selected and not selected.
This attention matrix is then used to compute the input embedding of the next layer, thus affecting the updated KV values of the next layer. 
As elaborated in \S\ref{subsec:token-selection}, capturing the full cross-attention of the selected tokens is important since high cross-attention can exist among any tokens, not only the selected ones.

%Recomputing the KV of a token $\TokenIndex$ on layer $\LayerIndex$ may not make its 

\begin{comment}

1. overhead proportional to number of selected tokens
2. kv of the selected tokens are updated with the cross-attention between them and all preceding tokens
3. kv of non-selected tokens are not changed

This ensures that the attention matrix captures the cross-attention between the selectively re-computed tokens and {\em all} preceding tokens.
This naturally affects the next layer's input $I_{\LayerIndex+1}$ and thus propagates to the KV values of the next layer.

\end{comment}


%However, we can first {\em permute} the order of the tokens on each layer to move the \HCA tokens and separate them from other tokens whose KV does not need to be updated. 
%The reason is the following insight, whose proof will be provided in \S\ref{??}.
%
%\begin{insight}
%The order of tokens on each layer does not affect the KV of each token.\jc{jiayi, this insight doesn't sound right. doesn't it mean you can arbitrarily shuffle the tokens and still get the same result?} \jiayi{A new version: The order of tokens on each layer does not affect the KV of each token if the attention mask is permuted accordingly}
%\end{insight}
%
%Once the \HCA tokens on a layer are moved together, the prefill computation can be done only on those tokens without affecting other tokens' KV.
%Figure~\ref{fig:selective_recompute} illustrates this process.
%So if only $r\%$ of tokens are selected as \HCA tokens, recomputing their KV only needs $r\%$ of computation overhead as a full prefill.

\subsection{Selecting which tokens to re-compute}
\label{subsec:token-selection}

To choose the tokens whose KV should be re-computed, we first notice that the attention deviation, defined in \S\ref{subsec:terminology}, is an aggregation of the token-wise attention deviation, \ie $||\Attention_{\LayerIndex}-\Attention_{\LayerIndex}^{\Full}||^2=\sum_{\TokenIndex}||\Attention_{\LayerIndex}[\TokenIndex]-\Attention_{\LayerIndex}^{\Full}[\TokenIndex]||^2$.

Therefore, to reduce attention deviation between $\Attention_{\LayerIndex}^{\Pre}$ and $\Attention_{\LayerIndex}^{\Full}$, our idea is to prioritize re-computing the KV of tokens $\TokenIndex$ on each layer whose token-wise attention deviations $||\Attention_{\LayerIndex}^{\Pre}[\TokenIndex]-\Attention_{\LayerIndex}^{\Full}[\TokenIndex]||$ are higher. 
To show its effect, Figure~\ref{??} uses three models on the dataset of \fillme (please see \S\ref{subsec:eval:setup} for details).\jc{jiayi, add the figure here please}
It shows the change of attention deviation of one layer $||\Attention_{\LayerIndex}^{\New}-\Attention_{\LayerIndex}^{\Full}||$ when we choose to recompute the $r\%$ of tokens $\TokenIndex$ who have the highest token-wise attention deviations $||\Attention_{\LayerIndex}^{\Pre}[\TokenIndex]-\Attention_{\LayerIndex}^{\Full}[\TokenIndex]||$.
As $r$ increases, the attention deviation gradually reduces, but the biggest drop happens when top few tokens with the highest are re-computed. 
Empirically, it indicates the following insight. 


\begin{insight}
On each layer $\LayerIndex$, re-computing the KV of a token who has a higher token-wise attention deviation (\ie $||\Attention_{\LayerIndex}^{\Pre}[\TokenIndex]-\Attention_{\LayerIndex}^{\Full}[\TokenIndex]||$) reduces the total attention deviation (\ie $||\Attention_{\LayerIndex}^{\New}-\Attention_{\LayerIndex}^{\Full}||$) by a greater amount. 
%Recomputing the KV of a token $\TokenIndex$ on layer $\LayerIndex$ will greatly reduce the Attention Deviation associated with this token, \ie $||\Attention_{\LayerIndex}^{\New}[\TokenIndex]-\Attention_{\LayerIndex}^{\Full}[\TokenIndex]||$.
\end{insight}



%\begin{figure}[t]
%\centering
%	\includegraphics[width=.99\columnwidth]{figs/aca_illustrated.pdf}
%    \tightcaption{Using token-wise attention deviation to identify which tokens to re-compute KV cache.}
%    \label{fig:aca}
%\end{figure}

%We call the top $r\%$ tokens on layer $\LayerIndex$ with highest token-wise attention deviation, {\em high-attention-deviation} (or {\em \HCA}) tokens on layer $\LayerIndex$.
Thus, if we need to re-compute the KV of, say 10\%, of tokens on a layer $\LayerIndex$, we should choose the 10\% of tokens who have the highest token-wise attention deviation.\footnote{An important side note is that in the pre-computed KV cache, the K vector of each chunk must be adjusted with the correct positional embedding. In the most popular positional embedding scheme (Rotary Positional Embedding or ROPE~\cite{??}), this correction is done simply by multiplying the K vector by a rotation matrix $\begin{pmatrix}
\cos m\theta & -\sin m\theta\\
\sin m\theta & \cos m\theta\\
\end{pmatrix}$. This step has negligible overhead (\S\ref{subsec:eval:overhead}).}
We refer to these tokens as the {\em high-attention-deviation} (or {\em \HCA}) tokens on layer $\LayerIndex$.
%10\% tokens with the highest \ACA, \ie top 10\% \HCA tokens.

Now that we know we should recompute KV for are the \HCA tokens, two natural questions remain. 

\vspace{0.2cm}
\noindent {\bf Do we need to re-compute the KV of most tokens?}
Fortunately, Figure~\ref{??} indicates that this is not always true. 
Re-computing 10-15\% of tokens can reduce the attention deviation by \fillme\%. 
The intuitive reason is the following:
\begin{insight}
Due to attention sparsity, the high attention only occurs between a small number of tokens and their preceding tokens in other chunks, so only a small number of tokens have a high token-wise attention deviation, \ie~\HCA tokens.
\end{insight}
{\em Attention sparsity} is a well-known property observed by prior research in many transformer models~\cite{liu2024scissorhands,h2o,choromanski2020rethinking,chen2021scatterbrain}.
If a token has very low attention with other chunks' tokens (\ie low cross-attention with other chunks), the token-wise attention deviation between $\Attention^{\Pre}$ and $\Attention^{\Full}$ will be low anyway. 
Only when attention is high between chunks, should KV re-computation be used.

\begin{figure}[t]
\centering
	\includegraphics[width=.99\columnwidth]{figs/ca_cdf.pdf}
    \tightcaption{Distribution of aggregated cross-attention (\ACA) of different tokens on one layer.\jiayi{Replotting this with our recomputation. Actually, I think using a separate graph might. The new graph should be the cdf containing only the recomputed ACA.}}
    \label{fig:acacdf}
\end{figure}

To validate this observation, Figure~\ref{fig:acacdf} uses the same models and dataset as Figure~\ref{??}. 
It shows the distribution of token-wise attention deviation on one layer.
We can see that a small fraction, about 10-15\%, of tokens have much higher token-wise attention deviation than others, which empirically corroborates the sparsity of cross-attention.



\vspace{0.2cm}
\noindent {\bf How to identify the \HCA tokens without knowing the true attention matrix?}
Naively, to identify the \HCA tokens, one must calculate the full attention matrix $\Attention_{\LayerIndex}^{\Pre}$ and $\Attention_{\LayerIndex}^{\Full}$ of each layer $\LayerIndex$ in the first place, but doing so is too expensive, and defeats the purpose of selective KV re-compute.
instead, we observe that the \HCA tokens on different layers are not independent:
%. we have the following observation:

\begin{insight}
Tokens with highest token-wise attention deviations on one layer are likely to have the highest token-wise attention deviations on the next layer. 
%The \HCA tokens on one layer is likely a subset of \HCA tokens on the previous layer. 
\end{insight}

More specifically, if token $\TokenIndex$ has a higher token-wise attention deviation than $\TokenIndex'$ on layer $\LayerIndex$, (\ie $||\Attention_{\LayerIndex}^{\Pre}[\TokenIndex]-\Attention_{\LayerIndex}^{\Full}[\TokenIndex]||>||\Attention_{\LayerIndex}^{\Pre}[\TokenIndex']-\Attention_{\LayerIndex}^{\Full}[\TokenIndex']||$), token $\TokenIndex$ will likely to have a higher token-wise attention deviation on the next layer $\LayerIndex+1$, (\ie $||\Attention_{\LayerIndex+1}^{\Pre}[\TokenIndex]-\Attention_{\LayerIndex+1}^{\Full}[\TokenIndex]||>||\Attention_{\LayerIndex+1}^{\Pre}[\TokenIndex']-\Attention_{\LayerIndex+1}^{\Full}[\TokenIndex']||$).
%on one layer $\LayerIndex$, if token $\TokenIndex$ has a higher \ACA than token $\TokenIndex'$, (\ie $\CA_{\LayerIndex, \TokenIndex}\geq\CA_{\LayerIndex, \TokenIndex}$), then on the the next layer $\LayerIndex+1$, token $\TokenIndex$ is likely to have a higher \ACA than token $\TokenIndex'$ (\ie $\CA_{\LayerIndex+1, \TokenIndex}\geq\CA_{\LayerIndex+1, \TokenIndex}$).

To put it concretely, if the top three \HCA tokens on the first layer are tokens 2, 3, and 5, these three tokens likely also have higher token-wise attention deviations than most other tokens. 
Figure~\ref{fig:rankcorr} uses the same setting as Figure~\ref{fig:acacdf} and shows the Jaccard's similarity score between the top 15\% \HCA tokens between two neighboring layers. 
The figure shows a consistently high similarity of \HCA tokens between different layers.\footnote{Note that the similarity of \HCA tokens does not mean the attention matrices are similar between layers.}
%Kendall's rank correlation scores between \ACA of the same token on two neighboring layers. 

The intuition behind this correlation is \fillme \jc{jiayi, please provide some explanation here}


\begin{figure}[t]
\centering
	\includegraphics[width=.99\columnwidth]{figs/ca_corr_bar_new.pdf}
    \tightcaption{Rank correlation of the Aggregated Cross-Attention (\ACA) per token between two consecutive layers.
    \jc{\st{mock figure. Jiayi, please update it with real numbers}}\jiayi{Scores don't look high enoug for now. Let me get figure 6 first then iterate on this}}
    \label{fig:rankcorr}
\end{figure}

\begin{figure}[t]
\centering
	\includegraphics[width=.99\columnwidth]{figs/selection_illustrated.pdf}
    \tightcaption{\name selects the \HCA (high-attention-deviation) tokens of one layer by computing the token-wise attention deviation of only the \HCA tokens selected from the previous layer and select the tokens among them with high token-wise attention deviation.}
    \label{fig:selection_illustrated}
\end{figure}



Given the substantial correlation between the \HCA tokens, a straightforward solution is that we can  perform prefill on the first layer first, and pick the \HCA tokens of the first layer and only update their KV on all other layers.
Since an LLM usually has over 30 layers, this process can save most of the compute compared to full KV re-compute. 
That said, using {\em only} the attention deviation of different tokens on the first layer may not be statistically reliable to pick \HCA tokens of all layers, especially deeper layers. 

Thus, we opt for a {\em gradual filtering} scheme (depicted in Figure~\ref{fig:selection_illustrated}).
If on average we want to pick $r\%$ \HCA tokens per layer, we will pick $r_1\%$ tokens based on the token-wise attention deviation on the first layer, with $r_1$ being slightly higher than $r$, and use them as the \HCA tokens on the second layer.
Then we recompute the KV of these $r_1\%$ \HCA tokens on the second layer and pick $r_2\%$ tokens who have highest token-wise attention deviation, with $r_2$ slightly less than $r_1$, as the \HCA tokens on the next layer, and so forth. 
Intuitively, this gradual-filtering scheme eventually picks the \HCA tokens who have relatively high attention deviation not only on the first layer, but also on a few other layers, which empirically is more statistically reliable to identify the \HCA tokens on each layers.  


%we only need to compute the \ACA of these three tokens on the next layer in order to pick its \HCA tokens. 

%As elaborated in \S\ref{subsec:modular}, the difference between the partially update attention matrix $\AttentionL{\LayerIndex}$ and the {\em fully recomputed} attention matrix $\AttentionL{\LayerIndex}^*$ 



\jc{junchen edit ends here}


==> sec_recompute_v5.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


%\section{Fast Context Fusing by Selective Recomputation}
\section{Fast KV Cache Fusing}
\label{sec:merge}

Given that {\em full KV re-compute} (\ie full prefill or prefix caching) can be too slow and {\em full KV reuse} (\ie modular caching) can have low quality, a natural question then is how to have both the low delay of full KV reuse {\em and} the high quality of full KV re-compute. 
Our goal therefore is the following:

\begin{goal}
When an LLM input includes multiple re-used text chunks, how to {\bf quickly} reduce the KV deviation, which caused by cross attention, such that the resulting forward attention matrix (indicating generation quality) has {\bf minimum difference} with the one produced by full KV re-compute. 
\end{goal}

To realize our goal, \name~{\em re-computes the KV of a selective subset of tokens} on each layer, while re-using other tokens' KV.\footnote{For simplicity, we use the terms KV and KV cache interchangeably.}
%\footnote{We also need to update the positional encoding for all tokens, but as explained shortly in \S\ref{subsec:positional}, doing so incurs minimum overhead.}
We explain how \name does so in three parts.
\S\ref{subsec:terminology} begins with the notations. 
\S\ref{subsec:partial-recompute} describes {\em how to re-compute} the KV of only a small subset of tokens with minimum overhead.
% (\S\ref{subsec:partial-recompute}).
Then \S\ref{subsec:token-selection} describes {\em how to select} the tokens on each layer whose KV will be re-computed.



\begin{table}[]
\small
\begin{tabular}{rl}
\hline
\textit{Notation} & \textit{Description} \\ \hline\hline
\begin{tabular}[c]{@{}r@{}}$\LayerIndex$ \\ $\TokenIndex$\\ $\ChunkIndex$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Layer index\\ Token index\\ Chunk index\end{tabular} \\ \hline
\begin{tabular}[c]{@{}r@{}}$\KV$\\ $\KV^{\Full}$\\ $\KV^{\Pre}$\\ $\KV^{\New}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}KV cache\\ Fully re-computed KV cache\\ Pre-computed KV cache\\ \name-updated KV cache\end{tabular} \\ \hline
\begin{tabular}[c]{@{}r@{}}$\KV[\LayerIndex]$\\ $\KV[\LayerIndex][\TokenIndex]$\end{tabular} & \begin{tabular}[c]{@{}l@{}}KV on layer $\LayerIndex$\\ KV on layer $\LayerIndex$ at token $\TokenIndex$\end{tabular} \\ \hline
\begin{tabular}[c]{@{}r@{}}$\Attention_{\LayerIndex}$\\ $\Attention_{\LayerIndex}[\TokenIndex]$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Attention matrix on layer $\LayerIndex$\\ Attention matrix on layer $\LayerIndex$ associated with token $\TokenIndex$\end{tabular} \\ \hline
%\begin{tabular}[c]{@{}r@{}}$\Attention_{\LayerIndex}$\\ $\Attention_{\LayerIndex}[\TokenIndex,\TokenIndex']$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Attention Matrix on layer $\LayerIndex$\\ Attention Matrix on layer $\LayerIndex$ between token $\TokenIndex$ and $\TokenIndex'$\end{tabular} \\ \hline
$\CA_{\LayerIndex,\TokenIndex}$ & Aggregated Cross-Attention of token $\TokenIndex$ on layer $\LayerIndex$ \\ \hline\end{tabular}
\caption{Summary of terminology\jiayi{Needs to be updated with Forward Attention FA}}
\label{tab:terminology}
\end{table}

%\mypara{Terminology}

\subsection{Terminology}
\label{subsec:terminology}

Table~\ref{tab:terminology} summarizes the notations used in this section.
%To formally describe our goal, we begin with the notations used in this section (summarized in Table~\ref{tab:terminology}).
%For a given KV cache $\KV$, we use $\KV[\LayerIndex]$ and $\KV[\LayerIndex][\TokenIndex]$ to denote the KV on layer $\LayerIndex$ and the KV on layer $\LayerIndex$ at token $\TokenIndex$, respectively.\footnote{For simplicity, we use the terms KV and KV cache interchangeably.}
For a given list of $\ChunkNum$ text chunks, 
we use $\KV^{\Full}$ to denote the KV cache of full KV re-compute, $\KV^{\Pre}$ to denote the pre-computed KV cache,  and $\KV^{\New}$ to denote the \name-updated KV cache. 
Here, each of these KV caches is a concatenation of KV caches $\KV_{\ChunkIndex}^{*}$ of different text chunks $\ChunkIndex$, $1\leq\ChunkIndex\leq\ChunkNum$. 

In addition, given a user instruction at the end,
we use $\ForwardAttention_{\LayerIndex}=\Func_\LayerIndex(\KV)$ to denote the forward attention on $\LayerIndex$ of the KV cache $\KV$.
Within an forward attention matrix $\ForwardAttention$, we use $\ForwardAttention[\TokenIndex][\UserTokenIndex]$ to denote the attention value between one token $\UserTokenIndex$ (in the user instruction) and another token $\TokenIndex$ among all preceding tokens (including the text chunks).
Correspondingly, we use $\ForwardAttention_{\LayerIndex}^{\Full}=\Func_\LayerIndex(\KV^{\Full}_{\LayerIndex})$, $\ForwardAttention_{\LayerIndex}^{\Pre}=\Func_\LayerIndex(\KV^{\Pre}_{\LayerIndex})$, and $\ForwardAttention_{\LayerIndex}^{\New}=\Func_\LayerIndex(\KV^{\New}_{\LayerIndex})$ to denote the forward attention matrix of $\KV^{\Full}$, $\KV^{\Pre}$, and $\KV^{\New}$, respectively.

%We use $\Attention_{\LayerIndex}=\Func_\LayerIndex(\KV)$ to denote the attention matrix on layer $\LayerIndex$ of a KV cache $\KV$.
%Within an attention matrix $\Attention$, we use $\Attention[\TokenIndex]$ to denote the submatrix of attention between one token $\TokenIndex$ and all preceding tokens.
%Correspondingly, we use $\Attention_{\LayerIndex}^{\Full}=\Func_\LayerIndex(\KV^{\Full})$, $\Attention_{\LayerIndex}^{\Pre}=\Func_\LayerIndex(\KV^{\Pre})$, and $\Attention_{\LayerIndex}^{\New}=\Func_\LayerIndex(\KV^{\New})$ to denote the attention matrix of $\KV^{\Full}$, $\KV^{\Pre}$, and $\KV^{\New}$, respectively.

%We denote the precomputed KV cache as $\KV^{\Pre}=[\KV_{1}^{\Pre},\dots,\KV_{\ChunkNum}^{\Pre}]$, where $\KV_{\ChunkIndex}^{\Pre}$ is the independently precomputed KV cache of text chunk $\ChunkIndex$, $1\leq\ChunkIndex\leq\ChunkNum$.

\mypara{Forward Attention Deviation}
Now, we define the {\em forward attention deviation} between a new KV cache $\KV$ and the fully re-computed $\KV^{\Full}$ on layer $\LayerIndex$ as the difference between forward attention matrices
$||\ForwardAttention-\ForwardAttention^{\Full}||$ (L2-norm).\footnote{We assume the $\KV$ has the same shape as $\KV^{\Full}$.}
%Similarly, we can define the {\em token-wise attention deviation} of a token $\TokenIndex$ as $||\Attention[\TokenIndex]-\Attention^{\Full}[\TokenIndex]||$.

%$\Func_\LayerIndex(\KV)$ and $\Func_\LayerIndex(\KV^{\Full})$.\footnote{Assume $\KV$ has the same shape as $\KV^{\Full}$.}
%We measure the difference by L2-norm. 
Using these notations, our goal can be formulated as how to quickly update the precomputed KV cache $\KV^{\Pre}$ to the new KV cache $\KV^{\New}$, such that the forward attention deviation of any layer $\LayerIndex$, $||\ForwardAttention_{\LayerIndex}^{\New}-\ForwardAttention_{\LayerIndex}^{\Full}||$, is minimized. 
%Note that the KV deviation between $\KV^{\Pre}$ and $\KV^{\Full}$ lies in the cross-attention between the chunks (\S\ref{??}). 
Note that the KV deviation between $\KV^{\Pre}$ and $\KV^{\Full}$ lies in the cross-attention between the chunks. KV deviation further affects the generation process through forward attention \jiayi{Need a visualization here}, reducing the forward attention deviation effectively recovers the cross-attention to the same as full KV recompute.
%the attention matrix contains the cross-attention between the chunks, 
\jiayi{updated 4.1}

\begin{comment}

the difference between the new attention matrix $\Attention_{\LayerIndex}^{\New}=\Func_\LayerIndex(\KV^{\New})$ and the fully recomputed attention matrix $\Attention_{\LayerIndex}^{\Full}=\Func_\LayerIndex(\KV^{\Full})$ is minimized for all layers, \ie $\min ||\Attention_{\LayerIndex}^{\New}-\Attention_{\LayerIndex}^{\Full}||, \forall \LayerIndex$.



For a different KV cache $\KV$ (which has the same shape as $\KV^{\Full}$), we define the {\em attention deviation} on layer $\LayerIndex$ as the deviation between 
its attention matrix 
$\Func_\LayerIndex(\KV)$ and 
the full recomputed attention matrix 
$\Func_\LayerIndex(\KV^{\Full})$


$||\Attention_{\LayerIndex}-\Attention_{\LayerIndex}^{\Full}||=||\Func_\LayerIndex(\KV^{\New})-\Func_\LayerIndex(\KV^{\New})||$, the difference between 



After updating the pre-computed KV cache, we denote the new KV as $\KV^{\New}$, whose resulting attention matrix on layer $\LayerIndex$ is $\Attention_{\LayerIndex}^{\New}=\Func_\LayerIndex(\KV^{\New})$.



Formally, our goal is to quickly update the precomputed KV cache $\KV^{\Pre}$ to a {\em partially updated} KV cache $\KV^{\New}$, such that the difference between the new attention matrix $\Attention_{\LayerIndex}^{\New}=\Func_\LayerIndex(\KV^{\New})$ and the fully recomputed attention matrix $\Attention_{\LayerIndex}^{\Full}=\Func_\LayerIndex(\KV^{\Full})$ is minimized for all layers, \ie $\min ||\Attention_{\LayerIndex}^{\New}-\Attention_{\LayerIndex}^{\Full}||, \forall \LayerIndex$.



$||\Attention_{\LayerIndex}^{\New}-\Attention_{\LayerIndex}^{\Full})||$, is minimized for all layers $\LayerIndex$.
and the fully recomputed attention matrix $\Attention_{\LayerIndex}^{\Full}=\Func_\LayerIndex(\KV^{\Full})$ is minimum for all layer index $\LayerIndex$.
Since the difference between $\Attention_{\LayerIndex}^{\New}$ and $\Attention_{\LayerIndex}^{\Full}$ lies in the cross-attention between the chunks, 
%the attention matrix contains the cross-attention between the chunks, 
minimizing the attention matrix difference effectively recovers the cross-attention to the same as full KV recompute.

\end{comment}



\subsection{Selectively re-computing KV cache}
\label{subsec:partial-recompute}

%Then in \S\ref{subsec:token-selection}, we will 
%\item Which tokens should be selected to be re-computed (\S\ref{subsec:token-selection}).
%\end{packeditemize}

\begin{figure}[t]
\centering
	\includegraphics[width=.99\columnwidth]{figs/selective_recompute.pdf}
    \tightcaption{}
    \label{fig:selective_recompute}
\end{figure}


\mypara{Workflow} 
The default implementation of prefill (depicted in Figure~\ref{fig:selective_recompute}(a)) does not ``skip'' tokens while only compute the KV of a subset of tokens. 
Instead, on each layer $\LayerIndex$, we apply a mask on the input embedding (depicted in Figure~\ref{fig:selective_recompute}(b)) in order to reduce it to the a subset of tokens (selected by the logic explained shortly).
It transforms the reduced input embedding into the resulting $Q_{\LayerIndex}$, $K_{\LayerIndex}$ and $V_{\LayerIndex}$ vectors will also be restricted to the selected tokens. 
Next, it expands the $K_{\LayerIndex}$ vector and $V_{\LayerIndex}$ vector by reusing the KV cache entries associated with the tokens not selected for re-computation on layer $\LayerIndex$, so the resulting attention matrix will include the attention between the selected tokens and all preceding tokens. 
Finally, it runs the same attention module to produce the input embedding of the next layer. 
These changes make little assumption on the exact transformer process and can be integrated with many popular transformers (more details in \S\ref{sec:impl}).

\jc{Jiayi, please mention some papers that also do this}

\mypara{Benefits} This procedure has two benefits.
First, the compute overhead is now proportional to the number of selected tokens. 
This is because it only does the computations associated with the selected tokens. 
Thus, if we re-compute $r\%$ of tokens per layer, the total compute overhead will be $r\%$ of full prefill. 
Empirically, the prefill delay is also about $r\%$ of the full prefill (see \S\ref{subsec:eval:??}).

Second, the KV of the selected tokens are updated to capture the cross-attention between them and all of their preceding tokens. 
This is because although attention matrix on each layer only has the entries of the selected tokens, it includes their attention with all preceding tokens, both selected and not selected.
This attention matrix is then used to compute the input embedding of the next layer, thus affecting the updated KV values of the next layer. 
%As elaborated in \S\ref{subsec:token-selection}, capturing the full cross-attention of the selected tokens is important since high cross-attention can exist among any tokens, not only the selected ones.

%Recomputing the KV of a token $\TokenIndex$ on layer $\LayerIndex$ may not make its 
\jiayi{Above is updated 4.2}

\begin{comment}

1. overhead proportional to number of selected tokens
2. kv of the selected tokens are updated with the cross-attention between them and all preceding tokens
3. kv of non-selected tokens are not changed

This ensures that the attention matrix captures the cross-attention between the selectively re-computed tokens and {\em all} preceding tokens.
This naturally affects the next layer's input $I_{\LayerIndex+1}$ and thus propagates to the KV values of the next layer.

\end{comment}


%However, we can first {\em permute} the order of the tokens on each layer to move the \HCA tokens and separate them from other tokens whose KV does not need to be updated. 
%The reason is the following insight, whose proof will be provided in \S\ref{??}.
%
%\begin{insight}
%The order of tokens on each layer does not affect the KV of each token.\jc{jiayi, this insight doesn't sound right. doesn't it mean you can arbitrarily shuffle the tokens and still get the same result?} \jiayi{A new version: The order of tokens on each layer does not affect the KV of each token if the attention mask is permuted accordingly}
%\end{insight}
%
%Once the \HCA tokens on a layer are moved together, the prefill computation can be done only on those tokens without affecting other tokens' KV.
%Figure~\ref{fig:selective_recompute} illustrates this process.
%So if only $r\%$ of tokens are selected as \HCA tokens, recomputing their KV only needs $r\%$ of computation overhead as a full prefill.

\subsection{Selecting which tokens to re-compute}
\label{subsec:token-selection}


%we first notice that the attention deviation, defined in \S\ref{subsec:terminology}, is an aggregation of the token-wise attention deviation, \ie $||\Attention_{\LayerIndex}-\Attention_{\LayerIndex}^{\Full}||^2=\sum_{\TokenIndex}||\Attention_{\LayerIndex}[\TokenIndex]-\Attention_{\LayerIndex}^{\Full}[\TokenIndex]||^2$.
To choose the tokens whose KV should be re-computed, 
we first notice that the forward attention deviation, defined in \S\ref{subsec:terminology}, can be written as a function of the KV caches, 
\ie $||\ForwardAttention_{\LayerIndex}-\ForwardAttention_{\LayerIndex}^{\Full}||^2=||\Func_\LayerIndex(\KV_{\LayerIndex})-\Func_\LayerIndex(\KV^{\Full}_{\LayerIndex})||^2$. \jiayi{We should add a intuitive transition saying deviation in X cause deviation in F(X)}

Therefore, to reduce attention forward deviation between $\Attention_{\LayerIndex}^{\Pre}$ and $\Attention_{\LayerIndex}^{\Full}$, our idea is to prioritize re-computing the KV of tokens $\TokenIndex$ on each layer whose token-wise KV deviation $||\KV_{\LayerIndex}^{\Pre}[\TokenIndex]-\KV_{\LayerIndex}^{\Full}[\TokenIndex]||$ are higher. 
To show its effect, Figure~\ref{??} uses three models on the dataset of \fillme (please see \S\ref{subsec:eval:setup} for details).\jc{jiayi, add the figure here please}
It shows the change of forward attention deviation of one layer $||\ForwardAttention_{\LayerIndex}^{\New}-\ForwardAttention_{\LayerIndex}^{\Full}||$ when we choose to recompute the $r\%$ of tokens $\TokenIndex$ who have the highest token-wise attention deviations $||\KV_{\LayerIndex}^{\Pre}[\TokenIndex]-\KV_{\LayerIndex}^{\Full}[\TokenIndex]||$.
As $r$ increases, the attention deviation gradually reduces, but the biggest drop happens when top few tokens with the highest are re-computed. 
Empirically, it indicates the following insight. 


\begin{insight}
On each layer $\LayerIndex$, re-computing the KV of a token who has a higher KV deviation (\ie $||\KV_{\LayerIndex}^{\Pre}[\TokenIndex]-\KV_{\LayerIndex}^{\Full}[\TokenIndex]||$) reduces the total forward attention deviation (\ie $||\ForwardAttention_{\LayerIndex}^{\New}-\ForwardAttention_{\LayerIndex}^{\Full}||$) by a greater amount. 
%Recomputing the KV of a token $\TokenIndex$ on layer $\LayerIndex$ will greatly reduce the Attention Deviation associated with this token, \ie $||\Attention_{\LayerIndex}^{\New}[\TokenIndex]-\Attention_{\LayerIndex}^{\Full}[\TokenIndex]||$.
\end{insight}



%\begin{figure}[t]
%\centering
%	\includegraphics[width=.99\columnwidth]{figs/aca_illustrated.pdf}
%    \tightcaption{Using token-wise attention deviation to identify which tokens to re-compute KV cache.}
%    \label{fig:aca}
%\end{figure}

%We call the top $r\%$ tokens on layer $\LayerIndex$ with highest token-wise attention deviation, {\em high-attention-deviation} (or {\em \HCA}) tokens on layer $\LayerIndex$.
Thus, if we need to re-compute the KV of, say 10\%, of tokens on a layer $\LayerIndex$, we should choose the 10\% of tokens who have the highest token-wise attention deviation.\footnote{An important side note is that in the pre-computed KV cache, the K vector of each chunk must be adjusted with the correct positional embedding. In the most popular positional embedding scheme (Rotary Positional Embedding or ROPE~\cite{??}), this correction is done simply by multiplying the K vector by a rotation matrix $\begin{pmatrix}
\cos m\theta & -\sin m\theta\\
\sin m\theta & \cos m\theta\\
\end{pmatrix}$. This step has negligible overhead (\S\ref{subsec:eval:overhead}).}
We refer to these tokens as the {\em high-KV-deviation} (or {\em \HKVD}) tokens on layer $\LayerIndex$.
%10\% tokens with the highest \ACA, \ie top 10\% \HCA tokens.

Now that we know we should recompute KV for are the \HKVD tokens, two natural questions remain. 

\jiayi{Jiayi stops here}


\vspace{0.2cm}
\noindent {\bf Do we need to re-compute the KV of most tokens?}
Fortunately, Figure~\ref{??} indicates that this is not always true. 
Re-computing 10-15\% of tokens can reduce the forward attention deviation by \fillme\%. 
The intuitive reason is the following:
\begin{insight}
Forward attention is affected more by tokens with high KV deviations \ie~\HKVD tokens. Due to attention sparsity, the high attention only occurs between a small number of tokens and their preceding tokens in other chunks, so only a small number of tokens are \HKVD tokens.
\end{insight}
{\em Attention sparsity} is a well-known property observed by prior research in many transformer models~\cite{liu2024scissorhands,h2o,choromanski2020rethinking,chen2021scatterbrain}.
If a token has very low attention with other chunks' tokens (\ie low cross-attention with other chunks), the token-wise KV deviation between $\Attention^{\Pre}$ and $\Attention^{\Full}$ will be low anyway. 
Only when attention is high between chunks (\ie high KV deviation), should KV re-computation be used.

\begin{figure}[t]
\centering
	\includegraphics[width=.99\columnwidth]{figs/ca_cdf.pdf}
    \tightcaption{Distribution of aggregated cross-attention (\ACA) of different tokens on one layer.\jiayi{Replotting this with our recomputation. Actually, I think using a separate graph might. The new graph should be the cdf containing only the recomputed ACA.}}
    \label{fig:acacdf}
\end{figure}

To validate this observation, Figure~\ref{fig:acacdf} uses the same models and dataset as Figure~\ref{??}. 
It shows the distribution of token-wise attention deviation on one layer.
We can see that a small fraction, about 10-15\%, of tokens have much higher token-wise attention deviation than others, which empirically corroborates the sparsity of cross-attention.



\vspace{0.2cm}
\noindent {\bf How to identify the \HCA tokens without knowing the true attention matrix?}
Naively, to identify the \HCA tokens, one must calculate the full attention matrix $\Attention_{\LayerIndex}^{\Pre}$ and $\Attention_{\LayerIndex}^{\Full}$ of each layer $\LayerIndex$ in the first place, but doing so is too expensive, and defeats the purpose of selective KV re-compute.
instead, we observe that the \HCA tokens on different layers are not independent:
%. we have the following observation:

\begin{insight}
Tokens with highest token-wise attention deviations on one layer are likely to have the highest token-wise attention deviations on the next layer. 
%The \HCA tokens on one layer is likely a subset of \HCA tokens on the previous layer. 
\end{insight}

More specifically, if token $\TokenIndex$ has a higher token-wise attention deviation than $\TokenIndex'$ on layer $\LayerIndex$, (\ie $||\Attention_{\LayerIndex}^{\Pre}[\TokenIndex]-\Attention_{\LayerIndex}^{\Full}[\TokenIndex]||>||\Attention_{\LayerIndex}^{\Pre}[\TokenIndex']-\Attention_{\LayerIndex}^{\Full}[\TokenIndex']||$), token $\TokenIndex$ will likely to have a higher token-wise attention deviation on the next layer $\LayerIndex+1$, (\ie $||\Attention_{\LayerIndex+1}^{\Pre}[\TokenIndex]-\Attention_{\LayerIndex+1}^{\Full}[\TokenIndex]||>||\Attention_{\LayerIndex+1}^{\Pre}[\TokenIndex']-\Attention_{\LayerIndex+1}^{\Full}[\TokenIndex']||$).
%on one layer $\LayerIndex$, if token $\TokenIndex$ has a higher \ACA than token $\TokenIndex'$, (\ie $\CA_{\LayerIndex, \TokenIndex}\geq\CA_{\LayerIndex, \TokenIndex}$), then on the the next layer $\LayerIndex+1$, token $\TokenIndex$ is likely to have a higher \ACA than token $\TokenIndex'$ (\ie $\CA_{\LayerIndex+1, \TokenIndex}\geq\CA_{\LayerIndex+1, \TokenIndex}$).

To put it concretely, if the top three \HCA tokens on the first layer are tokens 2, 3, and 5, these three tokens likely also have higher token-wise attention deviations than most other tokens. 
Figure~\ref{fig:rankcorr} uses the same setting as Figure~\ref{fig:acacdf} and shows the Jaccard's similarity score between the top 15\% \HCA tokens between two neighboring layers. 
The figure shows a consistently high similarity of \HCA tokens between different layers.\footnote{Note that the similarity of \HCA tokens does not mean the attention matrices are similar between layers.}
%Kendall's rank correlation scores between \ACA of the same token on two neighboring layers. 

The intuition behind this correlation is \fillme \jc{jiayi, please provide some explanation here}


\begin{figure}[t]
\centering
	\includegraphics[width=.99\columnwidth]{figs/ca_corr_bar_new.pdf}
    \tightcaption{Rank correlation of the Aggregated Cross-Attention (\ACA) per token between two consecutive layers.
    \jc{\st{mock figure. Jiayi, please update it with real numbers}}\jiayi{Scores don't look high enoug for now. Let me get figure 6 first then iterate on this}}
    \label{fig:rankcorr}
\end{figure}

\begin{figure}[t]
\centering
	\includegraphics[width=.99\columnwidth]{figs/selection_illustrated.pdf}
    \tightcaption{\name selects the \HCA (high-attention-deviation) tokens of one layer by computing the token-wise attention deviation of only the \HCA tokens selected from the previous layer and select the tokens among them with high token-wise attention deviation.}
    \label{fig:selection_illustrated}
\end{figure}



Given the substantial correlation between the \HCA tokens, a straightforward solution is that we can  perform prefill on the first layer first, and pick the \HCA tokens of the first layer and only update their KV on all other layers.
Since an LLM usually has over 30 layers, this process can save most of the compute compared to full KV re-compute. 
That said, using {\em only} the attention deviation of different tokens on the first layer may not be statistically reliable to pick \HCA tokens of all layers, especially deeper layers. 

Thus, we opt for a {\em gradual filtering} scheme (depicted in Figure~\ref{fig:selection_illustrated}).
If on average we want to pick $r\%$ \HCA tokens per layer, we will pick $r_1\%$ tokens based on the token-wise attention deviation on the first layer, with $r_1$ being slightly higher than $r$, and use them as the \HCA tokens on the second layer.
Then we recompute the KV of these $r_1\%$ \HCA tokens on the second layer and pick $r_2\%$ tokens who have highest token-wise attention deviation, with $r_2$ slightly less than $r_1$, as the \HCA tokens on the next layer, and so forth. 
Intuitively, this gradual-filtering scheme eventually picks the \HCA tokens who have relatively high attention deviation not only on the first layer, but also on a few other layers, which empirically is more statistically reliable to identify the \HCA tokens on each layers.  


%we only need to compute the \ACA of these three tokens on the next layer in order to pick its \HCA tokens. 

%As elaborated in \S\ref{subsec:modular}, the difference between the partially update attention matrix $\AttentionL{\LayerIndex}$ and the {\em fully recomputed} attention matrix $\AttentionL{\LayerIndex}^*$ 



\jc{junchen edit ends here}

==> sec_recompute_v6.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


%\section{Fast Context Fusing by Selective Recomputation}
\section{Fast KV Cache Fusing}
\label{sec:merge}

Given that {\em full KV re-compute} (\ie full prefill or prefix caching) can be too slow while {\em full KV reuse} has low quality, a natural question then is how to have both the speed of full KV reuse {\em and} the quality of full KV re-compute. 
Our goal, therefore, is the following:

\begin{goal}
When an LLM input includes multiple re-used text chunks, how to {\bf quickly} update the pre-computed KV cache, such that the cross attention (and subsequently the output text) has {\bf minimum difference} with the one produced by full KV re-compute. 
\end{goal}

To achieve our goal, we present \name, which {\em re-computes the KV of a selective subset of tokens} on each layer, while reusing other tokens' KV.\footnote{For simplicity, we use the terms KV and KV cache interchangeably.}
%\footnote{We also need to update the positional encoding for all tokens, but as explained shortly in \S\ref{subsec:positional}, doing so incurs minimum overhead.}
This section explains \name in three parts.
We begin with the notations (\S\ref{subsec:terminology}), and then describe {\em how to re-compute} the KV of only a small subset of tokens (\S\ref{subsec:partial-recompute}), and finally
% (\S\ref{subsec:partial-recompute}).
explain {\em how to select} the tokens on each layer whose KV will be re-computed (\S\ref{subsec:token-selection}).

\begin{table}[]
\small
\begin{tabular}{rl}
\hline
\textit{Notation} & \textit{Description} \\ \hline\hline
\begin{tabular}[c]{@{}r@{}}$\LayerIndex$ \\ $\TokenIndex$\\ $\ChunkIndex$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Layer index\\ Token index\\ Chunk index\end{tabular} \\ \hline
\begin{tabular}[c]{@{}r@{}}$\KV$\\ $\KV_{\LayerIndex}$\\ $\KV_{\LayerIndex}[\TokenIndex]$\\ $\KV^{\Full}$\\ $\KV^{\Pre}$\\ $\KV^{\New}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}KV cache\\ KV on layer $\LayerIndex$\\ KV on layer $\LayerIndex$ at token $\TokenIndex$\\ Fully re-computed KV cache\\ Pre-computed KV cache\\ \name-updated KV cache\end{tabular} \\ \hline
\begin{tabular}[c]{@{}r@{}}$\Attention_{\LayerIndex}$\\ $\Attention_{\LayerIndex}^{\Full}$\\ $\Attention_{\LayerIndex}^{\Pre}$\\ $\Attention_{\LayerIndex}^{\New}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Attention matrix on layer $\LayerIndex$\\ Fully re-computed attention matrix\\ Pre-computed attention matrix\\ \name-updated attention matrix\end{tabular} \\ \hline
$\KVD(\KV_{\LayerIndex}, \KV^{\Full}_{\LayerIndex})[\TokenIndex]$ & \begin{tabular}[c]{@{}l@{}}KV deviation of KV cache $\KV$ on \\ layer $\LayerIndex$ of token $\TokenIndex$ with $\KV_{\LayerIndex}^{\Full}[\TokenIndex]$\end{tabular} \\ \hline
$\CAD(\Attention_{\LayerIndex},\Attention_{\LayerIndex}^{\Full})$ & \begin{tabular}[c]{@{}l@{}}Cross-attention deviation between \\ $\Attention_{\LayerIndex}^{\Full}$ and $\Attention_{\LayerIndex}^{\Full}$ at the attention \\ between tokens of different chunks\end{tabular} \\ \hline
\end{tabular}
\caption{Summary of terminology}
\label{tab:terminology}
\end{table}


\begin{figure}[t]
\centering
	\includegraphics[width=.99\columnwidth]{figs/deviations.pdf}
    \tightcaption{Simplified depiction of KV cache and attention matrix per layer, and the KV deviation and cross-attention deviation between pre-computed KV cache and full KV compute.}
    \label{fig:deviations}
\end{figure}


%\begin{table}[]
%\small
%\begin{tabular}{rl}
%\hline
%\textit{Notation} & \textit{Description} \\ \hline\hline
%\begin{tabular}[c]{@{}r@{}}$\LayerIndex$ \\ $\TokenIndex$\\ $\ChunkIndex$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Layer index\\ Token index\\ Chunk index\end{tabular} \\ \hline
%\begin{tabular}[c]{@{}r@{}}$\KV$\\ $\KV^{\Full}$\\ $\KV^{\Pre}$\\ $\KV^{\New}$\end{tabular} & \begin{tabular}[c]{@{}l@{}}KV cache\\ Fully re-computed KV cache\\ Pre-computed KV cache\\ \name-updated KV cache\end{tabular} \\ \hline
%\begin{tabular}[c]{@{}r@{}}$\KV[\LayerIndex]$\\ $\KV[\LayerIndex][\TokenIndex]$\end{tabular} & \begin{tabular}[c]{@{}l@{}}KV on layer $\LayerIndex$\\ KV on layer $\LayerIndex$ at token $\TokenIndex$\end{tabular} \\ \hline
%\begin{tabular}[c]{@{}r@{}}$\Attention_{\LayerIndex}$\\ $\Attention_{\LayerIndex}[\TokenIndex]$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Attention matrix on layer $\LayerIndex$\\ Attention matrix on layer $\LayerIndex$ associated with token $\TokenIndex$\end{tabular} \\ \hline
%%\begin{tabular}[c]{@{}r@{}}$\Attention_{\LayerIndex}$\\ $\Attention_{\LayerIndex}[\TokenIndex,\TokenIndex']$\end{tabular} & \begin{tabular}[c]{@{}l@{}}Attention Matrix on layer $\LayerIndex$\\ Attention Matrix on layer $\LayerIndex$ between token $\TokenIndex$ and $\TokenIndex'$\end{tabular} \\ \hline
%$\CA_{\LayerIndex,\TokenIndex}$ & Aggregated Cross-Attention of token $\TokenIndex$ on layer $\LayerIndex$ \\ \hline\end{tabular}
%\caption{Summary of terminology\jiayi{This table needs update?}}
%\label{tab:terminology}
%\end{table}

%\mypara{Terminology}



\subsection{Terminology}
\label{subsec:terminology}

Table~\ref{tab:terminology} summarizes the notations used in this section.
%To formally describe our goal, we begin with the notations used in this section (summarized in Table~\ref{tab:terminology}).
%For a given KV cache $\KV$, we use $\KV[\LayerIndex]$ and $\KV[\LayerIndex][\TokenIndex]$ to denote the KV on layer $\LayerIndex$ and the KV on layer $\LayerIndex$ at token $\TokenIndex$, respectively.\footnote{For simplicity, we use the terms KV and KV cache interchangeably.}
For a given list of $\ChunkNum$ text chunks, 
we use $\KV^{\Full}$ to denote the KV cache from full KV re-compute, $\KV^{\Pre}$ to denote the pre-computed KV cache,  and $\KV^{\New}$ to denote the \name-updated KV cache. 
Here, each of these KV caches is a concatenation of KV caches associated with different text chunks.

As depicted in Figure~\ref{fig:deviations}, on each layer, the KV cache $\KV_{\LayerIndex}$ produces the attention matrix $\Attention_{\LayerIndex}$, which then affects the input and the KV on the next layer. (For clarity, we omitted the Q vectors.)
The attention matrix on each layer contains the cross-attention which is the attention between tokens from different chunks. 

The difference between the full KV re-compute (full prefill) and the full KV re-use are two-fold. 

\begin{packeditemize}
\item {\bf KV deviation:}
We define the {\em KV deviation} of a KV cache $\KV$ on layer $\LayerIndex$ of token $\TokenIndex$ as the absolute difference between $\KV_{\LayerIndex}[\TokenIndex]$ and $\KV_{\LayerIndex}^{\Full}[\TokenIndex]$, denoted as $\KVD(\KV_{\LayerIndex}, \KV^{\Full}_{\LayerIndex})[\TokenIndex]$. 
It measures how much different the given KV is on a particular token and layer compared to the full-prefilled KV cache.
%the deviation between the two KV caches at each token on this layer.
We will later use the KV deviation to identify which tokens' KV has higher deviation and thus need to be updated. 

\item {\bf Cross-attention deviation:}
Similarly, for an attention matrix $\Attention_{\LayerIndex}$ on layer $\LayerIndex$, we define the {\em cross-attention deviation}, denoted as $\CAD(\Attention_{\LayerIndex}, \Attention_{\LayerIndex}^{\Full})$, to be the L-2 norm\jc{Jiayi, need to update} of its difference with $\Attention_{\LayerIndex}^{\Full}$ at the attention between tokens from different chunks. 
We focus on the cross-attention, rather than the attention between any tokens, because missing the cross-attention is the primary reason for the poor quality of full KV reuse (\S\ref{subsec:modular}). 

\end{packeditemize}





%$\Func_\LayerIndex(\KV)$ and $\Func_\LayerIndex(\KV^{\Full})$.\footnote{Assume $\KV$ has the same shape as $\KV^{\Full}$.}
%We measure the difference by L2-norm. 
Using these notations, our goal can be formulated as how to quickly update the precomputed KV cache $\KV^{\Pre}$ to the new KV cache $\KV^{\New}$, such that the cross-attention deviation $\CAD(\Attention^{\New}_{\LayerIndex},\Attention^{\Full}_{\LayerIndex})$ on any layer $\LayerIndex$, is minimized. 



\subsection{Selectively re-computing KV cache}
\label{subsec:partial-recompute}

%Then in \S\ref{subsec:token-selection}, we will 
%\item Which tokens should be selected to be re-computed (\S\ref{subsec:token-selection}).
%\end{packeditemize}
\begin{figure}[t]
\centering
	\includegraphics[width=.99\columnwidth]{figs/selective_recompute.pdf}
    \tightcaption{Illustrated contrast between (a) full KV recompute and (b) selective KV recompute on one layer.}
    \label{fig:selective_recompute}
\end{figure}


For now, let us assume we have already selected a subset of tokens to re-compute on each layer (we will explain how to select them in \S\ref{subsec:token-selection}). 
Here, we describe how \name re-computes the KV of these selected tokens on each layer. 

\mypara{Workflow} 
The default implementation of prefill (depicted in Figure~\ref{fig:selective_recompute}(a)) does not ``skip'' tokens while only compute the KV of a subset of tokens. 
Instead, \name runs the following steps (depicted in Figure~\ref{fig:selective_recompute}(b)):
\begin{packeditemize}
\item It first applies a mask on the input of each layer $\LayerIndex$ to reduce it to the a subset of selected tokens.
\item It then transforms the reduced input into the $Q_{\LayerIndex}$, $K_{\LayerIndex}$ and $V_{\LayerIndex}$ vectors will also be restricted to the selected tokens. 
\item It then expands the $K_{\LayerIndex}$ vector and $V_{\LayerIndex}$ vector by reusing the KV cache entries associated with the un-selected tokens on layer $\LayerIndex$, so that the attention matrix includes attention between selected tokens and all other tokens.
%will include the attention between these un-selected tokens.
\item Finally, it runs the same attention module to produce the input of the next layer. 
\end{packeditemize}
These changes make little assumption on the exact transformer process and can be integrated with many popular transformers (more details in \S\ref{sec:impl}).


\jc{Jiayi, please mention some papers that also do this}

\mypara{Benefits} The selective KV recompute procedure enjoys two benefits.
First, the compute overhead is proportional to the number of selected tokens. 
This is because it only runs computation associated with the selected tokens. 
If we re-compute $r\%$ of tokens per layer, the total compute overhead will be $r\%$ of full prefill. 
Empirically, our evaluation also shows that the prefill delay is about $r\%$ of the full prefill as well (see \S\ref{sec:eval}).

Second, by re-computing the KV of a particular token, we also re-computes the cross-attention between it and its preceding tokens. 
%the KV of the selected tokens are updated based on the cross-attention between them and all of their preceding tokens. 
This is because although attention matrix on each layer only has the entries of the selected tokens, it includes their attention with all preceding tokens, including the non-selected tokens. 
This attention matrix is then used to compute the input embedding of the next layer, thus also affecting the KV values of the next layer. 
%As elaborated in \S\ref{subsec:token-selection}, capturing the full cross-attention of the selected tokens is important since high cross-attention can exist among any tokens, not only the selected ones.



%However, we can first {\em permute} the order of the tokens on each layer to move the \HCA tokens and separate them from other tokens whose KV does not need to be updated. 
%The reason is the following insight, whose proof will be provided in \S\ref{??}.
%
%\begin{insight}
%The order of tokens on each layer does not affect the KV of each token.\jc{jiayi, this insight doesn't sound right. doesn't it mean you can arbitrarily shuffle the tokens and still get the same result?} \jiayi{A new version: The order of tokens on each layer does not affect the KV of each token if the attention mask is permuted accordingly}
%\end{insight}
%
%Once the \HCA tokens on a layer are moved together, the prefill computation can be done only on those tokens without affecting other tokens' KV.
%Figure~\ref{fig:selective_recompute} illustrates this process.
%So if only $r\%$ of tokens are selected as \HCA tokens, recomputing their KV only needs $r\%$ of computation overhead as a full prefill.

\subsection{Selecting which tokens to re-compute}
\label{subsec:token-selection}


%we first notice that the attention deviation, defined in \S\ref{subsec:terminology}, is an aggregation of the token-wise attention deviation, \ie $||\Attention_{\LayerIndex}-\Attention_{\LayerIndex}^{\Full}||^2=\sum_{\TokenIndex}||\Attention_{\LayerIndex}[\TokenIndex]-\Attention_{\LayerIndex}^{\Full}[\TokenIndex]||^2$.
Next, we explain how to choose the tokens whose KV should be re-computed on each layer in order to reduce the cross-attention deviation.
We first notice, from Figure~\ref{fig:deviations}, that the cross-attention deviation on each layer results from the KV deviation on previous layers.
Thus, our intuition is to prioritize re-computing the KV of tokens who have high KV deviations.
Of course, this intuitive scheme is {\em not} feasible as it needs to know full-prefilled KV cache, and we will make it practical shortly.

\begin{figure}[t]
\centering
	\includegraphics[width=.99\columnwidth]{figs/ca_reduce_final.pdf}
    \tightcaption{Cross attention deviation is reduced by re-computing \HCA tokens}
    \label{fig:ca_reduction}
\end{figure}

To show effectiveness of selecting tokens with high KV deviations, Figure~\ref{fig:ca_reduction} uses three models on the dataset of Musique (please see \S\ref{subsec:eval:setup} for details).
It shows the change of cross-attention deviation of layer $\LayerIndex$, 
$\CAD(\Attention_{\LayerIndex}, \Attention_{\LayerIndex}^{\Full})$, after we use the aforementioned scheme (\S\ref{subsec:partial-recompute}) to select and re-compute the $r\%$ of tokens $\TokenIndex$ who have the highest KV deviation 
$\KVD(\KV_{\LayerIndex}, \KV^{\Full}_{\LayerIndex})[\TokenIndex]$.
As the recompute ratio ($r$) increases, the cross-attention deviation gradually reduces, and the biggest drops happen when the top few tokens with the highest KV deviations are re-computed. 
Empirically, it suggests the following insight. 



\begin{insight}
On each layer $\LayerIndex$, re-computing the KV of a token $\TokenIndex$ who has a higher KV deviation (\ie $\KVD(\KV_{\LayerIndex}, \KV^{\Full}_{\LayerIndex})[\TokenIndex]$) reduces the total forward attention deviation (\ie $\CAD(\Attention_{\LayerIndex}, \Attention_{\LayerIndex}^{\Full})$) by a greater amount. 
%Recomputing the KV of a token $\TokenIndex$ on layer $\LayerIndex$ will greatly reduce the Attention Deviation associated with this token, \ie $||\Attention_{\LayerIndex}^{\New}[\TokenIndex]-\Attention_{\LayerIndex}^{\Full}[\TokenIndex]||$.
\end{insight}

Thus, if we need to re-compute the KV of, say 10\%, of tokens on a layer $\LayerIndex$, we should choose the 10\% of tokens who have the highest KV deviations.\footnote{An important side note is that in the pre-computed KV cache, the K vector of each chunk must be adjusted with the correct positional embedding. In the most popular positional embedding scheme (Rotary Positional Embedding or ROPE~\cite{su2024roformer}), this correction is done simply by multiplying the K vector by a rotation matrix $\begin{pmatrix}
\cos m\theta & -\sin m\theta\\
\sin m\theta & \cos m\theta\\
\end{pmatrix}$. The rotation matrix in n-dimensional space is shown in Appendix \ref{sec:appendix_pos}. This step has negligible overhead (\S\ref{subsec:fusor_eval}).} 
We refer to these tokens as the {\bf High-KV-Deviation} (or {\bf \HCA}) tokens on layer $\LayerIndex$.

Now that we know we should recompute KV for the \HCA tokens, two natural questions arise. 



\vspace{0.2cm}
\noindent {\bf Do we need to re-compute KV for most tokens?}
%Fortunately, Figure~\ref{??} indicates that this is not always true. 
In \S\ref{sec:eval}, we empirically show that choosing 10-20\% tokens as \HCA tokens and re-computing their KV suffices to greatly reduce the cross-attention deviation and preserve generation quality.
%Re-computing 10-15\% of tokens can reduce the forward attention deviation by \fillme\%. 

This can be intuitively explained by {\em attention sparsity}, a well-studied property observed in many transformer models by prior research~\cite{liu2024scissorhands,h2o,choromanski2020rethinking,chen2021scatterbrain}. 
It says that in an attention matrix, high attention typically only occurs between a small number of tokens and their preceding tokens. 
To validate this observation, Figure~\ref{fig:acacdf} uses the same models and dataset as Figure~\ref{fig:ca_reduction}. 
It shows the distribution of KV deviation on one layer.
We can see that a small fraction, about 10-15\%, of tokens have much higher KV deviation than others, which corroborates the sparsity of cross-attention.

If a token has very low attention with other chunks' tokens (\ie low cross-attention with other chunks), the KV deviation between $\Attention^{\Pre}$ and $\Attention^{\Full}$ will be low and thus do not need to be re-computed.
Only when a token has a high attention with other chunks (\ie high KV deviation),\jc{Jiayi, the logic here is broken, why high attention means high kv deviation?} should its KV be re-computed.

%The intuitive reason is the following:
%\begin{insight}
%Due to attention sparsity, the high attention only occurs between a small number of tokens and their preceding tokens in other chunks, so only a few tokens' KV 
%
%Forward attention is affected more by tokens with high KV deviations \ie~\HKVD tokens. Due to attention sparsity, the high attention only occurs between a small number of tokens and their preceding tokens in other chunks, so only a small number of tokens are \HKVD tokens.
%\end{insight}
%{\em Attention sparsity} is a well-known property observed by prior research in many transformer models~\cite{liu2024scissorhands,h2o,choromanski2020rethinking,chen2021scatterbrain}.
%If a token has very low attention with other chunks' tokens (\ie low cross-attention with other chunks), the token-wise KV deviation between $\Attention^{\Pre}$ and $\Attention^{\Full}$ will be low anyway. 
%Only when attention is high between chunks (\ie high KV deviation), should KV re-computation be used.

\begin{figure}[t]
\centering
	\includegraphics[width=.99\columnwidth]{figs/kv_dev.pdf}
    \tightcaption{Distribution of KV deviation of different tokens on one layer.}
    \label{fig:acacdf}
\end{figure}




\vspace{0.2cm}
\noindent {\bf How to identify the \HCA tokens without knowing the true attention matrix?}
Naively, to identify the \HCA tokens, one must calculate the full attention matrix $\Attention_{\LayerIndex}^{\Pre}$ and $\Attention_{\LayerIndex}^{\Full}$ of each layer $\LayerIndex$ in the first place, but doing so is too expensive, and defeats the purpose of selective KV re-compute.
instead, we observe that the \HCA tokens on different layers are not independent:
%. we have the following observation:

\begin{insight}
Tokens with highest KV deviations on one layer are likely to have the highest KV deviations on the next layer. 
%The \HCA tokens on one layer is likely a subset of \HCA tokens on the previous layer. 
\end{insight}

%More specifically, if token $\TokenIndex$ has a higher token-wise attention deviation than $\TokenIndex'$ on layer $\LayerIndex$, (\ie $||\Attention_{\LayerIndex}^{\Pre}[\TokenIndex]-\Attention_{\LayerIndex}^{\Full}[\TokenIndex]||>||\Attention_{\LayerIndex}^{\Pre}[\TokenIndex']-\Attention_{\LayerIndex}^{\Full}[\TokenIndex']||$), token $\TokenIndex$ will likely to have a higher token-wise attention deviation on the next layer $\LayerIndex+1$, (\ie $||\Attention_{\LayerIndex+1}^{\Pre}[\TokenIndex]-\Attention_{\LayerIndex+1}^{\Full}[\TokenIndex]||>||\Attention_{\LayerIndex+1}^{\Pre}[\TokenIndex']-\Attention_{\LayerIndex+1}^{\Full}[\TokenIndex']||$).
%on one layer $\LayerIndex$, if token $\TokenIndex$ has a higher \ACA than token $\TokenIndex'$, (\ie $\CA_{\LayerIndex, \TokenIndex}\geq\CA_{\LayerIndex, \TokenIndex}$), then on the the next layer $\LayerIndex+1$, token $\TokenIndex$ is likely to have a higher \ACA than token $\TokenIndex'$ (\ie $\CA_{\LayerIndex+1, \TokenIndex}\geq\CA_{\LayerIndex+1, \TokenIndex}$).

To put it concretely, if the top three \HCA tokens on the first layer are tokens 2, 3, and 5, these three tokens will likely also have higher KV deviations than most other tokens on the second layer. 
Figure~\ref{fig:rankcorr} uses the same setting as Figure~\ref{fig:acacdf} and shows the Spearman's rank correlation score between the KV deviation of tokens between two neighboring layers. 
The figure shows a consistently high similarity of \HCA tokens between different layers.\footnote{We should clarify that although the \HCA tokens are similar across layers, the attention matrices between layers can still be quite different.} 
%similar between layers.\jiayi{What's the point of this footnote}}
%Kendall's rank correlation scores between \ACA of the same token on two neighboring layers. 

The intuition behind this correlation lies in the previous observation that the input embedding of each token changes slowly between layers in transformer models~\cite{liu2023deja,phang2021finesim}. Therefore, KV cache between layers should also bear similarity as KV cache is generated from the inut embedding with a linear transformation.


\begin{figure}[t]
\centering
	\includegraphics[width=.99\columnwidth]{figs/kv_corr_bar.pdf}
    \tightcaption{Rank correlation of the KV deviation per token between two consecutive layers.
    }
    \label{fig:rankcorr}
\end{figure}





Given the substantial correlation between the \HCA tokens, a straightforward solution is that we can  perform prefill on the first layer first, and pick the \HCA tokens of the first layer and only update their KV on all other layers.
Since an LLM usually has over 30 layers, this process can save most of the compute compared to full KV re-compute. 
That said, using {\em only} the attention deviation of different tokens on the first layer may not be statistically reliable to pick \HCA tokens of all layers, especially deeper layers. 

\begin{figure}[t]
\centering
%	\includegraphics[width=.99\columnwidth]{figs/selection_illustrated.pdf}
	\includegraphics[width=.99\columnwidth]{figs/selection_illustrated_v2.pdf}
    \tightcaption{\name selects the \HCA (high KV deviation) tokens of one layer by computing KV deviation of only the \HCA tokens selected from the previous layer and select the tokens among them with high KV deviation.}
    \label{fig:selection_illustrated}
\end{figure}

Thus, we opt for a {\em gradual filtering} scheme (depicted in Figure~\ref{fig:selection_illustrated}).
If on average we want to pick $r\%$ \HCA tokens per layer, we will pick $r_1\%$ tokens based on the token-wise attention deviation on the first layer, with $r_1$ being slightly higher than $r$, and use them as the \HCA tokens on the second layer.
Then we recompute the KV of these $r_1\%$ \HCA tokens on the second layer and pick $r_2\%$ tokens who have highest token-wise attention deviation, with $r_2$ slightly less than $r_1$, as the \HCA tokens on the next layer, and so forth. 
Intuitively, this gradual-filtering scheme eventually picks the \HCA tokens who have relatively high attention deviation not only on the first layer, but also on a few other layers, which empirically is more statistically reliable to identify the \HCA tokens on each layers.  


